Separable and Localized System Level Synthesis for Large-Scale Systems

A major challenge faced in the design of large-scale cyber-physical systems, such as power systems, the Internet of Things or intelligent transportation systems, is that traditional distributed optimal control methods do not scale gracefully, neither in controller synthesis nor in controller implementation, to systems composed of millions, billions or even trillions of interacting subsystems. This paper shows that this challenge can now be addressed by leveraging the recently introduced System Level Approach (SLA) to controller synthesis. In particular, in the context of the SLA, we define suitable notions of separability for control objective functions and system constraints such that the global optimization problem (or iterate update problems of a distributed optimization algorithm) can be decomposed into parallel subproblems. We then further show that if additional locality (i.e., sparsity) constraints are imposed, then these subproblems can be solved using local models and local decision variables. The SLA is essential to maintaining the convexity of the aforementioned problems under locality constraints. As a consequence, the resulting synthesis methods have $O(1)$ complexity relative to the size of the global system. We further show that many optimal control problems of interest, such as (localized) LQR and LQG, $\mathcal{H}_2$ optimal control with joint actuator and sensor regularization, and (localized) mixed $\mathcal{H}_2/\mathcal{L}_1$ optimal control problems, satisfy these notions of separability, and use these problems to explore tradeoffs in performance, actuator and sensing density, and average versus worst-case performance for a large-scale power inspired system.

==> Abstract_v2.tex <==
This paper presents a new control paradigm with favorable capability to handle implementation constraints on distributed controllers, which is particularly suitable for large-scale applications. By parameterizing all stabilizing controllers in terms of the closed loop transfer matrices, we show that the controller can be implemented by the desired closed loop transfer matrices directly with guaranteed internal stability. We then introduce an additional convex set constraint on the admissible closed loop transfer matrices, and cast the distributed optimal control problem as a convex optimization problem. This general formulation unifies many previous results in the field of distributed control, including quadratically invariant constraints as a special case. In addition, when sparsity constraints are imposed on the closed loop transfer matrices, the controller achieving the desired closed loop response can be implemented in a localized and scalable way. For some specific convex objective such as the $\mathcal{H}_2$ norm, the synthesis of the optimal controller can further be done in a localized and parallel way, regardless the dimension of the global system. Simulation shows that our optimal controller, with its constraints on locality, settling time, and communication delay, can achieve similar performance to an idealized centralized optimal one.
%novel output feedback control scheme for localizable distributed systems. 
%These are systems for which the effect of each local disturbance can be localized in closed loop despite communications delays between controllers, akin to spatio-temporal dead-beat control with delays.
%By parametrizing all stabilizing controllers in terms of the closed loop transfer matrix, 
%
%Specifically, we introduce the idea of state feedback localizability as a generalization of controllability into space-time domain, and characterize state feedback localizable systems in terms of the feasibility of a set of linear equations.
%We then formulate the localized LQR (LLQR) problem for state feedback localizable system, and show that the global optimal solution can be computed in a completely localized and parallel way. 
%The solution of each LLQR sub-problem can be used for controller synthesis by a local update algorithm, and each local controller only need to collect information from a localized region to compute its control action.
%All these properties are extremely favorable for large-scale control systems, as the synthesis and the implementation of the controller can all be done in a localized and parallel way, regardless the dimension of the global system. 
%Specifically, we show that when a model changes locally, we only need to re-synthesize some of the local controllers to ensure global optimality, which supports incremental design of the plant. 
%Simulation shows that our optimal controller, with its constraints on locality, settling time, and communication delay, can achieve similar performance to an idealized centralized optimal one.
%In particular, we synthesize a localized optimal controller for a large-scale unstable system with $10^{6}$ states, and achieve $99\%$ global optimality.

==> Abstract_v3.tex <==
This paper presents a scalable algorithm to synthesize a nearly optimal controller for a class of large-scale systems.
Our approach is based on the localized optimal control framework developed in the first part of this two-part paper.
%In the first part of this two-part paper, we introduced the notion of localizability as a convex set constraint imposed on the admissible closed loop transfer matrices, and formulated the localized optimal control problem as a convex optimization problem. 
%In this paper, we discuss how to use the localized optimal control framework to enhance the scalability of both controller implementation and controller synthesis for large-scale networked systems.
%design and implement controllers for large-scale networked systems in a localized and scalable way.
%First, we show that when the closed loop transfer matrices admit a localized (sparse) solution, the controller achieving the desired closed loop response can always be implemented in a localized and thus scalable way. 
%This holds true for localized optimal control problem with any performance metric.
%Then, 
%Specifically, we introduce the notion of decomposability such that the optimal control problem can be solved in a localized and scalable way.
We identify the conditions in which the localized optimal control problem can be solved in a localized and scalable way.
%Then, we identify the conditions in which the synthesis of the controller can be done in a localized and scalable way.
%We introduce the notion of decomposability on the performance metric and the localizability constraint of the localized optimal control problem. 
Specifically, when the problem is decomposable, the global optimization problem can be decomposed into parallel local subproblems.
%When both the performance metric and the localizability constraint are decomposable, the global optimization problem can be decomposed into several local optimization sub-problems. 
%These sub-problems can be solved in a parallel yet iterative way. 
Each local subproblem only depends on the local plant model information, and the complexity of solving each subproblem is independent to the size of the global network.
As a result, the synthesis algorithm for decomposable problems can be scaled to arbitrary large-scale network if parallel computation is available.  
We identify several class of decomposable problems, including the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem and the $\mathcal{H}_2$ optimal control with sensor and actuator regularization.
%Using the notion of decomposability, we identify several classes of optimal control problems that can be solved in a scalable way.
Simulation shows that our localized optimal controller, with its additional sparsity constraint, settling time constraint, and communication delay constraint, can achieve similar transient performance to an idealized centralized optimal one, but far more superior in terms of the scalability of controller synthesis and implementation. 
The algorithm is demonstrated on a system with $12800$ states composed of randomized heterogeneous and dynamically coupled subsystems -- here the distributed and centralized optimal controllers cannot be computed.

%novel output feedback control scheme for localizable distributed systems. 
%These are systems for which the effect of each local disturbance can be localized in closed loop despite communications delays between controllers, akin to spatio-temporal dead-beat control with delays.
%By parametrizing all stabilizing controllers in terms of the closed loop transfer matrix, 
%
%Specifically, we introduce the idea of state feedback localizability as a generalization of controllability into space-time domain, and characterize state feedback localizable systems in terms of the feasibility of a set of linear equations.
%We then formulate the localized LQR (LLQR) problem for state feedback localizable system, and show that the global optimal solution can be computed in a completely localized and parallel way. 
%The solution of each LLQR sub-problem can be used for controller synthesis by a local update algorithm, and each local controller only need to collect information from a localized region to compute its control action.
%All these properties are extremely favorable for large-scale control systems, as the synthesis and the implementation of the controller can all be done in a localized and parallel way, regardless the dimension of the global system. 
%Specifically, we show that when a model changes locally, we only need to re-synthesize some of the local controllers to ensure global optimality, which supports incremental design of the plant. 
%Simulation shows that our optimal controller, with its constraints on locality, settling time, and communication delay, can achieve similar performance to an idealized centralized optimal one.
%In particular, we synthesize a localized optimal controller for a large-scale unstable system with $10^{6}$ states, and achieve $99\%$ global optimality.

==> Implementation_old.tex <==
\subsection{Localized Implementation}
Note that the optimization problem \eqref{eq:LOC} is convex if the objective function is convex and the localizability constraint $\s$ in \eqref{eq:main_S} is a convex set. In this paper, we further express the localizability constraint $\s$ as the intersection of three convex set components: the locality (sparsity) constraint $\Ell$, the finite impulse response (FIR) constraint $\FT$, and an arbitrary convex set component $\Sother$. In this case, the localized optimal control problem is given by
\begin{eqnarray}
\underset{\{\tf R, \tf M,\tf N, \tf L\}}{\text{minimize}} \quad && g(\tf R,\tf M,\tf N,\tf L) \nonumber\\
\text{subject to} \quad && \eqref{eq:main_1} - \eqref{eq:main_stable} \nonumber \\
&& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \cap \Sother. \label{eq:localized}
\end{eqnarray}
We assume that the problem \eqref{eq:localized} has a feasible solution.

The components of the localizability constraint in \eqref{eq:localized} is interpreted in the following way. The constraint $\Sother$ includes any convex constraint imposed by the system, including the information sharing constraint $\C$ as one of its component. Constraints $\FT$ and $\Ell$ are the additional constraints we imposed to enhance the scalability of controller synthesis and controller implementation. For example, the constraint $\FT$ restricts the optimization variables to have finite impulse responses of horizon $T$. In this case, problem \eqref{eq:localized} becomes a finite dimensional convex program. In addition, the controller achieving the desired closed loop response can be implemented by FIR filters using the structure given in Theorem \ref{thm:1}. The role of $\Ell$ is explained as follows.

Theorem \ref{thm:1} shows how the sparsity of the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ translates into the implementation complexity of a controller as in \eqref{eq:implementation}. If the rows of these transfer matrices are suitably sparse, then each sub-controller only needs to collect a small number of measurements and controller internal states to compute its control law. The locality constraint $\Ell$ is the mechanism that we use to impose this sparsity.  

We begin by defining the notion of the $d$-outgoing and incoming sets at a subsystem $j$. To do so, we let the distance $\dist{j}{i}$ from subsystem $j$ to subsystem $i$ be given by the length of the shortest path from node $j$ to node $i$ in the graph $\mathcal{G}$.  We say that a set  $\mathcal{D}$ of subsystems is of size $d$ if $\dist{i}{j}\leq d$ for all $i,j \in \mathcal{D}$.  We then define the $d$-outgoing set of subsystem $j$ as $\Down{j}{d}:= \{i | \text{dist}(j \to i) \leq d\}$, and the $d$-incoming set of subsystem $j$ as $\Up{j}{d} := \{i | \text{dist}(i \to j) \leq d\}$ -- by definition, both of these sets are of size $d$.  Our approach to making the controller synthesis task specified in optimization problem \eqref{eq:localized} scalable is to confine, or \emph{localize} the effects of the process and sensor disturbances to a $d$-outgoing set at each subsystem $j$, for a size $d$ much smaller than that of $\mathcal{V}$.  As we make precise in the sequel, this implies that each sub-controller $j$ only needs to collect data from subsystems $i$ contained in its $d$-incoming set $\Up{j}{d}$.
%To help the readers follow the content, we create the following simple example in the form of \eqref{eq:interconnected}. This example is used to illustrate several ideas throughout the paper.
%\begin{example}
%Consider a network system with an undirected interaction topology as illustrated in Fig. \ref{fig:Chart105}. Each subsystem $i$ is assumed to have a scalar state $x_i$, a scalar control $u_i$, and a scalar measurement $y_i$. The dynamics for each subsystem $i$ are given by
%\begin{eqnarray}
%x_i[k+1] &=& x_i[k] + u_i[k] + \sum_{j \in \mathcal{N}_i} x_j[k] + \delta_{x_i}[k]\nonumber\\
%y_i[k] &=& x_i[k] + \delta_{y_i}[k]. \label{eq:interconnected_s}
%\end{eqnarray}
%As the interaction graph is undirected, we have that $\Down{j}{d} =  \Up{j}{d}$ for all $j$ and $d$. For example, $\Down{1}{2} =  \Up{1}{2} = \{1,2,3,4\}$.
%\end{example}
%\begin{figure}[h!]
%      \centering
%      \includegraphics[width=0.32\textwidth]{./figure/Topology.pdf}
%      \caption{Illustrative Example}
%      \label{fig:Chart105}     
%\end{figure}
\begin{example}
For a system \eqref{eq:interconnected} with interaction graph illustrated in Fig.
\ref{fig:Chart105}, the $2$-incoming and $2$-outgoing sets of subsystem $5$ are
given by $\Up{5}{2} = \{2,3,4,5\}$ and $\Down{5}{2} = \{5,6,7,8,9,10\}$,
respectively.
\end{example}
\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Topology2.pdf}
     \caption{Illustration of the $2$-incoming and $2$-outgoing sets of subsystem $5$.}
     \label{fig:Chart105}
\end{figure}

With this approach in mind, we say that the transfer matrix $\tf R$ mapping the state disturbance $\ttf \delta_x$ to the state $\tf x$, as defined in \eqref{eq:desired}, is $d$-localized if its impulse response can be appropriately covered by $d$-outgoing sets.  In particular, if we let $\tf R_{ij}$ denote the transfer function from the perturbation $\ttf \delta_{x_j}$ at sub-system $j$ to the state $\tf x_i$ at sub-system $i$, then the map $\tf R$ is $d$-localized if and only if for every subsystem $j$, $\tf R_{ij} = 0$ for all $i \not \in \Down{j}{d}$.  In words, this says that the transfer matrix $\tf R$ is $d$-localized if and only if the effect of each disturbance is contained, or localized, to within a region of size $d$.  This definition can be extended to the remaining transfer matrices $\tf N$, $\tf M$, and  $\tf L$ of \eqref{eq:desired} in a natural way.  The closed loop response \eqref{eq:desired} of the system is said to be $d$-localized if its constituent components $(\tf R,\tf N,\tf M,\tf L)$ are as well.  Finally, the subspace $\Ell$ in \eqref{eq:localized} imposes a $d$-localized constraint if it constrains its elements to be $d$-localized closed loop responses.
%In addition, we define a localized closed loop response as follows. 
%Consider the transfer matrix $R$ that maps the perturbation $\delta_x$ to the internal variable $x$. Denote $R_{ij}$ the submatrix of $R$ that maps the perturbation $\delta_{x_j}$ at sub-system $j$ to the state $x_i$ at sub-system $i$. The transfer matrix $R$ is said to be $d$-localized if $R_{ij} = 0$ for $i \not \in $ Down$(j,d)$ for all $j$. In this case, we say that the effect of each local perturbation $\delta_{x_j}$ is localized within the region Down$(j,d)$. We can define $d$-localized property for $N, M, L$ in \eqref{eq:desired} in a similar way. A closed loop transfer matrix in \eqref{eq:desired} is said to be $d$-localized if all its four components $(R,N,M,L)$ are $d$-localized.

%Given a transfer matrix $G$ mapping the perturbation $\delta_x$ or $\delta_y$ to the internal variable $x$ or $u$. Denote $G_{ij}$ the submatrix of $G$ that maps the perturbation $\delta_{x_j}$ or $\delta_{y_j} $at sub-system $j$ to the internal variable $x_i$ or $u_i$ at sub-system $i$. A transfer matrix $G$ is said to be $d$-localized if $G_{ij} = 0$ for $i \not \in $ Down$(j,d)$ for all $j$. In this case, we say that the effect of each local perturbation $\delta_{x_j}$ or $\delta_{y_j}$ is localized within the region Down$(j,d)$. A closed loop transfer matrix in \eqref{eq:desired} is said to be $d$-localized if all its four components $(R,N,M,L)$ are $d$-localized.

%Now we consider the case in which $\s$ enforces a $d$-localized constraint on $(R,N,M,L)$. 
With these definitions and results in hand, our approach to synthesizing a controller that is scalable to implement is straightforward: we choose the subspace $\Ell$ to be a $d$-localized constraint and select a horizon $T$ for the FIR subspace $\FT$.  Whereas the first constraint ensures that the transfer matrices solving optimization problem \eqref{eq:localized} are $d$-localized, the second constraint is simply imposed to make the optimization problem finite dimensional.  The resulting optimization problem \eqref{eq:localized} is easily seen to be convex as the constraints are all affine: if it is feasible, then the resulting closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ can be used to implement a controller as specified by Theorem \ref{thm:1} (note that the modified transfer matrices $( \tilde{\tf R},  \tilde{\tf M},  \tilde{\tf N})$ are also $d$-localized).  Further, since the effect of each disturbance is localized to a region of size $d$ (i.e., since the closed loop response is $d$-localized), each sub-controller only needs to collect data from other subsystems that are at most a distance $d$ away.  In particular, this means that the row sparsity of the transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ is defined by the $d$-incoming sets of the system, and thus the control action $\tf u_i$ and internal state $\ttf \beta_i$ of sub-controller $i$ can be computed by collecting the data $(\tf y_j, \ttf \beta_j)$ from subsystems $j$ in the $d$-incoming set $\Up{i}{d}$.  This discussion shows that a controller synthesized via optimization problem \eqref{eq:localized} and implemented according to Theorem \ref{thm:1} is scalable to implement, as the amount of information collected at a given subsystem is specified by the $d$-localized constraint $\Ell$, and hence is independent of the number of subsystems $n$.

Before proceeding, we note that although optimization problem \eqref{eq:localized} is convex for any affine constraint set $\Ell$, it is not necessarily feasible.  This is because the subsystems are dynamically coupled to each other (as per \eqref{eq:interconnected}), and hence it may not always be possible to localize the effect of a disturbance affecting subsystem $j$ to a pre-specified $d$-outgoing set $\Down{j}{d}$.  Intuitively, optimization problem \eqref{eq:localized} is feasible when the communication constraint in $\Sother$ is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant.  In this way, the necessary sub-controllers can take action \emph{before} a disturbance perturbs their subsystem and stop it from propagating to the rest of the system.  Implicit in this argument are the assumptions that information can be shared quickly between sub-controllers, and that sensors and actuators are strategically placed (these assumptions are discussed in detail in \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}).

Based on this intuition, we provide simple rules for how to select the size $d$ of the localized subspace constraint $\Ell$, the horizon $T$ of the FIR subspace constraint $\FT$, as well as a principled approach to designing the actuation scheme of the system (i.e., the matrix $B_2$) in the paper \cite{2015_Wang_Reg}.  For the remainder of the paper, we assume that the constraint sets $\Ell$ and $\FT$ are given, and that the communication, actuation and sensing architecture of the system is such that optimization problem \eqref{eq:localized} is feasible.

%First, we should note that a localized closed loop response does not mean that the open loop response is localized, so our method is still applicable for large-scale coupled network systems. 
%However, we do need some assumptions to ensure the existence of a localized closed loop response: (1) the communication speed is faster than the speed of disturbance propagated in the plant, and (2) the locations of the sensor and actuator are properly chosen. 
%Therefore, even though the open loop response is coupled to each other, it is still possible to achieve a $d$-localized closed loop response by designing the control action properly.
 %Note that our method do require the following assumptions: (1) fast information sharing, and (2) properly chosen locations of sensor and actuator.
%These conditions are discussed in our other works \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}. In particular, we give some simple rules to \emph{design} the spatio-temporal constraint $\s$ and the actuator locations ($B_2$) in \cite{2015_Wang_Reg}. In this paper, we assume that $\s$ is given before synthesis.
%
% 
%
%
%
%As mentioned the localized subspace constraint $\Ell$ and FIR horizon $T$ are design parameters in the controller synthesis problem.  We provide simple rules for how to select these parameters, as well as a principled approach to designing the actuation scheme of the system (i.e., the matrix $B_2$) in our companion paper  \cite{2015_Wang_Reg}.  For the remainder of the paper, we assume that the horizon $T$ has been set and that the subspace constraint $\Ell$ is $d$-localized.  
%Now we use $\s$ in \eqref{eq:local_S} to enforce the $d$-localized constraint on the closed loop. If \eqref{eq:local1} - \eqref{eq:local_S} is still feasible, then Theorem \ref{thm:1} suggests that the controller achieving the desired localized closed loop can be realized using $d$-localized stable transfer matrices $(\tilde{R}^+, \tilde{N}, \tilde{M}, L)$ by \eqref{eq:implementation}. By interpreting the implementation \eqref{eq:implementation} row at a time, we can show that the control information $(u_i, \beta_i)$ at each sub-system $i$ can be computed by collecting the information $(y_j, \beta_j)$ locally within the set $j \in \text{Up}(i,d)$. This implies that the controller can be implemented in a localized and scalable way. 
%For instance, local controller $u_i$ can be computed using only \emph{some} measurement $y_j$ and \emph{some} controller state $\beta_j$, as long as the $i$th rows of the matrices $\tilde{M}$ and $L$ are sparse. If we specify the sparsity pattern on the closed loop transfer matrices properly, local controller $u_i$ only needs to collect the information locally to compute its control action.

%Another benefit of our formulation is that \eqref{eq:local_obj} - \eqref{eq:local_S} is a \emph{convex} optimization problem for \emph{arbitrary} sparsity constraint $\s$, which is different from the traditional formulation \eqref{eq:trad}. The mathematical relation between the traditional formulation and our new formulation is beyond the scope of this paper. We just emphasize that both the synthesis and implementation of our method are done in the \emph{closed loop transfer matrices domain}, which avoids the non-convexity in \eqref{eq:trad}.

%\textcolor{blue}{For example, one may want the control action $u_1$ at node $1$ in Fig. \ref{fig:Chart105} to use the measurements $y_i$ from node $i = 1, \dots, 5$ only. This is equivalently saying that the delay from measurements $y_i$ for node $i = 6, \dots, 10$ to the control action $u_1$ at node $1$ is set to be infinity. This information sharing constraint is not QI, and \eqref{eq:trad} becomes non-convex. In fact, using the delay interpretation of QI in \cite{2010_Rotkowitz_QI_delay}, the sparsity constraint for a plant with strongly connected topology is not QI in general.}

==> Implementation_v1.tex <==
In this section, we discuss how to use \eqref{eq:localized} to design a distributed controller that is scalable to implement. We begin with the general idea on how to specify the locality constraint $\Ell$ in \eqref{eq:localized} as a constraint for controller implementation. We then focus on a special class of locality constraint and discuss its relation to the interconnected topology of the networked system. Finally, we discuss some technical conditions on the system in which \eqref{eq:localized} is feasible with the locality constraint.

\subsection{General Idea}
%Note that the optimization problem \eqref{eq:LOC} is convex if the objective function is convex and the localizability constraint $\s$ in \eqref{eq:main_S} is a convex set. In this paper, we further express the localizability constraint $\s$ as the intersection of three convex set components: the locality (sparsity) constraint $\Ell$, the finite impulse response (FIR) constraint $\FT$, and an arbitrary convex set component $\Sother$. In this case, the localized optimal control problem is given by
%\begin{eqnarray}
%\underset{\{\tf R, \tf M,\tf N, \tf L\}}{\text{minimize}} \quad && g(\tf R,\tf M,\tf N,\tf L) \nonumber\\
%\text{subject to} \quad && \eqref{eq:main_1} - \eqref{eq:main_stable} \nonumber \\
%&& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \cap \Sother. \label{eq:localized}
%\end{eqnarray}
%We assume that the problem \eqref{eq:localized} has a feasible solution.
%The components of the localizability constraint in \eqref{eq:localized} is interpreted in the following way. The constraint $\Sother$ includes any convex constraint imposed by the system, including the information sharing constraint $\C$ as one of its component. Constraints $\FT$ and $\Ell$ are the additional constraints we imposed to enhance the scalability of controller synthesis and controller implementation. 
Theorem \ref{thm:1} shows how the sparsity of the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ translates into the implementation complexity of a controller as in \eqref{eq:implementation}. If the rows of these transfer matrices are suitably sparse, then each sub-controller only needs to collect the information from a small number of subsystems to compute its control law. The locality constraint $\Ell$ is the mechanism that we use to impose this sparsity.  

% General principle
The role of the locality constraint $\Ell$ is two fold: we can interpret $\Ell$ as a constraint on the desired closed loop response, and/or a constraint for controller implementation. As an example, consider the closed loop transfer matrix $\tf N_{ij}$ which maps the disturbance $\ttf{\delta_{y_j}}$ at subsystem $j$ to the state $\tf{x_i}$ at subsystem $i$. When we impose the constraint $\tf N_{ij} = 0$, we try to make the state $\tf{x_i}$ uncorrelated to $\ttf{\delta_{y_j}}$ in the \emph{closed loop}. Suppose that \eqref{eq:main_1} - \eqref{eq:main_stable} remains feasible with the additional constraint $\tf N_{ij} = 0$. Applying Theorem \ref{thm:1}, the desired closed loop response can be achieved by the implementation \eqref{eq:implementation}, so the disturbance $\ttf{\delta_{y_j}}$ does not affect the state $\tf{x_i}$ in the closed loop. Meanwhile, as the controller is implemented by \eqref{eq:implementation}, the controller state $\ttf{\beta_i}$ at subsystem $i$ can be computed without knowing the measurement $\tf{y_j}$ at subsystem $j$. In other words, the constraint $\tf N_{ij} = 0$ can be considered as a sparsity constraint for controller implementation. The same argument holds for $\tf R$, $\tf M$, $\tf N$, and $\tf L$ for any $i$ and $j$.

%The locality constraint $\Ell$ can also be interpreted as a constraint for controller implementation. For instance, suppose that there exists a feasible solution of \eqref{eq:main_1} - \eqref{eq:main_stable} with the constraint $\tf L_{ij} = 0$. The controller achieving the desired closed loop response can be implemented by \eqref{eq:implementation}. As $\tf L_{ij} = 0$, the controller $\tf{u_i}$ at subsystem $i$ can be computed without knowing the measurement $\tf{y_j}$ at subsystem $j$. The same argument holds for $\tf R$, $\tf M$, and $\tf N$ with any $i$ and $j$ as well.
%Combining the above two arguments, we have the following general principle:
%\begin{principle}
%If the variable $(x_i, u_i)$ can be made unaffected by the disturbance $(\delta_{x_j}, \delta_{y_j})$ in closed loop, then the controller 
%\end{principle}
%
%\begin{remark}
%This 
%\end{remark}

From the above argument, we can impose the sparsity constraint on the closed loop transfer matrices to make the controller scalable to implement. Note that the optimization problem \eqref{eq:localized} is convex for any locality constraint $\Ell$. This is one of the primary advantage of the localized optimal control framework over the distributed optimal control framework in \eqref{eq:trad}, where the sparsity constraint imposed on \eqref{eq:trad_info} generally makes the problem non-convex. However, it should be noted that \eqref{eq:localized} may not be feasible with respect to an arbitrary locality constraint $\Ell$. Some design issues of the locality constraint is discussed in the last subsection of this section.

%In other words, the sparsity constraint imposed on the controller implementation is convex with respect to the localized optimal control problem.
%\eqref{eq:localized} with the controller implementation \eqref{eq:implementation}. 
%over the  

%For instance, let $(u_j, \beta_j, y_j)$ be the information at subsystem $j$. Due to the communication constraint, this information can only be shared with subsystem $k$ within some set $k \in \mathcal{V}_j$. In this case, we impose the constraint such that $\tf R_{ij} = 0$, $\tf M_{ij} = 0$, $\tf N_{ij} = 0$, and $\tf L_{ij} = 0$ for all $i \not \in \mathcal{V}_j$. Using the controller implementation \eqref{eq:implementation}, 
%we can impose the constraint such that $\tf R_{ij} = 0$, $\tf M_{ij} = 0$, $\tf N_{ij} = 0$, and $\tf L_{ij} = 0$ for all $i \not \in \mathcal{V}_j$. 
%suppose that the control action $u_i$ at sub-system $i$ does not have access to the measurement $y_j$
%By imposing the sparsity constraints on the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ through the locality constraint $\Ell$, the controller achieving the desired closed loop response can be implemented by sparse transfer matrices $(\tf{\tilde{R}^+}, \tf{\tilde{M}}, \tf{\tilde{N}}, \tf L)$ as in \eqref{eq:implementation} in a localized and scalable way.

% Feasibility
% Benefit / hold true for any g, S / partial nestedness
%Note that any sparsity constraint imposed through \eqref{eq:main_S} is a convex set constraint, so the optimization problem \eqref{eq:LOC} is convex. The reason why the localized optimal control framework can avoid the non-convexity present in the QI framework is that both the controller synthesis and controller implementation are performed in the \emph{closed loop transfer matrices} domain. 

%The locality constraint $\Ell$ is the mechanism that we use to impose this sparsity.  
%Although the localizability constraint seems to be a constraint for the closed loop response, it can also be interpreted as a constraint for controller implementation as the controller can be implemented using the closed loop transfer matrices. 
%By imposing the sparsity constraints on the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ through \eqref{eq:main_S}, the controller achieving the desired closed loop response can be implemented by sparse transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ in a localized and scalable way. 
%For example, the constraint $\FT$ restricts the optimization variables to have finite impulse responses of horizon $T$. In this case, problem \eqref{eq:localized} becomes a finite dimensional convex program. In addition, the controller achieving the desired closed loop response can be implemented by FIR filters using the structure given in Theorem \ref{thm:1}. The role of $\Ell$ is explained as follows.

\subsection{Physical Interpretation}
To help the reader get the intuition of our method, we focus on a special class of locality constraint called the $d$-localized constraint \cite{2014_Wang_Allerton, 2015_Wang_H2} in this subsection. The $d$-localized constraint is specified according to the interconnected topology of the networked system with a single parameter $d$. We begin by the following definitions.
\begin{definition}
Consider the interconnected system \eqref{eq:interconnected} with an interaction graph $\mathcal{G}$. The distance from subsystem $j$ to subsystem $i$ is defined by the length of the shortest path from node $j$ to node $i$ in the graph $\mathcal{G}$, and is denoted by $\dist{j}{i}$.
\end{definition}
%With the notion of distance, we define the $d$-outgoing and incoming sets at a subsystem $j$ as follows.
\begin{definition}
The $d$-outgoing set of subsystem $j$ is defined by $\Down{j}{d}:= \{i | \dist{j}{i} \leq d\}$, and the $d$-incoming set of subsystem $j$ is defined by $\Up{j}{d} := \{i | \dist{i}{j} \leq d\}$.
\end{definition}

%We begin by defining the notion of the $d$-outgoing and incoming sets at a subsystem $j$. To do so, we let the distance $\dist{j}{i}$ from subsystem $j$ to subsystem $i$ be given by the length of the shortest path from node $j$ to node $i$ in the graph $\mathcal{G}$.  
%We say that a set $\mathcal{D}$ of subsystems is of size $d$ if $\dist{i}{j}\leq d$ for all $i,j \in \mathcal{D}$. By definition, both the sets $\Down{j}{d}$ and $\Up{j}{d}$ are of size $d$. 
%We then define the $d$-outgoing set of subsystem $j$ as $\Down{j}{d}:= \{i | \text{dist}(j \to i) \leq d\}$, and the $d$-incoming set of subsystem $j$ as $\Up{j}{d} := \{i | \text{dist}(i \to j) \leq d\}$ -- by definition, both of these sets are of size $d$.  
%To help the readers follow the content, we create the following simple example in the form of \eqref{eq:interconnected}. This example is used to illustrate several ideas throughout the paper.
%\begin{example}
%Consider a network system with an undirected interaction topology as illustrated in Fig. \ref{fig:Chart105}. Each subsystem $i$ is assumed to have a scalar state $x_i$, a scalar control $u_i$, and a scalar measurement $y_i$. The dynamics for each subsystem $i$ are given by
%\begin{eqnarray}
%x_i[k+1] &=& x_i[k] + u_i[k] + \sum_{j \in \mathcal{N}_i} x_j[k] + \delta_{x_i}[k]\nonumber\\
%y_i[k] &=& x_i[k] + \delta_{y_i}[k]. \label{eq:interconnected_s}
%\end{eqnarray}
%As the interaction graph is undirected, we have that $\Down{j}{d} =  \Up{j}{d}$ for all $j$ and $d$. For example, $\Down{1}{2} =  \Up{1}{2} = \{1,2,3,4\}$.
%\end{example}
%\begin{figure}[h!]
%      \centering
%      \includegraphics[width=0.32\textwidth]{./figure/Topology.pdf}
%      \caption{Illustrative Example}
%      \label{fig:Chart105}     
%\end{figure}
\begin{example}
For a system \eqref{eq:interconnected} with interaction graph illustrated in Fig.
\ref{fig:Chart105}, the $2$-incoming and $2$-outgoing sets of subsystem $5$ are
given by $\Up{5}{2} = \{2,3,4,5\}$ and $\Down{5}{2} = \{5,6,7,8,9,10\}$,
respectively.
\end{example}
\begin{figure}[h!]
     \centering
     \includegraphics[width=0.25\textwidth]{./figure/Topology2.pdf}
     \caption{Illustration of the $2$-incoming and $2$-outgoing sets of subsystem $5$.}
     \label{fig:Chart105}
\end{figure}

%Our approach to making the controller synthesis task specified in optimization problem \eqref{eq:localized} scalable is to confine, or \emph{localize} the effects of the process and sensor disturbances to a $d$-outgoing set at each subsystem $j$, for a size $d$ much smaller than that of $\mathcal{V}$.  As we make precise in the sequel, this implies that each sub-controller $j$ only needs to collect data from subsystems $i$ contained in its $d$-incoming set $\Up{j}{d}$.

To make the controller implementation scalable, we begin by \emph{localizing} the effects of the process and sensor disturbances at each subsystem $j$ to its $d$-outgoing set for a sufficiently small $d$. This leads to the $d$-localized constraint defined as follows.
\begin{definition}
Let $\tf R_{ij}$ denote the closed loop mapping from the perturbation $\ttf \delta_{x_j}$ at sub-system $j$ to the state $\tf x_i$ at sub-system $i$. The closed loop transfer matrix $\tf R$ is said to be $d$-localized if the effect of each perturbation $\ttf \delta_{x_j}$ is contained within the set $\Down{j}{d}$. Specifically, we have $\tf R_{ij} = 0$ for all $i \not \in \Down{j}{d}$ and for all $j$. 
\end{definition}

%Likewise, we can 
%Specifically, we say that the transfer matrix $\tf R$ mapping the state disturbance $\ttf \delta_x$ to the state $\tf x$, as defined in \eqref{eq:desired}, is $d$-localized if 
%, for a size $d$ much smaller than that of $\mathcal{V}$.
%With this approach in mind, we say that the transfer matrix $\tf R$ mapping the state disturbance $\ttf \delta_x$ to the state $\tf x$, as defined in \eqref{eq:desired}, is $d$-localized if its impulse response can be appropriately covered by $d$-outgoing sets. In particular, if we let $\tf R_{ij}$ denote the transfer function from the perturbation $\ttf \delta_{x_j}$ at sub-system $j$ to the state $\tf x_i$ at sub-system $i$, then the map $\tf R$ is $d$-localized if and only if for every subsystem $j$, $\tf R_{ij} = 0$ for all $i \not \in \Down{j}{d}$.  In words, this says that the transfer matrix $\tf R$ is $d$-localized if and only if the effect of each disturbance is contained, or localized, to within a region of size $d$. 
This definition can be extended to the remaining transfer matrices $\tf M$, $\tf N$, and  $\tf L$ of \eqref{eq:desired} in a natural way.  The closed loop response \eqref{eq:desired} of the system is said to be $d$-localized if its constituent components $(\tf R,\tf M,\tf N,\tf L)$ are as well.  Finally, the locality constraint $\Ell$ in \eqref{eq:localized} imposes a $d$-localized constraint if it constrains its elements to be $d$-localized closed loop responses.
%In addition, we define a localized closed loop response as follows. 
%Consider the transfer matrix $R$ that maps the perturbation $\delta_x$ to the internal variable $x$. Denote $R_{ij}$ the submatrix of $R$ that maps the perturbation $\delta_{x_j}$ at sub-system $j$ to the state $x_i$ at sub-system $i$. The transfer matrix $R$ is said to be $d$-localized if $R_{ij} = 0$ for $i \not \in $ Down$(j,d)$ for all $j$. In this case, we say that the effect of each local perturbation $\delta_{x_j}$ is localized within the region Down$(j,d)$. We can define $d$-localized property for $N, M, L$ in \eqref{eq:desired} in a similar way. A closed loop transfer matrix in \eqref{eq:desired} is said to be $d$-localized if all its four components $(R,N,M,L)$ are $d$-localized.

%Given a transfer matrix $G$ mapping the perturbation $\delta_x$ or $\delta_y$ to the internal variable $x$ or $u$. Denote $G_{ij}$ the submatrix of $G$ that maps the perturbation $\delta_{x_j}$ or $\delta_{y_j} $at sub-system $j$ to the internal variable $x_i$ or $u_i$ at sub-system $i$. A transfer matrix $G$ is said to be $d$-localized if $G_{ij} = 0$ for $i \not \in $ Down$(j,d)$ for all $j$. In this case, we say that the effect of each local perturbation $\delta_{x_j}$ or $\delta_{y_j}$ is localized within the region Down$(j,d)$. A closed loop transfer matrix in \eqref{eq:desired} is said to be $d$-localized if all its four components $(R,N,M,L)$ are $d$-localized.

%Now we consider the case in which $\s$ enforces a $d$-localized constraint on $(R,N,M,L)$. 
With these definitions and results in hand, our approach to synthesizing a controller that is scalable to implement is straightforward: we choose the subspace $\Ell$ to be a $d$-localized constraint and select a horizon $T$ for the FIR subspace $\FT$.  Whereas the first constraint ensures that the transfer matrices solving optimization problem \eqref{eq:localized} are $d$-localized, the second constraint is imposed to make the optimization problem finite dimensional. The resulting optimization problem \eqref{eq:localized} is easily seen to be convex as the constraints are all affine: if it is feasible, then the resulting closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ can be used to implement a controller as specified by Theorem \ref{thm:1} (note that the modified transfer matrices $( \tilde{\tf R}^+,  \tilde{\tf M},  \tilde{\tf N})$ are also $d$-localized).  Further, since the closed loop response is $d$-localized, each sub-controller only needs to collect data from other subsystems that are at most a distance $d$ away.  In particular, the row sparsity of the transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ is defined by the $d$-incoming sets of the system, and thus the control action $\tf u_i$ and internal state $\ttf \beta_i$ of sub-controller $i$ can be computed by collecting the data $(\tf y_j, \ttf \beta_j)$ from subsystems $j$ in the $d$-incoming set $\Up{i}{d}$. This discussion shows that a controller synthesized via optimization problem \eqref{eq:localized} and implemented according to Theorem \ref{thm:1} is scalable to implement, as the amount of information collected at a given subsystem is specified by the $d$-localized constraint $\Ell$, and hence is independent of the number of subsystems $n$.

\subsection{Feasibility and Design Issues}
Before proceeding, we note that although optimization problem \eqref{eq:localized} is convex for any affine constraint set $\Ell$, it is not necessarily feasible.  This is because the subsystems are dynamically coupled to each other (as per \eqref{eq:interconnected}), and hence it may not always be possible to localize the effect of a disturbance affecting subsystem $j$ to a pre-specified $d$-outgoing set $\Down{j}{d}$.  Intuitively, optimization problem \eqref{eq:localized} is feasible when the communication constraint (contained in the component $\Sother$ in \eqref{eq:localized}) is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant.  In this way, the necessary sub-controllers can take action \emph{before} a disturbance perturbs their subsystem and stop it from propagating to the rest of the system.  Implicit in this argument are the assumptions that information can be shared quickly between sub-controllers, and that sensors and actuators are strategically placed (these assumptions are discussed in detail in \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}).

Based on this intuition, we provide simple rules for how to select the size $d$ of the localized subspace constraint $\Ell$, the horizon $T$ of the FIR subspace constraint $\FT$, as well as a principled approach to designing the actuation scheme of the system (i.e., the matrix $B_2$) in the paper \cite{2015_Wang_Reg}.  For the remainder of the paper, we assume that the constraint sets $\Ell$ and $\FT$ are given, and that the communication, actuation and sensing architecture of the system is such that optimization problem \eqref{eq:localized} is feasible.

%First, we should note that a localized closed loop response does not mean that the open loop response is localized, so our method is still applicable for large-scale coupled network systems. 
%However, we do need some assumptions to ensure the existence of a localized closed loop response: (1) the communication speed is faster than the speed of disturbance propagated in the plant, and (2) the locations of the sensor and actuator are properly chosen. 
%Therefore, even though the open loop response is coupled to each other, it is still possible to achieve a $d$-localized closed loop response by designing the control action properly.
 %Note that our method do require the following assumptions: (1) fast information sharing, and (2) properly chosen locations of sensor and actuator.
%These conditions are discussed in our other works \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}. In particular, we give some simple rules to \emph{design} the spatio-temporal constraint $\s$ and the actuator locations ($B_2$) in \cite{2015_Wang_Reg}. In this paper, we assume that $\s$ is given before synthesis.
%
% 
%
%
%
%As mentioned the localized subspace constraint $\Ell$ and FIR horizon $T$ are design parameters in the controller synthesis problem.  We provide simple rules for how to select these parameters, as well as a principled approach to designing the actuation scheme of the system (i.e., the matrix $B_2$) in our companion paper  \cite{2015_Wang_Reg}.  For the remainder of the paper, we assume that the horizon $T$ has been set and that the subspace constraint $\Ell$ is $d$-localized.  
%Now we use $\s$ in \eqref{eq:local_S} to enforce the $d$-localized constraint on the closed loop. If \eqref{eq:local1} - \eqref{eq:local_S} is still feasible, then Theorem \ref{thm:1} suggests that the controller achieving the desired localized closed loop can be realized using $d$-localized stable transfer matrices $(\tilde{R}^+, \tilde{N}, \tilde{M}, L)$ by \eqref{eq:implementation}. By interpreting the implementation \eqref{eq:implementation} row at a time, we can show that the control information $(u_i, \beta_i)$ at each sub-system $i$ can be computed by collecting the information $(y_j, \beta_j)$ locally within the set $j \in \text{Up}(i,d)$. This implies that the controller can be implemented in a localized and scalable way. 
%For instance, local controller $u_i$ can be computed using only \emph{some} measurement $y_j$ and \emph{some} controller state $\beta_j$, as long as the $i$th rows of the matrices $\tilde{M}$ and $L$ are sparse. If we specify the sparsity pattern on the closed loop transfer matrices properly, local controller $u_i$ only needs to collect the information locally to compute its control action.

%Another benefit of our formulation is that \eqref{eq:local_obj} - \eqref{eq:local_S} is a \emph{convex} optimization problem for \emph{arbitrary} sparsity constraint $\s$, which is different from the traditional formulation \eqref{eq:trad}. The mathematical relation between the traditional formulation and our new formulation is beyond the scope of this paper. We just emphasize that both the synthesis and implementation of our method are done in the \emph{closed loop transfer matrices domain}, which avoids the non-convexity in \eqref{eq:trad}.

%\textcolor{blue}{For example, one may want the control action $u_1$ at node $1$ in Fig. \ref{fig:Chart105} to use the measurements $y_i$ from node $i = 1, \dots, 5$ only. This is equivalently saying that the delay from measurements $y_i$ for node $i = 6, \dots, 10$ to the control action $u_1$ at node $1$ is set to be infinity. This information sharing constraint is not QI, and \eqref{eq:trad} becomes non-convex. In fact, using the delay interpretation of QI in \cite{2010_Rotkowitz_QI_delay}, the sparsity constraint for a plant with strongly connected topology is not QI in general.}

==> Intro_v4.tex <==
\IEEEPARstart{L}{arge-scale} networked systems permeate both modern life and academic research, with familiar examples including the Internet, smart grid, wireless sensor networks, and biological networks in science and medicine. The scale of these systems pose fundamental challenge for controller design: simple local controllers generated by heuristics cannot guarantee global performance (or at times even stability), whereas a traditional centralized controller is neither scalable to compute, nor physically implementable. Specifically, the synthesis of a centralized optimal controller requires solving a large-scale optimization problem with the knowledge of \emph{global} plant model. In addition, the information in the network is assumed to be collected \emph{instantaneously}. The scale of the problem and the practical communication delay degrade the performance of centralized scheme substantially and make it unappealing to large systems.
 
In order to incorporate realistic communication constraints amongst sensors, actuators, and controllers into the control design process, the field of distributed (decentralized) optimal control has emerged. By imposing an additional subspace constraint on the controller, a distributed optimal control problem is commonly formulated as
\begin{eqnarray}
\underset{\tf K}{\text{minimize  }} && || f(\tf P,\tf K) || \nonumber\\
\text{subject to }  && \tf K \text{ internally stabilizes } \tf P \nonumber\\
&& \tf K \in \C,  \label{eq:intro}
\end{eqnarray}
where $\tf P$ is the plant, $\tf K$ the controller, $f(\tf P,\tf K)$ the closed-loop mapping, and $\C$ the information sharing constraint that $\tf K$ needs to satisfy. The tractability of \eqref{eq:intro} depends on the relations between the information sharing constraint $\C$ and the plant $\tf P$, and it can be NP-hard for certain information structures \cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. It has been shown that \eqref{eq:intro} admits a convex reformulation in the Youla domain \cite{1976_Youla_parameterization} if \cite{2006_Rotkowitz_QI_TAC} and only if \cite{2014_Lessard_convexity} $\C$ is quadratically invariant (QI) with respect to the plant.
%Roughly speaking, constraints imposed by communication networks that allow exchange of information between controllers faster than dynamics propagate through the plant can be handled in a convex way.
Roughly speaking, quadratic invariance condition holds when the communication speed is faster than the speed of disturbance propagation in the physical system \cite{2010_Rotkowitz_QI_delay}. 
With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal, 2014_Lamperski_state, 2014_Matni_Hinf, 2012_Lessard_two_player, 2014_Lessard_Hinf, 2013_Scherer_Hinf, 2011_Shah_poset_causal} in finding finite dimensional reformulations of the optimal control problem or deriving explicit formulas for specific structured systems.

%Much progress has been made \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal, 2014_Lamperski_state, 2014_Matni_Hinf, 2012_Lessard_two_player, 2014_Lessard_Hinf, 2013_Scherer_Hinf, 2011_Shah_poset_causal} on extending the QI for specific structure or finite dimensional reformulation of the optimal control problem in recent years.
%With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made on the field of distributed control.
%If the information sharing constraint is quadratically invariant (QI) with respect to the plant, then the distributed optimal control problem can be formulated in a convex manner \cite{2006_Rotkowitz_QI_TAC, 2010_Rotkowitz_QI_delay} by Youla parametrization \cite{1976_Youla_parameterization}.  With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made in finding finite dimensional reformulations of the optimal control problem.

%Although the communication delay constraint is well-handled in the field of distributed control, the synthesis and the implementation of those controllers are still not scalable.
%As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}.  Although the computed controllers respect the information sharing constraints of the problem, 
Although the distributed optimal control problem with a QI information sharing constraint is computationally tractable (i.e., convex), both the controller synthesis and implementation scale with the dimension of the full system, and thus are not practical for large systems.
%As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large-scale systems: \emph{scalability}. 
%In all of the above, the resulting optimal controller is as difficult to compute as its centralized counterpart, and even more demanding to implement.
In fact, for a plant with a strongly connected topology, even as simple as a chain, the QI condition implies that local measurements need to be shared among \emph{all} sub-controllers in the network (which can be inferred from \cite{2010_Rotkowitz_QI_delay} and \cite{2009_Swigart_graph_QI}). This then implies that finding an optimal sparse controller $\tf K$ in \eqref{eq:intro} (which is defined as the transfer function from measurement to control action) for a strongly connected plant cannot be formulated in a convex manner in the Youla domain. 

%Based on this discussion, we argue that the closed loop behavior achieved by these distributed optimal controllers should be viewed as fundamental limits on performance, that we should strive to attain via more \emph{scalable} and \emph{realistically implementable} control schemes.

The idea of designing localized (sparse) controllers to improve scalability and ease of implementation has been applied on some special class of systems, such as the spatially invariant systems \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant, 2005_Jovanovic_localized} and the spatial decaying systems \cite{2008_Motee_distributed, 2014_Motee_spatially_decaying}. 
Regularization \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting}, convex approximation \cite{2014_Fazelnia_ODC, 2014_Sznaier}, and spatial truncation \cite{2009_Motee_spatial_truncation} have also been used in hopes of finding a near optimal distributed static feedback controller that is scalable to implement. These methods have been successful in extending the size of systems for which a distributed controller can be computed, but there is still a limit to their scalability as they often rely on an underlying centralized synthesis procedure. 
The methods described in \cite{2004_Dullerud, 2013_Farokhi_model} may provide scalable ways to synthesize distributed controller with limited model information, but they can be conservative. 
Finally, it is not clear if these methods can be extended to compute a dynamic controller that incorporates information sharing constraints.

%Although the nonconvex problem can possibly be solved approximately \cite{2014_Fazelnia_ODC, 2011_Rotkowitz_subspace}, the computational complexity of the approximated algorithm still does not scale gracefully to large scale the size of the network requires solving a large-scale optimization problem with the knowledge of global plant model information.
%Regularization or approximation have also been used in hopes of finding a sparse controller. Representative works include sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting} and spatial truncation method \cite{2009_Motee_spatial_truncation}.
%The synthesis of these methods, however, is still centralized, which requires global plant model information. 
%Part of the reason is that the controller synthesis and implementation of those methods are in the ``$K$" domain.

In our previous works \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_H2}, we point out the fact that a localized (and thus sparse and scalable) controller implementation does not necessarily imply that the transfer matrix $\tf K$ in \eqref{eq:intro} needs to be sparse. In fact, by using implicit implementations of the controller (which allow the communication of both \emph{measurements and controller states}, or \emph{estimated disturbance and reference trajectory}), we show that the distributed controller can be implemented in a localized way even when the transfer matrix $\tf K$ is not sparse. Therefore, we change the last constraint $\tf K \in \C$ in \eqref{eq:intro} slightly and formulate the localized optimal control problem as
%\footnote{If we want to find a non-strictly proper optimal controller for a discrete time system, we search for proper $L$ instead of strictly proper $L$ in \eqref{eq:main_stable}.}
\begin{subequations} \label{eq:LOC}
\begin{align}
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize    }} & \quad g(\tf R,\tf M,\tf N,\tf L) \label{eq:main_obj}\\
\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} = 
\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:main_1} \\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix}
\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:main_2} \\
&  \tf R, \tf M, \tf N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad \tf L \in \mathcal{RH}_{\infty} \label{eq:main_stable}\\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \mathcal{S} \label{eq:main_S}
\end{align}
\end{subequations}
where $\tf R, \tf M, \tf N, \tf L$ are \emph{closed loop transfer matrices} (this will be formally defined in Section \ref{sec:parameter}), $g(.)$ a convex objective function, $(A, B_2, C_2)$ the state space matrices of the plant model, and $\mathcal{S}$ a convex set. The goal of this two-part paper is to show that the new formulation in \eqref{eq:LOC} has various benefits over the traditional formulation in \eqref{eq:intro}, especially on handling the constraint \eqref{eq:main_S} for large-scale systems.

The two-part paper is organized in the following way. In the first part of the paper, we establish the fundamental theory of the localized optimal control problem \eqref{eq:LOC}. We focus on the mathematical relations between the distributed optimal control formulation \eqref{eq:intro} and the localized optimal control formulation \eqref{eq:LOC}, and show that \eqref{eq:LOC} contains a much broader class of convex problems than \eqref{eq:intro}. In the second part of the paper, we explain why the formulation \eqref{eq:LOC} is much more favorable to apply on large-scale networked systems. In particular, under some technical conditions, the localized optimal controller for a large-scale system can both be designed \emph{and} implemented in a localized and scalable way. 

The rest of the first-part paper is structured as follows. Section \ref{sec:prelim} introduces the system model and the traditional formulation \eqref{eq:intro}. We then explain why the formulation \eqref{eq:intro} is not amenable to large-scale problems, which motivates our work on the alternative formulation \eqref{eq:LOC}. The discussion in Section \ref{sec:parameter} focuses on the constraints \eqref{eq:main_1} - \eqref{eq:main_stable}. In particular, we show that the solution $(\tf R, \tf M, \tf N, \tf L)$ for \eqref{eq:main_1} - \eqref{eq:main_stable} parameterizes \emph{all achievable stable closed loop transfer matrices}, and the parameterization of all stabilizing controller can be constructed by the transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ directly. In Section \ref{sec:localizability}, we include the localizability constraint \eqref{eq:main_S} and the objective function \eqref{eq:main_obj} into the discussion. Specifically, we introduce the notion of $\mathcal{S}$-\emph{localizability} as the feasibility of \eqref{eq:main_1} - \eqref{eq:main_S}, and discuss the relations between the conventional formulation \eqref{eq:intro} and the new formulation \eqref{eq:LOC}. Several classes of $\mathcal{S}$-localizability constraint are discussed in Section \ref{sec:class}. In particular, we show that the QI constraints, controllability and observability constraints, and the $(d,T)$-localizability constraints \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton} are all special case of $\mathcal{S}$-localizability constraint.
When sparsity constraint is imposed through \eqref{eq:main_S}, the controller achieving the desired closed loop response can further be implemented by sparse transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ in a localized and scalable way.
Finally, conclusions are given in Section \ref{sec:conclusion}.
%contains a wide range of different problems as special cases, including distributed control problem with QI constraints, the controllability and observability problems of a network system, and our previous work on $(d,T)$-localizable systems \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}. 
%The objective function \eqref{eq:main_obj} is discussed in Section \ref{sec:synthesis}. 
%we discuss how to apply our alternative formulation for large-scale controller synthesis with implementation constraints. 
%In addition, for some specific objective functions, such as the $\mathcal{H}_2$ norm with some sparsity constraints, the optimization problem \eqref{eq:main_obj} - \eqref{eq:main_S} can be solved in a localized and parallel way by utilizing the technique in distributed optimization. 
%In Section \ref{sec:synthesis}, we show that for certain objective functions with certain $\mathcal{S}$-localizability constraint, the optimization problem \eqref{eq:main_obj} - \eqref{eq:main_S} can be decomposed into several localized optimization problems.
%For each localized optimization subroutine, only the \emph{localized plant model information} is required. 
%This provides a scalable way to synthesize the localized optimal controller for large-scale systems.
%Finally, simulation results are shown in Section \ref{sec:simu}, and the conclusions and some future research direction are summarized in Section \ref{sec:conclusion}.

\subsection*{Comparison With Prior Publications by the Authors} 
In this paper, we establish a coherent theoretical framework for our previous results in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_H2, 2015_Wang_LDKF} based on the parameterization of all stabilizing controllers using the closed loop transfer matrices. 
With this new framework, we generalize our previous results substantially in the following sense.
\begin{enumerate}
\item We show that the solution $(\tf R, \tf M, \tf N, \tf L)$ in \eqref{eq:main_1} - \eqref{eq:main_stable} parameterizes the closed loop achieved by an internally stabilizing controller. We also give an explicit formula to parameterize all internally stabilizing controller using the closed loop transfer matrices.
\item Based on the parameterization of all internally stabilizing controllers, we extend the output feedback scheme in \cite{2014_Wang_Allerton} to unstable plants. In addition, we provide a rigorous proof on the internally stability of the controller structures proposed in \cite{2014_Wang_CDC} and \cite{2014_Wang_Allerton}.
\item The notion of $\mathcal{S}$-localizability constraint is introduced as an additional convex set constraint imposed on the closed loop transfer matrices, which is a generalization of $(d,T)$-localizability constraints proposed in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}. We further show that the QI constraint, controllability and observability constraints, and many other constraints can all be interpreted as special cases of $\mathcal{S}$-localizability constraint.
%\item The robustness of the localized controller implementation with respect to model uncertainty or various source of error is rigorously analyzed. In particular, we give a simple sufficient condition on output feedback stabilizability for \emph{nearly} localizable systems.
%\item We provide a localized synthesis algorithm for the localized optimal controller with decomposable performance metrics. This is a generalization of our previous works in \cite{2014_Wang_CDC} and \cite{2015_Wang_H2}, which focus on quadratic objective functions.
%localized synthesis algorithm for a class of $\mathcal{H}_2$ problem based on the alternating direction method of multipliers (ADMM)\cite{BoydADMM}.
\end{enumerate}

%With this innovation on controller implementation, we create a whole new control theory, which we call \emph{localized distributed control}, that is extremely favorable for large-scale systems.

%Specifically, we argue that \eqref{eq:intro} is not the only way, and even not a good way, to formulate the optimal control problem with communication constraint.

%Specifically, in \cite{2014_Wang_ACC}, we introduced the notion of a state feedback localizable system. The basic concept is the following observation: when the communication speed is faster than the speed of disturbance propagation, it is possible to localize the effect of each local disturbance. We define this as the notion of state feedback localizability of a system, which is a natural extension of controllability in a space-time region. We show in \cite{2014_Wang_ACC, 2014_Wang_CDC} that a state feedback localizable system achieves the following properties.

%\textbf{Closed Loop Response}
%\begin{enumerate}
%\item The effect of each local disturbance is limited in a localized region in finite time.
%\item The transient performance can be close to the idealized centralized global optimal one by selecting the localized region appropriately. 
%\end{enumerate}
%
%\textbf{Controller Implementation}
%\begin{enumerate}
%\item The controller achieving the desired closed loop response can be implemented in a \emph{localized} way by FIR filters. Each local controller only needs to communicate with some of its neighbors to generate its control action.
%\item The controller can be implemented with communication delay as long as the communication speed is faster than the speed of disturbance propagation.
%\end{enumerate}
%
%\textbf{Controller Synthesis}
%\begin{enumerate}
%\item For linear quadratic regulator (LQR) cost, the global optimal controller (subject to localized constraints) can be synthesized in a localized way by solving localized LQR (LLQR) problems following a local update procedure.
%\item Each LLQR sub-problem only depends on the plant model locally. When the plant model changes locally, only some local optimization problems need to be resolved to maintain global optimality. This allows incremental design when the physical system expands.
%\end{enumerate}

%The implication of these properties is that we have a systematic way to practically synthesize and implement the controller for a large-scale system with nearly optimal transient performance. In addition, disturbance propagation can be limited in a localized region without using a centralized coordinator. Both features significantly enhance robustness and scalability for a large-scale system. Note that many of these properties cannot be achieved with the formulation in \eqref{eq:intro}.

%\subsection{Comparison to other works}
%Besides the works in distributed optimal control, the idea of localized closed loop response, localized implementation, and localized synthesis have been addressed separately in different line of research.

%The idea of designing localized (sparse) controllers to improve scalability and ease of implementation has been applied on spatially invariant systems \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant}, and the inverse optimality condition is analyzed in \cite{2005_Jovanovic_localized}.
%In fact, the distributed optimal controller for a spatially invariant system is shown to have an inherent degree of localization, which makes the 
%The spatial localization property of the distributed optimal controller have been analyzed
%For instance, the localized optimal controller has been applied on spatially invariant systems in \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant}%For instance, it has been shown that the optimal controller for a spatially invariant system have an inherent degree of localization \cite{2002_Bamieh_spatially_invariant} and thus 
%It should also be noted that similar approaches to convex distributed optimal controller synthesis have been applied to spatially invariant systems satisfying a funnel causality property \cite{2002_Bamieh_spatially_invariant, 2005_Bamieh_spatially_invariant}.
%The method is generalized into spatial decaying systems in \cite{2008_Motee_distributed, 2014_Motee_spatially_decaying}. Regularization or approximation have also been used in hopes of finding a sparse controller. Representative works include sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting} and spatial truncation method \cite{2009_Motee_spatial_truncation}.

%Although the above-mentioned methods provide a scalable way to implement the distributed controller, the synthesis procedure is still centralized, which requires global plant model beforehand. The methods described in 
%\cite{2004_Dullerud, 2008_Borrelli_LQR, 2013_Farokhi_model} can provide scalable way to synthesize distributed controller with limited model information, but the method can be quite conservative. Part of the reason is that the controller synthesis and implementation of those methods are in the ``$K$" domain.

%\subsection{Contribution}
%We derived a direct relation between the closed loop response of the system and the controller implementation achieving the desired closed loop.  Building on these results, in \cite{2014_Wang_CDC} we showed how the computation and implementation of a linear quadratic regulator (LQR) optimal localizing state feedback law can be done in a completely localized (and hence scalable) manner. The result is further extended to output feedback in \cite{2014_Wang_Allerton}. Surprisingly, simulations in \cite{2014_Wang_CDC, 2014_Wang_Allerton} showed that the proposed localized controller achieved performance similar to that of a centralized optimal one, while being far superior in terms of the sparsity of implementation and the closed loop response.  We emphasize once again that this latter property is key for the scalability of this scheme.
%This paper provides a localized and thus scalable way to synthesize and implement the state feedback distributed controller for large-scale systems with arbitrary interconnected topology. 
%It is an extension of our previous result in \cite{2014_Wang_ACC, 2014_Wang_CDC} in the following sense.
%\begin{enumerate}
%\item The robustness of the localized controller implementation is rigorously analyzed by an extended notion of internal stability.
%\item A localized algorithm that computes the lower bound of global optimality is proposed. By comparing the relative cost of the feasible solution (upper bound) and the lower bound, one can dynamically choose the size of the localized region for each local disturbance.
%\item A simple condition on the spatial localizability is given. This provides a guideline for actuator placement that ensures spatial localizability. 
%\end{enumerate}
% 
%With these three extensions, we test our algorithm on a large-scale randomized example. With the scalable lower bound algorithm, we show that our controller achieve nearly global optimality without actually computing the cost of an idealized centralized controller. Finally, some of the notation and derivation in \cite{2014_Wang_ACC, 2014_Wang_CDC} are refined in this paper to enhance generality and readability.

%This paper summarizes our previous results on localized distributed control into a generalized framework. Specifically, we extend the result in \cite{2014_Wang_Allerton} to unstable system by redefining the notion of internal stability. The notion of localizability is also restated as a generalization of controllability and observability. Based on that, the localized distributed optimal control problem is formulated as a finite dimensional affinely constrained convex program, which can be solved by a localized way by standard distributed optimization technique. The controller can also be implemented in a localized way, and the robustness of the implementation is analyzed. Simulation shows that our localized (scalable) controller implementation can achieve similar transient response to a centralized optimal one.

%\subsection{Outline}
%The rest of this paper is organized as follows. Section \ref{sec:problem} introduces some preliminaries and formulate the LLQR problem. The spatio-temporal constraints in LLQR is then formally defined in Section \ref{sec:st_cons}. In Section \ref{sec:state}, we define the notion of state feedback localizability in terms of the feasibility of a set of linear equations, and show that the feasibility of the equations can be verified in a localized and parallel way. We then show that the LLQR problem can be decomposed in a similar way in Section \ref{sec:LLQR}. The localized implementation and synthesis procedure for the LLQR controller are provided in Section \ref{sec:imp}. Some extensions are discussed in Section \ref{sec:ext}, and the simulation results are shown in Section \ref{sec:simu}. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%The rest of this paper is organized as follows. Section \ref{sec:prelim} introduces the system model, spatio-temporal constraints, and some preliminaries on graph theory and distributed control. Section \ref{sec:state} starts with an illustrative example, and formally defines the notion of state feedback localizability later on. The localized LQR (LLQR) problem is formulated in Section \ref{sec:LLQR}. In particular, we show that LLQR problem can be solved by a completely localized and distributed way, and the resulting controller can also be implemented in a localized way. Section \ref{sec:output} extends the result into output feedback, and the localized distributed optimal control problem is formulated and solved in \ref{sec:localized}. Once again, both the controller synthesis and implementation are localized. Simulation results are shown in Section \ref{sec:simu} to illustrate the effectiveness of our method. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%The rest of this paper is organized as follows.

%\textbf{Mathematical Notations: } $\mathcal{RH}_{\infty}$ denotes the set of all real-rational stable proper transfer functions. $z$ is the variable of the z-transform. 
%Throughout this paper, we use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system.


==> LLQG_Intro_v2.tex <==
\IEEEPARstart{L}{arge-scale} networked systems have received much attention in industry and academia in recent years. The application area is extremely diverse, ranging from the Internet, transportation networks, power networks, wireless sensor networks, to biological network systems. The scale of these systems introduces fundamental challenge for controller design: the computational complexity of synthesizing and implementing a controller must be traded off against the closed loop performance that it achieves. For instance, although a centralized optimal controller achieves a globally optimal closed loop, it can be difficult to compute for large-scale systems, and impossible to implement due to realistic communication constraints between sensors, actuators and sub-controllers.%Specifically, the synthesis of the optimal centralized controller requires solving a large-scale optimization problem with the knowledge of \emph{global} plant model. In addition, the information in the network is assumed to be transmitted to the \emph{whole} network \emph{instantaneously}. The scale of the problem and the practical communication delay degrade the performance of centralized scheme substantially and make it unappealing to those systems.

In order to address some of these issues, the field of distributed (decentralized) optimal control has emerged, and allows for realistic communication constraints amongst local sensors, actuators, and sub-controllers to be explicitly incorporated into the design process. 
%By imposing an additional subspace constraints on the controller, a distributed optimal control problem is commonly formulated as
%\begin{eqnarray}
%\underset{K}{\text{minimize  }} && || F(P,K) || \nonumber\\
%\text{subject to }  && K \text{ stabilizes } P \nonumber\\
%&& K \in \mathcal{S}_c  \label{eq:intro}
%\end{eqnarray}
%where $P$ is the global plant, $K$ the controller, $F(P,K)$ the closed-loop mapping, and $\mathcal{S}_c$ the subspace constraint that $K$ needs to satisfy. 
%The information sharing constraint is commonly described by an additional subspace constraint imposed on the controller, 
%Specifically, a distributed optimal control problem is commonly formulated by incorporating an additional information sharing constraint on controller $\tf K$ (the transfer matrix from \emph{measurements} to \emph{control actions}) in the centralized optimal control formulation. 
A distributed optimal control problem is commonly formulated by imposing an information sharing constraint on the set of all internally stabilizing controller in the centralized optimal control problem.
%The communication constraint is commonly described by an information sharing constraint imposed on the set of all internally stabilizing controller.
The additional information sharing constraint makes the distributed optimal control problem significantly harder than its centralized counterpart, and certain problems are indeed NP-hard \cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. 
%The tractability of the resulting problem depends on the relationship between the information sharing constraint and the open loop system, and certain problems can indeed be NP-hard \cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. 
It has been shown that the distributed optimal control problem admits a convex reformulation in the Youla domain if \cite{2006_Rotkowitz_QI_TAC} and only if \cite{2014_Lessard_convexity} the information sharing constraint is quadratically invariant (QI) with respect to the plant.
%In the seminal works \cite{2006_Rotkowitz_QI_TAC} and recently in \cite{2014_Lessard_convexity}, the authors show that \eqref{eq:intro} admits a convex reformulation in the Youla domain \cite{1976_Youla_parameterization} if and only if $\mathcal{S}_c$ is quadratically invariant (QI) with respect to the plant. 
With the identification of quadratic invariance as a means of convexifying the distributed optimal control problem, tractable solutions for various types of distributed objectives and constraints have been developed \cite{2012_Lessard_two_player, 2014_Lamperski_H2_journal, 2014_Lamperski_state, 2014_Sabau_QI, 2014_Matni_Hinf, 2014_Lessard_Hinf, 2013_Scherer_Hinf}.
%Roughly speaking, QI condition holds when the communication speed is faster than the speed of disturbance propagation in the physical system \cite{2010_Rotkowitz_QI_delay}. 
%Much progress has been made \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal, 2014_Lamperski_state, 2014_Matni_Hinf, 2012_Lessard_two_player, 2014_Lessard_Hinf, 2013_Scherer_Hinf, 2014_Tanaka_Triangular, 2010_Shah_H2_poset, 2011_Shah_poset_causal} on extending the result of QI for specific structure or finite dimensional reformulation of the optimal control problem in recent years.

As promising and impressive as all of the results have been, the QI theory also suggests a fundamental difficulty of extending the distributed optimal control framework to large-scale systems. 
For a strongly connected networked system, an optimal controller $\tf K$ (the transfer matrix from measurements to control actions) can only be solved for in a convex manner via Youla parameterization if $\tf K$ is dense (this follows from the conditions identified in \cite{2010_Rotkowitz_QI_delay}).
This then implies that each sub-controller in the network needs to exchange information to the entire networked system to compute its control action, which does not scale gracefully to large systems.
%Using the conditions identified in \cite{2010_Rotkowitz_QI_delay}, a sparsity constraint imposed on the controller $\tf K$ generally makes the resulting distributed optimal control problem non-convex when the networked system has a strongly connected topology.
%In fact, for a strongly connected networked system, 
%an information sharing constraint is QI if and only if the local measurement taken by each sensor is shared among \emph{all} sub-controllers in the network (this follows from the conditions identified in ). 
%When a plant is strongly connected, an optimal controller $\tf K$ (the transfer function from measurements $\tf y$ to control actions $\tf u$) can only be solved for in a convex manner via Youla parameterization if $\tf K$ is dense, i.e., if each sub-controller needs to collect the entire measurement $\tf y$ of the system to compute its control action.
%Although the distributed optimal control problem with a QI information sharing constraint is computationally tractable (i.e., convex), both the controller synthesis and implementation scale with the dimension of the full system, and thus are not practical for large systems.
%However, the QI control scheme is not scalable for large-scale systems either -- the resulting optimal controller is as difficult to compute as its centralized counterpart, and even more demanding to implement. 
In order to improve scalability and ease of implementation, techniques based on regularization \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting}, convex approximation \cite{2014_Fazelnia_ODC, 2014_Sznaier, 2015_DJ}, and spatial truncation \cite{2009_Motee_spatial_truncation} have been used in hopes of finding a sparse feedback controller that is scalable to implement. 
These methods have been successful in extending the size of systems for which a distributed controller can be implemented, but there is still a limit to their scalability as they often rely on an underlying centralized synthesis procedure.
%the synthesis procedure of these methods are centralized.
%Further, it is not clear if these methods can be extended to compute a dynamic controller that incorporates information sharing constraints.
%Even though the non-convex problem corresponding to a sparse $K$ may be solved via convex relaxation \cite{2014_Fazelnia_ODC} or spatial truncation \cite{2009_Motee_spatial_truncation}, 
%Regularization or approximation have been used in hopes of finding a sparse $K$, including sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting}, spatial truncation method \cite{2009_Motee_spatial_truncation}, or on spatial decaying systems \cite{2008_Motee_distributed, 2014_Motee_spatially_decaying}. 
%The synthesis of these methods, however, is still centralized. 
%However, the synthesis procedure of these methods are still centralized.
%In particular, these methods involve solving a large-scale optimization problem with the knowledge of global plant model beforehand, which is not scalable.
%In addition, the methods in \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting, 2009_Motee_spatial_truncation} are aimed at finding sparse static state-feedback controllers, and so it is not clear if they have natural extensions to incorporate output feedback and delay constraints. 
%In contrast, we propose a controller synthesis methodology that scales to systems of arbitrary size.
%Although the nonconvex problem is possible to be solved approximately \cite{2014_Fazelnia_ODC, 2011_Rotkowitz_subspace}, the synthesis of distributed optimal controller still requires solving large-scale optimization problem with the knowledge of global plant model beforehand, which is highly unrealistic.
%Based on this discussion, we argue that the closed loop behavior achieved by these distributed optimal controllers should be viewed as fundamental limits on performance, that we should strive to attain via more \emph{scalable} and \emph{realistically implementable} control schemes.
%The idea of designing localized (sparse) controllers to improve scalability and ease of implementation has been applied on special systems, such as the spatially invariant systems \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant, 2005_Jovanovic_localized}. The method is generalized into spatial decaying systems in \cite{2008_Motee_distributed, 2014_Motee_spatially_decaying}. Regularization or approximation have also been used in hopes of finding a sparse controller. Representative works include sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting} and spatial truncation method \cite{2009_Motee_spatial_truncation}.
%The synthesis of these methods, however, is still centralized, which requires global plant model beforehand. The methods described in \cite{2004_Dullerud, 2008_Borrelli_LQR, 2013_Farokhi_model} can provide scalable ways to synthesize distributed controller with limited model information, but the method can be quite conservative. 
%Part of the reason is that the controller synthesis and implementation of those methods are in the ``$K$" domain.

In the first part of this two-part paper \cite{2015_PartI}, we proposed the \emph{localized optimal control framework} as an alternative way to incorporate constraints into the optimal control problem. The key idea is to design the closed loop response of the feedback system first, then construct an internally stabilizing controller to achieve the desired closed loop response. Conceptually, the localized optimal control problem is formulated in the form of
\begin{subequations} \label{eq:clock}
\begin{align}
\underset{\ttf{\Phi}}{\text{minimize  }} \quad & g(\ttf{\Phi}) \label{eq:clock1}\\
\text{subject to }  \quad & \ttf{\Phi} \text{ stable and achievable } \label{eq:clock2}\\
& \ttf{\Phi} \in \s,  \label{eq:clock3}
\end{align}
\end{subequations}
where $\ttf{\Phi}$ is the desired closed loop response (this will be formally defined in Section \ref{sec:prelim}), $g(\cdot)$ a convex objective function, and $\mathcal{S}$ a convex set constraint. We showed in \cite{2015_PartI} that \eqref{eq:clock} characterizes the largest known class of convex problems in optimal control -- the class of QI constraint is a strict subset of $\s$-localizability constraint. In addition, we showed that by imposing a sparsity constraint through $\s$, the controller achieving the desired closed loop response can be implemented in a localized and thus scalable way if we allow the communication of both \emph{measurements} and \emph{controller's internal states}. 

%pointed out that the fundamental difficulty of extending the QI theory to large-scale problems is because the synthesis and implementation for distributed optimal controller are done in different domains. 
%Specifically, the controller synthesis is solved in the Youla domain, while the controller is implemented using the transfer matrix $\tf K$. 
%To overcome this difficulty, we proposed an alternative way to incorporate structured constraints in the domain of \emph{closed loop transfer matrices}.
%the fact that a localized (and thus sparse and scalable) controller implementation does not necessarily require the transfer matrix $\tf K$ to be sparse. 
%By using implicit implementations of the controller (which allow the communication of both \emph{measurements} and \emph{controller's internal states}), we showed that the distributed controller can be implemented in a localized way even when the transfer matrix $\tf K$ is not sparse. 
%Specifically, we formulated the localized optimal control problem as
%\begin{subequations} \label{eq:clock}
%\begin{align}
%\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize    }} & \quad g(\tf R,\tf M,\tf N,\tf L) \label{eq:main_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:main_1} \\
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:main_2} \\
%&  \tf R, \tf M, \tf N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad \tf L \in \mathcal{RH}_{\infty} \label{eq:main_stable}\\
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \s \label{eq:main_S}
%\end{align}
%\end{subequations}
%where $\tf R, \tf M, \tf N, \tf L$ are closed loop transfer matrices (this will be formally introduced in Section \ref{sec:prelim}), $g(\cdot)$ a convex objective function, $(A, B_2, C_2)$ the state space matrices of the plant model, and $\mathcal{S}$ a convex set constraint. We showed that the solution $(\tf R, \tf M, \tf N, \tf L)$ of \eqref{eq:main_1} - \eqref{eq:main_stable} parameterizes all achievable stable closed loop transfer matrices, and an internally stabilizing controller achieving the desired closed loop response can be constructed by the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ if we allow the communication of both \emph{measurements} and \emph{controller's internal states} between sub-controllers. We then introduced an additional convex set constraint in \eqref{eq:main_S}, which is called the $\mathcal{S}$-localizability constraint. 
%We showed in \cite{2015_PartI} that a large class of structured constraints can be interpreted as special cases of $\mathcal{S}$-localizability constraint. In particular, we showed that the formulation \eqref{eq:clock} characterize a much broader class of convex problems than the QI framework.
%The optimization problem \eqref{eq:clock} is convex as long as the objective function $g(\cdot)$ is convex and the localizability constraint $\s$ forms a convex set. We showed in \cite{2015_PartI} that the formulation \eqref{eq:clock} characterize a much broader class of convex problems than the QI framework.

In this paper, we propose a scalable algorithm to synthesize a nearly optimal controller for some class of large-scale systems. Specifically, we introduce the notion of \emph{decomposability} on the objective function $g(\cdot)$ and the localizability constraint $\s$ such that the global optimization problem \eqref{eq:clock} can be \emph{solved} in a localized and distributed way.
%discuss how to apply the localized optimal control formulation \eqref{eq:clock} on large-scale systems. 
%Our approach is to impose the sparsity constraint on the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ through the localizability constraint \eqref{eq:main_S}. 
%If \eqref{eq:clock} remains feasible under the additional sparsity constraint, then the controller achieving the desired closed loop response can be implemented by sparse transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ in a localized and scalable way. 
%In addition, if the objective function $g(\cdot)$ and the localizability constraint $\s$ further satisfy the \emph{decomposability} conditions, then the large-scale convex problem \eqref{eq:clock} can be \emph{solved} in a localized and distributed way. Specifically, 
We combine the distributed optimization techniques such as alternating direction method of multipliers (ADMM) \cite{BoydADMM} with the localizability constraint \eqref{eq:clock3} to decompose the global problem \eqref{eq:clock} into parallel local subproblems. Each local subproblem only needs to use the plant model information locally. In addition, the complexity of solving each subproblem is completely independent to the size of the global network, which means that our synthesis method can be scaled to arbitrary large systems if parallel computation is available. We give several examples of decomposable problems, including the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem and the co-design of $\mathcal{H}_2$ optimal control with its sensor and actuator locations. These problems can all be solved in an extremely scalable way.

%Although the optimization problem \eqref{eq:clock} is convex, it is still a large-scale optimization problem that may not be scalable to solve. In this paper, we identify the technical conditions on the objective function in \eqref{eq:main_obj} and the localizability constraint in \eqref{eq:main_S} such that the optimization problem \eqref{eq:clock} can be solved in a scalable way. Specifically, we introduce the notion of decomposability of the performance metric $g(\cdot)$ and the localizability constraint $\mathcal{S}$. There are two type of decomposable problems: (a) directly decomposable, and (b) decomposable with respect to distributed optimization. For the first type of the problem, the global optimization problem can be decomposed directly into multiple local subproblems. These subproblems can be solved in a parallel manner, and each subproblem only depends on the local plant model information. The complexity of solving each subproblem is completely independent to the size of the global network, which is extremely scalable. Specific examples include the localized linear quadratic regulator (LLQR) method proposed in \cite{2014_Wang_CDC}.
%The second type is the generalization of the first type, where we use distributed optimization techniques such as alternating direction method of multipliers (ADMM) \cite{BoydADMM} as an iterative algorithm to solve \eqref{eq:clock}. If each subroutine of the algorithm is directly decomposable, then the global optimization problem can also be solved in a localized and scalable way. We identify several classes of decomposable problems, including the localized linear quadratic Gaussian (LLQG) problem \cite{2015_Wang_H2} and the LLQR control with actuator regularization \cite{2015_Wang_Reg} as special cases.

%By scalable, we mean that the complexity of the optimization problem scale linearly with respect to the size of the global network system. 
%In addition to a scalable, or localized, implementation, we show that if a system can be localized via state-feedback controller, then the resulting localized linear quadratic regulator (LLQR) optimal controller can be synthesized in a scalable, parallel and localized way \cite{2014_Wang_CDC}.
%Specifically, we show that the LLQR optimal control problem can be decomposed into several subproblems that can be solved in parallel, each defined in terms of a local subset of the controller and system and admitting an analytic solution. 
%However, this technique does not extend to the output feedback setting \cite{2014_Wang_Allerton} because there is an additional constraint that introduces a coupling in the optimization problem.
%In this paper, we pose and solve the localized linear quadratic Gaussian (LLQG) problem, i.e., we solve the output feedback localized optimal control problem with an $\mathcal{H}_2$ (LQG) performance metric.  We show that by combining the alternating direction method of multipliers (ADMM) with the LLQR decomposition technique, we can synthesize an LLQG optimal controller in a scalable, parallel and localized way. Thus the LLQG controller can be both synthesized and implemented in a scalable way, with the complexity of each task independent of the global system size.

The rest of the paper is organized as follows. In Section \ref{sec:prelim}, we introduce the system model, recall the distributed optimal control formulation and comment on its scalability limitations, and recall relevant results from the first part of the paper \cite{2015_PartI}.
%In Section \ref{sec:imp}, we discuss how to use the localized optimal control framework to design a controller that is scalable to implement. 
%Section \ref{sec:sf} and Section \ref{sec:of} discuss the scalability of controller synthesis. 
%We focus on a special case of \eqref{eq:clock} in Section \ref{sec:sf}, where the optimization problem can be decomposed directly into local subproblems without using distributed optimization.  
In Section \ref{sec:sf}, we focus on a special case of \eqref{eq:clock} in which the optimization problem can be decomposed directly into local subproblems without using distributed optimization. 
%We show how to solve \eqref{eq:clock} in a localized and scalable way when the problem is directly decomposable.
%To deal with the general case, we combine the distributed optimization technique with the direct decomposition method in Section \ref{sec:of}. We introduce the notion of decomposability of the problem \eqref{eq:clock}, in which the 
%and identify the technical conditions
The general case is studied in Section \ref{sec:of}, where we identify the technical conditions on the decomposability of problem \eqref{eq:clock}. When the problem is decomposable, we can use distributed optimization combined with the direct decomposition technique to solve  \eqref{eq:clock} in a localized yet iterative way. We also give many examples of decomposable optimal control problems.
%Additionally, we show that the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem and the $\mathcal{H}_2$ optimal control with sensor and actuator regularization are both decomposable problems.
%The general case is discussed in \eqref{eq:clock}, 
%some classes of directly decomposable problems, and show that these problems can be solved in a scalable way. In Section \ref{sec:of}, we introduce the notion of decomposability with respect to distributed optimization, and show that the $\mathcal{H}_2$ optimal control, mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control, and $\mathcal{H}_2$ optimal control with sensor and actuator regularization are all decomposable problems. 
Simulation results are shown in Section \ref{sec:simu} to demonstrate the effectiveness of our method. Specifically, we synthesize a localized $\mathcal{H}_2$ optimal controller for a system with $12800$ states composed of dynamically coupled heterogeneous subsystems, and demonstrate the optimal co-design of localized controller with sensor placement on a system with $3200$ states. Finally, conclusions and some future research directions are summarized in Section \ref{sec:conclusion}.

%we recall the LLQR decomposition of the state-feedback problem, as it is a key component of our proposed computational scheme. We then use the LLQR decomposition in combination with the ADMM algorithm to show how the LLQG optimal control problem can be solved in a scalable way in \S\ref{sec:output}.  We end with \S\ref{sec:simu}, where we show the effectiveness of our method by synthesizing the LLQG optimal controller for a system with $\sim10^4$ states composed of dynamically coupled heterogeneous subsystems. 

\subsection*{Comparison With Prior Publications by the Authors}
In this paper, we identify the decomposability condition of the localized optimal control problem \eqref{eq:clock}, and propose a general algorithm to solve all kinds of decomposable problems in a localized and scalable way. 
%Based on the localized optimal control framework established in the first part of the paper \cite{2015_PartI}, we introduce the notion of decomposability of the problem \eqref{eq:clock}. We propose a general algorithm to solve \eqref{eq:clock} in a localized and scalable way when the objective and the localizability constraint satisfy the decomposability conditions. 
This provides a unified framework for our previous results in \cite{2014_Wang_CDC, 2015_Wang_H2, 2015_Wang_Reg}. Some specific extensions are summarized as follows.
\begin{enumerate} [(a)]
\item The notion of decomposable objective function is defined, which includes the quadratic objective \cite{2014_Wang_CDC, 2015_Wang_H2} and the actuator regularizer \cite{2015_Wang_Reg} as special cases.
%The quadratic objective \cite{2014_Wang_CDC, 2015_Wang_H2} and the actuator regularizer \cite{2015_Wang_Reg} are special cases of decomposable objective function defined in this paper.
% We also introduce some new class of decomposable objective functions.
\item We introduce the notion of decomposability on the localizability constraint, which generalizes the spatiotemporal constraint considered in \cite{2014_Wang_CDC, 2015_Wang_H2, 2015_Wang_Reg} substantially. 
%Some new classes of decomposable constraints such as the one that appeared in mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control are introduced.
%$\mathcal{L}_1$ norm bound on the closed loop transfer matrix are introduced. 
\item We provide a unified algorithm to solve all decomposable problems, and propose some variants and specialization of the algorithm for specific problems.
%\item We lift several technical assumptions of our prior works. For instance, we extend the row/column-wise decomposition into row/column-wise partition, which allows us to deal with locally correlated disturbances. In addition, we propose a more general dimensional reduction algorithm (see Remark \ref{rmk:1}).
%for the localized optimal controller with decomposable performance metrics. This is a generalization of our previous works in \cite{2014_Wang_CDC} and \cite{2015_Wang_H2}, which focus on quadratic objective functions.
%localized synthesis algorithm for a class of $\mathcal{H}_2$ problem based on the alternating direction method of multipliers (ADMM)\cite{BoydADMM}.
\end{enumerate}

%The goal of this two-part paper is to show that the new formulation in \eqref{eq:clock} has various benefits over the traditional formulation in \eqref{eq:intro}, especially on handling the constraint \eqref{eq:main_S} for large-scale systems.
%In previous work \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}, we introduced the notion of a localizable system.  These are systems for which a distributed controller exists that achieves a closed loop response in which the effect of each disturbance is limited to a local neighborhood (we make this precise in \S\ref{sec:prelim}). We showed that if a system is localizable, then a controller achieving the desired localized closed loop response can be implemented in a scalable way if we allow the communication of both \emph{measurements} and \emph{controller internal states} between sub-controllers. In particular, this means that each sub-controller $i$ only needs to collect a subset of the measurements and controller internal states to compute its control action.
%implementation is always localizable if we allow the communication of both \emph{measurements and controller}
%point out the fact that a localized (and thus sparse and scalable) controller implementation does not necessarily imply that $K$ (the transfer function from measurements to control actions) needs to be sparse. 
%By using implicit implementations of the controller (which allows the communication of both \emph{measurements and control action}, or \emph{estimated disturbance and reference trajectory}), we show that the distributed controller can be implemented in a localized way as long as a localized closed loop response exists.
%We derive a direct relati
%pointed out that the limitation of the QI framework is due to the transformation of ons between the closed loop response and the (implicit) controller implementation achieving the desired closed loop. 
%The result is extended to output feedback localizable system in \cite{2014_Wang_Allerton}, where the controller achieving the desired localized closed loop response can be implemented in a localized way. However, the synthesis of the output feedback problem is no longer localized in \cite{2014_Wang_Allerton}.
%This method not only avoids the non-convex nature in \eqref{eq:intro}, but also guarantees structured realizability \cite{2013_Lessard_structure} of the controller.
%decomposable performance metric. %Some familiar examples of decomposable performance metrics include a class of $\mathcal{H}_2$ norm and $\mathcal{L}_1$ system norm, where we focus our discussion mainly on $\mathcal{H}_2$ norm due to its popularity.
%further show that \eqref{eq:main_S} can be \emph{solved} in a localized way, given that the objective is $\mathcal{H}_2$ norm and $\mathcal{S}$ is sparse. Specifically, we combine the technique of distributed optimization and localized linear quadratic regulator (LLQR) \cite{2014_Wang_CDC} to decompose \eqref{eq:main_S} into several local optimization problems. Moreover, each local optimization problem only depends on \emph{local plant model} information. 
%inherits the favorable properties of the LLQR controller on large-scale systems, including localized implementation and synthesis using local plant model.
%an output feedback localizable system with a $\mathcal{H}_2$ objective. This completes our previous work in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton} by offering a scalable $\mathcal{H}_2$ synthesis algorithm for large-scale output feedback localizable systems. 

%\subsubsection*{Notation}  We use lower and upper case Latin letters such as $x$ and $M$ to denote vectors and matrices, respectively, and lower and upper case boldface Latin letters such as $\tf x$ and $\tf M$ to denote signals and transfer matrices, respectively.  We use calligraphic letters such as $\s$ to denote subspaces.  We use $\RHinf$ to denote the space of stable, proper real-rational transfer matrices, and $\FT$ to denote the space of finite impulse response transfer matrices with horizon $T$, i.e., $\FT := \{ \tf G \in \RHinf \, | \,, \tf G = \sum_{t=0}^T\frac{1}{z^t}G_t\}$. 

%we will discuss on how to apply our alternative formulation for large-scale controller synthesis with implementation constraints. Specifically, when sparsity constraint is imposed on \eqref{eq:main_S}, the controller achieving the desired closed loop response can be implemented in a localized way by sparse transfer matrices $R, M, N, L$ directly. In addition, for some specific objective functions, such as the $\mathcal{H}_2$ norm with some sparsity constraints, the optimization problem \eqref{eq:main_obj} - \eqref{eq:main_S} can be solved in a localized and parallel way by utilizing the technique in distributed optimization. For each localized optimization subroutine, only the \emph{localized plant model} information is required. Finally, simulation results are shown in Section \ref{sec:simu}, and the conclusions and some future research direction are summarized in Section \ref{sec:conclusion}.

%\textit{Comparison With Prior Publications by the Authors: } In this paper, we establish a coherent theoretical framework for our previous results in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton} based on a parameterization of all stabilizing controllers and the notion of internal stability on our particular controller architecture. With this new framework, we generalize our previous results substantially in the following sense.
%\begin{enumerate}
%\item The output feedback scheme in \cite{2014_Wang_Allerton} is generalized to unstable plant.
%\item The notion of $\mathcal{S}$-localizability is introduced, which is a generalization of $(d,T)$-localizability in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}. We further show that QI constraint is a special case of $\mathcal{S}$-localizability constraint.
%\item The robustness of the localized controller implementation with respect to model uncertainty or various source of error is rigorously analyzed. In particular, we give a simple sufficient condition on output feedback stabilizability for \emph{nearly} localizable systems.
%\item We provide a localized synthesis algorithm for a class of $\mathcal{H}_2$ problem based on the alternating direction method of multipliers (ADMM)\cite{BoydADMM}.
%\end{enumerate}



==> LLQG_Prelim_v1.tex <==
We begin by introducing the interconnected system model that we consider in this paper. We then explain why the distributed optimal control formulation has an intrinsic difficulty to scale to large systems. We then recall the results of \cite{2015_PartI} in which we defined the localized optimal control framework. This section ends with the problem statement of the paper.

%\subsection{System Model}
%In this paper, we consider a discrete time linear time invariant system (LTI) with dynamics given by
%\begin{eqnarray}
%x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber\\
%y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics} 
%\end{eqnarray}
%where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. 
%Equation \eqref{eq:dynamics} can be written in state space form as
%\begin{equation}
%\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & D_{11} & D_{12} \\ C_2 & D_{21} & D_{22} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
%\end{equation}
%where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. We refer to $\tf P$ the open loop plant model. The stability of $\tf P$ is determined by the matrix $A$. In this paper, a square matrix $A$ is called a stable matrix if its spectral radius is less than $1$, i.e., all the eigenvalues of $A$ lie within the unit circle. We assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable. In this case, the open loop plant $\tf P$ is stable if and only if $A$ is a stable matrix. 

\subsection{Interconnected System Model}
\input{Model_v2}
%We consider distributed systems described by linear time-invariant (LTI) dynamics and composed of a collection of subsystems that interact with each other according to a network topology specified by the interaction graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$. Here $\mathcal{V} = \{1, \dots, n\}$ denotes the set of subsystems: to each subsystem $i$ we associate a state vector $x_i$, control action $u_i$, and measurement $y_i$; and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems: an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$. We use $|\mathcal{V}|$ and $|\mathcal{E}|$ to denote the cardinality of the set $\mathcal{V}$ and $\mathcal{E}$, respectively. Defining the (incoming) neighbor set $\mathcal{N}_i$ of subsystem $i$ to be $\mathcal{N}_i = \{j | (i,j) \in \mathcal{E}\}$, may then write the dynamics of subsystem $i$ as
%\begin{eqnarray}
%x_i[k+1] &=& A_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[k] + B_{ii} u_i[k] + \delta_{x_i}[k] \nonumber\\
%y_i[k] &=& C_{ii} x_i[k] + \delta_{y_i}[k], \label{eq:interconnected}
%\end{eqnarray}
%where $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ are matrices of compatible dimensions, and $\delta_{x_i}$ and $\delta_{y_i}$ denote state and measurement perturbations, respectively. 
%The following is a simple example in the form of \eqref{eq:interconnected}.
%%, which is used to illustrate several ideas throughout this paper.
%\begin{example}
%Consider a network system with interconnected topology given by Fig. \ref{fig:Chart105}. Each sub-system $x_i$ is assumed to have two interacting scalar states $x_{i,1}, x_{i,2}$, a sensor on $x_{i,1}$, and an actuator on $x_{i,2}$. The interaction between two neighboring sub-systems is illustrated in Fig. \ref{fig:inter}, where $x_{i,1}$ can affect $x_{j,2}$ if $i$ and $j$ are neighbor. This model is inspired from the second-order dynamics in power network or mechanical system. Specifically, consider a second-order equation
%\begin{equation}
%m_i \ddot{\theta_i} + d_i \dot{\theta_i} = -\sum_{j \in \mathcal{N}_i} k_{ij} (\theta_i - \theta_j) + w_i + u_i \nonumber
%\end{equation}
%for some scalar $\theta_i$.
%If we define the state vector by $x_i = [\theta_i \quad \dot{\theta_i}]^\top$, take the measurement on $\theta_i$, and use $e^{A \Delta t} \approx I + A \Delta t$ to discretize the plant, we get a discretized plant model with interaction graph described by Fig. \ref{fig:inter}.
%\end{example}
%\begin{figure}[t!]
%      \centering
%      \subfigure[Interconnected topology]{%
%      \includegraphics[width=0.35\textwidth]{./figure/Topology.pdf}
%      \label{fig:Chart105}}      
%      \subfigure[Interaction between neighboring sub-systems]{%
%      \includegraphics[width=0.35\textwidth]{./figure/Interaction.pdf}
%      \label{fig:inter}}      
%      \caption{Illustrative Example}
%\end{figure}
%
%More generally, we consider global system model with dynamics given by
%\begin{eqnarray}
%x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber\\
%y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics} 
%\end{eqnarray}
%where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. We use $n_x, n_y$, and $n_u$ to denote the dimension of $x, y$, and $u$, respectively. In this paper, we are particularly interested in the case in which the matrices $(A,B_2,C_2)$ are large-scale but fairly sparse. For example, if the global system model $(A,B_2,C_2)$ is constructed by the interconnected system model described in \eqref{eq:interconnected}, then we have
%\begin{equation}
%A = \begin{bmatrix} A_{11} & \cdots & A_{1n} \\ \vdots & \ddots & \vdots \\ A_{n1} & \cdots & A_{nn} \end{bmatrix} \nonumber
%\end{equation}
%and $B_2 = \textbf{diag}(B_{11}, \dots, B_{nn})$ and $C_2 = \textbf{diag}(C_{11}, \dots, C_{nn})$. When the number of nodes of the interaction graph is large and the interconnected topology is sparse ($|\mathcal{E}| \ll n^2$), the matrices $(A,B_2,C_2)$ are all large-scale but sparse. The goal of this paper is to exploit the sparsity pattern of the system matrices $(A,B_2,C_2)$ to derive a scalable algorithm for controller synthesis. Note that our method can be applied on general system matrices. In particular, the matrices $B_2$ and $C_2$ does not need to be block diagonal as in the interconnected system model \eqref{eq:interconnected}. Throughout the paper, we assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable.
%
%Let the disturbances be given by $\delta_x = B_1 w$ and $\delta_y = D_{21} w$ for some matrices $B_1$ and $D_{12}$, and a disturbance vector $w$. Let $\bar{z}$ be a controlled output given by $\bar{z}[k] = C_1 x[k] + D_{12} u[k]$. The system equations in \eqref{eq:dynamics} can then be written in transfer function form as
%\begin{equation}
%\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & {0} & D_{12} \\ C_2 & D_{21} & {0} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
%\end{equation}
%where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. 

%This example is inspired from the discrete time double integrator model in mechanical or power system. The method described in this paper can generalize to other sub-system models with arbitrary interconnected topology as well.
%Although this example is extremely simple, our method can be applied on a much broader class of problems. In particular, we demonstrate our algorithm on a large system with randomized topology, randomized entries, sparse actuation, and sparse sensing in Section \ref{sec:simu}.}

\subsection{Limitation of Distributed Optimal Control Framework}
Interconnected systems \eqref{eq:interconnected} pose fundamental challenge to controller synthesis -- the additional information sharing constraint between sub-controllers usually make the distributed optimal control problem non-convex.
%Designing controllers for interconnected systems \eqref{eq:interconnected} can be very challenging for two distinct reasons: (i) in general, the optimal control problem may be intractable \cite{1968_Witsenhausen_counterexample}, and (ii) even if the problem is tractable, the resulting synthesis problem may not scale gracefully to large systems. 
%Although recent work \cite{2006_Rotkowitz_QI_TAC} has been very successful in identifying tractable (i.e., convex) classes of such problems, as described in the introduction, there has been less focus on scalability. 
%Before describing our scalable controller synthesis framework, 
Here we briefly recall the distributed optimal control framework, and show why scalability issues may arise when dealing with large systems.
%(i) the effect of sub-system interaction $A_{ij}$ is strong, and (ii) the number of sub-systems $n$ is large. The distributed method and the completely local method can handle one of the situations above, but not both.
%By completely local method, for an extreme case, the controller is implemented \emph{and} designed in a purely local way. Specifically, each local control rule is given by $u_i = K_i y_i$, where $K_i$ is designed with the local plant model $(A_{ii}, B_{ii}, C_{ii})$ \emph{only}. Clearly, such control scheme is scalable to arbitrary large $n$, but does not guarantee global stability if the effect of $A_{ij}$ is not negligible.
%We also assume that each sub-system can communicate and collaborate with each other. The general goal is to design a global control action $u = [u_1^\top, \dots, u_n^\top]^\top$ as a function of the global measurement $y = [y_1^\top, \dots, y_n^\top]^\top$ that achieves internal stability and some sort of optimality.
%When the number $n$ go large, localized implementation, localized model information, localized synthesis
%The interconnected system model can also be written in the global form as

Consider a dynamic output feedback control law $\tf u = \tf K \tf y$. The distributed optimal control problem of minimizing the norm of the closed loop transfer matrix from external disturbance $\tf w$ to regulated output $ \tf{\bar{z}}$ is commonly formulated as
%of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$.} of the closed loop transfer function from $w$ to $\bar{z}$ is formulated as
\begin{subequations}\label{eq:trad}
\begin{align}
\underset{\tf K}{\text{minimize  }} \quad & ||\tf P_{11} + \tf P_{12} \tf K(I-\tf P_{22}\tf K)^{-1} \tf P_{21}\| \label{eq:trad_obj}\\
\text{subject to  } \quad & \tf K \text{ internally stabilizes } \tf P \label{eq:trad_stable}\\ 
& \tf K \in \K \label{eq:trad_info}
\end{align}
\end{subequations}
where the subspace constraint $\tf K \in \K$ enforces information sharing constraints between the sub-controllers. When $\K$ is a subspace constraint, it has been shown that \eqref{eq:trad} is convex if \cite{2006_Rotkowitz_QI_TAC, 2014_Sabau_QI} and only if \cite{2011_QIN, 2014_Lessard_convexity} $\K$ is quadratically invariant (QI) with respect to $\tf P_{22}$, i.e., $\tf K \tf P_{22} \tf K \in \K$ for all $\tf K \in \K$. 
Roughly speaking, QI condition holds when sub-controllers are able to share information with each other at least as quickly as their control actions propagate through the plant \cite{2010_Rotkowitz_QI_delay}.

%If QI condition is satisfied, we have $\K = \Q$ and thus \eqref{eq:trad2} is a convex program. 
%The set of internally stabilizing controller is commonly characterized by Youla parameterization \cite{1976_Youla_parameterization}. For simplicity, we only consider the situation when $\tf P$ is open loop stable. In this case, the Youla parameter is given by $\tf Q = \tf K(I- \tf P_{22} \tf K)^{-1}$, and the optimization problem \eqref{eq:trad} can be equivalently formulated as
%\begin{eqnarray}
%\underset{\tf Q}{\text{minimize  }} &&|| \tf P_{11} + \tf P_{12} \tf Q \tf P_{21}|| \nonumber\\
%\text{subject to } && \tf Q \in \RHinf \nonumber\\
%&& \tf Q \in \Q,  \label{eq:trad2}
%\end{eqnarray}
%where the set $\Q$ is given by $\Q = \{ \tf K(I- \tf P_{22} \tf K)^{-1} | \tf K \in \K \}$. The convexity of \eqref{eq:trad2} depends solely on the convexity of the set $\Q$.
%It was shown in \cite{2006_Rotkowitz_QI_TAC} that if the constraint set $\mathcal{C}$ is quadratically invariant with respect to $\tf P_{22}$ then the optimal control problem admits a convex reformulation. 

When the interconnected system \eqref{eq:interconnected} is strongly connected, the transfer matrix $\tf P_{22} = C_2 (zI-A)^{-1} B_2$ is always dense even though the matrices $(A,B_2,C_2)$ are fairly sparse. In this case, a sparsity constraint $\K$ imposed on $\tf K$ in \eqref{eq:trad} is not QI, and \eqref{eq:trad} cannot be reformulated in a convex manner in the Youla domain.
%induces a non-convex constraint set $\Q$ on $\tf Q$ in \eqref{eq:trad2}, which makes the distributed optimal control problem non-convex. 
In other words, for a strongly connected plant, the distributed optimal control problem is convex only when the transfer matrix $\tf K$ is dense, i.e. each local measurement $\tf y_i$ needs to be shared among \emph{all} the sub-controllers in the network. This controller implementation does not scale gracefully to large systems.
%Assume that for a given constraint $\mathcal{C}$, the optimal controller $\tf K$ can be computed: the implementation complexity of $\tf K$ is then determined by the densest row $\tf K_i$ of $\tf K$.  Specifically, if we consider the control action taken at subsystem $i$, which is specified by $\tf u_i = \tf K_i \tf y$, then if $\tf K_i$ is completely dense then subsystem $i$ must collect measurements from every other subsystem $j \in \mathcal{V}$.  As the number of subsystems grows large, this then leads to a very complex controller implementation.  A natural solution to this problem is to impose sparsity constraints on the controller $\tf K$ such that each row only has a small number of nonzero terms -- in this way each subsystem $i$ only needs to collect a small number of measurements to compute its control action.  Unfortunately, this naive approach fails if the dynamics of $\tf P_{22}$ are strongly connected because in that case, any sparse constraint set $\mathcal{C}$ is not QI with respect to $\tf P_{22}$.  
Although recent methods based on convex relaxations \cite{2014_Fazelnia_ODC} can be used to solve certain cases of the non-convex optimal control problem \eqref{eq:trad} approximately with a sparse constraint set $\K$, the underlying synthesis optimization problem is still large-scale and does not admit a scalable reformulation. The need to address scalability, both in the \emph{synthesis} and \emph{implementation} of a controller, is the driving motivation behind the localized optimal control framework, which we recall in the next subsection.

%It has been shown that \eqref{eq:trad} admits a convex reformulation in the Youla domain if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$. The class of QI constraint, however, is not amenable for large-scale problem. This is due to the fact that the sparsity constraint on $K$ is generally not QI for a plant with strongly connected topology (which can be inferred from the delay interpretation of QI in \cite{2010_Rotkowitz_QI_delay}). For instance, even when $A$ in \eqref{eq:dynamics} is as sparse as a tridiagonal matrix, the QI condition requires all the local measurements to be shared among \emph{every controllers} in the network. 
%It is true that the controller implementation for \eqref{eq:trad} is scalable to large $n$ when $\s_c$ is a sparsity constraint. In this case, however, \eqref{eq:trad} is generally non-convex and hard to solve if the plant has a strongly connected topology. 
%The delay constraint for QI
%As alluded to in the introduction, the class of QI constraint is not amenable for large-scale problem. This is due to the fact that the sparsity constraint on $K$ is generally not QI for a plant with strongly connected topology\footnote{This means that $P_{22}$ is not sparse} \cite{2010_Rotkowitz_QI_delay, 2009_Swigart_graph_QI}. Even when $A$ in \eqref{eq:dynamics} is as sparse as a tridiagonal matrix, the QI condition requires all the local measurements to be shared among \emph{every controllers} in the network. Such a controller implementation is not scalable to large systems. In addition, \eqref{eq:trad} is a large-scale optimization problem, and it is generally hard to solve in a scalable way.
%It can be seen that the objective function in \eqref{eq:trad} is not convex in $K$. As a result, Youla parameterization is used to reformulate \eqref{eq:trad} in terms of the Youla parameter, and it admits a convex reformulation if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$.
%Traditionally, Youla parameterization is used to reformulate \eqref{eq:trad} into a convex manner. It is known that the constraint $\s_c$ remains convex on the Youla parameter if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$.

\subsection{Localized Optimal Control Framework}
%Our previous work on localized optimal control \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton} is built on the observation 
In the first part of this two-part paper \cite{2015_PartI}, we introduced a more general framework to incorporate constraints in the optimal control problem. The key idea is to design the closed loop response first, then construct an internally stabilizing controller to achieve the desired closed loop response. %based on the notion of \emph{closed loop transfer matrices}. 
For an LTI system with dynamics given by \eqref{eq:dynamics}, the closed loop transfer matrices $\{\tf R, \tf M, \tf N, \tf L\}$ are defined by the relation
\begin{equation}
\begin{bmatrix} \tf x \\ \tf u \end{bmatrix} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} \ttf{\delta_x} \\ \ttf{\delta_y} \end{bmatrix}. \label{eq:desired}
\end{equation}
where $\ttf{\delta_x} = B_1 \tf w$ is the disturbance on the state vector, and $\ttf{\delta_y} = D_{21} \tf w$ is the disturbance on the measurement. We showed that the parameterization of all stable achievable closed loop transfer matrices $\{\tf R, \tf M, \tf N, \tf L\}$ is described by the solution of the following equations:
\begin{subequations} \label{eq:achievable}
\begin{align}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} &= 
\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:main_1} \\
\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix}
\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} &= 
\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:main_2} \\
\tf R, \tf M, \tf N \in \frac{1}{z} \mathcal{RH}_{\infty}, & \quad \tf L \in \mathcal{RH}_{\infty}. \label{eq:main_stable}
\end{align}
\end{subequations}
The parameterization of all internally stabilizing controller is given by the following theorem.
%The following theorem gives an implementation of the controller that achieves the desired closed loop response.
\begin{theorem}
Suppose that a set of transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ satisfy the constraints \eqref{eq:main_1} - \eqref{eq:main_stable}. Then an internally stabilizing controller yielding the desired closed loop response \eqref{eq:desired} can be implemented as
\begin{subequations}\label{eq:implementation}
\begin{align}
z \ttf{\beta} &= \tilde{\tf R}^+ \ttf{\beta} + \tilde{\tf N} \tf y \label{eq:imple1}\\
\tf u &=  \tilde{\tf M} \ttf{\beta} + \tf L \tf y \label{eq:imple2}
\end{align}
\end{subequations}
where $ \tilde{\tf R}^+ = z(I - z\tf R)$, $\tilde{\tf N} = -z\tf N$, $\tilde{\tf M} = z\tf M$, $\tf L$ are in $\RHinf$. \label{thm:1} Further, the solutions of \eqref{eq:main_1} - \eqref{eq:main_stable} with the implementation \eqref{eq:implementation} parameterize all internally stabilizing controller. 
\end{theorem}
\begin{remark}
Equations \eqref{eq:implementation} can be considered as a natural extension of the state space realization of a controller $\tf K$, which is given by
\begin{eqnarray}
z \ttf{\xi} &=& A_K \ttf{\xi} + B_K \tf y \nonumber\\
\tf u &=& C_K \ttf{\xi} + D_K \tf y. \label{eq:sss}
\end{eqnarray}
Here we extend the constant matrices $A_K, B_K, C_K, D_K$ in \eqref{eq:sss} into stable proper transfer matrices $\tf{\tilde{R}^{+}}, \tf{\tilde{M}}, \tf{\tilde{N}}, \tf L$ in \eqref{eq:implementation}. As a result, the variable $\ttf{\beta}$ in \eqref{eq:imple2} is called the \emph{controller's internal state}.
\end{remark}

From Theorem \ref{thm:1}, we know that the constraints \eqref{eq:main_1} - \eqref{eq:main_stable} is equivalent to the internally stabilizing constraint in \eqref{eq:trad_stable}. We formulate the \emph{localized optimal control problem} by
%The key observation of the localized optimal control framework \cite{2015_PartI} is that the controller need not be implemented as a map $\tf K$ from measurements $\tf y$ to control actions $\tf u$, but rather admits a parameterization in terms of four closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ that define the closed loop maps from $\ttf{\delta_x}$ and $\ttf{\delta_y}$ to the state $\tf x$ and control action $\tf u$. Specifically, these closed loop maps are defined by the equation
%By working directly with these transfer matrices, suitably structured controllers and controller synthesis problems can be defined that address the issues of scalable synthesis and implementation described above.
\begin{subequations} \label{eq:LOC}
\begin{align}
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize  }} \quad & g(\tf R,\tf M,\tf N,\tf L) \label{eq:main_obj}\\
\text{subject to }  \quad & \eqref{eq:main_1} - \eqref{eq:main_stable} \label{eq:main_affine}\\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \s \label{eq:main_S}
\end{align}
\end{subequations}
where $g(\cdot)$ is a convex objective function and $\mathcal{S}$ a convex set constraint. 
%In our previous works, we point out that the distributed controller does not need to be implemented directly by $K$, so $K$ need not be sparse. Instead, we introduce four closed loop transfer matrices $(R,M,N,L)$ to link the relation between closed loop response, controller implementation, and controller synthesis. 
%In the first part of the paper \cite{2015_PartI}, we showed that for a system with dynamics given by \eqref{eq:dynamics}, there exists an internally stabilizing controller that achieves the desired closed loop response in \eqref{eq:desired} if and only if \eqref{eq:main_1} - \eqref{eq:main_stable} is feasible. More specifically, we have the following theorem from \cite{2015_PartI}.

We now compare the localized optimal control formulation \eqref{eq:LOC} with the conventional distributed optimal control formulation \eqref{eq:trad}.  Recall that the objective function in \eqref{eq:trad_obj} is the norm of the closed loop transfer matrix from $\tf w$ to $\tf{\bar{z}}$. We can rewrite \eqref{eq:trad_obj} in terms of the closed loop transfer matrices defined in \eqref{eq:desired} as
\begin{equation}
||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||, \label{eq:trad_obj2}
\end{equation}
which is a special case of the convex objective function $g(\cdot)$ in \eqref{eq:main_obj}. The subspace constraint $\tf K \in \K$ in \eqref{eq:trad_info} does not necessary correspond to a convex set constraint $\s$ in \eqref{eq:main_S}. However, we showed in \cite{2015_PartI} that when the subspace constraint $\K$ is QI with respect to $\tf P_{22}$, the corresponding set constraint $\s$ in \eqref{eq:main_S} is always a convex set. In other words, all the convex problems that can be identified using the QI theory can be identified using the localized formulation \eqref{eq:LOC}. On the other hand, we can identify many other convex problems that does not satisfy the QI condition \cite{2015_PartI}. One particular interesting example is the sparsity constraint considered in this paper.

%\begin{remark}
%Whereas the distributed optimal control framework requires a transformation between the optimization variable $\tf Q$ and the controller $\tf K$, we directly implement the controller in terms of the optimization variables $(\tf R, \tf M, \tf N, \tf L)$. In doing so, we are able to avoid the issues of non-convexity caused by a sparsity constraint set $\K$ -- however, it is possible to impose constraints that lead to an infeasible problem, and thus our results are still consistent with established results on the hardness of distributed control subject to non-classical information patterns \cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}.
%\end{remark}

%such that the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ satisfy
%\begin{equation}
%\begin{bmatrix} \tf x \\ \tf u \end{bmatrix} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} \ttf{\delta_x} \\ \ttf{\delta_y} \end{bmatrix}\label{eq:desired}
%\end{equation}
%if and only if $( z \tf R, z \tf M, z \tf N, \tf L)\in\RHinf$ and
%\begin{subequations}
%\begin{align}
% \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:local1} \\
% \begin{bmatrix} \tf R &\tf N \\ \tf M & \tf L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix}. \label{eq:local2} 
%\end{align}
%\end{subequations}
%and $\s$ a spatio-temporal constraint on the closed loop transfer matrices. In general, constraint $\s$ is the intersection of the following three different constraints: (i) the delay constraint $\mathcal{C}$ imposed by the communication network, (ii) the locality (sparsity) constraint $\mathcal{L}$ to enhance scalability, and (iii) the finite impulse response (FIR) constraint $\mathcal{F}$ to make the optimization problem \eqref{eq:local_obj} - \eqref{eq:local_S} finite dimensional. In the rest of this paper, we focus our discussion on the role of the locality (sparsity) component of $\s$. Consider the following theorem from \cite{2014_Wang_Allerton}.

%\input{Implementation_old}
\subsection{Localized Implementation} \label{sec:imp}
In \cite{2015_PartI}, we showed how to use the $\s$-localizability constraint in \eqref{eq:main_S} to design a controller that is scalable to implement. 
We first express the localizability constraint $\s$ \eqref{eq:main_S} as the intersection of three convex set components: the locality (sparsity) constraint $\Ell$, the finite impulse response (FIR) constraint $\FT$, and an arbitrary convex set component $\Sother$. 
This leads to the localized optimal control problem given by
\begin{eqnarray}
\underset{\{\tf R, \tf M,\tf N, \tf L\}}{\text{minimize}} \quad && g(\tf R,\tf M,\tf N,\tf L) \nonumber\\
\text{subject to} \quad && \eqref{eq:main_1} - \eqref{eq:main_stable} \nonumber \\
&& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \cap \Sother \label{eq:localized}
\end{eqnarray}
with $\s = \Ell \cap \FT \cap \Sother$. 
%We have $\s = \Ell \cap \FT \cap \Sother$.
The constraint $\Sother$ includes any convex constraint imposed by the system. For instance, the information sharing constraint $\C$ can be a component of $\Sother$. Constraints $\Ell$ and $\FT$ are the additional constraints we imposed. The locality constraint $\Ell$ on a transfer matrix $\tf G$ is a collection of the sparsity constraints with the form $\tf G_{ij} = 0$ for some $i$ and $j$. The constraint $\FT$ restricts the optimization variables to have finite impulse responses of horizon $T$, which makes \eqref{eq:localized} a finite dimensional convex program. 

Our approach to design a controller that is scalable to implement is to impose sparsity constraint on the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ through the locality constraint $\Ell$. 
Theorem \ref{thm:1} shows how the sparsity of the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ translates into the implementation complexity of a controller as in \eqref{eq:implementation}. 
For instance, if the rows of these transfer matrices are suitably sparse, then each sub-controller only needs to collect a small number of measurements and controller internal states to compute its control law. 
This holds true for arbitrary objective function $g(\cdot)$ and arbitrary set constraint $\Sother$.

%The locality constraint $\Ell$ is the mechanism that we use to impose this sparsity.  

It should be noted that although optimization problem \eqref{eq:localized} is convex for any affine constraint set $\Ell$, it is not necessarily feasible. 
In \cite{2015_Wang_Reg, 2015_PartI}, we showed that a necessary condition for the existence of a sparse (localized) closed loop response for a strongly connected plant is that the communication speed between sub-controllers is faster than the speed of disturbance propagation in the plant.
%constraint in $\Sother$ is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant. 
This condition is slightly more strict than the communication speed condition for QI to hold. However, as long as a localized closed loop response exists, we only need to use fast but \emph{local} communication to implement the controller.
%This is because the subsystems are dynamically coupled to each other (as per \eqref{eq:interconnected}), and hence it may not always be possible to localize the effect of a disturbance affecting subsystem $j$ to a pre-specified $d$-outgoing set $\Down{j}{d}$. 
%Intuitively, optimization problem \eqref{eq:localized} is feasible when the communication constraint in $\Sother$ is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant. 
%In this way, the necessary sub-controllers can take action \emph{before} a disturbance perturbs their subsystem and stop it from propagating to the rest of the system.  Implicit in this argument are the assumptions that information can be shared quickly between sub-controllers, and that sensors and actuators are strategically placed (these assumptions are discussed in detail in \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}).

\subsection{Problem Statement}
In the first part of this two-part paper, we showed that by imposing additional constraints $\Ell$ and $\FT$ in \eqref{eq:localized}, we can design a localized optimal controller that is scalable to implement. In this paper, we further show that localized optimal controller can be \emph{synthesized} in a localized and scalable way if the objective function $g(\cdot)$ and the localizability constraint set $\s$ satisfy certain technical condition. 

%The goal of this paper is to use the constraints $\Ell$ and $\FT$ to enhance the scalability of controller synthesis and controller implementation for large-scale systems. The scalability of controller implementation is discussed in Section \ref{sec:imp}, while the scalability of controller synthesis is discussed in Section \ref{sec:sf} and Section \ref{sec:of}. 
%We have thus far argued that localized controllers are scalable to implement -- what remains to be shown is that they are also scalable to synthesize. The goal of this paper is to identify the technical conditions on the objective function $g(\cdot)$ and the convex component $\Sother$ such that the optimization problem \eqref{eq:localized} can be solved in a scalable manner. 
%Although the optimization problem \eqref{eq:local_obj} - \eqref{eq:local_S} is convex, it is still a \emph{large-scale} optimization problem. The goal of this paper is to provide a scalable algorithm to \emph{solve} \eqref{eq:local_obj} - \eqref{eq:local_S} in a localized way with \eqref{eq:local_obj} being the LQG cost.
%Our approach is to exploit the structure of locality constraint $\Ell$ and the interconnection graph underlying the dynamics \eqref{eq:dynamics} to decompose the large-scale global optimization problem \eqref{eq:localized} into easily solved sub-problems of moderate size. In what follows we present an ADMM based algorithm for solving problem \eqref{eq:localized} that requires each subsystem $j$ to solve a sub-problem defined only by the state-space parameters of subsystems contained in its $d$-outgoing and $d$-incoming sets $\Down{j}{d}$ and $\Up{j}{d}$, respectively. In addition, the computation performed at each subsystem can be done parallel: thus the computational complexity, memory usage and parallel computation time needed at each subsystem are only a function of the size of the $d$-incoming and $d$-outgoing sets of the system.

%our previous works do not discuss on how to solve \eqref{eq:local1} - \eqref{eq:local_S} in a localized way, so the synthesis procedure is not scalable. 
%In this paper, we will show that \eqref{eq:local1} - \eqref{eq:local_S} can also be solved in a localized way for a $\mathcal{H}_2$ norm objective.
%Compare with disturbance localization and Bullo's decoupling control law
%when there may not exist a natural partition, decomposition
%design constraint (partial model information), implementation constraint
%In this paper, we are interested in the case when the matrices in \eqref{eq:dynamics} are \emph{large} but \emph{sparse}. We aim to develop a method that exploits the sparsity structure of these matrices to enhance scalability of controller synthesis and implementation. 
%In this paper, we will reformulate \eqref{eq:trad} in terms of the \emph{closed loop transfer matrices} rather than Youla parameter. With a slightly change in the last constraint in \eqref{eq:trad}, we characterize a much broader class of convex problems in the field of distributed control.



==> LLQG_Prelim_v2.tex <==
We first discuss the challenges of control design for large-scale interconnected systems. We then explain why the distributed optimal control formulation has an intrinsic difficulty to scale to large-scale interconnected systems. We then recall the results of \cite{2015_PartI} in which we defined the localized optimal control framework. This section ends with the problem statement of the paper.

%\subsection{System Model}
%In this paper, we consider a discrete time linear time invariant system (LTI) with dynamics given by
%\begin{eqnarray}
%x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber\\
%y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics} 
%\end{eqnarray}
%where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. 
%Equation \eqref{eq:dynamics} can be written in state space form as
%\begin{equation}
%\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & D_{11} & D_{12} \\ C_2 & D_{21} & D_{22} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
%\end{equation}
%where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. We refer to $\tf P$ the open loop plant model. The stability of $\tf P$ is determined by the matrix $A$. In this paper, a square matrix $A$ is called a stable matrix if its spectral radius is less than $1$, i.e., all the eigenvalues of $A$ lie within the unit circle. We assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable. In this case, the open loop plant $\tf P$ is stable if and only if $A$ is a stable matrix. 

\subsection{Optimal Control for Interconnected Systems} \label{sec:challenge}
\input{Model_v2}
%We consider distributed systems described by linear time-invariant (LTI) dynamics and composed of a collection of subsystems that interact with each other according to a network topology specified by the interaction graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$. Here $\mathcal{V} = \{1, \dots, n\}$ denotes the set of subsystems: to each subsystem $i$ we associate a state vector $x_i$, control action $u_i$, and measurement $y_i$; and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems: an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$. We use $|\mathcal{V}|$ and $|\mathcal{E}|$ to denote the cardinality of the set $\mathcal{V}$ and $\mathcal{E}$, respectively. Defining the (incoming) neighbor set $\mathcal{N}_i$ of subsystem $i$ to be $\mathcal{N}_i = \{j | (i,j) \in \mathcal{E}\}$, may then write the dynamics of subsystem $i$ as
%\begin{eqnarray}
%x_i[k+1] &=& A_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[k] + B_{ii} u_i[k] + \delta_{x_i}[k] \nonumber\\
%y_i[k] &=& C_{ii} x_i[k] + \delta_{y_i}[k], \label{eq:interconnected}
%\end{eqnarray}
%where $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ are matrices of compatible dimensions, and $\delta_{x_i}$ and $\delta_{y_i}$ denote state and measurement perturbations, respectively. 
%The following is a simple example in the form of \eqref{eq:interconnected}.
%%, which is used to illustrate several ideas throughout this paper.
%\begin{example}
%Consider a network system with interconnected topology given by Fig. \ref{fig:Chart105}. Each sub-system $x_i$ is assumed to have two interacting scalar states $x_{i,1}, x_{i,2}$, a sensor on $x_{i,1}$, and an actuator on $x_{i,2}$. The interaction between two neighboring sub-systems is illustrated in Fig. \ref{fig:inter}, where $x_{i,1}$ can affect $x_{j,2}$ if $i$ and $j$ are neighbor. This model is inspired from the second-order dynamics in power network or mechanical system. Specifically, consider a second-order equation
%\begin{equation}
%m_i \ddot{\theta_i} + d_i \dot{\theta_i} = -\sum_{j \in \mathcal{N}_i} k_{ij} (\theta_i - \theta_j) + w_i + u_i \nonumber
%\end{equation}
%for some scalar $\theta_i$.
%If we define the state vector by $x_i = [\theta_i \quad \dot{\theta_i}]^\top$, take the measurement on $\theta_i$, and use $e^{A \Delta t} \approx I + A \Delta t$ to discretize the plant, we get a discretized plant model with interaction graph described by Fig. \ref{fig:inter}.
%\end{example}
%\begin{figure}[t!]
%      \centering
%      \subfigure[Interconnected topology]{%
%      \includegraphics[width=0.35\textwidth]{./figure/Topology.pdf}
%      \label{fig:Chart105}}      
%      \subfigure[Interaction between neighboring sub-systems]{%
%      \includegraphics[width=0.35\textwidth]{./figure/Interaction.pdf}
%      \label{fig:inter}}      
%      \caption{Illustrative Example}
%\end{figure}
%
%More generally, we consider global system model with dynamics given by
%\begin{eqnarray}
%x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber\\
%y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics} 
%\end{eqnarray}
%where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. We use $n_x, n_y$, and $n_u$ to denote the dimension of $x, y$, and $u$, respectively. In this paper, we are particularly interested in the case in which the matrices $(A,B_2,C_2)$ are large-scale but fairly sparse. For example, if the global system model $(A,B_2,C_2)$ is constructed by the interconnected system model described in \eqref{eq:interconnected}, then we have
%\begin{equation}
%A = \begin{bmatrix} A_{11} & \cdots & A_{1n} \\ \vdots & \ddots & \vdots \\ A_{n1} & \cdots & A_{nn} \end{bmatrix} \nonumber
%\end{equation}
%and $B_2 = \textbf{diag}(B_{11}, \dots, B_{nn})$ and $C_2 = \textbf{diag}(C_{11}, \dots, C_{nn})$. When the number of nodes of the interaction graph is large and the interconnected topology is sparse ($|\mathcal{E}| \ll n^2$), the matrices $(A,B_2,C_2)$ are all large-scale but sparse. The goal of this paper is to exploit the sparsity pattern of the system matrices $(A,B_2,C_2)$ to derive a scalable algorithm for controller synthesis. Note that our method can be applied on general system matrices. In particular, the matrices $B_2$ and $C_2$ does not need to be block diagonal as in the interconnected system model \eqref{eq:interconnected}. Throughout the paper, we assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable.
%
%Let the disturbances be given by $\delta_x = B_1 w$ and $\delta_y = D_{21} w$ for some matrices $B_1$ and $D_{12}$, and a disturbance vector $w$. Let $\bar{z}$ be a controlled output given by $\bar{z}[k] = C_1 x[k] + D_{12} u[k]$. The system equations in \eqref{eq:dynamics} can then be written in transfer function form as
%\begin{equation}
%\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & {0} & D_{12} \\ C_2 & D_{21} & {0} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
%\end{equation}
%where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. 

%This example is inspired from the discrete time double integrator model in mechanical or power system. The method described in this paper can generalize to other sub-system models with arbitrary interconnected topology as well.
%Although this example is extremely simple, our method can be applied on a much broader class of problems. In particular, we demonstrate our algorithm on a large system with randomized topology, randomized entries, sparse actuation, and sparse sensing in Section \ref{sec:simu}.}

\subsection{Distributed Optimal Control Framework}
In order to incorporate the communication delay constraints between sub-controllers into the control design process, a common way is imposing an additional subspace constraint $\tf K \in \K$ in \eqref{eq:centralized}. For instance, suppose that there is $\tau$ steps of time delay to transmit the measurement $y_j$ to the control $u_i$. Then we impose the constraints $K_{ij}[t] = 0$ for $t = 0, \dots, \tau -1$. This leads to the distributed optimal control problem given by
%Interconnected systems \eqref{eq:interconnected} pose fundamental challenge to controller synthesis -- the additional information sharing constraint between sub-controllers usually make the distributed optimal control problem non-convex.
%Designing controllers for interconnected systems \eqref{eq:interconnected} can be very challenging for two distinct reasons: (i) in general, the optimal control problem may be intractable \cite{1968_Witsenhausen_counterexample}, and (ii) even if the problem is tractable, the resulting synthesis problem may not scale gracefully to large systems. 
%Although recent work \cite{2006_Rotkowitz_QI_TAC} has been very successful in identifying tractable (i.e., convex) classes of such problems, as described in the introduction, there has been less focus on scalability. 
%Before describing our scalable controller synthesis framework, 
%Here we briefly recall the distributed optimal control framework, and show why scalability issues may arise when dealing with large systems.
%(i) the effect of sub-system interaction $A_{ij}$ is strong, and (ii) the number of sub-systems $n$ is large. The distributed method and the completely local method can handle one of the situations above, but not both.
%By completely local method, for an extreme case, the controller is implemented \emph{and} designed in a purely local way. Specifically, each local control rule is given by $u_i = K_i y_i$, where $K_i$ is designed with the local plant model $(A_{ii}, B_{ii}, C_{ii})$ \emph{only}. Clearly, such control scheme is scalable to arbitrary large $n$, but does not guarantee global stability if the effect of $A_{ij}$ is not negligible.
%We also assume that each sub-system can communicate and collaborate with each other. The general goal is to design a global control action $u = [u_1^\top, \dots, u_n^\top]^\top$ as a function of the global measurement $y = [y_1^\top, \dots, y_n^\top]^\top$ that achieves internal stability and some sort of optimality.
%When the number $n$ go large, localized implementation, localized model information, localized synthesis
%The interconnected system model can also be written in the global form as
%Consider a dynamic output feedback control law $\tf u = \tf K \tf y$. The distributed optimal control problem of minimizing the norm of the closed loop transfer matrix from external disturbance $\tf w$ to regulated output $ \tf{\bar{z}}$ is commonly formulated as
%of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$.} of the closed loop transfer function from $w$ to $\bar{z}$ is formulated as
\begin{subequations}\label{eq:trad}
\begin{align}
\underset{\tf K}{\text{minimize  }} \quad & ||\tf P_{11} + \tf P_{12} \tf K(I-\tf P_{22}\tf K)^{-1} \tf P_{21}\| \label{eq:trad_obj}\\
\text{subject to  } \quad & \tf K \text{ internally stabilizes } \tf P \label{eq:trad_stable}\\ 
& \tf K \in \K. \label{eq:trad_info}
\end{align}
\end{subequations}
%where the subspace constraint $\tf K \in \K$ enforces information sharing constraints between the sub-controllers. 
The additional information sharing constraint \eqref{eq:trad_info} makes the distributed optimal control problem significantly more difficult than the centralized one. 
When $\K$ is a subspace constraint, it has been shown that \eqref{eq:trad} is convex if \cite{2006_Rotkowitz_QI_TAC} and only if \cite{2014_Lessard_convexity} $\K$ is quadratically invariant (QI) with respect to $\tf P_{22}$, i.e., $\tf K \tf P_{22} \tf K \in \K$ for all $\tf K \in \K$. 
Roughly speaking, QI condition holds when sub-controllers are able to share information with each other at least as quickly as their control actions propagate through the plant \cite{2010_Rotkowitz_QI_delay}. This allows us to design distributed controller subject to practical communication delay constraints.

%If QI condition is satisfied, we have $\K = \Q$ and thus \eqref{eq:trad2} is a convex program. 
%The set of internally stabilizing controller is commonly characterized by Youla parameterization \cite{1976_Youla_parameterization}. For simplicity, we only consider the situation when $\tf P$ is open loop stable. In this case, the Youla parameter is given by $\tf Q = \tf K(I- \tf P_{22} \tf K)^{-1}$, and the optimization problem \eqref{eq:trad} can be equivalently formulated as
%\begin{eqnarray}
%\underset{\tf Q}{\text{minimize  }} &&|| \tf P_{11} + \tf P_{12} \tf Q \tf P_{21}|| \nonumber\\
%\text{subject to } && \tf Q \in \RHinf \nonumber\\
%&& \tf Q \in \Q,  \label{eq:trad2}
%\end{eqnarray}
%where the set $\Q$ is given by $\Q = \{ \tf K(I- \tf P_{22} \tf K)^{-1} | \tf K \in \K \}$. The convexity of \eqref{eq:trad2} depends solely on the convexity of the set $\Q$.
%It was shown in \cite{2006_Rotkowitz_QI_TAC} that if the constraint set $\mathcal{C}$ is quadratically invariant with respect to $\tf P_{22}$ then the optimal control problem admits a convex reformulation. 

However, the QI theory has less emphasis on the scalability of controller synthesis and implementation. For instance, when the interconnected system \eqref{eq:interconnected} is strongly connected, the transfer matrix $\tf P_{22} = C_2 (zI-A)^{-1} B_2$ is always dense even though the matrices $(A,B_2,C_2)$ are highly sparse. In this case, a sparsity constraint $\K$ imposed on $\tf K$ in \eqref{eq:trad} is not QI, and \eqref{eq:trad} cannot be reformulated in a convex manner in the Youla domain.
%induces a non-convex constraint set $\Q$ on $\tf Q$ in \eqref{eq:trad2}, which makes the distributed optimal control problem non-convex. 
In other words, for a strongly connected plant, the distributed optimal control problem is convex only when the transfer matrix $\tf K$ is dense, i.e., each local measurement $\tf y_i$ needs to be shared among all the sub-controllers in the network. 
%This controller implementation does not scale gracefully to large systems.
%Assume that for a given constraint $\mathcal{C}$, the optimal controller $\tf K$ can be computed: the implementation complexity of $\tf K$ is then determined by the densest row $\tf K_i$ of $\tf K$.  Specifically, if we consider the control action taken at subsystem $i$, which is specified by $\tf u_i = \tf K_i \tf y$, then if $\tf K_i$ is completely dense then subsystem $i$ must collect measurements from every other subsystem $j \in \mathcal{V}$.  As the number of subsystems grows large, this then leads to a very complex controller implementation.  A natural solution to this problem is to impose sparsity constraints on the controller $\tf K$ such that each row only has a small number of nonzero terms -- in this way each subsystem $i$ only needs to collect a small number of measurements to compute its control action.  Unfortunately, this naive approach fails if the dynamics of $\tf P_{22}$ are strongly connected because in that case, any sparse constraint set $\mathcal{C}$ is not QI with respect to $\tf P_{22}$.  
Although recent methods based on convex relaxations \cite{2014_Fazelnia_ODC} can be used to solve certain cases of the non-convex optimal control problem \eqref{eq:trad} approximately with a sparse constraint set $\K$, the underlying synthesis optimization problem is still large-scale and does not admit a scalable reformulation. The need to address scalability, both in the \emph{synthesis} and \emph{implementation} of a controller, is the driving motivation behind the localized optimal control framework, which we recall in the next subsection.

%It has been shown that \eqref{eq:trad} admits a convex reformulation in the Youla domain if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$. The class of QI constraint, however, is not amenable for large-scale problem. This is due to the fact that the sparsity constraint on $K$ is generally not QI for a plant with strongly connected topology (which can be inferred from the delay interpretation of QI in \cite{2010_Rotkowitz_QI_delay}). For instance, even when $A$ in \eqref{eq:dynamics} is as sparse as a tridiagonal matrix, the QI condition requires all the local measurements to be shared among \emph{every controllers} in the network. 
%It is true that the controller implementation for \eqref{eq:trad} is scalable to large $n$ when $\s_c$ is a sparsity constraint. In this case, however, \eqref{eq:trad} is generally non-convex and hard to solve if the plant has a strongly connected topology. 
%The delay constraint for QI
%As alluded to in the introduction, the class of QI constraint is not amenable for large-scale problem. This is due to the fact that the sparsity constraint on $K$ is generally not QI for a plant with strongly connected topology\footnote{This means that $P_{22}$ is not sparse} \cite{2010_Rotkowitz_QI_delay, 2009_Swigart_graph_QI}. Even when $A$ in \eqref{eq:dynamics} is as sparse as a tridiagonal matrix, the QI condition requires all the local measurements to be shared among \emph{every controllers} in the network. Such a controller implementation is not scalable to large systems. In addition, \eqref{eq:trad} is a large-scale optimization problem, and it is generally hard to solve in a scalable way.
%It can be seen that the objective function in \eqref{eq:trad} is not convex in $K$. As a result, Youla parameterization is used to reformulate \eqref{eq:trad} in terms of the Youla parameter, and it admits a convex reformulation if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$.
%Traditionally, Youla parameterization is used to reformulate \eqref{eq:trad} into a convex manner. It is known that the constraint $\s_c$ remains convex on the Youla parameter if and only if $\s_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \s_c$ for all $K \in \s_c$.

\subsection{Localized Optimal Control Framework}
%Our previous work on localized optimal control \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton} is built on the observation 
In the first part of this two-part paper \cite{2015_PartI}, we introduced a more general framework to incorporate constraints into the optimal control problem. The key idea is to reformulate the optimal control problem in the domain of \emph{closed loop transfer matrices}.
%design the closed loop response first, then construct an internally stabilizing controller to achieve the desired closed loop response. %based on the notion of \emph{closed loop transfer matrices}. 
For an LTI system with dynamics given by \eqref{eq:dynamics}, the closed loop transfer matrices $\{\tf R, \tf M, \tf N, \tf L\}$ are defined by the relation
\begin{equation}
\begin{bmatrix} \tf x \\ \tf u \end{bmatrix} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} \ttf{\delta_x} \\ \ttf{\delta_y} \end{bmatrix}. \label{eq:desired}
\end{equation}
%where $\ttf{\delta_x} = B_1 \tf w$ is the disturbance on the state vector, and $\ttf{\delta_y} = D_{21} \tf w$ is the disturbance on the measurement. 
We showed that the parameterization of all stable achievable closed loop transfer matrices $\{\tf R, \tf M, \tf N, \tf L\}$ is described by the solution of the following equations:
\begin{subequations} \label{eq:achievable}
\begin{align}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} &= 
\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:main_1} \\
\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix}
\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} &= 
\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:main_2} \\
\tf R, \tf M, \tf N \in \frac{1}{z} \mathcal{RH}_{\infty}, & \quad \tf L \in \mathcal{RH}_{\infty}. \label{eq:main_stable}
\end{align}
\end{subequations}
The parameterization of all internally stabilizing controller is given by the following theorem.
%The following theorem gives an implementation of the controller that achieves the desired closed loop response.
\begin{theorem}
Suppose that a set of transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ satisfy the constraints \eqref{eq:main_1} - \eqref{eq:main_stable}. Then an internally stabilizing controller yielding the desired closed loop response \eqref{eq:desired} can be implemented as
\begin{subequations}\label{eq:implementation}
\begin{align}
z \ttf{\beta} &= \tilde{\tf R}^+ \ttf{\beta} + \tilde{\tf N} \tf y \label{eq:imple1}\\
\tf u &=  \tilde{\tf M} \ttf{\beta} + \tf L \tf y \label{eq:imple2}
\end{align}
\end{subequations}
where $ \tilde{\tf R}^+ = z(I - z\tf R)$, $\tilde{\tf N} = -z\tf N$, $\tilde{\tf M} = z\tf M$, $\tf L$ are in $\RHinf$. \label{thm:1} Further, the solutions of \eqref{eq:main_1} - \eqref{eq:main_stable} with the implementation \eqref{eq:implementation} parameterize all internally stabilizing controller. 
\end{theorem}
\begin{remark}
Equations \eqref{eq:implementation} can be considered as a natural extension of the state space realization of a controller $\tf K$, which is given by
\begin{eqnarray}
z \ttf{\xi} &=& A_K \ttf{\xi} + B_K \tf y \nonumber\\
\tf u &=& C_K \ttf{\xi} + D_K \tf y. \label{eq:sss}
\end{eqnarray}
Here we extend the constant matrices $A_K, B_K, C_K, D_K$ in \eqref{eq:sss} into stable proper transfer matrices $\tf{\tilde{R}^{+}}, \tf{\tilde{M}}, \tf{\tilde{N}}, \tf L$ in \eqref{eq:implementation}. As a result, the variable $\ttf{\beta}$ in \eqref{eq:imple2} is called the \emph{controller's internal state}.
\end{remark}

From Theorem \ref{thm:1}, we know that the constraints \eqref{eq:main_1} - \eqref{eq:main_stable} is equivalent to the internally stabilizing constraint in \eqref{eq:trad_stable}. The complete form of the localized optimal control problem \eqref{eq:clock} is then given by
%The key observation of the localized optimal control framework \cite{2015_PartI} is that the controller need not be implemented as a map $\tf K$ from measurements $\tf y$ to control actions $\tf u$, but rather admits a parameterization in terms of four closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ that define the closed loop maps from $\ttf{\delta_x}$ and $\ttf{\delta_y}$ to the state $\tf x$ and control action $\tf u$. Specifically, these closed loop maps are defined by the equation
%By working directly with these transfer matrices, suitably structured controllers and controller synthesis problems can be defined that address the issues of scalable synthesis and implementation described above.
\begin{subequations} \label{eq:LOC}
\begin{align}
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize  }} \quad & g(\tf R,\tf M,\tf N,\tf L) \label{eq:main_obj}\\
\text{subject to }  \quad & \eqref{eq:main_1} - \eqref{eq:main_stable} \label{eq:main_affine}\\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \s \label{eq:main_S}
\end{align}
\end{subequations}
where $g(\cdot)$ is a convex objective function and $\mathcal{S}$ a convex set constraint. 
%In our previous works, we point out that the distributed controller does not need to be implemented directly by $K$, so $K$ need not be sparse. Instead, we introduce four closed loop transfer matrices $(R,M,N,L)$ to link the relation between closed loop response, controller implementation, and controller synthesis. 
%In the first part of the paper \cite{2015_PartI}, we showed that for a system with dynamics given by \eqref{eq:dynamics}, there exists an internally stabilizing controller that achieves the desired closed loop response in \eqref{eq:desired} if and only if \eqref{eq:main_1} - \eqref{eq:main_stable} is feasible. More specifically, we have the following theorem from \cite{2015_PartI}.
We showed in \cite{2015_PartI} that \eqref{eq:LOC} is a generalization of \eqref{eq:trad} in the following sense: (i) all the convex problems that can be identified using the QI theory are convex in the localized formulation \eqref{eq:LOC}, while there are some convex problems that cannot be identified using the theory of QI, and (ii) the objective function in \eqref{eq:LOC} is more general. Specifically, the objective function in \eqref{eq:trad_obj} can be written as
\begin{equation}
||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||, \label{eq:trad_obj2}
\end{equation}
which is a special case of the convex objective function $g(\cdot)$ in \eqref{eq:main_obj}.

%We now compare the localized optimal control formulation \eqref{eq:LOC} with the distributed optimal control formulation \eqref{eq:trad}.  Recall that the objective function in \eqref{eq:trad_obj} is the norm of the closed loop transfer matrix from $\tf w$ to $\tf{\bar{z}}$. We can rewrite \eqref{eq:trad_obj} in terms of the closed loop transfer matrices defined in \eqref{eq:desired} as
%\begin{equation}
%||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||, \label{eq:trad_obj2}
%\end{equation}
%which is a special case of the convex objective function $g(\cdot)$ in \eqref{eq:main_obj}. The subspace constraint $\tf K \in \K$ in \eqref{eq:trad_info} does not necessary correspond to a convex set constraint $\s$ in \eqref{eq:main_S}. However, we showed in \cite{2015_PartI} that when the subspace constraint $\K$ is QI with respect to $\tf P_{22}$, the corresponding set constraint $\s$ in \eqref{eq:main_S} is always a convex set. In other words, all the convex problems that can be identified using the QI theory can be identified using the localized formulation \eqref{eq:LOC}. On the other hand, we can identify many other convex problems that does not satisfy the QI condition \cite{2015_PartI}. One particular interesting example is the sparsity constraint considered in this paper.
%
%\begin{remark}
%Whereas the distributed optimal control framework requires a transformation between the optimization variable $\tf Q$ and the controller $\tf K$, we directly implement the controller in terms of the optimization variables $(\tf R, \tf M, \tf N, \tf L)$. In doing so, we are able to avoid the issues of non-convexity caused by a sparsity constraint set $\K$ -- however, it is possible to impose constraints that lead to an infeasible problem, and thus our results are still consistent with established results on the hardness of distributed control subject to non-classical information patterns \cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}.
%\end{remark}

%such that the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ satisfy
%\begin{equation}
%\begin{bmatrix} \tf x \\ \tf u \end{bmatrix} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} \ttf{\delta_x} \\ \ttf{\delta_y} \end{bmatrix}\label{eq:desired}
%\end{equation}
%if and only if $( z \tf R, z \tf M, z \tf N, \tf L)\in\RHinf$ and
%\begin{subequations}
%\begin{align}
% \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:local1} \\
% \begin{bmatrix} \tf R &\tf N \\ \tf M & \tf L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix}. \label{eq:local2} 
%\end{align}
%\end{subequations}
%and $\s$ a spatio-temporal constraint on the closed loop transfer matrices. In general, constraint $\s$ is the intersection of the following three different constraints: (i) the delay constraint $\mathcal{C}$ imposed by the communication network, (ii) the locality (sparsity) constraint $\mathcal{L}$ to enhance scalability, and (iii) the finite impulse response (FIR) constraint $\mathcal{F}$ to make the optimization problem \eqref{eq:local_obj} - \eqref{eq:local_S} finite dimensional. In the rest of this paper, we focus our discussion on the role of the locality (sparsity) component of $\s$. Consider the following theorem from \cite{2014_Wang_Allerton}.

%\input{Implementation_old}
%\subsection{Localized Implementation} \label{sec:imp}
In \cite{2015_PartI}, we showed how to use the convex set constraint \eqref{eq:main_S} to design a controller that is scalable to implement. 
We first express the constraint set $\s$ in \eqref{eq:main_S} as the intersection of three convex set components: the locality (sparsity) constraint $\Ell$, the finite impulse response (FIR) constraint $\FT$, and an arbitrary convex set component $\Sother$, i.e., $\s = \Ell \cap \FT \cap \Sother$. The locality constraint $\Ell$ on a transfer matrix $\tf G$ is a collection of the sparsity constraints with the form $\tf G_{ij} = 0$ for some $i$ and $j$. The constraint $\FT$ restricts the optimization variables to have finite impulse responses of horizon $T$, which makes \eqref{eq:localized} a finite dimensional convex program. The constraint $\Sother$ includes any convex constraint imposed by the system. This leads to the localized optimal control problem given by
\begin{eqnarray}
\underset{\{\tf R, \tf M,\tf N, \tf L\}}{\text{minimize}} \quad && g(\tf R,\tf M,\tf N,\tf L) \nonumber\\
\text{subject to} \quad && \eqref{eq:main_1} - \eqref{eq:main_stable} \nonumber \\
&& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \cap \Sother. \label{eq:localized}
\end{eqnarray}
%We have $\s = \Ell \cap \FT \cap \Sother$.
%For instance, the information sharing constraint $\C$ can be a component of $\Sother$. Constraints $\Ell$ and $\FT$ are the additional constraints we imposed.  

Our approach to design a controller that is scalable to implement is to impose sparsity constraint on the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ through the locality constraint $\Ell$. 
Theorem \ref{thm:1} shows how the sparsity of the closed loop transfer matrices $(\tf R, \tf M, \tf N, \tf L)$ translates into the implementation complexity of a controller as in \eqref{eq:implementation}. 
For instance, if the rows of these transfer matrices are suitably sparse, then each sub-controller only needs to collect a small number of measurements and controller internal states to compute its control law. In particular, the complexity to implement each sub-controller can be made to be independent to the size of the global network.
In contrast to the distributed optimal control framework \eqref{eq:trad}, the localized optimal control framework \eqref{eq:LOC} offers a \emph{convex} way to design a controller that is scalable to implement. This holds true for arbitrary objective function $g(\cdot)$ and arbitrary set constraint $\Sother$.

%The locality constraint $\Ell$ is the mechanism that we use to impose this sparsity.  
\begin{remark}
It should be noted that although optimization problem \eqref{eq:localized} is convex for any affine constraint set $\Ell$, it is not necessarily feasible. 
In \cite{2015_Wang_Reg, 2015_PartI}, we showed that a necessary condition for the existence of a sparse (localized) closed loop response for a strongly connected plant is that the communication speed between sub-controllers is faster than the speed of disturbance propagation in the plant.
%constraint in $\Sother$ is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant. 
This condition is slightly more strict than the communication speed condition for QI to hold. However, as long as a localized closed loop response exists, we only need to use fast but \emph{local} communication to implement the controller.
%This is because the subsystems are dynamically coupled to each other (as per \eqref{eq:interconnected}), and hence it may not always be possible to localize the effect of a disturbance affecting subsystem $j$ to a pre-specified $d$-outgoing set $\Down{j}{d}$. 
%Intuitively, optimization problem \eqref{eq:localized} is feasible when the communication constraint in $\Sother$ is such that information about a disturbance can be transmitted faster than the disturbance propagates through the plant. 
%In this way, the necessary sub-controllers can take action \emph{before} a disturbance perturbs their subsystem and stop it from propagating to the rest of the system.  Implicit in this argument are the assumptions that information can be shared quickly between sub-controllers, and that sensors and actuators are strategically placed (these assumptions are discussed in detail in \cite{2014_Wang_CDC, 2014_Wang_Allerton, 2015_Wang_Reg}).
\end{remark}

\subsection{Problem Statement}
We already showed that by imposing additional constraints $\Ell$ and $\FT$ in \eqref{eq:localized}, we can design a localized optimal controller that is scalable to implement. In this paper, we further show that localized optimal controller can be \emph{synthesized} in a localized and scalable way if the objective function $g(\cdot)$ and the localizability constraint set $\s$ satisfy certain technical condition. By scalable, we mean that the complexity to synthesize each sub-controller in the network is independent to the size of the global network ($O(1)$ complexity). This offers a unified framework to address the three challenges mentioned in Section \ref{sec:challenge} simultaneously.

%The goal of this paper is to use the constraints $\Ell$ and $\FT$ to enhance the scalability of controller synthesis and controller implementation for large-scale systems. The scalability of controller implementation is discussed in Section \ref{sec:imp}, while the scalability of controller synthesis is discussed in Section \ref{sec:sf} and Section \ref{sec:of}. 
%We have thus far argued that localized controllers are scalable to implement -- what remains to be shown is that they are also scalable to synthesize. The goal of this paper is to identify the technical conditions on the objective function $g(\cdot)$ and the convex component $\Sother$ such that the optimization problem \eqref{eq:localized} can be solved in a scalable manner. 
%Although the optimization problem \eqref{eq:local_obj} - \eqref{eq:local_S} is convex, it is still a \emph{large-scale} optimization problem. The goal of this paper is to provide a scalable algorithm to \emph{solve} \eqref{eq:local_obj} - \eqref{eq:local_S} in a localized way with \eqref{eq:local_obj} being the LQG cost.
%Our approach is to exploit the structure of locality constraint $\Ell$ and the interconnection graph underlying the dynamics \eqref{eq:dynamics} to decompose the large-scale global optimization problem \eqref{eq:localized} into easily solved sub-problems of moderate size. In what follows we present an ADMM based algorithm for solving problem \eqref{eq:localized} that requires each subsystem $j$ to solve a sub-problem defined only by the state-space parameters of subsystems contained in its $d$-outgoing and $d$-incoming sets $\Down{j}{d}$ and $\Up{j}{d}$, respectively. In addition, the computation performed at each subsystem can be done parallel: thus the computational complexity, memory usage and parallel computation time needed at each subsystem are only a function of the size of the $d$-incoming and $d$-outgoing sets of the system.

%our previous works do not discuss on how to solve \eqref{eq:local1} - \eqref{eq:local_S} in a localized way, so the synthesis procedure is not scalable. 
%In this paper, we will show that \eqref{eq:local1} - \eqref{eq:local_S} can also be solved in a localized way for a $\mathcal{H}_2$ norm objective.
%Compare with disturbance localization and Bullo's decoupling control law
%when there may not exist a natural partition, decomposition
%design constraint (partial model information), implementation constraint
%In this paper, we are interested in the case when the matrices in \eqref{eq:dynamics} are \emph{large} but \emph{sparse}. We aim to develop a method that exploits the sparsity structure of these matrices to enhance scalability of controller synthesis and implementation. 
%In this paper, we will reformulate \eqref{eq:trad} in terms of the \emph{closed loop transfer matrices} rather than Youla parameter. With a slightly change in the last constraint in \eqref{eq:trad}, we characterize a much broader class of convex problems in the field of distributed control.



==> LLQG_Sensor_Actuator.tex <==
\subsection{LLQG with Sensor Actuator Regularization}\label{sec:sar}
We summarize all the techniques described in this section on the LLQG problem with sensor actuator regularization. This problem is used in Section \ref{sec:simu} as a case study example.
\begin{example}
The LLQG problem with sensor actuator regularization is formulated by 
\begin{subequations} \label{eq:h2l1}
\begin{align} 
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & \eqref{eq:h2_sar} \label{eq:h2l1-1}\\
%||\begin{bmatrix} C_1 & D_{12} \end{bmatrix}\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \lambda \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} 
\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \C \cap \Ell \cap \FT. \label{eq:h2l1-3}
\end{align}
\end{subequations}
where $\C$ encodes the communication delay constraint. %\footnote{The communication delay constraint is specified by the sparsity constraint imposed on each spectral component of $\tf R$, $\tf M$, $\tf N$, and $\tf L$. Consider the controller implementation in \eqref{eq:implementation}. For example, suppose that there is $\tau$ time steps of delay to transmit the measurement $y_j$ to the control $u_i$. Then, we impose the constraint $L_{ij}[t] = 0$ for $t = 0, \dots, \tau - 1$.}
We assume that the matrix $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ in \eqref{eq:h2l1-1} is identity, and $\begin{bmatrix} B_1^\top & D_{12}^\top \end{bmatrix}^\top$ is diagonal. Problem \eqref{eq:h2l1} is decomposable, and thus can be solved by the algorithm \eqref{eq:admm} in a scalable way. Specifically, the $\mathcal{H}_2$ norm and the sensor regularizer belong to the column-wise decomposable component of the objective function, while the actuator regularizer belongs to the row-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
\end{example}

Once the row-wise and the column-wise decomposable components are identified, we decompose the subroutines \eqref{eq:admm1} and \eqref{eq:admm2} into parallel local subproblems. In this example, each local subproblem can be evaluated in analytic form. For the actuator regularizer in the row-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic2}. For the transfer matrix $\begin{bmatrix} \tf R^\top & \tf M^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic1}. 
%Here we discuss the analytic solution for the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part.
For the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the objective function is given by the sum of a convex quadratic and a $\ell_2$ norm, and the constraint is a linear subspace. As $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ is identity, the leading coefficient of the quadratic objective is identity. In this case, the optimization problem can be rewritten into the form as the one in Example \ref{ex:analytic2}, with an additional linear subspace constraint. We can show that the analytic solution is given by a projection onto a linear subspace followed by a vectorial soft-thresholding. 

Finally, the weights $\mu_i$ and $\lambda_i$ in the regularizers \eqref{eq:act_norm} and \eqref{eq:sen_norm} can be properly chosen to further enhance row/column-wise sparsity. We use the reweighted $\ell_1$ algorithm proposed in \cite{Reweighted} to iteratively set the weights and solve \eqref{eq:h2l1} multiple times. Let $\mu_i^{(0)} = \mu_0$ for $i = 1, \dots, n_u$ and $\lambda_i^{(0)} = \lambda_0$ for $i = 1, \dots, n_y$.
Let $(\tf R^{(k)}, \tf M^{(k)}, \tf N^{(k)}, \tf L^{(k)})$ be the optimal solution of \eqref{eq:h2l1} when the weights are given by $\{ \mu_i^{(k)} \}_{i=1}^{n_u}$ and $\{ \lambda_i^{(k)} \}_{i=1}^{n_y}$. We update the weights at iteration $(k+1)$ by
\begin{subequations}
\begin{align}
\mu_i^{(k+1)} &= ( \, || e_i^\top \begin{bmatrix} \tf M^{(k)} & \tf L^{(k)} \end{bmatrix} ||_{\mathcal{H}_2} + \epsilon )^{-1} \nonumber\\
\lambda_i^{(k+1)} &= ( \, || \begin{bmatrix} \tf N^{(k)} \\ \tf L^{(k)} \end{bmatrix} e_i ||_{\mathcal{H}_2} + \epsilon )^{-1} 
\end{align}
\end{subequations}
for some small $\epsilon$. It is shown in \cite{Reweighted} that this reweighted scheme usually results in sparser solution.



==> Localizability_v1.tex <==
The objective function \eqref{eq:main_obj} and the convex set constraint \eqref{eq:main_S} are introduced in this section, which leads to the notion of $\mathcal{S}$-localizability. The general formulation of the optimization problem is given first. We then show that many constraints, including the QI constraints, controllability and observability constraint, and the sparsity constraints, can all be considered as special cases of $\mathcal{S}$-localizability constraint. 
%This section ends up with a detailed robustness analysis of our control scheme in the presence of computation error or model uncertainty by the characterization of \emph{nearly} localizable systems. 

\subsection{General Formulation}
With the parameterization of all stabilizing controller in \eqref{eq:output_fb1} - \eqref{eq:output_fb3}, we now introduce an objective function and an additional constraint imposed on the closed loop transfer matrices. The localized optimal control problem is then formulated by
%formulate the constrained optimization problem as
\begin{eqnarray}
\underset{\{R,M,N,L\}}{\text{minimize    }} && g(R,M,N,L) \nonumber\\
\text{subject to } && \eqref{eq:output_fb1} - \eqref{eq:output_fb3} \nonumber \\
&& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:main_SS}
\end{eqnarray}
where $g(.)$ is the objective function, and $\mathcal{S}$ is a constraint imposed on the closed loop transfer matrices. The feasibility of \eqref{eq:main_SS} is defined as the $\mathcal{S}$-localizability of the system $(A,B_2,C_2)$. In general, we consider the case in which the objective function $g(.)$ is convex with respect to the closed loop transfer matrices, and the constraint $\mathcal{S}$ is a convex set. In this case, \eqref{eq:main_SS} is a convex optimization problem. 

The following example describes the relation between the conventional distributed optimal control formulation \eqref{eq:trad} and our alternative formulation \eqref{eq:main_SS}.
\begin{example}
The objective function in the traditional distributed optimal control formulation \eqref{eq:trad} can be written as
\begin{eqnarray}
g(R,M,N,L) = ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} + D_{11} ||, \nonumber \\ \label{eq:tra_obj}
\end{eqnarray}
which is a convex function of the closed loop transfer matrices. The subspace constraint $K \in \mathcal{S}_c$ in \eqref{eq:trad} does not necessary correspond to a convex set $\mathcal{S}$ in \eqref{eq:main_SS} in general. However, as will be shown in the next subsection, when $\mathcal{S}_c$ is QI with respect to $P_{22}$, the corresponding $\mathcal{S}$ in \eqref{eq:main_SS} is always a convex set. This then implies that all the convex problems in the conventional formulation are convex in our alternative formulation, given that $\mathcal{S}_c$ in \eqref{eq:trad} is a subspace constraint. 
\end{example}

The advantages of our formulation \eqref{eq:main_SS} is twofold: (1) we can identify a much larger class of convex problems in distributed control using the localizability constraint $\mathcal{S}$, and (2) we can deal with more general objective functions.

For the localizability constraint $\mathcal{S}$, note that any sparsity constraint imposed through $\mathcal{S}$ in \eqref{eq:main_SS} is always a convex constraint, but the sparsity constraint imposed on $K$ generally makes the problem \eqref{eq:trad} non-convex. Although the constraint $\mathcal{S}$ in \eqref{eq:main_SS} seems to be a constraint imposed on the closed loop response, it can also be interpreted as a constraint for controller implementation -- if we implement the controller using the structure given in Figure \ref{fig:of}. In this case, the controller achieving the desired closed loop response can be implemented in a localized and thus scalable way. This property makes the formulation \eqref{eq:main_SS} extremely favorable for large-scale systems.

%\begin{remark}
%When the closed loop transfer matrices belong to a convex set $\mathcal{S}$, the corresponding $K$ in the traditional formulation \eqref{eq:trad} generally belong to a non-convex set. 
%\end{remark}

The objective function in \eqref{eq:main_SS} is not limited to the form of \eqref{eq:tra_obj}. For instance, we can define a convex objective consisting of the closed loop transfer matrices in Table \ref{Table:1}. This means that we can deal with the case in which there exists internal additive noise $\delta_\beta$ within the controller structure. We can penalize the internal variable $\beta$ as well.
% which takes into account the effect of $\delta_x, \delta_y, \delta_u, \delta_\beta$ all at once.
This is clearly more general than the traditional optimal control problem \eqref{eq:trad}.

%We now discuss the relation between the conventional distributed optimal control formulation \eqref{eq:trad} and our alternative formulation \eqref{eq:main_SS}. It can be shown that the objective function in \eqref{eq:trad} is equivalent to
%\begin{equation}
%g(R,M,N,L) = ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} + D_{11} || , \nonumber
%\end{equation}
%which is a convex function. 

%We will give a detail discussion in Section \ref{sec:synthesis}.
%It should be noted that 
 
\subsection{Special Cases}
In this subsection, we discuss some special classes of $\mathcal{S}$-localizability constraint.
%show that QI constraint for distributed control and FIR constraint for deadbeat control are both special cases of $\mathcal{S}$-localizability constraint. 

\subsubsection{Quadratic Invariance Constraints}
The following theorem states that QI constraint is a special case of $\mathcal{S}$-localizability constraint.

\begin{theorem}
Assume that the subspace constraint $\mathcal{S}_c$ in \eqref{eq:trad} is quadratically invariant with respect to $P_{22}$. Then, \eqref{eq:trad} can be equivalently formulated as
\begin{eqnarray}
\underset{\{R,M,N,L\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} + D_{11} || \nonumber\\
\text{subject to } && \eqref{eq:output_fb1} - \eqref{eq:output_fb3} \nonumber \\
&& L \in \mathcal{S}_c \label{eq:qieq}
\end{eqnarray} \label{thm:qi}
\end{theorem}
\begin{proof}
As \eqref{eq:output_fb1} - \eqref{eq:output_fb3} corresponds to the stabilizing constraint, we only need to show that $K \in \mathcal{S}_c$ if and only if $L \in \mathcal{S}_c$. By definition, $L$ is the closed loop transfer matrix from $\delta_y$ to $u$. From $y = P_{22}u + \delta_u$, we have $L = K (I - P_{22} K)^{-1}$. Using the QI theorem in \cite{2006_Rotkowitz_QI_TAC}, we have $K \in \mathcal{S}_c$ if and only if $L = K (I - P_{22} K)^{-1} \in \mathcal{S}_c$, which completes the proof.
%Let
%\begin{subequations}
%\begin{align}
%(zI-A) x &= B_2 u + \delta_x \nonumber\\
%y &= C_2 x + D_{22} u + \delta_y \nonumber\\
%u &= K y, \nonumber
%\end{align}
%\end{subequations}
%and $P_{22} = C_2 (zI-A)^{-1} B_2 + D_{22}$. By definition, $L$ is the closed loop transfer matrix from $\delta_y$ to $u$. We can derive 
\end{proof}
%After solving \eqref{eq:qieq}, we can either construct the controller by $R, M, N, L, D_{22}$ directly, or compute $K$ by $K = (I+\tilde{K}D_{22})^{-1}\tilde{K}$, with $\tilde{K} = L - M R^{-1} N$. 

Note that the result in Theorem \ref{thm:qi} holds true regardless the stability of open loop plant $A$. We do not need to assume the existence of an initial strongly stabilizing controller as in \cite{2006_Rotkowitz_QI_TAC}, and we do not need to perform a doubly coprime factorization as in \cite{2014_Sabau_QI}.

\subsubsection{Finite Impulse Response Constraints}
Another interesting case is the FIR constraint for a discrete time system. For example, we can impose the constraint in \eqref{eq:main_SS} such that $R, M, N, L$ are all FIRs with length $T$. Similar to the alternative definition of stabilizability and detectability in \eqref{eq:state_fb1} - \eqref{eq:state_fb2} and \eqref{eq:state_est1} - \eqref{eq:state_est2}, we can define the notion of $T$-step controllability and $T$-step observability as follows.
\begin{definition}[$T$-step controllability and observability]
The pair $(A,B_2)$ is said to be $T$-step controllable if the following equations are feasible.
\begin{subequations}
\begin{align}
& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \nonumber\\
& R = \sum_{i=1}^{T} \frac{1}{z^i} R[i], \quad M = \sum_{i=1}^{T} \frac{1}{z^i} M[i]. \nonumber
\end{align}
\end{subequations} 
Similarly, the pair $(A,C_2)$ is said to be $T$-step observable if the following equations are feasible.
\begin{subequations}
\begin{align}
& \begin{bmatrix} R & N \end{bmatrix} \begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = I  \nonumber\\
& R = \sum_{i=1}^{T} \frac{1}{z^i} R[i], \quad N = \sum_{i=1}^{T} \frac{1}{z^i} N[i]. \nonumber
\end{align}
\end{subequations} 
\end{definition}
\begin{remark}
Note that the definition of $T$-step controllability is that the state can be driven to zero from arbitrary initial condition within $T$ steps. If we want to drive the state to arbitrary final state from any initial condition ($T$-step reachability), we need an additional condition that the matrix $[A \quad B_2]$ has full column rank.
\end{remark}

Imposing a FIR constraint on the closed loop transfer matrices has several advantages:
\begin{enumerate}
  \item The closed loop response of an impulse disturbance is FIR, which implies a short settling time in closed loop.
  \item The controller can be implemented by FIR filters with the structure in Figure \ref{fig:of}
  \item The infinite dimensional convex program in \eqref{eq:main_SS} becomes a \emph{finite dimensional affinely constrained convex program} because the number of variables is finite when the FIR constraint is imposed.
\end{enumerate}
In other words, the FIR constraint is beneficial for both controller synthesis, controller implementation, and closed loop settling time -- with some tradeoffs in the transient response such as maximum overshoot. The interesting fact here is that the additional constraint in \eqref{eq:main_SS} sometimes make the problem easier to solve. This is also true when the convex set constraint is a sparsity constraint. %In Section \ref{sec:synthesis}, we will show that sparsity constraint allows us to synthesize and implement the controller in a localized way, while achieving 

\subsubsection{Spatio-Temporal Constraints}
Assume that $P_{22}$ is strictly proper, i.e. $D_{22} = 0$. Similar to the FIR constraint, the sparsity constraints imposed on $R, M, N, L$ in \eqref{eq:main_SS} can have added benefit on the scalability of controller implementation. As our controller is implemented by $R, M, N, L$ directly as in Figure \ref{fig:of}, a localized (sparse) closed loop response implies a localized (sparse) controller implementation -- this allows the control scheme to be applied on an arbitrary large-scale system.

The $(d,T)$-localizability constraint -- spatio-temporal constraints

%In particular, when sparsity constraint is imposed on the closed loop transfer matrices, the controller achieving the desired closed loop response can be implemented in a localized way -- 
%For simplicity of presentation, we use the chain model to illustrate the idea. The method described in this paper can generalize to arbitrary plant topology immediately as in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}.
%When sparsity constraints is imposed
%The problem of structural realizability is automatically satisfied


\subsubsection{Other Convex Constraints}
Finally, it should be noted that many other interesting problems can also be formulated by \eqref{eq:main_SS}. For instance, the convex set constraint in \eqref{eq:main_SS} can be the sublevel sets of any convex function. Therefore, the mixed $\mathcal{H}_2 / \mathcal{H}_{\infty}$ control problem can be formulated by \eqref{eq:main_SS}. 

%$T$-step controllability - distinguish between reachability and controllability
%state feedback
%Disturbance localization? H2 Hinf mixed
%\input{Nearly_local}


==> Model_v1.tex <==
Consider a discrete time linear time invariant (LTI) system with dynamics given by
\begin{eqnarray}
x[t+1] &=& A x[t] + B_2 u[t] + \delta_x [t] \nonumber\\
y[t] &=& C_2 x[t] + \delta_y [t] \label{eq:dynamics} 
\end{eqnarray}
where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are the state vector, control action, measurement, process disturbance, and sensor disturbance, respectively. We use $n_x, n_y$, and $n_u$ to denote the dimension of $x, y$, and $u$, respectively. Let the disturbances be given by $\delta_x = B_1 w$ and $\delta_y = D_{21} w$ for some matrices $B_1$ and $D_{12}$, and a disturbance vector $w$. Let $\bar{z}$ be a controlled output given by $\bar{z}[t] = C_1 x[t] + D_{12} u[t]$. The system equations in \eqref{eq:dynamics} can then be written in transfer function form as
\begin{equation}
\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & {0} & D_{12} \\ C_2 & D_{21} & {0} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
\end{equation}
where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. 

In this paper, we are particularly interested in the case that the matrices $(A,B_2,C_2)$ are large-scale but fairly sparse. This is motivated by the interconnected system model given as follows.
\begin{example}\label{ex:1}
Consider a collection of LTI subsystems that interact with each other according to an interaction graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$. Here $\mathcal{V} = \{1, \dots, n\}$ denotes the set of subsystems. We denote $x_i, u_i,$ and $y_i$ the state vector, control action, and measurement of subsystem $i$. The set $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems -- an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$.
%For each subsystem $i$ we associate a state vector $x_i$, control action $u_i$, and measurement $y_i$; and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems: an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$. 
%Denote $|\mathcal{V}|$ and $|\mathcal{E}|$ the cardinality of the set $\mathcal{V}$ and $\mathcal{E}$, respectively. 
We define the (incoming) neighbor set $\mathcal{N}_i$ of subsystem $i$ to be $\mathcal{N}_i = \{j | (i,j) \in \mathcal{E}\}$. The dynamics of subsystem $i$ is then given by
\begin{eqnarray}
x_i[t+1] &=& A_{ii} x_i[t] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[t] + B_{ii} u_i[t] + \delta_{x_i}[t] \nonumber\\
y_i[t] &=& C_{ii} x_i[t] + \delta_{y_i}[t], \label{eq:interconnected}
\end{eqnarray}
where $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ are matrices of compatible dimensions, and $\delta_{x_i}$ and $\delta_{y_i}$ are the perturbations on state and measurement, respectively. Define $x$, $u$, $y$, $\delta_x$, and $\delta_y$ the stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. We can construct the global system model \eqref{eq:dynamics} from the interconnected system model \eqref{eq:interconnected} with
\begin{equation}
A = \begin{bmatrix} A_{11} & \cdots & A_{1n} \\ \vdots & \ddots & \vdots \\ A_{n1} & \cdots & A_{nn} \end{bmatrix} \nonumber
\end{equation}
and $B_2 = \textbf{diag}(B_{11}, \dots, B_{nn})$ and $C_2 = \textbf{diag}(C_{11}, \dots, C_{nn})$. When the number of subsystems is large and the interconnected topology is sparse, the matrices $(A,B_2,C_2)$ are all large-scale but fairly sparse.
%($|\mathcal{E}| \ll |\mathcal{V}|^2$), 
\end{example}

The goal of this paper is to exploit the sparsity pattern of the system matrices $(A,B_2,C_2)$ to propose a scalable algorithm for controller synthesis. Our method can be applied on arbitrary system matrices $(A,B_2,C_2)$: the matrices $B_2$ and $C_2$ does not need to be block diagonal as in Example \ref{ex:1}. Throughout the paper, we assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable.


==> Model_v2.tex <==

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.45\textwidth]{./figure/Interconnection4.pdf}
     \caption{Interconnected Systems}
     \label{fig:interconnected}
\end{figure}

We begin by considering a chain of $n$ dynamically coupled discrete time linear time invariant (LTI) subsystems shown in Figure \ref{fig:interconnected}. Each subsystem $i$ is assumed to have a state vector $x_i$, a control action $u_i$, and a measurement $y_i$. The dynamics of subsystem $i$ is assumed to be given by
\begin{eqnarray}
x_i[t+1] &=& A_{ii} x_i[t] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[t] + B_{ii} u_i[t] + \delta_{x_i}[t] \nonumber\\
y_i[t] &=& C_{ii} x_i[t] + \delta_{y_i}[t], \label{eq:interconnected}
\end{eqnarray}
where $\mathcal{N}_i$ is the (incoming) neighbor set of subsystem $i$, $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ some matrices of compatible dimensions, and $\delta_{x_i}$ and $\delta_{y_i}$ the process disturbance and sensor disturbance, respectively. 
%A typical interconnected system is shown in Figure \ref{fig:interconnected}.
% that interact with each other according to an interaction graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$. Here $\mathcal{V} = \{1, \dots, n\}$ denotes the set of subsystems. We denote $x_i, u_i,$ and $y_i$ the state vector, control action, and measurement of subsystem $i$. The set $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems -- an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$.
%For each subsystem $i$ we associate a state vector $x_i$, control action $u_i$, and measurement $y_i$; and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these subsystems: an edge $(i,j)$ is in $\mathcal{E}$ if and only if the state $x_j$ of subsystem $j$ directly affects the state $x_i$ of subsystem $i$. 
%Denote $|\mathcal{V}|$ and $|\mathcal{E}|$ the cardinality of the set $\mathcal{V}$ and $\mathcal{E}$, respectively. 
%We define the (incoming) neighbor set $\mathcal{N}_i$ of subsystem $i$ to be $\mathcal{N}_i = \{j | (i,j) \in \mathcal{E}\}$. 
Define $x$, $u$, $y$, $\delta_x$, and $\delta_y$ the stacked vectors of the subsystem states, controls, measurements, and process and sensor disturbances, respectively. The $n$ interconnected system models \eqref{eq:interconnected} can be written into a global system model as
%We can construct the global system model from the interconnected system model \eqref{eq:interconnected} as
\begin{eqnarray}
x[t+1] &=& A x[t] + B_2 u[t] + \delta_x [t] \nonumber\\
y[t] &=& C_2 x[t] + \delta_y [t] \label{eq:dynamics} 
\end{eqnarray}
where $(A,B_2,C_2)$ are appropriate augmented matrices of the system matrices in \eqref{eq:interconnected}.  
%with
%\begin{equation}
%A = \begin{bmatrix} A_{11} & \cdots & A_{1n} \\ \vdots & \ddots & \vdots \\ A_{n1} & \cdots & A_{nn} \end{bmatrix}, \nonumber
%\end{equation}
%$B_2 = \textbf{diag}(B_{11}, \dots, B_{nn})$, and $C_2 = \textbf{diag}(C_{11}, \dots, C_{nn})$. 
We use $n_x, n_y$, and $n_u$ to denote the dimension of $x, y$, and $u$, respectively. Let the disturbances be given by $\delta_x = B_1 w$ and $\delta_y = D_{21} w$ for some matrices $B_1$ and $D_{12}$, and a disturbance vector $w$. Let $\bar{z}$ be a controlled output given by $\bar{z}[t] = C_1 x[t] + D_{12} u[t]$. The system equations in \eqref{eq:dynamics} can then be written in transfer function form as
\begin{equation}
\tf P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & {0} & D_{12} \\ C_2 & D_{21} & {0} \end{array} \right] = \begin{bmatrix} \tf P_{11} & \tf P_{12} \\ \tf P_{21} & \tf P_{22} \end{bmatrix} \nonumber
\end{equation}
where $\tf P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. Consider a dynamic output feedback control law $\tf u = \tf K \tf y$. The traditional centralized optimal control problem of minimizing the norm of the closed loop transfer matrix from external disturbance $\tf w$ to regulated output $ \tf{\bar{z}}$ is then given by
%of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$.} of the closed loop transfer function from $w$ to $\bar{z}$ is formulated as
\begin{subequations}\label{eq:centralized}
\begin{align}
\underset{\tf K}{\text{minimize  }} \quad & ||\tf P_{11} + \tf P_{12} \tf K(I-\tf P_{22}\tf K)^{-1} \tf P_{21}\| \label{eq:cent_obj}\\
\text{subject to  } \quad & \tf K \text{ internally stabilizes } \tf P. \label{eq:cent_stable}
\end{align}
\end{subequations}

%The goal of the optimal control problem is to design a feedback strategy from measurement $y$ to control action $u$ to mitigate the effect of disturbances $\delta_x$ and $\delta_y$.
%\begin{equation}
%A = \begin{bmatrix} A_{11} & \cdots & A_{1n} \\ \vdots & \ddots & \vdots \\ A_{n1} & \cdots & A_{nn} \end{bmatrix} \nonumber
%\end{equation}
%and $B_2 = \textbf{diag}(B_{11}, \dots, B_{nn})$ and $C_2 = \textbf{diag}(C_{11}, \dots, C_{nn})$. When the number of subsystems is large and the interconnected topology is sparse, the matrices $(A,B_2,C_2)$ are all large-scale but fairly sparse.
%Consider a discrete time linear time invariant (LTI) system with dynamics given by
%where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are the state vector, control action, measurement, process disturbance, and sensor disturbance, respectively. 
%In this paper, we are particularly interested in the case that the matrices $(A,B_2,C_2)$ are large-scale but fairly sparse. This is motivated by the interconnected system model given as follows.

%It is readily seem that the
%In this paper, we consider three different challenges of controller design for large-scale interconnected systems:
The centralized optimal control framework \eqref{eq:centralized} does not work well on large-scale interconnected systems due to three distinctive reasons:
\begin{enumerate}[(a)]
\item Communication delays: Problem \eqref{eq:centralized} does not incorporate communication delay constraints between sub-controllers shown in Figure \ref{fig:interconnected}.
%The communication between sub-controllers shown in Figure \ref{fig:interconnected} are subject to some communication delays. We must incorporate this practical communication delays constraint into the optimal control problem \eqref{eq:centralized}, so the controller being designed is practically implementable. 
\item Scalability of controller implementation: The controller $\tf K$ in \eqref{eq:centralized} is typically dense without specific sparsity structure. This means that each measurement $y_i$ needs to be shared among all the sub-controllers in the network, which does not scale gracefully to large systems.
\item Scalability of controller synthesis: Problem \eqref{eq:centralized} is a large-scale optimization problem, which cannot be solved in a scalable and distributed way.
\end{enumerate}
The goal of this paper is to address these three challenges of controller design for large-scale interconnected systems.
%e following subsections, we will show that the distributed optimal control framework can address the issue of communication delays, but has a 

\begin{remark}
The method described in this paper can be applied to system matrices $(A,B_2,C_2)$ with any sparsity pattern. In particular, we do not require $B_2$ and $C_2$ to be block diagonal.
\end{remark}
%The goal of this paper is to exploit the sparsity pattern of the system matrices $(A,B_2,C_2)$ to propose a scalable algorithm for controller synthesis. Our method can be applied on arbitrary system matrices $(A,B_2,C_2)$: the matrices $B_2$ and $C_2$ does not need to be block diagonal as in Example \ref{ex:1}. Throughout the paper, we assume that the realization $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable.


==> Nearly_local.tex <==
\subsection{Nearly Localizable Systems}
In the above, the basic assumption is that the constraints in \eqref{eq:main_SS} are satisfied \emph{exactly}. In practice, a system $(A, B_2, C_2)$ may be only \emph{nearly} $\mathcal{S}$-localizable. One interesting question is: if the closed loop response $R, M, N, L$ can be only approximately $\mathcal{S}$-localizable, can we still implement a stabilizing controller in a localized way using Figure \ref{fig:sf} or \ref{fig:of}? In this subsection, we will give a simple sufficient condition on output feedback stabilizability for nearly localizable systems. The plant model $P_{22}$ is assumed to be strictly proper in this subsection.

\subsubsection{State Feedback}
We consider state feedback first as it gives a simple necessary and sufficient condition on global stabilizability when \eqref{eq:main_SS} cannot be solved exactly. This happens when there is computation error, model uncertainty, discretization error, or simply because the system is not localizable. All these sources of error can be analyzed simultaneously by defining a perturbation transfer matrix $\Delta_{RM} \in \RHinf$ satisfying
\begin{subequations}
\begin{align}
& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I+\Delta_{RM} \label{eq:near_sf1}\\
& \begin{bmatrix} R \\ M \end{bmatrix} \in \mathcal{S} \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:near_sf2}
\end{align}
\end{subequations}
Here, $(A,B_2)$ in \eqref{eq:near_sf1} represents the \emph{actual} system model, and $(R,M)$ in \eqref{eq:near_sf1} - \eqref{eq:near_sf2} represents the \emph{actual} controller implementation. More specifically, the controller is implemented by the structure given in Figure \ref{fig:sf} with a pair of stable $\mathcal{S}$-localizable transfer matrices $(R,M)$ in \eqref{eq:near_sf1} - \eqref{eq:near_sf2}. The solution $(R,M)$, however, is \emph{not} the actual closed loop response since $\Delta_{RM}$ is not zero. The error may come from various sources. For example, the controller $(R,M)$ may be designed from a biased plant model $(A^{(b)}, B_2^{(b)})$, or we truncate the solution $(R,M)$ to force it satisfying the convex set constraint. The perturbation transfer matrix $\Delta_{RM}$ characterizes all the mismatch between actual system and actual controller implementation. The following theorem gives a necessary and sufficient condition for internal stability in the presence of $\Delta_{RM}$.
\begin{theorem}
The state feedback controller with structure given by Figure \ref{fig:sf} internally stabilizes the plant if and only if $(I + \Delta_{RM})^{-1}$ is stable.
\end{theorem}
\begin{proof}
This can be done by calculating the actual closed loop transfer matrices from $(\delta_x, \delta_y, \delta_u)$ to $(x, u, w_e)$ as in Theorem \ref{thm:sf}, with \eqref{eq:state_fb1} replaced by \eqref{eq:near_sf1}. The nine closed loop transfer matrices are summarized in Table \ref{Table:2}, where $I_\Delta = (I+\Delta_{RM})^{-1}$. Clearly, if $I_\Delta$ is stable, then all the transfer functions in Table \ref{Table:2} will be stable. If $I_\Delta$ is unstable, then the closed loop maps from $\delta_x$ to $w_e$ will be unstable, and the structure in Figure \ref{fig:sf} lose internal stability. Therefore, the stability of $(I + \Delta_{RM})^{-1}$ is necessary and sufficient for the internal stability of Figure \ref{fig:sf}.
\end{proof}

\begin{table}[h!]
 \caption{Closed Loop Maps With Non-localizability}
 \label{Table:2}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c | c | c |}
    \hline 
    & $\delta_x$ & $\delta_y$ & $\delta_u$ \\ \hline
    $x$ & $R I_\Delta$ & $(I - \tilde{R}) I_\Delta (I - \frac{1}{z} A) - I$ & $R I_\Delta B_2$ \\ \hline
    $u$ & $M I_\Delta$ & $\tilde{M} I_\Delta (I - \frac{1}{z} A)$ & $I + M I_\Delta B_2$ \\ \hline
    $w_e$ & $\frac{1}{z} I_\Delta$ & $I_\Delta (I - \frac{1}{z} A)$ & $\frac{1}{z} I_\Delta B_2$ \\ \hline
    \end{tabular}
\end{center}
\end{table}

Note that in the present of $\Delta_{RM}$, the closed loop response is no longer exactly localizable. However, when $\Delta_{RM}$ is small enough, $I_\Delta = (I+\Delta_{RM})^{-1}$ will be stable, and the structure in Figure \ref{fig:sf} achieves global stability. The robustness of the controller structure allows us to use approximated solution to implement the localized controller when the constraint \eqref{eq:main_SS} is not exactly satisfied.
%for nearly localizable systems.

\subsubsection{Output Feedback}
The analysis for output feedback nearly localizable system follows the similar fashion, but is substantially more complicated. Assume that $(A, B_2, C_2)$ is the actual plant model and controller is implemented by Figure \ref{fig:of} with four stable $\mathcal{S}$-localizable transfer matrices $(R, M, N, L)$. The non-localizability can be characterized by perturbation matrices $(\Delta_{RM}, \Delta_{RN}, \Delta_{M}, \Delta_{N})$ as
\begin{eqnarray}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} R & N \\ M & L \end{bmatrix} &=& 
\begin{bmatrix} I + \Delta_{RM} & \Delta_{N} \end{bmatrix} \label{eq:matrix_3} \\
\begin{bmatrix} R & N \\ M & L \end{bmatrix}
 \begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} &=& 
\begin{bmatrix} I + \Delta_{RN} \\ \Delta_{M} \end{bmatrix} \label{eq:matrix_4} \\
R, M, N \in \frac{1}{z} \RHinf && L \in \RHinf \nonumber\\
\begin{bmatrix} R & N \\ M & L \end{bmatrix} &\in& \mathcal{S}. \nonumber
\end{eqnarray}
Note that the perturbation matrices are always stable since $(R, M, N, L)$ are stable, and $\Delta_{RM}$ and $\Delta_{RN}$ are strictly proper due to the implementation in Figure \ref{fig:of}. The perturbation matrices satisfy a relation
\begin{equation}
\Delta_{N} C_2 - \Delta_{RM} (zI-A) = B_2 \Delta_{M} - (zI-A) \Delta_{RN}, \nonumber
\end{equation}
which can be directly verified by combining \eqref{eq:matrix_3} and \eqref{eq:matrix_4}. 
%We will derive a sufficient condition for those errors such that the localized implementation \eqref{eq:rhc} stabilized the original plant.
Define
\begin{eqnarray}
G_{\Delta} &=& \Delta_{N} C_2 - \Delta_{RM} (zI-A) \nonumber\\
G_1 &=& (I+\Delta_{RN})^{-1} \nonumber\\
G_2 &=& (I+\Delta_{RM})^{-1} \nonumber\\
G_3 &=& (I+R G_2 G_{\Delta} G_1)^{-1} \nonumber\\
G_4 &=& (I+G_2 G_{\Delta} G_1 R)^{-1}. \label{eq:G_delta}
\end{eqnarray}
Using the matrix identity from \cite{Matrix}
\begin{equation}
(I + A B)^{-1} = I - A (I + B A)^{-1}B, \nonumber
\end{equation}
we have
\begin{equation}
G_4 = I - G_2 G_\Delta G_1 G_3 R. \nonumber
\end{equation}
Therefore, if $G_1, G_2, G_3$ are stable, then $G_4$ must be stable. Similarly, if $G_1, G_2, G_4$ are stable, then $G_3$ will be stable. The following theorem gives a sufficient condition on internal stability of Figure \ref{fig:of}.

\begin{theorem}
If $G_1, G_2, G_3$ in \eqref{eq:G_delta} are stable, then the implementation in Figure \ref{fig:of} is internally stable. Figure \ref{fig:of} is internally stable if and only if all the closed loop transfer matrices in Table \ref{Table:3} and \ref{Table:4} are stable. \label{thm:5}
\end{theorem}
\begin{proof}
This can be done by calculating the closed loop transfer matrices from $(\delta_x, \delta_y, \delta_u, \delta_\beta)$ to $(x, u, y, \beta)$ as in Theorem \ref{fig:of}, with \eqref{eq:output_fb1} - \eqref{eq:output_fb2} replaced by \eqref{eq:matrix_3} - \eqref{eq:matrix_4}. The calculation, however, is not as straightforward as the state feedback case. Therefore, we will show how to derive the closed loop map from $\delta_x$ to $x$ as an example. 

From Figure \ref{fig:of}, we have
\begin{equation}
\beta = - \frac{1}{z} R^{-1} N y + \frac{1}{z^2} R^{-1} \delta_\beta. \nonumber
\end{equation}
Therefore,
\begin{eqnarray}
u &=& L y + z M \beta + \delta_u \nonumber \\
&=& (L - M R^{-1} N) y + \frac{1}{z} M R^{-1} \delta_\beta + \delta_u. \nonumber
\end{eqnarray}
Define $\widehat{K} = L - M R^{-1} N$ and calculate the dynamics of $x$ in Figure \ref{fig:of}, we have
\begin{equation}
(zI - A - B_2 \widehat{K} C_2) x = \delta_x + B_2 \widehat{K} \delta_y + B_2 \delta_u + \frac{1}{z} B_2 M R^{-1} \delta_\beta. \nonumber
\end{equation}
As $\widehat{K}$ is proper, $(zI - A - B_2 \widehat{K} C_2)$ is invertible. We define $\widehat{R} = (zI - A - B_2 \widehat{K} C_2)^{-1}$, which is the actual transfer function from $\delta_x$ to $x$. We will show that $\widehat{R}$ is stable when $G_1, G_2, G_3$ are stable.

We start from the equation
\begin{eqnarray}
&&(zI - A - B_2 \widehat{K} C_2) \nonumber\\
&=& (zI - A - B_2 Q C_2 + B_2 M R^{-1} N C_2). \nonumber
\end{eqnarray}
Substituting $B_2 Q C_2$, $B_2 M$, and $N C_2$ from \eqref{eq:matrix_3} and \eqref{eq:matrix_4}, this equation will eventually lead to
\begin{eqnarray}
&&(zI - A - B_2 \widehat{K} C_2) \nonumber\\
&=& (I+\Delta_{RM}) R^{-1} (I+\Delta_{RN}) + G_\Delta \nonumber\\
&=& G_2^{-1} (R^{-1} + G_2 G_{\Delta} G_1) G_1^{-1}. \nonumber
\end{eqnarray}
Therefore,
\begin{eqnarray}
\widehat{R} &=& (zI - A - B_2 \widehat{K} C_2)^{-1} \nonumber\\
&=& G_1 (R^{-1} + G_2 G_{\Delta} G_1)^{-1} G_2 \nonumber\\
&=& G_1 [R^{-1} (I + R G_2 G_{\Delta} G_1)]^{-1} G_2 \nonumber\\
&=& G_1 G_3 R G_2 \nonumber\\
&=& G_1 R G_4 G_2.
\end{eqnarray}
If $G_1, G_2, G_3$ are stable, then $\widehat{R}$ is stable.

Table \ref{Table:3} and \ref{Table:4} summarize all closed loop transfer matrices. Similar to Theorem \ref{thm:of}, a necessary and sufficient condition for the stability of Figure \ref{fig:of} is that all the closed loop transfer matrices in Table \ref{Table:3} and \ref{Table:4} being stable. Clearly, if $G_1, G_2, G_3$ are stable, then all the transfer matrices in Table \ref{Table:3} and \ref{Table:4} are stable. Therefore, the stability of $G_1, G_2, G_3$ is a sufficient condition for the stability of Figure \ref{fig:of}.
\end{proof}

%\begin{table*}[t]
% \caption{Closed Loop Maps With Non-localizability}
% \label{Table:3}
%\begin{center}
%\begin{subtable}
%\centering
%\renewcommand{\arraystretch}{2}
%    \begin{tabular}{| c | c | c | c | c | c |}
%    \hline 
%    & $\delta_x$ & $\delta_y$ & $\delta_u$ & $\delta_\beta$ \\ \hline
%    $x$ & $\widehat{R} = G_1 G_3 R G_2$ & $\widehat{N} = G_1 G_3 N - \widehat{R} \Delta_N$ & $\widehat{R} B_2$ & $T_{x\beta}$ \\ \hline
%    $u$ & $\widehat{M} = M G_4 G_2 - \Delta_M \widehat{R}$ & $L - \widehat{M} \Delta_N - \Delta_M \widehat{N} - \Delta_M \widehat{R} \Delta_N - M G_2 G_\Delta G_1 G_3 N$ & $I + \widehat{M} B_2$ & $T_{u\beta}$ \\ \hline
%    $y$ & $C_2 \widehat{R}$ & $I + C_2 \widehat{N}$ & $C_2 \widehat{R} B_2$ & $C_2 T_{x\beta}$ \\ \hline
%    $\beta$ & $T_{\beta x}$ & $T_{\beta y}$ & $T_{\beta x} B_2$ & $T_{\beta \beta}$ \\ \hline
%    \end{tabular}
%    %\caption{First part}
%    %\label{tab:sub1}
%\end{subtable} \\ \hfill
%
%\begin{subtable}
%\centering
%\renewcommand{\arraystretch}{2}
%    \begin{tabular}{| c |}
%    \\ \hline
%    $T_{x\beta} = \frac{1}{z} [\widehat{R}(zI-A) - G_1 G_3]$ \\ \hline     
%    \end{tabular}
%\end{subtable} 
%\end{center}
%\end{table*}

%\begin{table*}[t]
% \caption{Closed Loop Maps With Non-localizability}
% %\label{Table:3}
%\begin{center}
%\renewcommand{\arraystretch}{2}
%    \begin{tabular}{| c | c | c | c | c | c |}
%    \hline 
%    & $\delta_x$ & $\delta_y$ & $\delta_u$ & $\delta_\beta$ \\ \hline
%    $x$ & $\widehat{R} = G_1 G_3 R G_2$ & $\widehat{N} = G_1 G_3 N - \widehat{R} \Delta_N$ & $\widehat{R} B_2$ & $T_{x\beta} = \frac{1}{z} [\widehat{R}(zI-A) - G_1 G_3]$ \\ \hline
%    $u$ & $\widehat{M} = M G_4 G_2 - \Delta_M \widehat{R}$ & $L - \widehat{M} \Delta_N - \Delta_M \widehat{N} - \Delta_M \widehat{R} \Delta_N - M G_2 G_\Delta G_1 G_3 N$ & $I + \widehat{M} B_2$ & $\frac{1}{z} [\widehat{M}(zI-A) + M G_2 G_\Delta G_1 G_3 + \Delta_M G_1 G_3]$ \\ \hline
%    $y$ & $C_2 \widehat{R}$ & $I + C_2 \widehat{N}$ & $C_2 \widehat{R} B_2$ & $C_2 T_{x\beta}$ \\ \hline
%    $\beta$ & $T_{\beta x} = -\frac{1}{z} [(zI-A) \widehat{R} - G_4 G_2]$ & $-\frac{1}{z} [(zI-A) \widehat{N} + G_2 G_\Delta G_1 G_3 N + G_4 G_2 \Delta_N]$ & $T_{\beta x} B_2$ & $\frac{1}{z^2}[(zI-A) G_1 G_3 + G_4 G_2 (zI-A) + G_2 G_\Delta G_1 G_3 - (zI-A) \widehat{R} (zI-A)]$ \\ \hline
%    \end{tabular}
%\end{center}
%\end{table*}

\begin{table*}[t]
 \caption{Closed Loop Maps With Non-localizability - Part I}
 \label{Table:3}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c | c | c |}
    \hline 
    & $\delta_x$ & $\delta_y$ & $\delta_u$ \\ \hline
    $x$ & $\widehat{R} = G_1 G_3 R G_2$ & $\widehat{N} = G_1 G_3 N - \widehat{R} \Delta_N$ & $\widehat{R} B_2$ \\ \hline
    $u$ & $\widehat{M} = M G_4 G_2 - \Delta_M \widehat{R}$ & $L - \widehat{M} \Delta_N - \Delta_M \widehat{N} - \Delta_M \widehat{R} \Delta_N - M G_2 G_\Delta G_1 G_3 N$ & $I + \widehat{M} B_2$ \\ \hline
    $y$ & $C_2 \widehat{R}$ & $I + C_2 \widehat{N}$ & $C_2 \widehat{R} B_2$ \\ \hline
    $\beta$ & $-\frac{1}{z} [(zI-A) \widehat{R} - G_4 G_2]$ & $-\frac{1}{z} [(zI-A) \widehat{N} + G_2 G_\Delta G_1 G_3 N + G_4 G_2 \Delta_N]$ & $-\frac{1}{z} [(zI-A) \widehat{R} - G_4 G_2] B_2$ \\ \hline
    \end{tabular}
\end{center}
\end{table*}

\begin{table*}[t]
 \caption{Closed Loop Maps With Non-localizability - Part II}
 \label{Table:4}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c |}
    \hline 
    & $\delta_\beta$ \\ \hline
    $x$ & $\frac{1}{z} [\widehat{R}(zI-A) - G_1 G_3]$ \\ \hline
    $u$ & $\frac{1}{z} [\widehat{M}(zI-A) + M G_2 G_\Delta G_1 G_3 + \Delta_M G_1 G_3]$ \\ \hline
    $y$ & $\frac{1}{z} C_2 [\widehat{R}(zI-A) - G_1 G_3]$ \\ \hline
    $\beta$ & $\frac{1}{z^2}[(zI-A) G_1 G_3 + G_4 G_2 (zI-A) + G_2 G_\Delta G_1 G_3 - (zI-A) \widehat{R} (zI-A)]$ \\ \hline
    \end{tabular}
\end{center}
\end{table*}

%\begin{table*}[t]
% \caption{Closed Loop Maps With Non-localizability}
% \label{Table:4}
%\begin{center}
%\renewcommand{\arraystretch}{2}
%    \begin{tabular}{| c | c | c | c | c | c |}
%    \hline 
%    & $\delta_x$ & $\delta_y$ & $\delta_u$ & $\delta_\beta$ \\ \hline
%    $x$ & $\widehat{R} = G_1 G_3 R G_2$ & $\widehat{N} = G_1 G_3 N - \widehat{R} \Delta_N$ & $\widehat{R} B_2$ & $T_{x\beta} = \frac{1}{z} [\widehat{R}(zI-A) - G_1 G_3]$ \\ \hline
%    $u$ & $\widehat{M} = M G_4 G_2 - \Delta_M \widehat{R}$ & $L - \widehat{M} \Delta_N - \Delta_M \widehat{N} - \Delta_M \widehat{R} \Delta_N - M G_{\Delta 2} N$ & $I + \widehat{M} B_2$ & $\frac{1}{z} [\widehat{M}(zI-A) + M G_{\Delta 2} + \Delta_M G_1 G_3]$ \\ \hline
%    $y$ & $C_2 \widehat{R}$ & $I + C_2 \widehat{N}$ & $C_2 \widehat{R} B_2$ & $C_2 T_{x\beta}$ \\ \hline
%    $\beta$ & $T_{\beta x} = -\frac{1}{z} [(zI-A) \widehat{R} - G_4 G_2]$ & $-\frac{1}{z} [(zI-A) \widehat{N} + G_{\Delta 2} N + G_4 G_2 \Delta_N]$ & $T_{\beta x} B_2$ & $\frac{1}{z^2}[(zI-A) G_1 G_3 + G_4 G_2 (zI-A) + G_{\Delta 2} - (zI-A) \widehat{R} (zI-A)]$ \\ \hline
%    \end{tabular}
%\end{center}
%\end{table*}

%\begin{widetext}
%\begin{equation}
%\widehat{R} = 
%\end{equation}
%\end{widetext}

%For Theorem \ref{thm:5}, a necessary and sufficient condition for the stability of Figure \ref{fig:of} is that all the closed loop transfer matrices in Table \ref{Table:3} and \ref{Table:4} being stable. 

Theorem \ref{thm:5} can be simplified for some particular source of error. For instance, assume that the actual plant model is given by $(A+\delta_A, B_2, C_2)$, and $\delta_A$ is the only source of error. We have $\Delta_{RM} = -\delta_{A}R$, $\Delta_{N} = -\delta_{A}N$, $\Delta_{RN} = -R \delta_{A}$, $\Delta_M = -M \delta_A$, and
\begin{eqnarray}
G_\Delta &=& \Delta_N C_2 - \Delta_{RM} (zI - A - \delta_A) \nonumber\\
&=& \delta_A (I-R \delta_A) \nonumber \\
G_3 &=& I - R \delta_A. \nonumber
\end{eqnarray}
We can show that if $(I-R \delta_A)^{-1}$ is stable, then the system is internally stable. For instance, some closed loop transfer matrices are given by
\begin{eqnarray}
\widehat{R} &=& (I - R \delta_A)^{-1} R \nonumber\\
\widehat{N} &=&  (I - R \delta_A)^{-1} N \nonumber\\
\widehat{M} &=&  M(I + \delta_A (I - R \delta_A)^{-1} R) \nonumber\\
\widehat{L} &=& L + M \delta_A (I - R \delta_A)^{-1} N. \nonumber
\end{eqnarray}
If $\delta_A$ is in the set $||\delta_A||_{\mathcal{H}_\infty} \leq \gamma$, then we know that a sufficient condition for internal stability is $||R||_{\mathcal{H}_\infty} < 1 / \gamma$. Similarly, if the actual plant model is given by $(A, B_2+\delta_B, C_2)$ and $\delta_B$ is the only source of error. A sufficient condition for internal stability for all $||\delta_B||_{\mathcal{H}_\infty} \leq \gamma$ is given by $||M||_{\mathcal{H}_\infty} < 1 / \gamma$.

%Therefore, if the implementation \eqref{eq:rhc} can stabilizing the plant $A+\delta_A$ if $(I - R \delta_A)^{-1}$ is stable. 
%
%Formulation of gain margin maximization problem based on $|| B_2 M ||_{\mathcal{H}_{\infty}}$



==> Output_v1.tex <==
%In the previous section, we discussed the direct decomposability of the optimization problem \eqref{eq:localized} when either $B_2$ or $C_2$ are invertible. The original problem can then be simplified significantly into \eqref{eq:sf_lop}. 
In this section, we discuss how to solve the general output feedback problem \eqref{eq:LOC} in a scalable way with arbitrary $B_2$ and $C_2$. In this case, the problem is not directly decomposable due to the coupling constraints \eqref{eq:main_1} and \eqref{eq:main_2}. We introduce the notion of decomposability with respect to distributed optimization for the objective function and the localizability constraint in \eqref{eq:LOC}, which is a substantial generalization of direct decomposability described in the previous section. When both the objective function and the localizability constraint are decomposable and convex, we can use the ADMM algorithm to decompose the problem \eqref{eq:LOC} into two subroutines. Each subroutine can be solved in a localized and scalable way using the direct decomposition method described in the previous section. We show that many class of problems satisfy this general decomposability condition. Examples include the $\mathcal{H}_2$ optimal control problem with sensor and actuator regularization and the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem.

%solve the output feedback problem \eqref{eq:localized} in a localized and scalable way. We give several classes of 
%In this section, we discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%State feedback is discussed first due to
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Decomposability with respect to Distributed Optimization}
We begin by simplifying the notation of \eqref{eq:LOC}. We use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. Denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$ and $\tf Z_{AC}$ the transfer matrix $\begin{bmatrix} zI-A^\top & -C_2^\top \end{bmatrix}^\top$. Let $J_B$ be the matrix in the right-hand-side of \eqref{eq:main_1} and $J_C$ be the matrix in the right-hand-side of \eqref{eq:main_2}. The original optimization problem \eqref{eq:LOC} can be written as
\begin{subequations} \label{eq:of_lop}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:of-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = J_B \label{eq:of-2} \\
& \ttf{\Phi} \tf Z_{AC} = J_C \label{eq:of-3} \\
& \ttf{\Phi} \in \s. \label{eq:of-4}
\end{align}
\end{subequations}
Here the stability constraint \eqref{eq:main_stable} is included in the set constraint $\s$ in \eqref{eq:of-4}. 

The primary difference between the output feedback problem \eqref{eq:of_lop} and the state feedback problem \eqref{eq:sf_lop2} is the additional constraint \eqref{eq:of-3}. The column-wise decomposition technique does not apply to the output feedback problem \eqref{eq:of_lop} directly because the constraint \eqref{eq:of-3} does not admit a column-wise decomposition. However, we note that the optimization variable $\ttf{\Phi}$ in constraint \eqref{eq:of-3} can be solved row at a time. Our strategy is to use distributed optimization techniques such as ADMM to decouple problem \eqref{eq:of_lop} into a row-wise decomposable component and a column-wise decomposable component. If the objective function \eqref{eq:of-1} and the localizability constraint \eqref{eq:of-4} can be split into a row-wise decomposable component and a column-wise decomposable component, we can then solve the localized output feedback optimal control problem \eqref{eq:of_lop} in a localized yet iterative way. 
%It is then natural to use distributed optimization techniques such as ADMM to decouple the constraints \eqref{eq:of-2} and \eqref{eq:of-3}, and solve 

From the definition of the closed loop transfer matrices \eqref{eq:desired}, the number of rows and columns of $\ttf{\Phi}$ in \eqref{eq:of_lop} are given by $(n_x + n_u)$ and $(n_x+n_y)$, respectively. Let $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ be a partition of the set $\{1, \dots, n_x+n_u\}$, and $\{ \Set q_1, \dots, \Set q_{\hat{m}} \}$ be a partition of the set $\{1, \dots, n_x+n_y\}$. The decomposability of the objective function \eqref{eq:of-1} is defined as follows.
%The optimization variable $\ttf{\Phi}$ can be partitioned column-wisely into the set $\{ \Sub{\ttf{\Phi}}{ : }{\Set p_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\Set p_m} \}$. 
%Define decomposability for the objective and the localizability constraint
%Let $\{\Phi_j\}_{j=1}^n$ be a column-wise partition of $\Phi$, and $\{(\Phi^\top)_j\}_{j=1}^{n'}$ be a row-wise partition of $\Phi$ (a column-wise partition of $\Phi^\top$).
%Let $\{p_j\}_{j=1}^n$ be a column-wise partition for $CL$ (a partition on the perturbation $[\delta{x}; \delta{y}]$), and $\{p'_j\}_{j=1}^{n'}$ a row-wise partition for $CL$ (a partition on the internal variable $[x; u]$). 
%The decomposability for the objective function and the localizability constraint are defined as follows.
\begin{definition} \label{dfn:do}
The convex objective function $g(\ttf{\Phi})$ in \eqref{eq:of_lop} is said to be \emph{decomposable} with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\hat{m}}\}$ if $g(\ttf{\Phi})$ can be written as the sum of two convex functions $\tilde{g}(\ttf{\Phi})$ and $\hat{g}(\ttf{\Phi})$, where $\tilde{g}(\ttf{\Phi})$ is directly decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ and $\hat{g}(\ttf{\Phi})$ is directly decomposable with respect to the column-wise partition $\{ \Set q_1, \dots, \Set q_{\hat{m}} \}$. Specifically, we have 
\begin{eqnarray}
g(\ttf{\Phi}) &=& \tilde{g}(\ttf{\Phi}) + \hat{g}(\ttf{\Phi}) \nonumber\\
\tilde{g}(\ttf{\Phi}) &=& \sum_{j=1}^{\tilde{m}} \tilde{g}_j(\Sub{\ttf{\Phi}}{\Set p_j}{:}) \nonumber\\
\hat{g}(\ttf{\Phi}) &=& \sum_{j=1}^{\hat{m}} \hat{g}_j(\Sub{\ttf{\Phi}}{:}{\Set q_j}) \label{eq:obj_decom2}
\end{eqnarray}
for some convex functions $\tilde{g}_j(\cdot)$ for $j = 1, \dots, \tilde{m}$, and $\hat{g}_j(\cdot)$ for $j = 1, \dots, \hat{m}$.  
\end{definition}

In the rest of this paper, when we say an objective function is \emph{decomposable}, we mean that the objective function satisfy the conditions in \eqref{eq:obj_decom2} for some row-wise and column-wise partition. The directly decomposable objective function defined in Definition \ref{dfn:dd} is a special class of decomposable objective function with $\tilde{g}(\cdot) = 0$. The decomposability of the localizability constraint \eqref{eq:of-4} is defined as follows.
%\begin{remark}
%From the definition, every directly decomposable objective function is a decomposable objective function, but not the opposite. 
%\end{remark}
\begin{definition} \label{dfn:ss}
The convex set constraint $\s$ in \eqref{eq:of_lop} is said to be \emph{decomposable} with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\hat{m}}\}$ if $\s$ can be written as the intersection of two convex sets $\tilde{\s}$ and $\hat{\s}$, where $\tilde{\s}$ is directly decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ and $\hat{\s}$ is directly decomposable with respect to the column-wise partition $\{ \Set q_1, \dots, \Set q_{\hat{m}} \}$. Specifically, we have 
\begin{eqnarray}
\s &=& \tilde{\s} \cap \hat{\s} \nonumber\\
\ttf{\Phi} \in \tilde{\s} \quad &\Longleftrightarrow& \quad \bigcap_{j=1}^{\tilde{m}} \Sub{\ttf{\Phi}}{\Set p_j}{:} \in \tilde{\s}_j \nonumber\\
\ttf{\Phi} \in \hat{\s} \quad &\Longleftrightarrow& \quad \bigcap_{j=1}^{\hat{m}} \Sub{\ttf{\Phi}}{:}{\Set q_j} \in \hat{\s}_j \label{eq:sdecom}
\end{eqnarray}
for some convex sets $\tilde{\s}_j$ for $j = 1, \dots, \tilde{m}$ and $\hat{\s}_j$ for $j = 1, \dots, \hat{m}$.
\end{definition}

Similarly, when we say a localizability constraint is \emph{decomposable}, we mean that the localizability constraint satisfy the conditions in Definition \ref{dfn:ss}. The directly decomposable constraint defined in Definition \ref{dfn:s} is a special class of decomposable localizability constraint which discards the constraint set $\tilde{\s}$. 

\begin{remark} \label{rmk:lt}
In this paper, the localizability constraint $\s$ in \eqref{eq:of_lop} is expressed as $\s = \Ell \cap \FT \cap \Sother$. The locality constraint $\Ell$ and the FIR constraint $\FT$ are decomposable with respect to arbitrary row-wise and column-wise partition. Therefore, the decomposability of the localizability constraint $\s$ is determined by the decomposability of the constraint $\Sother$. If $\Sother$ is decomposable, we can express the original localizability constraint $\s$ as an intersection of the sets $\tilde{\s} = \Ell \cap \FT \cap \tilde{\Sother}$ and $\hat{\s} = \Ell \cap \FT \cap \hat{\Sother}$, where $\tilde{\Sother}$ is a row-wise decomposable component of $\Sother$ and $\hat{\Sother}$ a column-wise decomposable component of $\Sother$.
Note that the locality constraint and the FIR constraint are included in both $\tilde{\s}$ and $\hat{\s}$. As will be shown later, this is the key point to allow the subroutines of the ADMM algorithm to be solved in a finite dimensional and scalable way.
\end{remark}

%\begin{remark}
%From the definition, every directly decomposable localizability constraint is a decomposable localizability constraint, but not the opposite. 
%\end{remark}

%Consider the optimization problem
%\begin{subequations}
%\begin{align}
%\underset{\{R,M,N,L\}}{\text{minimize    }} & || \begin{bmatrix} R & \sigma_y N \\ \sigma_u M & \sigma_u \sigma_y L \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:h2_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:h2_1} \\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:h2_2} \\
%&  R, M, N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad L \in \mathcal{RH}_{\infty} \label{eq:h2_stable}\\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:h2_S}
%\end{align}
%\end{subequations}
%where $\sigma_u$ is the relative penalty between state deviation and control effort, $\sigma_y$ the relative magnitude of process disturbance and sensor disturbance. This corresponds to the case for some sparse $C_1, D_{21}, B_1, D_{21}$. Theoretically, the method described in this paper can generalize to arbitrary $C_1, D_{21}, B_1, D_{21}$, but it is effective only when those matrices are highly sparse.

%Assumptions (?)
Assume that the objective function and the localizability constraint in \eqref{eq:of_lop} are both decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\tilde{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\hat{m}}\}$. We can split the optimization problem \eqref{eq:of_lop} into a row-wise decomposable part and a column-wise decomposable part. Let $\ttf{\Psi}$ be a duplicate of the optimization variable $\ttf{\Phi}$. We define extended-real-value functions $\tilde{h}(\ttf{\Phi})$ and $\hat{h}(\ttf{\Psi})$ by
\begin{eqnarray}
&& \tilde{h}(\ttf{\Phi}) = \left\{ \begin{array}{ll}
\tilde{g}(\ttf{\Phi}) & \textrm{if } \eqref{eq:of-3}, \ttf{\Phi} \in \tilde{\s}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
&& \hat{h}(\ttf{\Psi}) = \left\{ \begin{array}{ll}
\hat{g}(\ttf{\Psi}) & \textrm{if } \eqref{eq:of-2}, \ttf{\Psi} \in \hat{\s}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
\label{eq:extended}
\end{eqnarray}
Problem \eqref{eq:of_lop} can then be equivalently formulated as
\begin{eqnarray}
\underset{\{ \ttf{\Phi}, \ttf{\Psi} \}}{\text{minimize    }} && \tilde{h}(\ttf{\Phi}) + \hat{h}(\ttf{\Psi}) \nonumber\\
\text{subject to }  && \ttf{\Phi} = \ttf{\Psi}. \label{eq:sub3}
\end{eqnarray}
Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}. Specifically, the ADMM algorithm for \eqref{eq:sub3} is given by
\begin{subequations}\label{eq:admm}
\begin{align}
\ttf{\Phi}^{k+1} &= \underset{\ttf{\Phi}}{\text{argmin }} \Big( \tilde{h}(\ttf{\Phi}) + \frac{\rho}{2} || \ttf{\Phi} - \ttf{\Psi}^{k} + \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm1} \\
\ttf{\Psi}^{k+1} &= \underset{\ttf{\Psi}}{\text{argmin }} \Big( \hat{h}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm2} \\
\ttf{\Lambda}^{k+1} &= \ttf{\Lambda}^{k} + \ttf{\Phi}^{k+1} - \ttf{\Psi}^{k+1} \label{eq:admm3}
\end{align}
\end{subequations}
where the square of the $\mathcal{H}_2$ norm is computed by \eqref{eq:h2_comp}. As the FIR constraint $\FT$ is imposed on $\ttf{\Phi}$ and $\ttf{\Psi}$ through the constraint sets $\tilde{\s}$ and $\hat{\s}$, subroutines \eqref{eq:admm1} and \eqref{eq:admm2} are both finite dimensional optimization problems.
%When the FIR constraint $\FT$ is imposed through 
%of a transfer matrix can be computed by the sum of the square of Frobenius norm of all its spectral components.

%The primary reason 
%The main advantage of using the ADMM algorithm to solve \eqref{eq:sub3} is 
Subroutines \eqref{eq:admm1} and \eqref{eq:admm2} can be further decomposed row-wise and column-wise, respectively. For instance, the optimization problem corresponding to subroutine \eqref{eq:admm2} can be written as
\begin{subequations} \label{eq:admm_lop}
\begin{align} 
\underset{\ttf{\Psi}}{\text{minimize }} \quad & \hat{g}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \label{eq:admmlop1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Psi} = J_B \label{eq:admmlop2} \\
& \ttf{\Psi} \in \hat{\s}. \label{eq:admmlop3}
\end{align}
\end{subequations}
This problem has the same form as \eqref{eq:sf_lop2} -- the right-hand-side of \eqref{eq:admmlop2} does not affect the direct decomposability of the problem. The $\mathcal{H}_2$ norm regularizer in \eqref{eq:admmlop1} is directly decomposable with respect to arbitrary column-wise partition.
%, so the objective function in \eqref{eq:admmlop1} is column-wise decomposable. 
As the function $\hat{g}(\cdot)$ and the localizability constraint $\hat{\s}$ are directly decomposable with respect to a given column-wise partition, we can use the decomposition technique described in the previous section to decompose problem \eqref{eq:admm_lop} into parallel subproblems. As $\hat{\s} = \Ell \cap \FT \cap \hat{\Sother}$, we can exploit the locality constraint and use the dimension reduction technique described in the previous section to further reduce the complexity of each subproblem from global scale to local scale. Overall, subroutine \eqref{eq:admm2} can be solved in a localized and scalable manner. Similarly, subroutine \eqref{eq:admm1} can also be solved using the direct decomposition technique through a row-wise partition. Equation \eqref{eq:admm3} can be computed element-wisely since it is a matrix addition. Therefore, \eqref{eq:admm1} - \eqref{eq:admm3} is a scalable algorithm to solve the localized output feedback problem \eqref{eq:of_lop} by using the row-wise and column-wise decomposition alternatively and iteratively.

%Note that $\tilde{h}(\Phi)$ admits a block column-wise decomposition as both $\tilde{g}(\Phi)$ and the localizability constraint $\mathcal{S}$ are both column-wise decomposable. As the $\mathcal{H}_2$ norm admits a column-wise decomposition for any partition, subproblem \eqref{eq:admm1} can be solved using the state feedback decomposition technique described in the previous subsection. When the localizability constraint $\mathcal{S}$ is highly sparse, subproblem \eqref{eq:admm1} can be solved in a localized and scalable way. 
%From the decomposability assumptions on the objective function and the localizability constraint, function $\tilde{h}(\Phi)$ admits a block column-wise decomposition. 
%and function $\hat{h}(\Psi)$ admits a block row-wise decomposition. 
%From the decomposability of the
%Subproblem \eqref{eq:admm1} reduces to be form of state feedback 
%can be solved in a localized way using LLQR with a column-wise decomposition on the objective function and the constraint. 

\subsection{Examples of Decomposable Problems}
In this subsection, we introduce several classes of decomposable objective functions and decomposable localizability constraints. All these problems can be solved using the ADMM algorithm described in the previous subsection in a scalable way.
\begin{example} \label{ex:b1}
Consider the objective function of the distributed optimal control problem in \eqref{eq:trad_obj2} with either the $\mathcal{H}_2$ norm or the element-wise $\ell_1$ norm defined in Example \ref{ex:l1}. Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} B_1^\top & D_{21}^\top \end{bmatrix} \Pi$ is block diagonal. Using a similar argument as in Example \ref{ex:perm}, we can find a column-wise partition to decompose the objective function in a column-wise manner. Likewise, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the objective function in a row-wise manner. In both cases, the objective function is directly decomposable and thus decomposable.
\end{example}
%\begin{example} \label{ex:c1}
%Similarly, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the objective function in a row-wise manner. This objective function is directly decomposable and thus decomposable.
%\end{example}
\begin{example}
Consider the weighted actuator norm defined in \cite{MC_CDC14, 2015_Wang_Reg}, which is given by
\begin{equation}
|| \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} = \sum_{i=1}^{n_u} \mu_i || e_i^\top \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{H}_2} \label{eq:act_norm} 
\end{equation}
where $\mu$ is a diagonal matrix with $\mu_i$ being its $i$th diagonal entry, and $e_i$ is a unit vector with $1$ on its $i$th entry and $0$ elsewhere. When $\mu$ is an identity matrix, the actuator norm \eqref{eq:act_norm} is equivalent to the $\ell_1 / \ell_2$ norm, or the group lasso \cite{2006_grouplasso} in the statistical learning literature. This norm acts as a regularizer to make the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ row-wise sparse, i.e., have many zero rows. Recall from Theorem \ref{thm:1} that the controller achieving the desired closed loop response can be implemented by \eqref{eq:implementation}. If the $i$th row of the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ is a zero row, then the $i$th component of the control action $u_i$ is always equal to zero. This means that we can remove the control action $u_i$ without changing the closed loop response. It is clear that the actuator norm defined in \eqref{eq:act_norm} is directly decomposable to arbitrary row-wise partition. This still holds true when the actuator norm is defined by the $\ell_1 / \ell_\infty$ norm. Similarly, consider the weighted sensor norm given by
\begin{equation}
|| \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} = \sum_{i=1}^{n_y} \lambda_i || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} e_i ||_{\mathcal{H}_2} \label{eq:sen_norm} 
\end{equation}
where $\lambda$ is a diagonal matrix with $\lambda_i$ being its $i$th diagonal entry. The sensor norm in \eqref{eq:sen_norm} is a regularizer to make the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ column-wise sparse. Using the controller implementation \eqref{eq:implementation}, the sensor norm can be treated as a regularizer on the measurement $y$. For instance, if the $i$th column of the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ is identical to zero, then we can ignore the measurement $y_i$ without changing the closed loop response. The sensor norm defined in \eqref{eq:act_norm} is directly decomposable with respect to any column-wise partition.
\end{example}
\begin{example}
From Definition \ref{dfn:do}, it is straightforward to see that the sum of multiple decomposable objective functions with the same partition is still decomposable with respect to the given partition. Therefore, we can combine all the decomposable objective functions above, and the resulting objective function is still decomposable. For instance, consider the $\mathcal{H}_2$ optimal control problem with sensor and actuator regularization. The objective function is given by
\begin{eqnarray}
g(\tf R,\tf M,\tf N,\tf L) &=& ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
&&+ || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} \label{eq:h2_sar}
\end{eqnarray}
where $\mu$ and $\lambda$ are the relative penalty between the $\mathcal{H}_2$ performance and the actuator and sensor regularizer, respectively. If there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal, then the objective function \eqref{eq:h2_sar} is decomposable. In this case, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise decomposable component, and the sensor regularizer belongs to the column-wise decomposable component.
\end{example}

Next, we consider some examples of decomposable localizability constraints beside the locality constraint $\Ell$ and the FIR constraint $\FT$ described in Remark \ref{rmk:lt}.
%, some other examples of decomposable localizability constraints are given as follows.
\begin{example}
Consider the $\mathcal{L}_1$ norm \cite{Munther_L1} of a FIR transfer matrix $\tf G \in \FT$, which is given by
\begin{equation}
|| \tf G ||_{\mathcal{L}_1} = \underset{i}{\text{max}} \quad \sum_{j} \sum_{t=1}^T | g_{ij}[t] |.\label{eq:L1_defn}
\end{equation}
The $\mathcal{L}_1$ norm is an induced norm from a $\ell_\infty$ input signal to a $\ell_\infty$ output signal. Suppose that the $\ell_\infty$ norm of the disturbance $\delta_x$ and $\delta_y$ in \eqref{eq:desired} is bounded, and we want to bound the $\ell_\infty$ norm of the state vector $x$ and the control action $u$. We can impose the constraint
\begin{equation}
|| \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} ||_{\mathcal{L}_1} \leq \gamma \label{eq:L1_cons}
\end{equation}
in the optimization problem \eqref{eq:of_lop} for some $\gamma$. The solution of \eqref{eq:L1_cons} forms a convex set because it is a sublevel set of a convex function. Therefore, we can consider \eqref{eq:L1_cons} as a localizability constraint. From the definition \eqref{eq:L1_defn}, the constraint \eqref{eq:L1_cons} is decomposable with respect to arbitrary row-wise partition. If we choose the $\mathcal{H}_2$ norm as the objective function and \eqref{eq:L1_cons} as the constraint, then the problem becomes a mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem. As both the objective and the constraint are decomposable, the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem is decomposable. %it is a directly decomposable constraint and thus a decomposable constraint. 
\end{example}
\begin{example}
From Definition \ref{dfn:ss}, the intersection of multiple decomposable constraints with the same partition is decomposable with respect to the given partition. Therefore, we can combine all the decomposable constraints described above, and the resulting localizability constraint is still decomposable. This property is extremely useful because all the decomposable constraints can be incorporated into the optimization problem in a sequential manner without breaking the decomposability of the problem. For instance, the combination of the locality constraint $\Ell$, the FIR constraint $\FT$, and the $\mathcal{L}_1$ constraint in \eqref{eq:L1_cons} is decomposable.
\end{example}
%The ADMM algorithm described in the previous subsection can be applied to any problem with a decomposable objective function and a decomposable localizability constraint.
%Here we consider a localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization. We explain how to solve this problem in a localized and scalable manner using the ADMM algorithm.
%\begin{example}
%A localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization is formulated by
%\begin{subequations} \label{eq:h2l1}
%\begin{align} 
%\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + \mu || \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + \lambda || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} \label{eq:h2l1-1}\\
%\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \label{eq:h2l1-3} \\
%& || \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} ||_{\mathcal{L}_1} \leq \gamma \label{eq:h2l1-4}.
%\end{align}
%\end{subequations}
%Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. In this case, problem \eqref{eq:h2l1} is decomposable. Specifically, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise decomposable component of the objective function, while the sensor regularizer belongs to the column-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2} and the $\mathcal{L}_1$ constraint \eqref{eq:h2l1-4}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
%\end{example}

%Without the constraint \eqref{eq:h2_2}, this optimization problem admits a column-wise decomposition as the LLQR problem. Similarly, without the constraint \eqref{eq:h2_1}, the optimization problem admits a row-wise decomposition. Specifically, we solve
%\begin{eqnarray}
%\begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_1}, \eqref{eq:h2_stable}, \eqref{eq:h2_S} \label{eq:sub1}
%\end{eqnarray}
%and
%\begin{eqnarray}
%\begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_2}, \eqref{eq:h2_stable}, \eqref{eq:h2_S}. \label{eq:sub2}
%\end{eqnarray}
%When the constraint \eqref{eq:h2_S} is a locality constraint, we can utilize the technique of LLQR to solve both \eqref{eq:sub1} and \eqref{eq:sub2} in a completely localized and parallel way.
%
%The optimal solution in \eqref{eq:sub1} and \eqref{eq:sub2} may not be the same. Therefore, we need to solve an extra optimization problem as
%\begin{eqnarray}
%\underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix}. \label{eq:sub3}
%\end{eqnarray}
%Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}.

\subsection{Convergence and Stopping Criteria}
In this subsection, we identify the technical conditions on problem \eqref{eq:of_lop} (or equivalently, \eqref{eq:sub3}) such that the ADMM algorithm \eqref{eq:admm1} - \eqref{eq:admm3} converges to an optimal solution. We make the following assumptions. 
\begin{assumption}
Problem \eqref{eq:of_lop} has a feasible solution in the relative interior of the set $\s$. \label{as:1}
\end{assumption}
\begin{assumption} 
The functions $\tilde{g}(\cdot)$ and $\hat{g}(\cdot)$ are closed, proper, and convex. \label{as:2}
\end{assumption}
\begin{assumption} 
The sets $\tilde{\s}$ and $\hat{\s}$ are closed and convex. \label{as:3}
\end{assumption}

Assumption \ref{as:1} implies feasibility and strong duality of \eqref{eq:of_lop} (or its equivalent formulation \eqref{eq:sub3}). Combining with Assumptions \ref{as:2} and \ref{as:3}, we know that the extended-real-value functions $\tilde{h}(\cdot)$ and $\hat{h}(\cdot)$ defined in \eqref{eq:extended} are closed, proper, and convex. Under these assumptions, problem \eqref{eq:sub3} satisfies the convergence conditions in \cite{BoydADMM}. From \cite{BoydADMM}, we have objective convergence, dual variable convergence ($\ttf{\Lambda}^{k} \to \ttf{\Lambda}^{*}$ as $k \to \infty$), and residual convergence ($\ttf{\Phi}^k - \ttf{\Psi}^k \to 0$ as $k \to \infty$). As long as the problem \eqref{eq:sub3} approaches feasibility and the optimal value of \eqref{eq:sub3} converges to the global optimal, we can use a feasible solution of \eqref{eq:sub3} to construct a controller that achieves the desired optimal closed loop response. Note that the optimization problem \eqref{eq:sub3} may not have a unique optimal point, so the optimization variable $\ttf{\Phi}^k$ and $\ttf{\Psi}^k$ does not necessary converge. If we further assume that the objective function $g(\cdot)$ is strongly convex with respect to $\ttf{\Phi}$, then problem \eqref{eq:sub3} has a unique optimal solution $\ttf{\Phi}^*$. In this case, objective convergence implies primal variable convergence, so we have $\ttf{\Phi}^k \to \ttf{\Phi}^*$ and $\ttf{\Psi}^k \to \ttf{\Phi}^*$ as $k \to \infty$.

The stopping criteria is designed from \cite{BoydADMM}, in which we use $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2}$ as primal infeasibility and $|| \ttf{\Psi}^k - \ttf{\Psi}^{k-1} ||_{\mathcal{H}_2}$ as dual infeasibility. The square of these two functions can be calculated in a localized and distributed way. The algorithm \eqref{eq:admm1} - \eqref{eq:admm3} terminates when $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2} < \epsilon^{pri}$ and $|| \ttf{\Psi}^k - \ttf{\Psi}^{k-1} ||_{\mathcal{H}_2} < \epsilon^{dual}$ for some feasibility tolerances $\epsilon^{pri}$ and $\epsilon^{dual}$.
%the primal and dual infeasibility are smaller than the feasibility tolerances $\epsilon^{pri}$ and $\epsilon^{dual}$, respectively.

In practice, we may not know the feasibility of \eqref{eq:of_lop} in advanced. In other words, we do not know whether Assumption \ref{as:1} holds. Consider the case that the ADMM subroutines \eqref{eq:admm1} - \eqref{eq:admm3} are solvable, but problem \eqref{eq:sub3} is infeasible. In this situation, the stopping criteria on primal infeasibility $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2} < \epsilon^{pri}$ may not be satisfied. To avoid infinite number of iterations, we can set a limit on the number of iterations in the ADMM algorithm. The convergence result of the ADMM algorithm should be regarded as a scalable algorithm to check the $\s$-localizability of the system matrices $(A,B_2,C_2)$ in \eqref{eq:of_lop}. If the ADMM algorithm does not converge, then we know that the system $(A,B_2,C_2)$ is not $\s$-localizable. Interested readers can refer to \cite{2015_Wang_Reg} on the design of the localizability constraint $\s$ to ensure the feasibility of \eqref{eq:of_lop} for some specific systems.

\subsection{Analytic Solution and Acceleration}
Suppose that Assumptions \ref{as:1} - \ref{as:3} hold. The ADMM algorithm presented in \eqref{eq:admm1} - \eqref{eq:admm3} is a special case of the proximal algorithm \cite{proximal, proximalBoyd, BoydADMM}. For certain type of objective functions $\tilde{h}(\cdot)$ and $\hat{h}(\cdot)$, the proximal operators can be evaluated analytically. In this situation, we only need to evaluate the proximal operators \emph{once}, and iterate \eqref{eq:admm1} and \eqref{eq:admm2} in closed form. This improves the overall computation time significantly. Here we explain how to express the solutions of \eqref{eq:admm1} and \eqref{eq:admm2} using proximal operators.

We focus our discussion on \eqref{eq:admm2}, or its equivalent formulation in \eqref{eq:admm_lop}, while the same argument holds for \eqref{eq:admm1} as well. Recall that the localizability constraint $\hat{\s}$ in \eqref{eq:admmlop3} is given by $\hat{\s} = \Ell \cap \FT \cap \hat{\Sother}$. We use the column-wise partition and the dimension reduction techniques described in Section \ref{sec:sf} (the procedure that simplifies \eqref{eq:sf_lop2} into \eqref{eq:decom3}) to simplify \eqref{eq:admm_lop} into
\begin{subequations} \label{eq:decom4}
\begin{align} 
\underset{\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}}{\text{minimize }} \quad & \hat{g}'_j(\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}) \nonumber\\
+ & \frac{\rho}{2} || \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} - \Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j} - \Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j} ||_{\mathcal{H}_2}^2 \label{eq:decom4-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{\Set t_j}{\Set r_j} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} = \Sub{J_B}{\Set t_j}{\Set p_j} \label{eq:decom4-2} \\
& \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} \in \Sub{\Ell}{\Set r_j}{\Set p_j} \cap \FT \cap \hat{\Sother}'_j \label{eq:decom4-3}
\end{align}
\end{subequations}
for $j = 1, \dots \hat{m}$. 
%The optimization variables of problem \eqref{eq:decom4} are the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. 
In \eqref{eq:decom4}, the transfer matrices $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, $\Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j}$, and $\Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j}$ are all FIRs with horizon $T$. We express the optimization variables of problem \eqref{eq:decom4} using a column vector defined by
\begin{equation}
\Psi_{v(j)} = \text{vec}(\begin{bmatrix} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[0] & \cdots & \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[T] \end{bmatrix}) \nonumber
\end{equation} 
where $\Psi_{v(j)}$ is the vectorization of all the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. Similarly, we define $\Phi_{v(j)}^{k+1}$ and $\Lambda_{v(j)}^k$ the vectorization of all the spectral components of $\Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j}$ and $\Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j}$, respectively.
%As the FIR constraint is imposed on the transfer matrix $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, the optimization variables of problem \eqref{eq:decom4} are the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. Let 
%\begin{equation}
%\Psi_{v(j)} = \text{vec}(\begin{bmatrix} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[0] & \cdots & \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[T] \end{bmatrix}). \nonumber
%\end{equation} 
%be the vectorization of all the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, which is a column vector. We can define $\Phi_{v(j)}^{k+1}$ and $\Lambda_{v(j)}^k$ in a similar manner. 
The optimization problem \eqref{eq:decom4} can then be written in the form of
\begin{subequations} \label{eq:decom5}
\begin{align} 
\underset{\Psi_{v(j)}}{\text{minimize }} \quad & g_{v(j)}(\Psi_{v(j)}) + \frac{\rho}{2} || \Psi_{v(j)} - \Phi_{v(j)}^{k+1} - \Lambda_{v(j)}^k ||_2^2 \label{eq:decom5-1}\\
\text{subject to } \quad & \Psi_{v(j)} \in \s_{v(j)} \label{eq:decom5-2}
\end{align}
\end{subequations}
where $g_{v(j)}(\cdot)$ is the vectorization form of $\hat{g}'_j(\cdot)$, and $\s_{v(j)}$ is the set constraint imposed by \eqref{eq:decom4-2} - \eqref{eq:decom4-3}. Define the indicator function by
\begin{equation}
\mathcal{I}_{\mathcal{D}}(x) = \left\{ \begin{array}{ll}
0 & x \in \mathcal{D}\\
\infty & x \not \in \mathcal{D}.
\end{array} \right. \nonumber
\end{equation}
Problem \eqref{eq:decom5} can be written as an unconstrained problem as
\begin{align}
\underset{\Psi_{v(j)}}{\text{minimize }} \quad &\mathcal{I}_{\s_{v(j)}}(\Psi_{v(j)}) + g_{v(j)}(\Psi_{v(j)}) \nonumber\\
&+ \frac{\rho}{2} || \Psi_{v(j)} - \Phi_{v(j)}^{k+1} - \Lambda_{v(j)}^k ||_2^2. \label{eq:decom6}
\end{align}
The solution of \eqref{eq:decom6} can be expressed using the proximal operator as
\begin{equation}
\Psi_{v(j)}^{k+1} = \textbf{prox}_{\mathcal{I}_{\s_{v(j)}} + \frac{1}{\rho} g_{v(j)}} ( \,\Phi_{v(j)}^{k+1} + \Lambda_{v(j)}^k \,). \label{eq:proximal}
\end{equation}
Equation \eqref{eq:proximal} is the solution of \eqref{eq:decom4} because \eqref{eq:decom6} is equivalent to \eqref{eq:decom4}.
%As problem \eqref{eq:decom6} is equivalent to problem \eqref{eq:decom4}, \eqref{eq:proximal} is the solution of \eqref{eq:decom4}. 
Therefore, the ADMM update \eqref{eq:admm2} can be carried out by the proximal operators \eqref{eq:proximal} for $j = 1, \dots \hat{m}$, all in the reduced dimension.

For certain type of objective functions, the proximal operator in \eqref{eq:proximal} can be evaluated analytically (see Ch. 6 of \cite{proximalBoyd}). Here we list a few examples.
\begin{example} \label{ex:analytic1}
%the objective functions $\tilde{g}(\cdot)$ and $\hat{g}(\cdot)$ are convex quadratic. The constraint sets $\tilde{\s}$ and $\hat{\s}$ are the 
Consider the localized linear quadratic Gaussian (LLQG) problem proposed in \cite{2015_Wang_H2}. The objective function is given in \eqref{eq:trad_obj2}, and the constraint is the intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the communication delay subspace constraint $\C$. When the global optimization problem is decomposed into multiple subproblems in the form of \eqref{eq:decom5}, each subproblem is a convex quadratic program restricted on an affine set. The proximal operator of this problem is an affine function \cite{2015_Wang_H2, proximalBoyd, BoydADMM}. We only need to calculate this affine function once. The iteration in \eqref{eq:admm1} - \eqref{eq:admm3} can then be carried out using multiple matrix multiplications in the reduced dimension, which significantly improves the overall computation time.
\end{example}
\begin{example} \label{ex:analytic2}
Consider the localized LQR (LLQR) problem with actuator regularization \cite{2015_Wang_Reg}. The column-wise part is identical to the LLQG example, so the update \eqref{eq:admm2} can be computed using matrix multiplication. Suppose that we use \eqref{eq:act_norm} as the actuator norm. The row-wise part can be decomposed and simplified into multiple unconstrained optimization problems with $g_{v(j)}(\cdot)$ being the $\ell_2$ norm of the variables. The proximal operator of this problem is a vectorial soft-thresholding \cite{2015_Wang_Reg, proximalBoyd}, which can be calculated in an efficient way. 
%If we use the $\ell_1 / \ell_\infty$ norm as the actuator norm, efficient algorithm to evaluate the proximal operator also exists \cite{proximalBoyd}.
\end{example}

Beside ADMM, there are other algorithms to solve the optimization problem \eqref{eq:sub3} in an efficient and scalable way. For instance, if either $\tilde{g}(\cdot)$ or $\hat{g}(\cdot)$ is strongly convex, we can use the alternating minimization algorithm (AMA) \cite{AMA} to simplify the ADMM algorithm. An alternative is the over-relax ADMM \cite{BoydADMM}. Finally, we can use the accelerated version of ADMM and AMA proposed in \cite{FastADMM}.

%\subsection{Localized Synthesis and Re-synthesis}
\subsection{LLQG with Sensor Actuator Regularization}\label{sec:sar}
We summarize all the techniques described in this section on the LLQG problem with sensor actuator regularization. This problem is used in Section \ref{sec:simu} as a case study example.
\begin{example}
The LLQG problem with sensor actuator regularization is formulated by 
\begin{subequations} \label{eq:h2l1}
\begin{align} 
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & \eqref{eq:h2_sar} \label{eq:h2l1-1}\\
%||\begin{bmatrix} C_1 & D_{12} \end{bmatrix}\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \lambda \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} 
\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \C \cap \Ell \cap \FT. \label{eq:h2l1-3}
\end{align}
\end{subequations}
where $\C$ encodes the communication delay constraint. \footnote{The communication delay constraint is specified by the sparsity constraint imposed on each spectral component of $\tf R$, $\tf M$, $\tf N$, and $\tf L$. Consider the controller implementation in \eqref{eq:implementation}. For example, suppose that there is $\tau$ time steps of delay to transmit the measurement $y_j$ to the control $u_i$. Then, we impose the constraint $L_{ij}[k] = 0$ for $k = 0, \dots, \tau - 1$.}
We assume that the matrix $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ in \eqref{eq:h2l1-1} is identity, and $\begin{bmatrix} B_1^\top & D_{12}^\top \end{bmatrix}^\top$ is diagonal. Problem \eqref{eq:h2l1} is decomposable, and thus can be solved by the algorithm \eqref{eq:admm} in a scalable way. Specifically, the $\mathcal{H}_2$ norm and the sensor regularizer belong to the column-wise decomposable component of the objective function, while the actuator regularizer belongs to the row-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
\end{example}

Once the row-wise and the column-wise decomposable components are identified, we decompose the subroutines \eqref{eq:admm1} and \eqref{eq:admm2} into parallel local subproblems. In this example, each local subproblem can be evaluated in analytic form. For the actuator regularizer in the row-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic2}. For the transfer matrix $\begin{bmatrix} \tf R^\top & \tf M^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic1}. 
%Here we discuss the analytic solution for the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part.
For the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the objective function is given by the sum of a convex quadratic and a $\ell_2$ norm, and the constraint is a linear subspace. As $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ is identity, the leading coefficient of the quadratic objective is identity. In this case, the optimization problem can be rewritten into the form as the one in Example \ref{ex:analytic2}, with an additional linear subspace constraint. We can show that the analytic solution is given by a projection onto a linear subspace followed by a vectorial soft-thresholding. 

Finally, the weights $\mu_i$ and $\lambda_i$ in the regularizers \eqref{eq:act_norm} and \eqref{eq:sen_norm} can be properly chosen to further enhance row/column-wise sparsity. We use the reweighted $\ell_1$ algorithm proposed in \cite{Reweighted} to iteratively set the weights and solve \eqref{eq:h2l1} multiple times. Let $\mu_i^{(0)} = \mu_0$ for $i = 1, \dots, n_u$ and $\lambda_i^{(0)} = \lambda_0$ for $i = 1, \dots, n_y$.
Let $(\tf R^{(k)}, \tf M^{(k)}, \tf N^{(k)}, \tf L^{(k)})$ be the optimal solution of \eqref{eq:h2l1} when the weights are given by $\{ \mu_i^{(k)} \}_{i=1}^{n_u}$ and $\{ \lambda_i^{(k)} \}_{i=1}^{n_y}$. We update the weights at iteration $(k+1)$ by
\begin{subequations}
\begin{align}
\mu_i^{(k+1)} &= ( \, || e_i^\top \begin{bmatrix} \tf M^{(k)} & \tf L^{(k)} \end{bmatrix} ||_{\mathcal{H}_2} + \epsilon )^{-1} \nonumber\\
\lambda_i^{(k+1)} &= ( \, || \begin{bmatrix} \tf N^{(k)} \\ \tf L^{(k)} \end{bmatrix} e_i ||_{\mathcal{H}_2} + \epsilon )^{-1} 
\end{align}
\end{subequations}
for some small $\epsilon$. It is shown in \cite{Reweighted} that this reweighted scheme usually results in sparser solution.



==> Output_v2.tex <==
%In the previous section, we discussed the direct decomposability of the optimization problem \eqref{eq:localized} when either $B_2$ or $C_2$ are invertible. The original problem can then be simplified significantly into \eqref{eq:sf_lop}. 
In this section, we discuss how to solve the general output feedback problem \eqref{eq:LOC} in a scalable way with arbitrary $B_2$ and $C_2$. In this case, the problem is not directly decomposable due to the coupling constraints \eqref{eq:main_1} and \eqref{eq:main_2}. We introduce the notion of decomposability with respect to distributed optimization for the objective function and the localizability constraint in \eqref{eq:LOC}, which is a substantial generalization of direct decomposability described in the previous section. When both the objective function and the localizability constraint are decomposable and convex, we can use the ADMM algorithm to decompose the problem \eqref{eq:LOC} into two subroutines. Each subroutine can be solved in a localized and scalable way using the direct decomposition method described in the previous section. We show that many class of problems satisfy this general decomposability condition. Examples include the $\mathcal{H}_2$ optimal control problem with sensor and actuator regularization and the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem.

%solve the output feedback problem \eqref{eq:localized} in a localized and scalable way. We give several classes of 
%In this section, we discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%State feedback is discussed first due to
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Decomposability with respect to Distributed Optimization}
We begin by simplifying the notation of \eqref{eq:LOC}. We use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. Denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$ and $\tf Z_{AC}$ the transfer matrix $\begin{bmatrix} zI-A^\top & -C_2^\top \end{bmatrix}^\top$. Let $J_B$ be the matrix in the right-hand-side of \eqref{eq:main_1} and $J_C$ be the matrix in the right-hand-side of \eqref{eq:main_2}. The original optimization problem \eqref{eq:LOC} can be written as
\begin{subequations} \label{eq:of_lop}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:of-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = J_B \label{eq:of-2} \\
& \ttf{\Phi} \tf Z_{AC} = J_C \label{eq:of-3} \\
& \ttf{\Phi} \in \s. \label{eq:of-4}
\end{align}
\end{subequations}
Here the stability constraint \eqref{eq:main_stable} is included in the set constraint $\s$ in \eqref{eq:of-4}. 

The primary difference between the output feedback problem \eqref{eq:of_lop} and the state feedback problem \eqref{eq:sf_lop2} is the additional constraint \eqref{eq:of-3}. The column-wise decomposition technique does not apply to the output feedback problem \eqref{eq:of_lop} directly because the constraint \eqref{eq:of-3} does not admit a column-wise decomposition. However, we note that the optimization variable $\ttf{\Phi}$ in constraint \eqref{eq:of-3} can be solved row at a time. Our strategy is to use distributed optimization techniques such as ADMM to decouple problem \eqref{eq:of_lop} into a row-wise decomposable component and a column-wise decomposable component. If the objective function \eqref{eq:of-1} and the localizability constraint \eqref{eq:of-4} can be split into a row-wise decomposable component and a column-wise decomposable component, we can then solve the localized output feedback optimal control problem \eqref{eq:of_lop} in a localized yet iterative way. 
%It is then natural to use distributed optimization techniques such as ADMM to decouple the constraints \eqref{eq:of-2} and \eqref{eq:of-3}, and solve 

From the definition of the closed loop transfer matrices \eqref{eq:desired}, the number of rows and columns of $\ttf{\Phi}$ in \eqref{eq:of_lop} are given by $(n_x + n_u)$ and $(n_x+n_y)$, respectively. Let $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ be a partition of the set $\{1, \dots, n_x+n_u\}$, and $\{ \Set q_1, \dots, \Set q_{\coldec{m}} \}$ be a partition of the set $\{1, \dots, n_x+n_y\}$. The decomposability of the objective function \eqref{eq:of-1} is defined as follows.
%The optimization variable $\ttf{\Phi}$ can be partitioned column-wisely into the set $\{ \Sub{\ttf{\Phi}}{ : }{\Set p_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\Set p_m} \}$. 
%Define decomposability for the objective and the localizability constraint
%Let $\{\Phi_j\}_{j=1}^n$ be a column-wise partition of $\Phi$, and $\{(\Phi^\top)_j\}_{j=1}^{n'}$ be a row-wise partition of $\Phi$ (a column-wise partition of $\Phi^\top$).
%Let $\{p_j\}_{j=1}^n$ be a column-wise partition for $CL$ (a partition on the perturbation $[\delta{x}; \delta{y}]$), and $\{p'_j\}_{j=1}^{n'}$ a row-wise partition for $CL$ (a partition on the internal variable $[x; u]$). 
%The decomposability for the objective function and the localizability constraint are defined as follows.
\begin{definition} \label{dfn:do}
The convex objective function $g(\ttf{\Phi})$ in \eqref{eq:of_lop} is said to be \emph{decomposable} with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\coldec{m}}\}$ if $g(\ttf{\Phi})$ can be written as the sum of two convex functions $\rowdec{g}(\ttf{\Phi})$ and $\coldec{g}(\ttf{\Phi})$, where $\rowdec{g}(\ttf{\Phi})$ is directly decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ and $\coldec{g}(\ttf{\Phi})$ is directly decomposable with respect to the column-wise partition $\{ \Set q_1, \dots, \Set q_{\coldec{m}} \}$. Specifically, we have 
\begin{eqnarray}
g(\ttf{\Phi}) &=& \rowdec{g}(\ttf{\Phi}) + \coldec{g}(\ttf{\Phi}) \nonumber\\
\rowdec{g}(\ttf{\Phi}) &=& \sum_{j=1}^{\rowdec{m}} \rowdec{g}_j(\Sub{\ttf{\Phi}}{\Set p_j}{:}) \nonumber\\
\coldec{g}(\ttf{\Phi}) &=& \sum_{j=1}^{\coldec{m}} \coldec{g}_j(\Sub{\ttf{\Phi}}{:}{\Set q_j}) \label{eq:obj_decom2}
\end{eqnarray}
for some convex functions $\rowdec{g}_j(\cdot)$ for $j = 1, \dots, \rowdec{m}$, and $\coldec{g}_j(\cdot)$ for $j = 1, \dots, \coldec{m}$.  
\end{definition}

In the rest of this paper, when we say an objective function is \emph{decomposable}, we mean that the objective function satisfy the conditions in \eqref{eq:obj_decom2} for some row-wise and column-wise partition. The directly decomposable objective function defined in Definition \ref{dfn:dd} is a special class of decomposable objective function with $\rowdec{g}(\cdot) = 0$. The decomposability of the localizability constraint \eqref{eq:of-4} is defined as follows.
%\begin{remark}
%From the definition, every directly decomposable objective function is a decomposable objective function, but not the opposite. 
%\end{remark}
\begin{definition} \label{dfn:ss}
The convex set constraint $\s$ in \eqref{eq:of_lop} is said to be \emph{decomposable} with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\coldec{m}}\}$ if $\s$ can be written as the intersection of two convex sets $\rowdec{\s}$ and $\coldec{\s}$, where $\rowdec{\s}$ is directly decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ and $\coldec{\s}$ is directly decomposable with respect to the column-wise partition $\{ \Set q_1, \dots, \Set q_{\coldec{m}} \}$. Specifically, we have 
\begin{eqnarray}
\s &=& \rowdec{\s} \cap \coldec{\s} \nonumber\\
\ttf{\Phi} \in \rowdec{\s} \quad &\Longleftrightarrow& \quad \bigcap_{j=1}^{\rowdec{m}} \Sub{\ttf{\Phi}}{\Set p_j}{:} \in \rowdec{\s}_j \nonumber\\
\ttf{\Phi} \in \coldec{\s} \quad &\Longleftrightarrow& \quad \bigcap_{j=1}^{\coldec{m}} \Sub{\ttf{\Phi}}{:}{\Set q_j} \in \coldec{\s}_j \label{eq:sdecom}
\end{eqnarray}
for some convex sets $\rowdec{\s}_j$ for $j = 1, \dots, \rowdec{m}$ and $\coldec{\s}_j$ for $j = 1, \dots, \coldec{m}$.
\end{definition}

Similarly, when we say a localizability constraint is \emph{decomposable}, we mean that the localizability constraint satisfy the conditions in Definition \ref{dfn:ss}. The directly decomposable constraint defined in Definition \ref{dfn:s} is a special class of decomposable localizability constraint which discards the constraint set $\rowdec{\s}$. 

\begin{remark} \label{rmk:lt}
In this paper, the localizability constraint $\s$ in \eqref{eq:of_lop} is expressed as $\s = \Ell \cap \FT \cap \Sother$. The locality constraint $\Ell$ and the FIR constraint $\FT$ are decomposable with respect to arbitrary row-wise and column-wise partition. Therefore, the decomposability of the localizability constraint $\s$ is determined by the decomposability of the constraint $\Sother$. If $\Sother$ is decomposable, we can express the original localizability constraint $\s$ as an intersection of the sets $\rowdec{\s} = \Ell \cap \FT \cap \rowdec{\Sother}$ and $\coldec{\s} = \Ell \cap \FT \cap \coldec{\Sother}$, where $\rowdec{\Sother}$ is a row-wise decomposable component of $\Sother$ and $\coldec{\Sother}$ a column-wise decomposable component of $\Sother$.
Note that the locality constraint and the FIR constraint are included in both $\rowdec{\s}$ and $\coldec{\s}$. As will be shown later, this is the key point to allow the subroutines of the ADMM algorithm to be solved in a finite dimensional and scalable way.
\end{remark}

%\begin{remark}
%From the definition, every directly decomposable localizability constraint is a decomposable localizability constraint, but not the opposite. 
%\end{remark}

%Consider the optimization problem
%\begin{subequations}
%\begin{align}
%\underset{\{R,M,N,L\}}{\text{minimize    }} & || \begin{bmatrix} R & \sigma_y N \\ \sigma_u M & \sigma_u \sigma_y L \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:h2_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:h2_1} \\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:h2_2} \\
%&  R, M, N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad L \in \mathcal{RH}_{\infty} \label{eq:h2_stable}\\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:h2_S}
%\end{align}
%\end{subequations}
%where $\sigma_u$ is the relative penalty between state deviation and control effort, $\sigma_y$ the relative magnitude of process disturbance and sensor disturbance. This corresponds to the case for some sparse $C_1, D_{21}, B_1, D_{21}$. Theoretically, the method described in this paper can generalize to arbitrary $C_1, D_{21}, B_1, D_{21}$, but it is effective only when those matrices are highly sparse.

%Assumptions (?)
Assume that the objective function and the localizability constraint in \eqref{eq:of_lop} are both decomposable with respect to the row-wise partition $\{ \Set p_1, \dots, \Set p_{\rowdec{m}}\}$ and the column-wise partition $\{ \Set q_1, \dots, \Set q_{\coldec{m}}\}$. We can split the optimization problem \eqref{eq:of_lop} into a row-wise decomposable part and a column-wise decomposable part. Let $\ttf{\Psi}$ be a duplicate of the optimization variable $\ttf{\Phi}$. We define extended-real-value functions $\rowdec{h}(\ttf{\Phi})$ and $\coldec{h}(\ttf{\Psi})$ by
\begin{eqnarray}
&& \rowdec{h}(\ttf{\Phi}) = \left\{ \begin{array}{ll}
\rowdec{g}(\ttf{\Phi}) & \textrm{if } \eqref{eq:of-3}, \ttf{\Phi} \in \rowdec{\s}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
&& \coldec{h}(\ttf{\Psi}) = \left\{ \begin{array}{ll}
\coldec{g}(\ttf{\Psi}) & \textrm{if } \eqref{eq:of-2}, \ttf{\Psi} \in \coldec{\s}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
\label{eq:extended}
\end{eqnarray}
Problem \eqref{eq:of_lop} can then be equivalently formulated as
\begin{eqnarray}
\underset{\{ \ttf{\Phi}, \ttf{\Psi} \}}{\text{minimize    }} && \rowdec{h}(\ttf{\Phi}) + \coldec{h}(\ttf{\Psi}) \nonumber\\
\text{subject to }  && \ttf{\Phi} = \ttf{\Psi}. \label{eq:sub3}
\end{eqnarray}
Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}. Specifically, the ADMM algorithm for \eqref{eq:sub3} is given by
\begin{subequations}\label{eq:admm}
\begin{align}
\ttf{\Phi}^{k+1} &= \underset{\ttf{\Phi}}{\text{argmin }} \Big( \rowdec{h}(\ttf{\Phi}) + \frac{\rho}{2} || \ttf{\Phi} - \ttf{\Psi}^{k} + \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm1} \\
\ttf{\Psi}^{k+1} &= \underset{\ttf{\Psi}}{\text{argmin }} \Big( \coldec{h}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm2} \\
\ttf{\Lambda}^{k+1} &= \ttf{\Lambda}^{k} + \ttf{\Phi}^{k+1} - \ttf{\Psi}^{k+1} \label{eq:admm3}
\end{align}
\end{subequations}
where the square of the $\mathcal{H}_2$ norm is computed by \eqref{eq:h2_comp}. As the FIR constraint $\FT$ is imposed on $\ttf{\Phi}$ and $\ttf{\Psi}$ through the constraint sets $\rowdec{\s}$ and $\coldec{\s}$, subroutines \eqref{eq:admm1} and \eqref{eq:admm2} are both finite dimensional optimization problems.
%When the FIR constraint $\FT$ is imposed through 
%of a transfer matrix can be computed by the sum of the square of Frobenius norm of all its spectral components.

%The primary reason 
%The main advantage of using the ADMM algorithm to solve \eqref{eq:sub3} is 
Subroutines \eqref{eq:admm1} and \eqref{eq:admm2} can be further decomposed row-wise and column-wise, respectively. For instance, the optimization problem corresponding to subroutine \eqref{eq:admm2} can be written as
\begin{subequations} \label{eq:admm_lop}
\begin{align} 
\underset{\ttf{\Psi}}{\text{minimize }} \quad & \coldec{g}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \label{eq:admmlop1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Psi} = J_B \label{eq:admmlop2} \\
& \ttf{\Psi} \in \coldec{\s}. \label{eq:admmlop3}
\end{align}
\end{subequations}
This problem has the same form as \eqref{eq:sf_lop2} -- the right-hand-side of \eqref{eq:admmlop2} does not affect the direct decomposability of the problem. The $\mathcal{H}_2$ norm regularizer in \eqref{eq:admmlop1} is directly decomposable with respect to arbitrary column-wise partition.
%, so the objective function in \eqref{eq:admmlop1} is column-wise decomposable. 
As the function $\coldec{g}(\cdot)$ and the localizability constraint $\coldec{\s}$ are directly decomposable with respect to a given column-wise partition, we can use the decomposition technique described in the previous section to decompose problem \eqref{eq:admm_lop} into parallel subproblems. As $\coldec{\s} = \Ell \cap \FT \cap \coldec{\Sother}$, we can exploit the locality constraint and use the dimension reduction technique described in the previous section to further reduce the complexity of each subproblem from global scale to local scale. Overall, subroutine \eqref{eq:admm2} can be solved in a localized and scalable manner. Similarly, subroutine \eqref{eq:admm1} can also be solved via the direct decomposition technique through a row-wise partition. Equation \eqref{eq:admm3} can be computed element-wisely since it is a matrix addition. Therefore, \eqref{eq:admm1} - \eqref{eq:admm3} is a scalable algorithm to solve the localized output feedback problem \eqref{eq:of_lop} by using row-wise and column-wise decomposition alternatively and iteratively.

%Note that $\rowdec{h}(\Phi)$ admits a block column-wise decomposition as both $\rowdec{g}(\Phi)$ and the localizability constraint $\mathcal{S}$ are both column-wise decomposable. As the $\mathcal{H}_2$ norm admits a column-wise decomposition for any partition, subproblem \eqref{eq:admm1} can be solved using the state feedback decomposition technique described in the previous subsection. When the localizability constraint $\mathcal{S}$ is highly sparse, subproblem \eqref{eq:admm1} can be solved in a localized and scalable way. 
%From the decomposability assumptions on the objective function and the localizability constraint, function $\rowdec{h}(\Phi)$ admits a block column-wise decomposition. 
%and function $\coldec{h}(\Psi)$ admits a block row-wise decomposition. 
%From the decomposability of the
%Subproblem \eqref{eq:admm1} reduces to be form of state feedback 
%can be solved in a localized way using LLQR with a column-wise decomposition on the objective function and the constraint. 

\subsection{Examples of Decomposable Problems}
In this subsection, we introduce several classes of decomposable objective functions and decomposable localizability constraints. All these problems can be solved using the ADMM algorithm described in the previous subsection in a scalable way.
\begin{example} \label{ex:b1}
Consider the objective function of the distributed optimal control problem in \eqref{eq:trad_obj2} with either the $\mathcal{H}_2$ norm or the element-wise $\ell_1$ norm defined in Example \ref{ex:l1}. Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} B_1^\top & D_{21}^\top \end{bmatrix} \Pi$ is block diagonal. Using a similar argument as in Example \ref{ex:perm}, we can find a column-wise partition to decompose the objective function in a column-wise manner. Likewise, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the objective function in a row-wise manner. In both cases, the objective function is directly decomposable and thus decomposable.
\end{example}
%\begin{example} \label{ex:c1}
%Similarly, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the objective function in a row-wise manner. This objective function is directly decomposable and thus decomposable.
%\end{example}
\begin{example}
Consider the weighted actuator norm defined in \cite{MC_CDC14, 2015_Wang_Reg}, which is given by
\begin{equation}
|| \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} = \sum_{i=1}^{n_u} \mu_i || e_i^\top \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{H}_2} \label{eq:act_norm} 
\end{equation}
where $\mu$ is a diagonal matrix with $\mu_i$ being its $i$th diagonal entry, and $e_i$ is a unit vector with $1$ on its $i$th entry and $0$ elsewhere. When $\mu$ is an identity matrix, the actuator norm \eqref{eq:act_norm} is equivalent to the $\ell_1 / \ell_2$ norm, or the group lasso \cite{2006_grouplasso} in the statistical learning literature. This norm acts as a regularizer to make the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ row-wise sparse, i.e., have many zero rows. Recall from Theorem \ref{thm:1} that the controller achieving the desired closed loop response can be implemented by \eqref{eq:implementation}. If the $i$th row of the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ is a zero row, then the $i$th component of the control action $u_i$ is always equal to zero. This means that we can remove the control action $u_i$ without changing the closed loop response. It is clear that the actuator norm defined in \eqref{eq:act_norm} is directly decomposable to arbitrary row-wise partition. This still holds true when the actuator norm is defined by the $\ell_1 / \ell_\infty$ norm. Similarly, consider the weighted sensor norm given by
\begin{equation}
|| \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} = \sum_{i=1}^{n_y} \lambda_i || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} e_i ||_{\mathcal{H}_2} \label{eq:sen_norm} 
\end{equation}
where $\lambda$ is a diagonal matrix with $\lambda_i$ being its $i$th diagonal entry. The sensor norm in \eqref{eq:sen_norm} is a regularizer to make the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ column-wise sparse. Using the controller implementation \eqref{eq:implementation}, the sensor norm can be treated as a regularizer on the measurement $y$. For instance, if the $i$th column of the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ is identical to zero, then we can ignore the measurement $y_i$ without changing the closed loop response. The sensor norm defined in \eqref{eq:act_norm} is directly decomposable with respect to any column-wise partition.
\end{example}
\begin{example}
From Definition \ref{dfn:do}, it is straightforward to see that the sum of multiple decomposable objective functions with the same partition is still decomposable with respect to the given partition. Therefore, we can combine all the decomposable objective functions above, and the resulting objective function is still decomposable. For instance, consider the $\mathcal{H}_2$ optimal control problem with sensor and actuator regularization. The objective function is given by
\begin{eqnarray}
g(\tf R,\tf M,\tf N,\tf L) &=& ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
&&+ || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} \label{eq:h2_sar}
\end{eqnarray}
where $\mu$ and $\lambda$ are the relative penalty between the $\mathcal{H}_2$ performance and the actuator and sensor regularizer, respectively. If there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal, then the objective function \eqref{eq:h2_sar} is decomposable. In this case, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise decomposable component, and the sensor regularizer belongs to the column-wise decomposable component.
\end{example}

Next, we consider some examples of decomposable localizability constraints beside the locality constraint $\Ell$ and the FIR constraint $\FT$ described in Remark \ref{rmk:lt}.
%, some other examples of decomposable localizability constraints are given as follows.
\begin{example}
Consider the $\mathcal{L}_1$ norm \cite{Munther_L1} of a FIR transfer matrix $\tf G \in \FT$, which is given by
\begin{equation}
|| \tf G ||_{\mathcal{L}_1} = \underset{i}{\text{max}} \quad \sum_{j} \sum_{t=1}^T | g_{ij}[t] |.\label{eq:L1_defn}
\end{equation}
The $\mathcal{L}_1$ norm is an induced norm from a $\ell_\infty$ input signal to a $\ell_\infty$ output signal. Suppose that the $\ell_\infty$ norm of the disturbance $\delta_x$ and $\delta_y$ in \eqref{eq:desired} is bounded, and we want to bound the $\ell_\infty$ norm of the state vector $x$ and the control action $u$. We can impose the constraint
\begin{equation}
|| \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} ||_{\mathcal{L}_1} \leq \gamma \label{eq:L1_cons}
\end{equation}
in the optimization problem \eqref{eq:of_lop} for some $\gamma$. The solution of \eqref{eq:L1_cons} forms a convex set because it is a sublevel set of a convex function. Therefore, we can consider \eqref{eq:L1_cons} as a localizability constraint. From the definition \eqref{eq:L1_defn}, the constraint \eqref{eq:L1_cons} is decomposable with respect to arbitrary row-wise partition. If we choose the $\mathcal{H}_2$ norm as the objective function and \eqref{eq:L1_cons} as the constraint, then the problem becomes a mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem. As both the objective and the constraint are decomposable, the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem is decomposable. %it is a directly decomposable constraint and thus a decomposable constraint. 
\end{example}
\begin{example}
From Definition \ref{dfn:ss}, the intersection of multiple decomposable constraints with the same partition is decomposable with respect to the given partition. Therefore, we can combine all the decomposable constraints described above, and the resulting localizability constraint is still decomposable. This property is extremely useful because all the decomposable constraints can be incorporated into the optimization problem in a sequential manner without breaking the decomposability of the problem. For instance, the combination of the locality constraint $\Ell$, the FIR constraint $\FT$, and the $\mathcal{L}_1$ constraint in \eqref{eq:L1_cons} is decomposable.
\end{example}
%The ADMM algorithm described in the previous subsection can be applied to any problem with a decomposable objective function and a decomposable localizability constraint.
%Here we consider a localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization. We explain how to solve this problem in a localized and scalable manner using the ADMM algorithm.
%\begin{example}
%A localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization is formulated by
%\begin{subequations} \label{eq:h2l1}
%\begin{align} 
%\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + \mu || \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + \lambda || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} \label{eq:h2l1-1}\\
%\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \label{eq:h2l1-3} \\
%& || \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} ||_{\mathcal{L}_1} \leq \gamma \label{eq:h2l1-4}.
%\end{align}
%\end{subequations}
%Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. In this case, problem \eqref{eq:h2l1} is decomposable. Specifically, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise decomposable component of the objective function, while the sensor regularizer belongs to the column-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2} and the $\mathcal{L}_1$ constraint \eqref{eq:h2l1-4}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
%\end{example}

%Without the constraint \eqref{eq:h2_2}, this optimization problem admits a column-wise decomposition as the LLQR problem. Similarly, without the constraint \eqref{eq:h2_1}, the optimization problem admits a row-wise decomposition. Specifically, we solve
%\begin{eqnarray}
%\begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_1}, \eqref{eq:h2_stable}, \eqref{eq:h2_S} \label{eq:sub1}
%\end{eqnarray}
%and
%\begin{eqnarray}
%\begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_2}, \eqref{eq:h2_stable}, \eqref{eq:h2_S}. \label{eq:sub2}
%\end{eqnarray}
%When the constraint \eqref{eq:h2_S} is a locality constraint, we can utilize the technique of LLQR to solve both \eqref{eq:sub1} and \eqref{eq:sub2} in a completely localized and parallel way.
%
%The optimal solution in \eqref{eq:sub1} and \eqref{eq:sub2} may not be the same. Therefore, we need to solve an extra optimization problem as
%\begin{eqnarray}
%\underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix}. \label{eq:sub3}
%\end{eqnarray}
%Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}.

\subsection{Convergence and Stopping Criteria}
In this subsection, we identify the technical conditions on problem \eqref{eq:of_lop} (or equivalently, \eqref{eq:sub3}) such that the ADMM algorithm \eqref{eq:admm1} - \eqref{eq:admm3} converges to an optimal solution. We make the following assumptions. 
\begin{assumption}
Problem \eqref{eq:of_lop} has a feasible solution in the relative interior of the set $\s$. \label{as:1}
\end{assumption}
\begin{assumption} 
The functions $\rowdec{g}(\cdot)$ and $\coldec{g}(\cdot)$ are closed, proper, and convex. \label{as:2}
\end{assumption}
\begin{assumption} 
The sets $\rowdec{\s}$ and $\coldec{\s}$ are closed and convex. \label{as:3}
\end{assumption}

Assumption \ref{as:1} implies feasibility and strong duality of \eqref{eq:of_lop} (or its equivalent formulation \eqref{eq:sub3}). Combining with Assumptions \ref{as:2} and \ref{as:3}, we know that the extended-real-value functions $\rowdec{h}(\cdot)$ and $\coldec{h}(\cdot)$ defined in \eqref{eq:extended} are closed, proper, and convex. Under these assumptions, problem \eqref{eq:sub3} satisfies the convergence conditions in \cite{BoydADMM}. From \cite{BoydADMM}, we have objective convergence, dual variable convergence ($\ttf{\Lambda}^{k} \to \ttf{\Lambda}^{*}$ as $k \to \infty$), and residual convergence ($\ttf{\Phi}^k - \ttf{\Psi}^k \to 0$ as $k \to \infty$). As long as the problem \eqref{eq:sub3} approaches feasibility and the optimal value of \eqref{eq:sub3} converges to the global optimal, we can use a feasible solution of \eqref{eq:sub3} to construct a controller that achieves the desired optimal closed loop response. Note that the optimization problem \eqref{eq:sub3} may not have a unique optimal point, so the optimization variable $\ttf{\Phi}^k$ and $\ttf{\Psi}^k$ does not necessary converge. If we further assume that the objective function $g(\cdot)$ is strongly convex with respect to $\ttf{\Phi}$, then problem \eqref{eq:sub3} has a unique optimal solution $\ttf{\Phi}^*$. In this case, objective convergence implies primal variable convergence, so we have $\ttf{\Phi}^k \to \ttf{\Phi}^*$ and $\ttf{\Psi}^k \to \ttf{\Phi}^*$ as $k \to \infty$.

The stopping criteria is designed from \cite{BoydADMM}, in which we use $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2}$ as primal infeasibility and $|| \ttf{\Psi}^k - \ttf{\Psi}^{k-1} ||_{\mathcal{H}_2}$ as dual infeasibility. The square of these two functions can be calculated in a localized and distributed way. The algorithm \eqref{eq:admm1} - \eqref{eq:admm3} terminates when $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2} < \epsilon^{pri}$ and $|| \ttf{\Psi}^k - \ttf{\Psi}^{k-1} ||_{\mathcal{H}_2} < \epsilon^{dual}$ for some feasibility tolerances $\epsilon^{pri}$ and $\epsilon^{dual}$.
%the primal and dual infeasibility are smaller than the feasibility tolerances $\epsilon^{pri}$ and $\epsilon^{dual}$, respectively.

In practice, we may not know the feasibility of \eqref{eq:of_lop} in advanced. In other words, we do not know whether Assumption \ref{as:1} holds. Consider the case that the ADMM subroutines \eqref{eq:admm1} - \eqref{eq:admm3} are solvable, but problem \eqref{eq:sub3} is infeasible. In this situation, the stopping criteria on primal infeasibility $|| \ttf{\Phi}^k - \ttf{\Psi}^k ||_{\mathcal{H}_2} < \epsilon^{pri}$ may not be satisfied. To avoid infinite number of iterations, we can set a limit on the number of iterations in the ADMM algorithm. The convergence result of the ADMM algorithm should be regarded as a scalable algorithm to check the $\s$-localizability of the system matrices $(A,B_2,C_2)$ in \eqref{eq:of_lop}. If the ADMM algorithm does not converge, then we know that the system $(A,B_2,C_2)$ is not $\s$-localizable. Interested readers can refer to \cite{2015_Wang_Reg} on the design of the localizability constraint $\s$ to ensure the feasibility of \eqref{eq:of_lop} for some specific systems.

\subsection{Analytic Solution and Acceleration}
Suppose that Assumptions \ref{as:1} - \ref{as:3} hold. The ADMM algorithm presented in \eqref{eq:admm1} - \eqref{eq:admm3} is a special case of the proximal algorithm \cite{proximal, proximalBoyd, BoydADMM}. For certain type of objective functions $\rowdec{h}(\cdot)$ and $\coldec{h}(\cdot)$, the proximal operators can be evaluated analytically. In this situation, we only need to evaluate the proximal operators \emph{once}, and iterate \eqref{eq:admm1} and \eqref{eq:admm2} in closed form. This improves the overall computation time significantly. Here we explain how to express the solutions of \eqref{eq:admm1} and \eqref{eq:admm2} using proximal operators.

We focus our discussion on \eqref{eq:admm2}, or its equivalent formulation in \eqref{eq:admm_lop}, while the same argument holds for \eqref{eq:admm1} as well. Recall that the localizability constraint $\coldec{\s}$ in \eqref{eq:admmlop3} is given by $\coldec{\s} = \Ell \cap \FT \cap \coldec{\Sother}$. We use the column-wise partition and the dimension reduction techniques described in Section \ref{sec:sf} (the procedure that simplifies \eqref{eq:sf_lop2} into \eqref{eq:decom3}) to simplify \eqref{eq:admm_lop} into
\begin{subequations} \label{eq:decom4}
\begin{align} 
\underset{\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}}{\text{minimize }} \quad & \coldec{g}_j(\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}) \nonumber\\
+ & \frac{\rho}{2} || \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} - \Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j} - \Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j} ||_{\mathcal{H}_2}^2 \label{eq:decom4-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{\Set t_j}{\Set r_j} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} = \Sub{J_B}{\Set t_j}{\Set p_j} \label{eq:decom4-2} \\
& \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j} \in \Sub{\Ell}{\Set r_j}{\Set p_j} \cap \FT \cap \coldec{\Sother}_j \label{eq:decom4-3}
\end{align}
\end{subequations}
for $j = 1, \dots \coldec{m}$. 
%The optimization variables of problem \eqref{eq:decom4} are the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. 
In \eqref{eq:decom4}, the transfer matrices $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, $\Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j}$, and $\Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j}$ are all FIRs with horizon $T$. We express the optimization variables of problem \eqref{eq:decom4} using a column vector defined by
\begin{equation}
\Psi_{v(j)} = \text{vec}(\begin{bmatrix} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[0] & \cdots & \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[T] \end{bmatrix}) \nonumber
\end{equation} 
where $\Psi_{v(j)}$ is the vectorization of all the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. Similarly, we define $\Phi_{v(j)}^{k+1}$ and $\Lambda_{v(j)}^k$ the vectorization of all the spectral components of $\Sub{\ttf{\Phi}^{k+1}}{\Set r_j}{\Set p_j}$ and $\Sub{\ttf{\Lambda}^{k}}{\Set r_j}{\Set p_j}$, respectively.
%As the FIR constraint is imposed on the transfer matrix $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, the optimization variables of problem \eqref{eq:decom4} are the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$. Let 
%\begin{equation}
%\Psi_{v(j)} = \text{vec}(\begin{bmatrix} \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[0] & \cdots & \Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}[T] \end{bmatrix}). \nonumber
%\end{equation} 
%be the vectorization of all the spectral components of $\Sub{\ttf{\Psi}}{\Set r_j}{\Set p_j}$, which is a column vector. We can define $\Phi_{v(j)}^{k+1}$ and $\Lambda_{v(j)}^k$ in a similar manner. 
The optimization problem \eqref{eq:decom4} can then be written in the form of
\begin{subequations} \label{eq:decom5}
\begin{align} 
\underset{\Psi_{v(j)}}{\text{minimize }} \quad & g_{v(j)}(\Psi_{v(j)}) + \frac{\rho}{2} || \Psi_{v(j)} - \Phi_{v(j)}^{k+1} - \Lambda_{v(j)}^k ||_2^2 \label{eq:decom5-1}\\
\text{subject to } \quad & \Psi_{v(j)} \in \s_{v(j)} \label{eq:decom5-2}
\end{align}
\end{subequations}
where $g_{v(j)}(\cdot)$ is the vectorization form of $\coldec{g}_j(\cdot)$, and $\s_{v(j)}$ is the set constraint imposed by \eqref{eq:decom4-2} - \eqref{eq:decom4-3}. Define the indicator function by
\begin{equation}
\mathcal{I}_{\mathcal{D}}(x) = \left\{ \begin{array}{ll}
0 & x \in \mathcal{D}\\
\infty & x \not \in \mathcal{D}.
\end{array} \right. \nonumber
\end{equation}
Problem \eqref{eq:decom5} can be written as an unconstrained problem as
\begin{align}
\underset{\Psi_{v(j)}}{\text{minimize }} \quad &\mathcal{I}_{\s_{v(j)}}(\Psi_{v(j)}) + g_{v(j)}(\Psi_{v(j)}) \nonumber\\
&+ \frac{\rho}{2} || \Psi_{v(j)} - \Phi_{v(j)}^{k+1} - \Lambda_{v(j)}^k ||_2^2. \label{eq:decom6}
\end{align}
The solution of \eqref{eq:decom6} can be expressed using the proximal operator as
\begin{equation}
\Psi_{v(j)}^{k+1} = \textbf{prox}_{\mathcal{I}_{\s_{v(j)}} + \frac{1}{\rho} g_{v(j)}} ( \,\Phi_{v(j)}^{k+1} + \Lambda_{v(j)}^k \,). \label{eq:proximal}
\end{equation}
Equation \eqref{eq:proximal} is the solution of \eqref{eq:decom4} because \eqref{eq:decom6} is equivalent to \eqref{eq:decom4}.
%As problem \eqref{eq:decom6} is equivalent to problem \eqref{eq:decom4}, \eqref{eq:proximal} is the solution of \eqref{eq:decom4}. 
Therefore, the ADMM update \eqref{eq:admm2} can be carried out by the proximal operators \eqref{eq:proximal} for $j = 1, \dots \coldec{m}$, all in the reduced dimension.

For certain type of objective functions, the proximal operator in \eqref{eq:proximal} can be evaluated analytically (see Ch. 6 of \cite{proximalBoyd}). Here we list a few examples.
\begin{example} \label{ex:analytic1}
%the objective functions $\rowdec{g}(\cdot)$ and $\coldec{g}(\cdot)$ are convex quadratic. The constraint sets $\rowdec{\s}$ and $\coldec{\s}$ are the 
Consider the localized linear quadratic Gaussian (LLQG) problem proposed in \cite{2015_Wang_H2}. The objective function is given in \eqref{eq:trad_obj2}, and the constraint is the intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the communication delay subspace constraint $\C$. When the global optimization problem is decomposed into multiple subproblems in the form of \eqref{eq:decom5}, each subproblem is a convex quadratic program restricted on an affine set. The proximal operator of this problem is an affine function \cite{2015_Wang_H2, proximalBoyd, BoydADMM}. We only need to calculate this affine function once. The iteration in \eqref{eq:admm1} - \eqref{eq:admm3} can then be carried out using multiple matrix multiplications in the reduced dimension, which significantly improves the overall computation time.
\end{example}
\begin{example} \label{ex:analytic2}
Consider the localized LQR (LLQR) problem with actuator regularization \cite{2015_Wang_Reg}. The column-wise part is identical to the LLQG example, so the update \eqref{eq:admm2} can be computed using matrix multiplication. Suppose that we use \eqref{eq:act_norm} as the actuator norm. The row-wise part can be decomposed and simplified into multiple unconstrained optimization problems with $g_{v(j)}(\cdot)$ being the $\ell_2$ norm of the variables. The proximal operator of this problem is a vectorial soft-thresholding \cite{2015_Wang_Reg, proximalBoyd}, which can be calculated in an efficient way. 
%If we use the $\ell_1 / \ell_\infty$ norm as the actuator norm, efficient algorithm to evaluate the proximal operator also exists \cite{proximalBoyd}.
\end{example}

Beside ADMM, there are other algorithms to solve the optimization problem \eqref{eq:sub3} in an efficient and scalable way. For instance, if either $\rowdec{g}(\cdot)$ or $\coldec{g}(\cdot)$ is strongly convex, we can use the alternating minimization algorithm (AMA) \cite{AMA} to simplify the ADMM algorithm. An alternative is the over-relax ADMM \cite{BoydADMM}. Finally, we can use the accelerated version of ADMM and AMA proposed in \cite{FastADMM}.

%\subsection{Localized Synthesis and Re-synthesis}
\subsection{LLQG with Sensor Actuator Regularization}\label{sec:sar}
We summarize all the techniques described in this section on the LLQG problem with sensor actuator regularization. This problem is used in Section \ref{sec:simu} as a case study example.
\begin{example}
The LLQG problem with sensor actuator regularization is formulated by 
\begin{subequations} \label{eq:h2l1}
\begin{align} 
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & \eqref{eq:h2_sar} \label{eq:h2l1-1}\\
%||\begin{bmatrix} C_1 & D_{12} \end{bmatrix}\begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \lambda \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} 
\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \C \cap \Ell \cap \FT. \label{eq:h2l1-3}
\end{align}
\end{subequations}
where $\C$ encodes the communication delay constraint. \footnote{The communication delay constraint is specified by the sparsity constraint imposed on each spectral component of $\tf R$, $\tf M$, $\tf N$, and $\tf L$. Consider the controller implementation in \eqref{eq:implementation}. For example, suppose that there is $\tau$ time steps of delay to transmit the measurement $y_j$ to the control $u_i$. Then, we impose the constraint $L_{ij}[k] = 0$ for $k = 0, \dots, \tau - 1$.}
We assume that the matrix $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ in \eqref{eq:h2l1-1} is identity, and $\begin{bmatrix} B_1^\top & D_{12}^\top \end{bmatrix}^\top$ is diagonal. Problem \eqref{eq:h2l1} is decomposable, and thus can be solved by the algorithm \eqref{eq:admm} in a scalable way. Specifically, the $\mathcal{H}_2$ norm and the sensor regularizer belong to the column-wise decomposable component of the objective function, while the actuator regularizer belongs to the row-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
\end{example}

Once the row-wise and the column-wise decomposable components are identified, we decompose the subroutines \eqref{eq:admm1} and \eqref{eq:admm2} into parallel local subproblems. In this example, each local subproblem can be evaluated in analytic form. For the actuator regularizer in the row-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic2}. For the transfer matrix $\begin{bmatrix} \tf R^\top & \tf M^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the analytic solution is given in Example \ref{ex:analytic1}. 
%Here we discuss the analytic solution for the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part.
For the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ in the column-wise decomposable part, the objective function is given by the sum of a convex quadratic and a $\ell_2$ norm, and the constraint is a linear subspace. As $\begin{bmatrix} C_1 & D_{21} \end{bmatrix}$ is identity, the leading coefficient of the quadratic objective is identity. In this case, the optimization problem can be rewritten into the form as the one in Example \ref{ex:analytic2}, with an additional linear subspace constraint. We can show that the analytic solution is given by a projection onto a linear subspace followed by a vectorial soft-thresholding. 

Finally, the weights $\mu_i$ and $\lambda_i$ in the regularizers \eqref{eq:act_norm} and \eqref{eq:sen_norm} can be properly chosen to further enhance row/column-wise sparsity. We use the reweighted $\ell_1$ algorithm proposed in \cite{Reweighted} to iteratively set the weights and solve \eqref{eq:h2l1} multiple times. Let $\mu_i^{(0)} = \mu_0$ for $i = 1, \dots, n_u$ and $\lambda_i^{(0)} = \lambda_0$ for $i = 1, \dots, n_y$.
Let $(\tf R^{(k)}, \tf M^{(k)}, \tf N^{(k)}, \tf L^{(k)})$ be the optimal solution of \eqref{eq:h2l1} when the weights are given by $\{ \mu_i^{(k)} \}_{i=1}^{n_u}$ and $\{ \lambda_i^{(k)} \}_{i=1}^{n_y}$. We update the weights at iteration $(k+1)$ by
\begin{subequations}
\begin{align}
\mu_i^{(k+1)} &= ( \, || e_i^\top \begin{bmatrix} \tf M^{(k)} & \tf L^{(k)} \end{bmatrix} ||_{\mathcal{H}_2} + \epsilon )^{-1} \nonumber\\
\lambda_i^{(k+1)} &= ( \, || \begin{bmatrix} \tf N^{(k)} \\ \tf L^{(k)} \end{bmatrix} e_i ||_{\mathcal{H}_2} + \epsilon )^{-1} 
\end{align}
\end{subequations}
for some small $\epsilon$. It is shown in \cite{Reweighted} that this reweighted scheme usually results in sparser solution.



==> Output_v3.tex <==
%In the previous section, we discussed the direct decomposability of the optimization problem \eqref{eq:localized} when either $B_2$ or $C_2$ are invertible. The original problem can then be simplified significantly into \eqref{eq:sf_lop}. 
In this section, we discuss how to solve the general form of the localized SLS problem \eqref{eq:localized} in a scalable way with arbitrary $B_2$ and $C_2$. Note that \eqref{eq:localized} is neither column-wise nor row-wise separable due to the coupling constraints \eqref{eq:main_1} and \eqref{eq:main_2}. 
We introduce the class of partially separable problems in this section, which is a substantial generalization of column/row-wise separable problems described in the previous section. When the SLO and the SLC are convex and partially separable, we can use ADMM algorithm to decouple \eqref{eq:localized} into two subroutines. Each subroutine can then be solved in a localized and scalable way using the column/row-wise separation method described in the previous section. 
%This section begins with the definition of generally separable problems. Then, 
We show that many constrained optimal control problems are partially separable. Examples include the localized $\mathcal{H}_2$ optimal control problem with sensor actuator regularization and the localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem. 
%Finally, we discuss the condition for the convergence of the ADMM algorithm, and give some specialization and variant to further accelerate the computation.

%solve the output feedback problem \eqref{eq:localized} in a localized and scalable way. We give several classes of 
%In this section, we discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%State feedback is discussed first due to
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Partially Separable Problems} \label{sec:ps}
We begin by simplifying the notation of \eqref{eq:localized}. We use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \nonumber
\end{equation}
to represent the system response we want to optimize for. Denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$ and $\tf Z_{AC}$ the transfer matrix $\begin{bmatrix} zI-A^\top & -C_2^\top \end{bmatrix}^\top$. Let $J_B$ be the matrix in the right-hand-side of \eqref{eq:main_1} and $J_C$ be the matrix in the right-hand-side of \eqref{eq:main_2}. The localized SLS problem \eqref{eq:localized} can be written as
\begin{subequations} \label{eq:of_lop}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:of-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = J_B \label{eq:of-2} \\
& \ttf{\Phi} \tf Z_{AC} = J_C \label{eq:of-3} \\
& \ttf{\Phi} \in \s \label{eq:of-4}
\end{align}
\end{subequations}
%Here the stability constraint \eqref{eq:main_stable} is included in the set constraint $\s$ in \eqref{eq:of-4}. 
with $\s = \Ell \cap \FT \cap \Sother$.
The goal of this section is to identify the technical conditions on $g(\cdot)$ and $\s$ in \eqref{eq:of_lop} so that the SLS problem \eqref{eq:of_lop} can be solved in a localized and scalable way.

The primary difference between the SLS problem \eqref{eq:of_lop} and its state feedback simplification \eqref{eq:sf_lop2} is the additional constraint \eqref{eq:of-3}. The column-wise separation technique does not apply to the SLS problem \eqref{eq:of_lop} directly because the constraint \eqref{eq:of-3} does not admit a column-wise separation. However, we note that the optimization variable $\ttf{\Phi}$ in constraint \eqref{eq:of-3} can be solved row at a time. Our strategy is to use distributed optimization techniques such as ADMM to decouple \eqref{eq:of_lop} into a row-wise separable component and a column-wise separable component. If the SLO \eqref{eq:of-1} and the SLC \eqref{eq:of-4} can be \emph{split} into a row-wise separable component and a column-wise separable component, then we can solve the localized SLS problem \eqref{eq:of_lop} in a localized yet iterative way. 
%It is then natural to use distributed optimization techniques such as ADMM to decouple the constraints \eqref{eq:of-2} and \eqref{eq:of-3}, and solve 

From the definition of the system response \eqref{eq:desired}, the number of rows and columns of $\ttf{\Phi}$ in \eqref{eq:of_lop} are given by $(n_x + n_u)$ and $(n_x+n_y)$, respectively. Let $\{ \rowps_1, \dots, \rowps_{q}\}$ be a partition of the set $\{1, \dots, n_x+n_u\}$, and $\{ \colps_1, \dots, \colps_{p} \}$ be a partition of the set $\{1, \dots, n_x+n_y\}$. We define partially separable SLO as follows.%The decomposability of the objective function \eqref{eq:of-1} is defined as follows.
%The optimization variable $\ttf{\Phi}$ can be partitioned column-wisely into the set $\{ \Sub{\ttf{\Phi}}{ : }{\rowps_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\rowps_m} \}$. 
%Define decomposability for the objective and the localizability constraint
%Let $\{\Phi_j\}_{j=1}^n$ be a column-wise partition of $\Phi$, and $\{(\Phi^\top)_j\}_{j=1}^{n'}$ be a row-wise partition of $\Phi$ (a column-wise partition of $\Phi^\top$).
%Let $\{p_j\}_{j=1}^n$ be a column-wise partition for $CL$ (a partition on the perturbation $[\delta{x}; \delta{y}]$), and $\{p'_j\}_{j=1}^{n'}$ a row-wise partition for $CL$ (a partition on the internal variable $[x; u]$). 
%The decomposability for the objective function and the localizability constraint are defined as follows.
\begin{definition} \label{dfn:do}
The convex system level objective $g(\ttf{\Phi})$ in \eqref{eq:of-1} is said to be \emph{partially separable} with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_{q}\}$ and the column-wise partition $\{ \colps_1, \dots, \colps_{p}\}$ if $g(\ttf{\Phi})$ can be written as the sum of two convex objectives $\rowdec{g}(\ttf{\Phi})$ and $\coldec{g}(\ttf{\Phi})$, where $\rowdec{g}(\ttf{\Phi})$ is row-wise separable with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_{q}\}$ and $\coldec{g}(\ttf{\Phi})$ is column-wise separable with respect to the column-wise partition $\{ \colps_1, \dots, \colps_{p} \}$. Specifically, we have 
\begin{eqnarray}
g(\ttf{\Phi}) &=& \rowdec{g}(\ttf{\Phi}) + \coldec{g}(\ttf{\Phi}) \nonumber\\
\rowdec{g}(\ttf{\Phi}) &=& \sum_{j=1}^{q} \rowdec{g}_j(\Sub{\ttf{\Phi}}{\rowps_j}{:}) \nonumber\\
\coldec{g}(\ttf{\Phi}) &=& \sum_{j=1}^{p} \coldec{g}_j(\Sub{\ttf{\Phi}}{:}{\colps_j}) \label{eq:obj_decom2}
\end{eqnarray}
for some convex functionals $\rowdec{g}_j(\cdot)$ for $j = 1, \dots, q$, and $\coldec{g}_j(\cdot)$ for $j = 1, \dots, p$.  
\end{definition}

%In the rest of this paper, when we say an objective function is \emph{separable}, we mean that the objective function satisfies the conditions in \eqref{eq:obj_decom2} for some row-wise and column-wise partition. 
Note that the column/row-wise separable SLO defined in Definition \ref{dfn:dd} and \ref{dfn:dd_row} are special cases of partially separable SLO. %with $\rowdec{g}(\cdot) = 0$. 
We define partially separable SLC \eqref{eq:of-4} as follows.
%\begin{remark}
%From the definition, every directly decomposable objective function is a decomposable objective function, but not the opposite. 
%\end{remark}
\begin{definition} \label{dfn:ss}
The convex system level constraint $\s$ in \eqref{eq:of-4} is said to be \emph{partially separable} with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_{q}\}$ and the column-wise partition $\{ \colps_1, \dots, \colps_{p}\}$ if $\s$ can be written as the intersection of two convex sets $\rowdec{\s}$ and $\coldec{\s}$, where $\rowdec{\s}$ is row-wise separable with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_{q}\}$ and $\coldec{\s}$ is column-wise separable with respect to the column-wise partition $\{ \colps_1, \dots, \colps_{p} \}$. Specifically, we have 
\begin{eqnarray}
\s &=& \rowdec{\s} \cap \coldec{\s} \nonumber\\
\ttf{\Phi} \in \rowdec{\s} \quad &\Longleftrightarrow& \quad \Sub{\ttf{\Phi}}{\rowps_j}{:} \in \rowdec{\s}_j, \forall j \nonumber\\
\ttf{\Phi} \in \coldec{\s} \quad &\Longleftrightarrow& \quad \Sub{\ttf{\Phi}}{:}{\colps_j} \in \coldec{\s}_j, \forall j \label{eq:sdecom}
\end{eqnarray}
for some convex sets $\rowdec{\s}_j$ for $j = 1, \dots, q$ and $\coldec{\s}_j$ for $j = 1, \dots, p$.
\end{definition}

%Similarly, when we say a set constraint is \emph{separable}, we mean that the set constraint satisfy the conditions in \eqref{eq:sdecom}. The column-wise separable constraint defined in Definition \ref{dfn:s} is a special class of separable constraint which discards the constraint set $\rowdec{\s}$. 
Similarly, the column/row-wise separable SLC defined in Definition \ref{dfn:s} and \ref{dfn:s_row} are special cases of partially separable SLC. %constraint which discards the constraint set $\rowdec{\s}$. 

\begin{remark} \label{rmk:lt}
Recall that the SLC set $\s$ in \eqref{eq:of_lop} is given by $\s = \Ell \cap \FT \cap \Sother$. The locality constraint $\Ell$ and the FIR constraint $\FT$ are partially separable with respect to arbitrary row-wise and column-wise partition. Therefore, the partial separability of the SLC $\s$ is determined by the partial separability of the set $\Sother$. If $\Sother$ is partially separable, we can express the original SLC $\s$ as an intersection of the sets $\rowdec{\s} = \Ell \cap \FT \cap \rowdec{\Sother}$ and $\coldec{\s} = \Ell \cap \FT \cap \coldec{\Sother}$, where $\rowdec{\Sother}$ is a row-wise separable component of $\Sother$ and $\coldec{\Sother}$ a column-wise separable component of $\Sother$.
Note that the locality constraint and the FIR constraint are included in both $\rowdec{\s}$ and $\coldec{\s}$. As will be shown later, this is the key point to allow the subroutines of the ADMM algorithm to be solved in a scalable way. % finite dimensional and
\end{remark}

%\begin{remark}
%From the definition, every directly decomposable localizability constraint is a decomposable localizability constraint, but not the opposite. 
%\end{remark}

%Consider the optimization problem
%\begin{subequations}
%\begin{align}
%\underset{\{R,M,N,L\}}{\text{minimize    }} & || \begin{bmatrix} R & \sigma_y N \\ \sigma_u M & \sigma_u \sigma_y L \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:h2_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:h2_1} \\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:h2_2} \\
%&  R, M, N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad L \in \mathcal{RH}_{\infty} \label{eq:h2_stable}\\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:h2_S}
%\end{align}
%\end{subequations}
%where $\sigma_u$ is the relative penalty between state deviation and control effort, $\sigma_y$ the relative magnitude of process disturbance and sensor disturbance. This corresponds to the case for some sparse $C_1, D_{21}, B_1, D_{21}$. Theoretically, the method described in this paper can generalize to arbitrary $C_1, D_{21}, B_1, D_{21}$, but it is effective only when those matrices are highly sparse.

%Assumptions (?)
Assume that the SLO and the SLC in \eqref{eq:of_lop} are both partially separable with respect to a row-wise partition $\{ \rowps_1, \dots, \rowps_{q}\}$ and a column-wise partition $\{ \colps_1, \dots, \colps_{p}\}$. In this case, we say that the SLS problem \eqref{eq:of_lop} is partially separable. 
%We can split the SLS problem \eqref{eq:of_lop} into a row-wise separable part and a column-wise separable part. 
Let $\ttf{\Psi}$ be a duplicate of the optimization variable $\ttf{\Phi}$. We define extended-real-value functionals $\rowdec{h}(\ttf{\Phi})$ and $\coldec{h}(\ttf{\Psi})$ by
\begin{eqnarray}
&& \rowdec{h}(\ttf{\Phi}) = \left\{ \begin{array}{ll}
\rowdec{g}(\ttf{\Phi}) & \textrm{if } \eqref{eq:of-3}, \ttf{\Phi} \in \rowdec{\s}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
&& \coldec{h}(\ttf{\Psi}) = \left\{ \begin{array}{ll}
\coldec{g}(\ttf{\Psi}) & \textrm{if } \eqref{eq:of-2}, \ttf{\Psi} \in \coldec{\s}\\
\infty & \textrm{otherwise.}
\end{array} \right. \label{eq:extended}
\end{eqnarray}
The SLS problem \eqref{eq:of_lop} can then be reformulated as
\begin{eqnarray}
\underset{\{ \ttf{\Phi}, \ttf{\Psi} \}}{\text{minimize    }} && \rowdec{h}(\ttf{\Phi}) + \coldec{h}(\ttf{\Psi}) \nonumber\\
\text{subject to }  && \ttf{\Phi} = \ttf{\Psi}. \label{eq:sub3}
\end{eqnarray}
Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}. Specifically, the ADMM algorithm for \eqref{eq:sub3} is given by
\begin{subequations}\label{eq:admm}
\begin{align}
\ttf{\Phi}^{k+1} &= \underset{\ttf{\Phi}}{\text{argmin }} \Big( \rowdec{h}(\ttf{\Phi}) + \frac{\rho}{2} || \ttf{\Phi} - \ttf{\Psi}^{k} + \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm1} \\
\ttf{\Psi}^{k+1} &= \underset{\ttf{\Psi}}{\text{argmin }} \Big( \coldec{h}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm2} \\
\ttf{\Lambda}^{k+1} &= \ttf{\Lambda}^{k} + \ttf{\Phi}^{k+1} - \ttf{\Psi}^{k+1} \label{eq:admm3}
\end{align}
\end{subequations}
where the square of the $\mathcal{H}_2$ norm is computed by \eqref{eq:h2_comp}. As the FIR constraint $\FT$ is imposed on $\ttf{\Phi}$ and $\ttf{\Psi}$ through the SLC sets $\rowdec{\s}$ and $\coldec{\s}$, subroutines \eqref{eq:admm1} and \eqref{eq:admm2} are both finite dimensional optimization problems.
%When the FIR constraint $\FT$ is imposed through 
%of a transfer matrix can be computed by the sum of the square of Frobenius norm of all its spectral components.

%The primary reason 
%The main advantage of using the ADMM algorithm to solve \eqref{eq:sub3} is 
Subroutines \eqref{eq:admm1} and \eqref{eq:admm2} can be further decomposed row-wisely and column-wisely, respectively. For instance, the optimization problem corresponding to subroutine \eqref{eq:admm2} is given by
\begin{subequations} \label{eq:admm_lop}
\begin{align} 
\underset{\ttf{\Psi}}{\text{minimize }} \quad & \coldec{g}(\ttf{\Psi}) + \frac{\rho}{2} || \ttf{\Psi} - \ttf{\Phi}^{k+1} - \ttf{\Lambda}^{k}||_{\mathcal{H}_2}^2 \label{eq:admmlop1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Psi} = J_B \label{eq:admmlop2} \\
& \ttf{\Psi} \in \coldec{\s}. \label{eq:admmlop3}
\end{align}
\end{subequations}
This problem has the same form as \eqref{eq:sf_lop2} -- the right-hand-side of \eqref{eq:admmlop2} does not affect the column-wise separability of the problem. 
The $\mathcal{H}_2$ norm regularizer in \eqref{eq:admmlop1} is column-wise separable with respect to arbitrary column-wise partition.
%, so the objective function in \eqref{eq:admmlop1} is column-wise decomposable. 
As the objective $\coldec{g}(\cdot)$ and the constraint $\coldec{\s}$ are column-wise separable with respect to a given column-wise partition, we can use the column-wise separation technique described in the previous section to decompose problem \eqref{eq:admm_lop} into parallel subproblems. Recall that we have $\coldec{\s} = \Ell \cap \FT \cap \coldec{\Sother}$. We can exploit the locality constraint and use the technique described in Section \ref{sec:CWSP} and Appendix \ref{sec:reduction} to further reduce the dimension of each subproblem from global scale to local scale. Overall, subroutine \eqref{eq:admm2} can be solved in a localized and scalable manner. Similarly, subroutine \eqref{eq:admm1} can also be solved via the row-wise separation. Equation \eqref{eq:admm3} can be computed element-wisely since it is a matrix addition. Therefore, \eqref{eq:admm1} - \eqref{eq:admm3} is a scalable algorithm to solve the localized SLS problem \eqref{eq:of_lop} by using row-wise and column-wise separation alternatively and iteratively.

%We prove that the ADMM algorithm \eqref{eq:admm1} - \eqref{eq:admm3} converges summarized in Appendix \ref{sec:ADMM}.

%We prove that the ADMM algorithm \eqref{eq:admm1} - \eqref{eq:admm3} converges to an optimal solution of \eqref{eq:of_lop} under certain technical conditions in Appendix \ref{sec:ADMM}.
We prove that the ADMM algorithm \eqref{eq:admm1} - \eqref{eq:admm3} converges to an optimal solution of \eqref{eq:of_lop} (or equivalently, \eqref{eq:sub3}) under the following assumptions. The details of the proof, as well as the stopping criteria of the algorithm, can be found in Appendix \ref{sec:ADMM}. %The details can be found in Appendix \ref{sec:ADMM}.
\begin{assumption}
Problem \eqref{eq:of_lop} has a feasible solution in the relative interior of the set $\s$. \label{as:1}
\end{assumption}
\begin{assumption} 
The functionals $\rowdec{g}(\cdot)$ and $\coldec{g}(\cdot)$ are closed, proper, and convex. \label{as:2}
\end{assumption}
\begin{assumption} 
The sets $\rowdec{\s}$ and $\coldec{\s}$ are closed and convex. \label{as:3}
\end{assumption}

%Note that $\rowdec{h}(\Phi)$ admits a block column-wise decomposition as both $\rowdec{g}(\Phi)$ and the localizability constraint $\mathcal{S}$ are both column-wise decomposable. As the $\mathcal{H}_2$ norm admits a column-wise decomposition for any partition, subproblem \eqref{eq:admm1} can be solved using the state feedback decomposition technique described in the previous subsection. When the localizability constraint $\mathcal{S}$ is highly sparse, subproblem \eqref{eq:admm1} can be solved in a localized and scalable way. 
%From the decomposability assumptions on the objective function and the localizability constraint, function $\rowdec{h}(\Phi)$ admits a block column-wise decomposition. 
%and function $\coldec{h}(\Psi)$ admits a block row-wise decomposition. 
%From the decomposability of the
%Subproblem \eqref{eq:admm1} reduces to be form of state feedback 
%can be solved in a localized way using LLQR with a column-wise decomposition on the objective function and the constraint. 

\subsection{Examples of Partially Separable Problems}
In this subsection, we give some examples of partially separable localized SLS problems in optimal control. All these problems can be solved using the ADMM algorithm \eqref{eq:admm} in a localized and scalable way. 

\subsubsection{Partially Separable Objectives}
We begin by considering some examples of partially separable SLO.
\begin{example} \label{ex:b1}
Consider the SLO of the distributed optimal control problem in \eqref{eq:trad_obj2}, with the norm given by either the square of the $\mathcal{H}_2$ norm or the element-wise $\ell_1$ norm defined in Example \ref{ex:l1}. Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} B_1^\top & D_{21}^\top \end{bmatrix} \Pi$ is block diagonal. Using a similar argument as in Example \ref{ex:perm}, we can find a column-wise partition to decompose the SLO in a column-wise manner. Likewise, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the SLO in a row-wise manner. In both cases, the SLO is column/row-wise separable and thus partially separable.
\end{example}
%\begin{example} \label{ex:c1}
%Similarly, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. We can find a row-wise partition to decompose the objective function in a row-wise manner. This objective function is directly decomposable and thus decomposable.
%\end{example}
\begin{example}
Consider the weighted actuator norm defined in \cite{MC_CDC14, 2015_Wang_Reg}, which is given by
\begin{equation}
|| \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} = \sum_{i=1}^{n_u} \mu_i || e_i^\top \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{H}_2} \label{eq:act_norm} 
\end{equation}
where $\mu$ is a diagonal matrix with $\mu_i$ being its $i$th diagonal entry, and $e_i$ is a unit vector with $1$ on its $i$th entry and $0$ elsewhere. When $\mu$ is an identity matrix, the actuator norm \eqref{eq:act_norm} is equivalent to the $\ell_1 / \ell_2$ norm, or the group lasso \cite{2006_grouplasso} in the statistical learning literature. This norm acts as a regularizer to make the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ row-wise sparse, i.e., have many zero rows. Recall from Theorem \ref{thm:1} that the controller achieving the desired system response can be implemented by \eqref{eq:implementation}. If the $i$th row of the transfer matrix $\begin{bmatrix} \tf M & \tf L \end{bmatrix}$ is a zero row, then the $i$th component of the control action $u_i$ is always equal to zero. This means that we can remove the control action $u_i$ without changing the closed loop response. It is clear that the actuator norm defined in \eqref{eq:act_norm} is row-wise separable with respect to arbitrary row-wise partition. This still holds true when the actuator norm is defined by the $\ell_1 / \ell_\infty$ norm. Similarly, consider the weighted sensor norm given by
\begin{equation}
|| \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} = \sum_{i=1}^{n_y} \lambda_i || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} e_i ||_{\mathcal{H}_2} \label{eq:sen_norm} 
\end{equation}
where $\lambda$ is a diagonal matrix with $\lambda_i$ being its $i$th diagonal entry. The sensor norm in \eqref{eq:sen_norm} is a regularizer to make the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ column-wise sparse. Using the controller implementation \eqref{eq:implementation}, the sensor norm can be treated as a regularizer on the measurement $y$. For instance, if the $i$th column of the transfer matrix $\begin{bmatrix} \tf N^\top & \tf L^\top \end{bmatrix}^\top$ is identical to zero, then we can ignore the measurement $y_i$ without changing the closed loop response. The sensor norm defined in \eqref{eq:act_norm} is column-wise separable with respect to any column-wise partition.
\end{example}
\begin{example}
From Definition \ref{dfn:do}, it is straightforward to see that the class of partially separable SLOs with the same partition are closed under summation.
%the sum of multiple partially separable objective functions with the same partition is still separable with respect to the given partition. 
Therefore, we can combine all the partially separable SLOs described above, and the resulting SLO is still partially separable. For instance, consider the SLO given by
%
\begin{eqnarray}
g(\tf R,\tf M,\tf N,\tf L) &=& || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
&&+ || \mu \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} \lambda ||_{\mathcal{Y}} \label{eq:h2_sar}
\end{eqnarray}
where $\mu$ and $\lambda$ are the relative penalty between the $\mathcal{H}_2$ performance, actuator and sensor regularizer, respectively. 
If there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal, then the SLO \eqref{eq:h2_sar} is partially separable. 
%In this case, 
Specifically, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise separable component, and the sensor regularizer belongs to the column-wise separable component.
\end{example}

\subsubsection{Partially Separable Constraints}
We consider some examples of partially separable SLCs beside the locality constraint $\Ell$ and the FIR constraint $\FT$ described in Remark \ref{rmk:lt}.
%, some other examples of decomposable localizability constraints are given as follows.
\begin{example}
Consider the $\mathcal{L}_1$ norm \cite{Munther_L1} of a FIR transfer matrix $\tf G \in \FT$, which is given by
\begin{equation}
|| \tf G ||_{\mathcal{L}_1} = \underset{i}{\text{max}} \quad \sum_{j} \sum_{t=0}^T | g_{ij}[t] |.\label{eq:L1_defn}
\end{equation}
The $\mathcal{L}_1$ norm is the induced norm of a $\ell_\infty$ input signal to a $\ell_\infty$ output signal. Suppose that the $\ell_\infty$ norm of the disturbance $w$ in \eqref{eq:desired} is bounded, and we want to bound the $\ell_\infty$ norm of the state vector $x$ and the control action $u$. We can impose the constraint
\begin{equation}
|| \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix}||_{\mathcal{L}_1} \leq \gamma \label{eq:L1_cons}
\end{equation}
in the optimization problem \eqref{eq:of_lop} for some $\gamma$. The solution of \eqref{eq:L1_cons} forms a convex set because it is a sublevel set of a convex function. Therefore, \eqref{eq:L1_cons} is a convex SLC. From the definition \eqref{eq:L1_defn}, the SLC \eqref{eq:L1_cons} is row-wise separable with respect to any row-wise partition. 
\end{example}
\begin{example}
From Definition \ref{dfn:ss}, the class of partially separable SLCs with the same partition are closed under intersection.
%the intersection of multiple separable constraints with the same partition is separable with respect to the given partition. 
Therefore, we can combine all the partially separable SLCs described above, and the resulting SLC is still partially separable. 
%all the decomposable constraints can be incorporated into the optimization problem in a sequential manner without breaking the decomposability of the problem. 
For instance, the combination of the locality constraint $\Ell$, the FIR constraint $\FT$, and the $\mathcal{L}_1$ constraint in \eqref{eq:L1_cons} is partially separable.
This property is extremely useful because it provides a unified framework to deal with all kinds of partially separable constraints at once.
\end{example}
%The ADMM algorithm described in the previous subsection can be applied to any problem with a decomposable objective function and a decomposable localizability constraint.
%Here we consider a localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization. We explain how to solve this problem in a localized and scalable manner using the ADMM algorithm.
%\begin{example}
%A localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem with sensor and actuator regularization is formulated by
%\begin{subequations} \label{eq:h2l1}
%\begin{align} 
%\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & ||\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
%& + \mu || \begin{bmatrix} \tf M & \tf L \end{bmatrix} ||_{\mathcal{U}} + \lambda || \begin{bmatrix} \tf N \\ \tf L \end{bmatrix} ||_{\mathcal{Y}} \label{eq:h2l1-1}\\
%\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2l1-2} \\
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \Ell \cap \FT \label{eq:h2l1-3} \\
%& || \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} ||_{\mathcal{L}_1} \leq \gamma \label{eq:h2l1-4}.
%\end{align}
%\end{subequations}
%Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal. In this case, problem \eqref{eq:h2l1} is decomposable. Specifically, the $\mathcal{H}_2$ norm and the actuator regularizer belong to the row-wise decomposable component of the objective function, while the sensor regularizer belongs to the column-wise decomposable component of the objective. The row-wise decomposable constraint includes the affine constraint \eqref{eq:main_2} and the $\mathcal{L}_1$ constraint \eqref{eq:h2l1-4}, and the column-wise decomposable constraint includes the affine constraint \eqref{eq:main_1}. Constraints \eqref{eq:main_stable} and \eqref{eq:h2l1-3} are included in both the row-wise component and the column-wise component to facilitate the scalability of solving \eqref{eq:admm1} and \eqref{eq:admm2}. 
%\end{example}

%Without the constraint \eqref{eq:h2_2}, this optimization problem admits a column-wise decomposition as the LLQR problem. Similarly, without the constraint \eqref{eq:h2_1}, the optimization problem admits a row-wise decomposition. Specifically, we solve
%\begin{eqnarray}
%\begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_1}, \eqref{eq:h2_stable}, \eqref{eq:h2_S} \label{eq:sub1}
%\end{eqnarray}
%and
%\begin{eqnarray}
%\begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_2}, \eqref{eq:h2_stable}, \eqref{eq:h2_S}. \label{eq:sub2}
%\end{eqnarray}
%When the constraint \eqref{eq:h2_S} is a locality constraint, we can utilize the technique of LLQR to solve both \eqref{eq:sub1} and \eqref{eq:sub2} in a completely localized and parallel way.
%
%The optimal solution in \eqref{eq:sub1} and \eqref{eq:sub2} may not be the same. Therefore, we need to solve an extra optimization problem as
%\begin{eqnarray}
%\underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix}. \label{eq:sub3}
%\end{eqnarray}
%Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}.

\subsubsection{Partially Separable Problems}
With some examples of partially separable SLOs and SLCs, we now consider two partially separable SLS problems: (i) localized $\mathcal{H}_2$ optimal control problem with sensor actuator regularization, and (ii) localized mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control. These two problems are used in Section \ref{sec:simu} as case study examples.

\begin{example}
The localized $\mathcal{H}_2$ optimal control with sensor actuator regularization is formulated by 
\begin{subequations} \label{eq:h2SA}
\begin{align} 
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & \eqref{eq:h2_sar} \label{eq:h2SA-1} \\
\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}  \label{eq:h2SA-2} \\
& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \C \cap \Ell \cap \FT. \label{eq:h2SA-3}
\end{align}
\end{subequations}
where $\C$ encodes the communication delay constraint. If there exists a permutation matrix $\Pi$ such that the matrix $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Pi$ is block diagonal, then \eqref{eq:h2SA} is partially separable. 
\end{example}
\begin{remark}
When the penalty of the sensor and actuator norms are zero, problem \eqref{eq:h2SA} reduces to a localized $\mathcal{H}_2$ optimal control problem. We also call this specialized problem as localized linear quadratic Gaussian (LLQG) \cite{2015_Wang_H2}.
\end{remark}


Problem \eqref{eq:h2SA} can be used to co-design a localized optimal controller and its sensing actuation interface by choosing the relative weight among the $\mathcal{H}_2$ performance, actuator and sensor norm. The weights $\mu_i$ and $\lambda_i$ in the regularizers \eqref{eq:act_norm} and \eqref{eq:sen_norm} can be properly chosen to further enhance row/column-wise sparsity. For instance, we can use the reweighted $\ell_1$ algorithm proposed in \cite{Reweighted} to iteratively set the weights and solve \eqref{eq:h2SA} multiple times. Let $\mu_i^{(0)} = \mu_0$ for $i = 1, \dots, n_u$ and $\lambda_i^{(0)} = \lambda_0$ for $i = 1, \dots, n_y$.
Let $(\tf R^{(k)}, \tf M^{(k)}, \tf N^{(k)}, \tf L^{(k)})$ be the optimal solution of \eqref{eq:h2SA} when the weights are given by $\{ \mu_i^{(k)} \}_{i=1}^{n_u}$ and $\{ \lambda_i^{(k)} \}_{i=1}^{n_y}$. We update the weights at iteration $(k+1)$ by
\begin{subequations}
\begin{align}
\mu_i^{(k+1)} &= ( \, || e_i^\top \begin{bmatrix} \tf M^{(k)} & \tf L^{(k)} \end{bmatrix} ||_{\mathcal{H}_2} + \epsilon )^{-1} \nonumber\\
\lambda_i^{(k+1)} &= ( \, || \begin{bmatrix} \tf N^{(k)} \\ \tf L^{(k)} \end{bmatrix} e_i ||_{\mathcal{H}_2} + \epsilon )^{-1} 
\end{align}
\end{subequations}
for some small $\epsilon$. It is shown in \cite{Reweighted} that this reweighted scheme usually results in sparser solution.

Next, we consider the localized mixed $\mathcal{H}_2/\mathcal{L}_1$ optimal control given as follows.
\begin{example}
The localized mixed $\mathcal{H}_2/\mathcal{L}_1$ optimal control problem is given by 
\begin{subequations} \label{eq:h2l1}
\begin{align} 
\underset{\{\tf R, \tf M, \tf N, \tf L\}}{\text{minimize }} \quad & || \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix}||_{\mathcal{H}_2}^2 \label{eq:h2l1-1} \\
\text{subject to } \quad & \eqref{eq:main_1} - \eqref{eq:main_stable}, \eqref{eq:L1_cons}, \eqref{eq:h2SA-3} \label{eq:h2l1-2}
\end{align}
\end{subequations}
which is partially separable.
\end{example}
%& \begin{bmatrix} \tf R & \tf N \\ \tf M & \tf L \end{bmatrix} \in \C \cap \Ell \cap \FT, \label{eq:h2l1-3}

The localized mixed $\mathcal{H}_2/\mathcal{L}_1$ optimal control problem can be used to design the tradeoff between average-case performance and worst-case performance. Specifically, the $\mathcal{H}_2$ objective in \eqref{eq:h2l1} is the expected value of the energy of state and control for AWGNs, which measures the average-case performance of the controller. The $\mathcal{L}_1$ constraint in \eqref{eq:L1_cons} is the $\ell_\infty$-$\ell_\infty$ induced norm, which measures the worst-case state and control deviation for $\ell_\infty$ bounded disturbance.

%If we choose the $\mathcal{H}_2$ norm as the objective function and \eqref{eq:L1_cons} as the constraint, then the problem becomes a mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem. As both the objective and the constraint are decomposable, the mixed $\mathcal{H}_2 / \mathcal{L}_1$ optimal control problem is decomposable. %it is a directly decomposable constraint and thus a decomposable constraint. 

\subsection{Analytic Solution and Acceleration}
Suppose that the Assumptions \ref{as:1} - \ref{as:3} in Section \ref{sec:ps} hold. The ADMM algorithm presented in \eqref{eq:admm} is a special case of the proximal algorithm \cite{proximal, proximalBoyd, BoydADMM}. For certain type of objective functionals $\rowdec{h}(\cdot)$ and $\coldec{h}(\cdot)$, the proximal operators can be evaluated analytically (see Ch. 6 of \cite{proximalBoyd}). In this situation, we only need to evaluate the proximal operators \emph{once}, and iterate \eqref{eq:admm1} and \eqref{eq:admm2} in closed form. This improves the overall computation time significantly. 
We explain how to express the solutions of \eqref{eq:admm1} and \eqref{eq:admm2} using proximal operators in detail in Appendix \ref{sec:appendix}. Here we list a few examples that the proximal operators can be evaluated analytically. 

%\input{Proximal}
%For certain type of objective functions, the proximal operator in \eqref{eq:proximal} can be evaluated analytically (see Ch. 6 of \cite{proximalBoyd}). Here we list a few examples.
\begin{example} \label{ex:analytic1}
%the objective functions $\rowdec{g}(\cdot)$ and $\coldec{g}(\cdot)$ are convex quadratic. The constraint sets $\rowdec{\s}$ and $\coldec{\s}$ are the 
Consider the LLQG problem proposed in \cite{2015_Wang_H2}.
%, which is a special case of \eqref{eq:h2SA} with zero penalty on sensor and actuator norms.
% The objective function is given in \eqref{eq:trad_obj2}, and the constraint is the intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the communication delay subspace constraint $\C$. 
When the global optimization problem is decomposed into parallel subproblems, each subproblem is a convex quadratic program restricted on an affine set. In this case, the proximal operator is an affine function \cite{2015_Wang_H2, proximalBoyd, BoydADMM}. We only need to calculate this affine function once. The iteration in \eqref{eq:admm1} - \eqref{eq:admm3} can then be carried out using multiple matrix multiplications in the reduced dimension, which significantly improves the overall computation time.
\end{example}
\begin{example} \label{ex:analytic2}
Consider the LLQR problem with actuator regularization \cite{2015_Wang_Reg}, which is the state feedback version of \eqref{eq:h2SA}. The column-wise separable part is identical to the LLQG example, so the update \eqref{eq:admm2} can be computed using matrix multiplication. Suppose that we use \eqref{eq:act_norm} as the actuator norm. 
We showed in \cite{2015_Wang_Reg} that the row-wise separable part can be simplified into multiple unconstrained optimization problems, with proximal operators given by vectorial soft-thresholding \cite{proximalBoyd}.
This offers an efficient way to update \eqref{eq:admm1}.
%The row-wise decomposable part can be simplified into multiple unconstrained optimization problems with objective given by the sum of a $\ell_2$ norm and a square of the $\ell_2$ norm
%$g_{v(j)}(\cdot)$ being the $\ell_2$ norm of the variables. 
%The proximal operator of this problem is a vectorial soft-thresholding \cite{2015_Wang_Reg, proximalBoyd}, which can be calculated in an efficient way. 
%If we use the $\ell_1 / \ell_\infty$ norm as the actuator norm, efficient algorithm to evaluate the proximal operator also exists \cite{proximalBoyd}.
\end{example}

Beside ADMM, there exists other distributed algorithms that can be used to solve the optimization problem \eqref{eq:sub3} in a localized and scalable way. For instance, if either $\rowdec{g}(\cdot)$ or $\coldec{g}(\cdot)$ is strongly convex, we can use the alternating minimization algorithm (AMA) \cite{AMA} to simplify the ADMM algorithm. Some other alternatives include the over-relax ADMM \cite{BoydADMM} and the accelerated version of ADMM and AMA proposed in \cite{FastADMM}.

%\subsection{Localized Synthesis and Re-synthesis}


==> Parameter_v1.tex <==
In this section, we show that the constraints \eqref{eq:main_1} - \eqref{eq:main_stable} is equivalent to the constraint ``$K$ stabilizes $P$" in \eqref{eq:trad}. We then give a parameterization of all stabilizing controller based on the closed loop transfer matrices in \eqref{eq:main_1} - \eqref{eq:main_stable}. The state feedback case is discussed first as it gives a simple, intuitive idea on how to construct a controller by closed loop transfer matrices. The discussion then extends to output feedback, which is the main focus of this paper.

%\subsection{Preliminaries}
%Some conventional definitions and lemmas are presented here.
%\begin{definition}
%A square matrix $A$ is said to be a \emph{stable matrix} if all its eigenvalues are contained in the unit disc.
%\end{definition}
%
%Note that $A$ is a stable matrix if and only if $(zI-A)^{-1}$ is a stable transfer function. 
%\begin{definition}
%The pair $(A,B_2)$ is said to be \emph{stabilizable} if there exists a matrix $F$ such that $A+B_2 F$ is a stable matrix. The pair $(A,C_2)$ is said to be \emph{detectable} if there exists a matrix $H$ such that $A+H C_2$ is a stable matrix.
%\end{definition}
%
%The following test on stabilizability and detectability is known as the PBH test.
%\begin{lemma}
%The pair $(A,B_2)$ is stabilizable if and only if the matrix $[zI-A \quad B_2]$ has full row rank for all $|z| \geq 1$. The pair $(A,C_2)$ is detectable if and only if the matrix $[zI-A^\top \quad C_2^\top]^\top$ has full column rank for all $|z| \geq 1$.
%\end{lemma}
%\begin{proof}
%See, for example, \cite{Zhou1996robust} or \cite{Dullerud_Paganini}.
%\end{proof}
%
%Traditionally, the notion of ``$K$ stabilizes $P$" can be checked by the input-output stability of the following configuration
%
%Internal stability for state space

\subsection{State Feedback}
Consider a state feedback problem
\begin{equation}
P = \left[ \begin{array}{c|cc} A & I & B_2 \\ \hline C_1 & \mathbf{0} & D_{12} \\ I & \mathbf{0} & \mathbf{0} \end{array} \right]. \label{eq:sfplant}
\end{equation}
The z-transform of the state dynamics is given by
\begin{equation}
(zI - A) x = B_2 u + w. \label{eq:zsfb}
\end{equation}
Define $R$ the closed loop transfer matrix from $w$ to $x$, $M$ the closed loop transfer matrix from $w$ to $u$. Equation \eqref{eq:zsfb} can be written as
\begin{equation}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I. \label{eq:rm}
\end{equation}
From \eqref{eq:zsfb} and causality, $R$ and $M$ must be strictly proper. Intuitively, the state feedback system \eqref{eq:zsfb}, or the pair $(A, B_2)$, is stabilizable if and only if we can find a stable solution $R, M \in \frac{1}{z} \mathcal{RH}_\infty$ in \eqref{eq:rm}. This idea is formally stated in the following lemma.
\begin{lemma}
The pair $(A, B_2)$ is stabilizable if and only if the following equations are feasible.
\begin{subequations}
\begin{align}
& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \label{eq:state_fb1}\\
& R, M \in \frac{1}{z} \mathcal{RH}_\infty \label{eq:state_fb2}
\end{align}
\end{subequations} \label{lemma:1}
\end{lemma}
\begin{proof}
By definition of stabilizability, there exists a matrix $F$ such that $A+B_2 F$ is a stable matrix. Using the state feedback control law $u = F x$, the closed loop transfer matrices are given by
\begin{equation}
\begin{bmatrix} R \\ M \end{bmatrix} = \left[ \begin{array}{c|c} A+B_2 F & I \\ \hline I & \mathbf{0} \\ F & \mathbf{0} \end{array} \right]. \label{eq:sfrm}
\end{equation}
Clearly, \eqref{eq:sfrm} is a solution satisfying \eqref{eq:state_fb1} - \eqref{eq:state_fb2}. On the other hand, \eqref{eq:state_fb2} implies that $R(z)$ and $M(z)$ do not have poles in $| z | \geq 1$.
%if there exists a solution $(R,M)$ in \eqref{eq:state_fb1} - \eqref{eq:state_fb2}, then $R(z)$ and $M(z)$ do not have poles in $| z | \geq 1$. 
With \eqref{eq:state_fb1}, we conclude that $\begin{bmatrix} zI - A & -B_2 \end{bmatrix}$ must has full row rank for all $| z | \geq 1$ as it is right invertible. This is equivalent saying that $(A, B_2)$ is stabilizable from the well-known PBH test \cite{Dullerud_Paganini}.
\end{proof}

The implication of Lemma \ref{lemma:1} is that \eqref{eq:state_fb1} - \eqref{eq:state_fb2} gives an alternative definition of state feedback stabilizability of a system. We show in the next theorem that the solution of \eqref{eq:state_fb1} - \eqref{eq:state_fb2} actually parameterize \emph{all} achievable closed loop response. Before that, we first show how to construct a feedback controller for any solution of \eqref{eq:state_fb1} - \eqref{eq:state_fb2}.

Given a state feedback controller $u = Kx$, it is straightforward to derive the relation $M = K R$. Instead of implementing the controller by $K$, we implement the controller by $R$ and $M$ directly. As will be shown in the next section, this is the key point to make the implementation constraint convex to the distributed optimal control problem. 
%Specifically, imposing a sparsity constraint on $R$ and $M$ is always convex, but a sparsity constraint on $K$ is rarely convex. 
Assume that the the closed loop transfer matrices $R$ and $M$ are finite impulse response (FIR) with length $T$. In \cite{2014_Wang_CDC}, we proposed a model predictive control (MPC) like controller implementation given by
\begin{subequations}
\begin{align}
w_e [k] &= x[k] - x_r [k] \label{eq:mpc1} \\
u[k] &= \sum_{\tau = 0}^{T-1} M[\tau+1] w_e [k-\tau] \label{eq:mpc2}\\
x_r [k+1] &= \sum_{\tau = 0}^{T-2} R[\tau+2] w_e [k-\tau]. \label{eq:mpc3}
\end{align}
\end{subequations}
In the above equations, the estimated disturbance $w_e$ is computed by the difference between state measurement $x$ and reference trajectory $x_r$, while the reference trajectory and the control action can be computed by the estimated disturbance. Routine calculation shows that the implementation \eqref{eq:mpc1} - \eqref{eq:mpc3} achieves the desired closed loop response $(R,M)$.

In this paper, we further show that implementation \eqref{eq:mpc1} - \eqref{eq:mpc3} internally stabilizes the plant regardless the stability of the open loop plant $A$, and all stabilizing linear state feedback controller can be implemented in this way. Consider the controller architecture given in Figure \ref{fig:sf}. We define $\tilde{R} = I - zR$ and $\tilde{M} = zM$. From \eqref{eq:rm}, we have $\tilde{R} = I - zR = -A R - B_2 M$. As $R, M \in \frac{1}{z} \mathcal{RH}_{\infty}$, we have $\tilde{R} \in \frac{1}{z} \mathcal{RH}_{\infty}$ and $\tilde{M} \in \mathcal{RH}_{\infty}$. Therefore, the configuration in Figure \ref{fig:sf} is well-posed. Note that the controller can be implemented by the stable filters $(\tilde{R},\tilde{M})$ directly without computing its state space form. Similar to the standard material \cite{Zhou1996robust, Dullerud_Paganini}, Figure \ref{fig:sf} is said to be \emph{internally stable} if all the internal variables go to zero from all initial conditions in the absence of external disturbance, i.e. $\delta_x, \delta_y, \delta_u = 0$. It can readily show that it suffices to check the stability of the nine closed loop transfer matrices from $(\delta_x, \delta_y, \delta_u)$ to $(x, u, w_e)$. The configuration in Figure \ref{fig:sf} is internally stable if and only if all the nine transfer matrices are stable.

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.45\textwidth]{./figure/SF.pdf}
      \caption{The proposed state feedback controller structure, with $\tilde{R} = I - zR$ and $\tilde{M} = zM$.}
      \label{fig:sf}
\end{figure}

From Figure \ref{fig:sf}, as $\tilde{R}$ is strictly proper, $(I - \tilde{R})$ is invertible and we have $K = \tilde{M} (I - \tilde{R})^{-1}$, or $K = (zM)(zR)^{-1}$. By an abuse of notation, we sometimes simply write $K = M R^{-1}$, with $R^{-1}$ a short hand of $z (zR)^{-1}$.\footnote{Note that as $R$ is strictly proper, $R^{-1}$ is not proper. However, $M R^{-1}$ is always proper.} The next theorem states that $K = M R^{-1}$ is a parameterization of all stabilizing controllers, and it indeed achieves the desired closed loop response $(R,M)$.

\begin{theorem}
The following are true:
\begin{enumerate}[i]
  \item The solution of \eqref{eq:state_fb1} - \eqref{eq:state_fb2} parameterizes all closed loop map from $\delta_x$ to $(x,u)$ achieved by a linear stabilizing state feedback controller. 
  \item A parameterization of all state feedback stabilizing controller is given by $K = M R^{-1}$, or equivalently, the architecture in Figure \ref{fig:sf}, for all $(R,M)$ satisfying \eqref{eq:state_fb1} - \eqref{eq:state_fb2}.
  \item The controller implementation in Figure \ref{fig:sf} internally stabilizes the plant, and achieves the desired closed loop map from $\delta_x$ to $(x,u)$ in the absence of perturbation $\delta_y$ and $\delta_u$.
  \end{enumerate} \label{thm:sf}
\end{theorem}
\begin{proof}
Given any stabilizing controller $u = Kx$ in state space form
\begin{equation}
K = \left[ \begin{array}{c|c} A_k & B_k \\ \hline C_k & D_k \end{array} \right], \nonumber
\end{equation}
the closed loop transfer matrices is given by
\begin{equation}
\begin{bmatrix} R \\ M \end{bmatrix} = \left[ \begin{array}{cc | c} A + B_2 D_k C_2 & B_2 C_k & I \\ B_k C_2 & A_k & \mathbf{0} \\ \hline I & \mathbf{0} & \mathbf{0} \\ D_k C_2 & C_k & \mathbf{0} \end{array} \right], \label{eq:ss_p1}
\end{equation}
which is a solution to \eqref{eq:state_fb1} - \eqref{eq:state_fb2}. For any solution $(R,M)$ of \eqref{eq:state_fb1} - \eqref{eq:state_fb2}, construct a controller by $K = M R^{-1}$, or equivalently, by Figure \ref{fig:sf}. After some calculation, the closed loop transfer matrices from $(\delta_x, \delta_y, \delta_u)$ to $(x, u, w_e)$ are shown to be
\begin{equation}
\begin{bmatrix} x \\ u \\ w_e \end{bmatrix} = \begin{bmatrix} R & -\tilde{R} - RA & R B_2 \\ M & \tilde{M} - MA & I+MB_2 \\ \frac{1}{z}I & I-\frac{1}{z}A & \frac{1}{z}B_2 \end{bmatrix} \begin{bmatrix} \delta_x \\ \delta_y \\ \delta_u \end{bmatrix}. \label{eq:sf_cl}
\end{equation}
As all nine transfer matrices in \eqref{eq:sf_cl} are stable, the implementation in Figure \ref{fig:sf} is internally stable. Furthermore, the desired closed loop response from $\delta_x$ to $(x,u)$ is achieved. Therefore, for any solution to \eqref{eq:state_fb1} - \eqref{eq:state_fb2}, we can achieve the desired closed loop response by a stabilizing controller $K = M R^{-1}$. This suggests that all the three statements in this theorem are true.
\end{proof}

The analysis in this subsection can be extended to state estimation problem readily. For example, the following corollary gives an alternative definition of detectability of $(A,C_2)$.
\begin{corollary}
The pair $(A, C_2)$ is detectable if and only if the following equations are feasible.
\begin{subequations}
\begin{align}
& \begin{bmatrix} R & N \end{bmatrix} \begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = I \label{eq:state_est1}\\
& R, N \in \frac{1}{z} \mathcal{RH}_\infty. \label{eq:state_est2}
\end{align}
\end{subequations}
\end{corollary}
The parameterization of all detectable observer can also be given by $R^{-1} N$ for any solution in \eqref{eq:state_est1} - \eqref{eq:state_est2}.

%The controller implemented by Figure \ref{fig:sf} also achieves some robustness with respect to model uncertainty. This will be analyzed in the next section.

\subsection{Output Feedback}
One straightforward way to construct an output feedback controller is combining a state feedback controller with a state estimator. We do not use this approach due to the following reasons: (i) the observer-based output feedback controller does not necessary parameterize all stabilizing controllers, and (ii) separation principle does not hold in general when there are implementation constraints. Nevertheless, combining a localized state feedback controller with a localized state estimator can still be a good heuristic to construct a sub-optimal localized output feedback controller. The detail is under current research.

Assume that $D_{22} = 0$ first. Consider a discrete time distributed system described by
\begin{eqnarray}
x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber \\
y[k] &=& C_2 x[k] + \delta_y [k], \nonumber
\end{eqnarray}
with an output feedback dynamic controller $u = K y$. As in \cite{2014_Wang_Allerton}, we define the closed loop transfer matrices from perturbations $(\delta_x, \delta_y)$ to $(x,u)$ as
\begin{equation}
\begin{bmatrix} x \\ u \end{bmatrix} = \begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix} \delta_x \\ \delta_y \end{bmatrix}. 
\end{equation}
These closed loop transfer matrices can also be expressed as a function of controller $K$. Substituting $u = Ky$ into the system equations, we have
\begin{equation}
(zI - A - B_2 K C_2) x = \delta_x + B_2 K \delta_y. \nonumber
\end{equation}
As $K$ is proper, $(zI-A-B_2 K C_2)$ is always invertible -- even when $A$ is unstable. By routine calculation, it can be shown that
\begin{align}
R &= (zI - A - B_2 K C_2)^{-1} \nonumber\\
M &= K C_2 R \nonumber\\
N &= R B_2 K \nonumber\\
L  &= K + K C_2 R B_2 K. \label{eq:K_relation}
\end{align}

Similar to the state feedback case, we would like to: (i) derive some algebraic relations that the closed loop transfer matrices need to satisfy, (ii) implement the controller directly by those closed loop transfer matrices, and (iii) show that the solution to these algebraic equations parameterizes all closed loop map and controller. 

%Similar to the state feedback case, we would like to derive some algebraic relations that a closed loop transfer matrix need to satisfy. From \eqref{eq:ss_relation}, one can actually check that the following relations are satisfied. 
%\begin{eqnarray}
%\begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} &=& 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:matrix_1} \\
%\begin{bmatrix} R & N \\ M & L \end{bmatrix}
% \begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} &=& 
%\begin{bmatrix} I \\ 0 \end{bmatrix}. \label{eq:matrix_2}
%\end{eqnarray}
\begin{lemma}
The realization $(A, B_2, C_2)$ is stabilizable and detectable if and only if the following equations are feasible.
\begin{subequations}
\begin{align}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} R & N \\ M & L \end{bmatrix} &= 
\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:output_fb1}\\
\begin{bmatrix} R & N \\ M & L \end{bmatrix}
 \begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} &= 
\begin{bmatrix} I \\ 0 \end{bmatrix}. \label{eq:output_fb2} \\
R, M, N \in \frac{1}{z} \mathcal{RH}_\infty, \quad & L \in \mathcal{RH}_\infty \label{eq:output_fb3}
\end{align}
\end{subequations} \label{lemma:2}
\end{lemma}
\begin{proof}
For one direction, note that the feasibility of \eqref{eq:output_fb1} - \eqref{eq:output_fb3} implies the feasibility of \eqref{eq:state_fb1} - \eqref{eq:state_fb2} and \eqref{eq:state_est1} - \eqref{eq:state_est2}, respectively. Therefore, $(A, B_2, C_2)$ is stabilizable and detectable.
For another direction, given a feasible solution $(R_1, M_1)$ in \eqref{eq:state_fb1} - \eqref{eq:state_fb2} and a feasible solution $(R_2, N_2)$ in \eqref{eq:state_est1} - \eqref{eq:state_est2}, we can construct a feasible solution of \eqref{eq:output_fb1} - \eqref{eq:output_fb3} by
\begin{subequations}
\begin{align}
R &= R_1 + R_2 - R_1 (zI-A) R_2 \label{eq:rmnl1}\\
M &= M_1 - M_1 (zI-A) R_2 \label{eq:rmnl2}\\
N &= N_2 - R_1 (zI-A) N_2 \label{eq:rmnl3}\\
L &= -M_1 (zI-A) N_2, \label{eq:rmnl4}
\end{align}
\end{subequations}
which completes the proof.
%It is straightforward to check that \eqref{eq:rmnl1} - \eqref{eq:rmnl4} gives a feasible solution to \eqref{eq:output_fb1} - \eqref{eq:output_fb3}.
\end{proof}

%How do we derive this? What's the intuition?
%Why do we implement the controller by this?
We will show in the next theorem that the solution of \eqref{eq:output_fb1} - \eqref{eq:output_fb3} actually parameterize \emph{all} achievable closed loop response. Before that, we will first show how to construct a feedback controller for any solution in \eqref{eq:output_fb1} - \eqref{eq:output_fb3}.

From \eqref{eq:K_relation}, we notice that $K = L - M R^{-1} N$. This relation leads to the controller architecture given in Figure \ref{fig:of}, where $\tilde{R}^+ = z\tilde{R} = z (I - zR)$, $\tilde{M} = zM$, and $\tilde{N} = -zN$. Similar to the state feedback case, we can show that $\tilde{R}^{+}, \tilde{M}, \tilde{N} \in \RHinf$, so the architecture is well-posed. The controller implementation of Figure \ref{fig:of} is governed by the following equations
\begin{eqnarray}
z \beta &=& \tilde{R}^{+} \beta + \tilde{N} y \nonumber\\
u &=& \tilde{M} \beta + L y. \label{eq:ss_like}
\end{eqnarray}
Equations \eqref{eq:ss_like} can be considered as an extension of 
state space realization of $K$, which is given by
\begin{eqnarray}
z \xi &=& A_K \xi + B_K y \nonumber\\
u &=& C_K \xi + D_K y. \label{eq:sss}
\end{eqnarray}
Note that we extend the constant matrices $A_K, B_K, C_K, D_K$ in \eqref{eq:sss} into stable (or FIR) proper transfer functions $\tilde{R}^{+}, \tilde{M}, \tilde{N}, L$ in \eqref{eq:ss_like}. Although the implementation in \eqref{eq:ss_like} seems to be more complicated than \eqref{eq:sss}, the benefit is that \emph{any} convex constraints imposing on $\tilde{R}^{+}, \tilde{M}, \tilde{N}, L$ are convex with respect to the optimal control problem - which is crucial for large-scale problems. On the other hand, the sparsity constraint imposing on $A_K, B_K, C_K, D_K$, or $K$ are generally non-convex.

%Therefore, \eqref{eq:ss_like} can be considered as a generalization of state space realization by extending constant matrices $(A_K, B_K, C_K, D_K)$
%Note that the controller in Figure \ref{fig:of} is given by $K = \tilde{M} (zI - \tilde{R}^+)^{-1} \tilde{N} + L$, or equivalently, $K = L - M R^{-1} N$. 

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.48\textwidth]{./figure/Output.pdf}
      \caption{The proposed output feedback controller structure, with $\tilde{R}^+ = z\tilde{R} = z(I - zR)$, $\tilde{M} = zM$, and $\tilde{N} = -zN$.}
      \label{fig:of}
\end{figure}

The following theorem states that \eqref{eq:output_fb1} - \eqref{eq:output_fb3} along with the architecture in Figure \ref{fig:of} give a parameterization of all stabilizing controllers.

\begin{theorem}
The following are true:
\begin{enumerate}[i]
  \item The solution to \eqref{eq:output_fb1} - \eqref{eq:output_fb3} parameterizes all closed loop map from $(\delta_x, \delta_y)$ to $(x,u)$ achieved by a linear stabilizing output feedback controller. 
  \item A parameterization of all stabilizing controller is given by $K = L - M R^{-1} N$, or equivalently, the architecture in Figure \ref{fig:of}, for all $(R, M, N, L)$ satisfying \eqref{eq:output_fb1} - \eqref{eq:output_fb3}.
  \item The controller implementation in Figure \ref{fig:of} internally stabilizes the plant, and achieves the desired closed loop map from $(\delta_x, \delta_y)$ to $(x,u)$ in the absence of perturbation $\delta_u$ and $\delta_\beta$.
  \end{enumerate} \label{thm:of}
\end{theorem}
\begin{proof}
The proof is similar to the one for state feedback. For any stabilizing $K$ written in state space form, the closed loop transfer matrices by definition can be written as 
\begin{equation}
\begin{bmatrix} R & N \\ M & L \end{bmatrix} = \left[ \begin{array}{cc | cc} A + B_2 D_k C_2 & B_2 C_k & I & B_2 D_k \\ B_k C_2 & A_k & \mathbf{0} & B_k \\ \hline I & \mathbf{0} & \mathbf{0} & \mathbf{0} \\ D_k C_2 & C_k & \mathbf{0} & D_k \end{array} \right]. \label{eq:ss_relation}
\end{equation}
It can be checked that \eqref{eq:ss_relation} is a feasible solution to \eqref{eq:output_fb1} - \eqref{eq:output_fb3}. Given any feasible solution to \eqref{eq:output_fb1} - \eqref{eq:output_fb3}, construct a controller by $K = L - M R^{-1} N$, or equivalently, by Figure \ref{fig:of}. For internal stability, it suffices to check the stability of the closed loop transfer matrices from $(\delta_x, \delta_y, \delta_u, \delta_\beta)$ to $(x, u, y, \beta)$. Those transfer matrices are summarized in Table \ref{Table:1}. As all sixteen transfer matrices in Table \ref{Table:1} are stable, the implementation in Figure \ref{fig:of} is internally stable. Furthermore, the desired closed loop response from $(\delta_x, \delta_y)$ to $(x,u)$ is achieved. Therefore, for any solution to \eqref{eq:output_fb1} - \eqref{eq:output_fb2}, we can achieve the desired closed loop response by a stabilizing controller $K = L - M R^{-1} N$. This suggests that all the three claims in this theorem are true.
\end{proof}

\begin{table}[h!]
 \caption{Closed Loop Maps from Perturbations to Internal Variables}
 \label{Table:1}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c | c | c | c |}
    \hline 
    & $\delta_x$ & $\delta_y$ & $\delta_u$ & $\delta_\beta$ \\ \hline
    $x$ & $R$ & $N$ & $R B_2$ & $\frac{1}{z} N C_2$ \\ \hline
    $u$ & $M$ & $L$ & $I + M B_2$ & $\frac{1}{z} L C_2$ \\ \hline
    $y$ & $C_2 R$ & $I + C_2 N$ & $C_2 R B_2$ & $\frac{1}{z} C_2 N C_2$ \\ \hline
    $\beta$ & $-\frac{1}{z} B_2 M$ & $-\frac{1}{z} B_2 L$ & $-\frac{1}{z} B_2 M B_2$ & $\frac{1}{z} I - \frac{1}{z^2} (A + B_2 L C_2)$ \\ \hline
    \end{tabular}
\end{center}
\end{table}

%Compare to state space realization
When $\delta_u = 0$ and $\delta_\beta = 0$, we have $\beta = -\frac{1}{z}B_2 u$ from Table \ref{Table:1}. We can come up with a simpler implementation $u = Ly - M B_2 u$. As shown in the next example, this implementation is internally stable when the system is open loop stable.
\begin{example}
From the identity $K = (I+M B_2)^{-1} L$, we have $u = Ly - M B_2 u$. The corresponding controller structure is given by Figure \ref{fig:alt1}. The closed loop transfer matrices can be shown to be
\begin{equation}
\begin{bmatrix} x \\ u \end{bmatrix} = \begin{bmatrix} R & N & R B_2 & (zI-A)^{-1} B_2 \\ M & L & I+MB_2 & I \end{bmatrix} \begin{bmatrix} \delta_x \\ \delta_y \\ \delta_u \\ \delta_\beta \end{bmatrix}. \nonumber
\end{equation}
When $A$ is a stable matrix, this implementation is internally stable. Similarly, from the identity $K = L (I+C_2 N)^{-1}$, we have the controller structure given by Figure \ref{fig:alt2}. The closed loop transfer matrices are
\begin{equation}
\begin{bmatrix} x \\ u \\ \beta \end{bmatrix} = \begin{bmatrix} R & N & R B_2 \\ M & L & I+MB_2 \\ C_2 (zI-A)^{-1} & I & C_2 (zI-A)^{-1} B_2 \end{bmatrix} \begin{bmatrix} \delta_x \\ \delta_y \\ \delta_u \end{bmatrix}. \nonumber
\end{equation}
Clearly, it is internally stable when $A$ is a stable matrix.
\end{example}
\begin{figure}[ht!]
      \centering
      \subfigure[Structure 1]{%
      \includegraphics[width=0.35\textwidth]{./figure/MB2.pdf}
      \label{fig:alt1}}
      
      \subfigure[Structure 2]{%
      \includegraphics[width=0.35\textwidth]{./figure/C2N.pdf}
      \label{fig:alt2}}
      
      \caption{Alternative controller structures for stable systems.}
\end{figure}

Finally, consider the case $D_{22} \not = 0$. We can simply define a new measurement $y_n = y - D_{22} u$, which leads to the structure in Figure \ref{fig:pof}. Note that the closed loop transfer matrices from $\delta_u$ change to
\begin{equation}
\begin{bmatrix} x \\ u \\ y \\ \beta \end{bmatrix} = \begin{bmatrix} R B_2 + N D_{22} \\ I+MB_2+LD_{22} \\ C_2 R B_2 + D_{22} + C_2 N D_{22} \\ -\frac{1}{z}B_2 (M B_2 + L D_{22}) \end{bmatrix} \delta_u. \nonumber
\end{equation}
\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.48\textwidth]{./figure/D22.pdf}
      \caption{The proposed output feedback controller structure for $D_{22} \not = 0$.}
      \label{fig:pof}
\end{figure}

%Internal robustness with respect to computation error


==> Physical_v1.tex <==
\begin{example}
Consider Fig. \ref{fig:Chart105} with state feedback (full sensing). Assume that the disturbance $\delta{x_1}$ at node $1$ is only allowed to affect the state $x_1$ and $x_2$ at node $1$ and node $2$ in closed loop. In addition, we want to achieve this by activating the control action $u_i$ from node $i = 1, \dots, 4$. In this case, a localized region for disturbance $\delta{x_1}$ can be constructed by Region$(x_1) = \{x_1, x_2, x_3, x_4\}$ as shown in Fig. \ref{fig:region}. The boundary of this localized region is the set $\{x_3, x_4\}$. Intuitively, by keeping the boundary being zero for all time, there is no way for the disturbance to \emph{escape} from the localized region through state propagation. In addition, the effects of all control actions are limited within the localized region. We can then solve \eqref{eq:sf_lopd} using the local state, control, and plant model defined within this localized region. \label{ex:3}
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.4\textwidth]{figure/Region.pdf}
      \caption{Localized Region}
      \label{fig:region}
\end{figure}
%Clearly, we need to activate $u_1, u_2, u_3$ in order to localize the disturbance. In this case, we can define $Region(x_1) = \{x_1, x_2, x_3\}$, $Ext(x_1) = \{x_4, x_5\}$, and $Bound(x_1) = \{x_3\}$. Note that $x_3$ is contained within the localized region since $u_3$ is actuated.
\end{example}

1. Formally define "affected states" and "activated control actions"
Split $\mathcal{S}_j$ into $\mathcal{S}_{R_j}$ and $\mathcal{S}_{M_j}$. 
To be specific, the notion of affected states and activated control actions are formally defined as follows.
\begin{definition}
The affected states and the activated control actions, nonzero position of $\mathcal{S}_j$
\end{definition}
\begin{example}
Graph example, intuition
\end{example}

2. Define the localized region as a union set (need to define the partition of matrix A)
For a particular local disturbance $\delta{x_j}$ with the spatio-temporal constraint $\mathcal{S}_j$, we can construct a localized region by taking the union of the following three sets:
\begin{enumerate}[(i)]
\item the affected states %($\{x_1, x_2\}$ in Example \ref{ex:3})
\item the states that can be affected by the activated control actions directly %($\{x_1, \dots, x_4\}$ in Example \ref{ex:3})
\item the states that are connected from the affected states, i.e. the set $\{ x_i | A_{ik} \not = 0, x_k \in \text{ affected states}\}$. %($\{x_1, \dots, x_4\}$ in Example \ref{ex:3})
\end{enumerate}
We denote the localized region for $\delta{x_j}$ by Region($x_j$).
\begin{example}
Graph example, intuition
\end{example}

For a localized region, the external region Ext$(.)$ is defined as its complement set. The boundary of a localized region is defined as the set of states that connect the localized region toward the external region, i.e. $\{ x_k | A_{ik} \not = 0, x_k \in \text{Region}(x_j), x_i \in \text{Ext}(x_j)\}$. Intuitively, the affected states can be considered as the \emph{internal region} of the localized region, and the boundary is the set that \emph{separates} the internal region from the external region. As long as the boundary states are keeping zero for all time, and the control actions do not affect the external region (which is ensured by construction rule (ii)), the solution of \eqref{eq:llqr-s} can be analyzed completely within the localized region. Construction rule (iii) ensures that the boundary states are included in the localized region. 

Algebraically, we can also calculate the localized region for $\delta{x_{\Set p_j}}$ by checking the block row-wise sparsity pattern of
\begin{equation}
SL = \Sp{\begin{bmatrix} zI - A & -B_2 \end{bmatrix}} \Sp{\mathcal{S}_j}. \nonumber
\end{equation}
The localized region can be alternatively defined as
\begin{equation}
\text{Region}(x_j) = \{i | SL_i \not = 0 \}.
\end{equation}

With the notion of localized region, we define the local state vector $x_{\ell}$ the stacked vector of $x_i$ for all $x_i \in \text{Region}(x_j)$. The local control vector $u_{\ell}$ is stacked vector of all activated local control action $u_i$. The local plant model $(A_\ell,B_{2 \ell})$ associated with Region$(x_j)$ is defined by selecting submatrices of $(A,B_2)$ consisting of the columns and rows associated with $x_\ell$ and $u_\ell$.

Let $e_\ell$ be the initial condition of the source of disturbance. The local convex set constraint $\mathcal{S}_\ell$ can be defined by selecting the block rows of $\mathcal{S}_j$ associated with $[x_\ell^\top u_\ell^\top]^\top$, and column corresponding to $e_\ell$.

%The construction of the localized region
%For completeness, we prove the equivalence in Appendix (see LLQR paper)
%To be specific, we define the localized region for state $j$ by a column sparsity pattern as
%\begin{equation}
%\text{sp}(\begin{bmatrix} zI - A & -B_2 \end{bmatrix}) \Sp{\mathcal{S}_j}. \nonumber
%\end{equation}
%Region(j) = \begin{bmatrix} \Sp{\bar{A}} & \Sp{B_2} \end{bmatrix} \Sp{\mathcal{S}_j}, \nonumber
%By an abuse of notation, we also interpret Region$(j)$ as a set of the positions of its nonzero entries. 
%Recall that $\mathcal{V}$ is the set of all sub-systems. We use a set $Region(j) \subseteq \mathcal{V}$ to denote the localized region for sub-system $j$, and $External(j) = \mathcal{V} \setminus Region(j)$ to denote the external region for sub-system $j$. The boundary of $Region(j)$ is defined as follows.
%\begin{definition}
%The boundary of $Region(j)$ is the set of all sub-systems that connect $Region(j)$ toward $External(j)$ and is denoted by $Bound(j)$. Specifically, we have
%\begin{equation}
%Bound(j) = \{ k | A_{ik} \not = 0, k \in Region(j), i \in External(j) \}. \nonumber
%%\footnote{The $A_{ik}$ here denotes the $(i,k)$-entries of $A$.} \nonumber
%\end{equation}
%\end{definition}

The algebraic definition can be calculated in a localized way.

\begin{example}
Each LLQR sub-problem can be expressed in the form as
\begin{eqnarray}
\underset{\{x_\ell, u_\ell \}}{\text{minimize    }} && || C_\ell x_\ell + D_\ell u_\ell ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A_\ell & -B_\ell \end{bmatrix} \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} = e_\ell \nonumber \\
&& \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} \in \mathcal{S}_\ell \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-l}
\end{eqnarray}
\end{example}

==> Prelim_v1.tex <==
\subsection{Mathematical Notations and Preliminaries} 
This paper works on discrete time system for simplicity of presentation. Some notation and definition are taken from \cite{2014_Lamperski_H2_journal} and \cite{2014_Matni_Hinf}. As standard, let $\mathbb{D} = \{ z \in \mathbb{C} : | z | < 1 \}$ be the unit disc of complex numbers, and $\bar{\mathbb{D}}$ be its closure. A mapping $G : (\mathbb{C} \cup \{ \infty\}) \ \bar{\mathbb{D}} \to \mathbb{C}^{p \times q}$ is said to be in $\mathcal{H}_2$ if it admits the following expansion
\begin{equation}
G = \sum_{i=0}^{\infty} \frac{1}{z^i} G[i]
\end{equation}
where $G[i] \in \mathbb{C}^{p \times q}$ and $\sum_{i=0}^{\infty} \Trace(G[i]^* G[i]) < \infty$. The square of the $\mathcal{H}_2$ norm of a system $G \in \mathcal{H}_2$ is given by $ || G ||_{\mathcal{H}_2}^2 = \sum_{i=0}^{\infty} \Trace(G[i]^* G[i])$. A mapping $G : (\mathbb{C} \cup \{ \infty\}) \ \bar{\mathbb{D}} \to \mathbb{C}^{p \times q}$ is in $\mathcal{H}_\infty$ if it is analytic, bounded, and has a well-defined limit almost everywhere on the unit circle. We use the prefix $\mathcal{R}$ to a set $\mathcal{X}$ to indicate the restriction to real-rational members of $\mathcal{X}$. Therefore, $\mathcal{RH}_{\infty} = \mathcal{RH}_2$ denote the set of all real-rational stable proper transfer functions. We also denote $\mathcal{RH}_{\infty}^{sp}$ the set of all real-rational, stable, and strictly proper transfer functions.

In this paper, we use $G[i]$ to denote the $i$-th spectral component of a transfer function $G$. In time domain, the order set $\{G[i]\}_{i=0}^{\infty}$ describes the impulse response of the system. Unless specified otherwise, we use $G_j$ represents the $j$-th column of a matrix-valued transfer function $G$, and $G_{ij}$ the $(i,j)$-entry of $G$. For a vector $x$, $x_j$ represents the $j$-th component of $x$.

\subsection{Sparsity Patterns}
In order to describe the sparsity pattern of a matrix, we define the support operator $\Sp{\cdot}: \mathbb{R}^{m \times n} \to \{0,1\}^{m \times n}$, where $\{\Sp{A}\}_{ij}=1$ if and only if $A_{ij}\neq0$, and $\{\Sp{A}\}_{ij}=0$ otherwise. We use $\cup$ and $\cap$ to represent the OR and AND operator on binary variables, respectively. The addition of two binary matrices $\s_1,\s_2 \in \{0,1\}^{m \times n}$ is defined by the rule
\begin{equation}
(\s_1 + \s_2)_{ij} = (\s_1)_{ij} \cup (\s_2)_{ij}. \nonumber
\end{equation}
In addition, we write $\s_1\subseteq \s_2$ when $\s_1 + \s_2=\s_2$. The product $\s_1 = \s_2 \s_3$ with binary matrices of compatible dimension is defined by the rule
\begin{equation}
(\s_1)_{ij} = \underset{k}{\cup} \, [ \, (\s_2)_{ik} \cap (\s_3)_{kj} \, ]. \nonumber
\end{equation}
where the $\cup$ operator is taken over all possible $k$. For a square binary matrix $\mathcal{S}_0$, we define the power $\mathcal{S}_{0}^{i+1} := \mathcal{S}_{0}^i \mathcal{S}_{0}$ for all positive integer $i$, and $\mathcal{S}_{0}^0 = I$. 

The sparsity pattern of a transfer function $R$ is described by a constraint space $\mathcal{S}_R(z) := \sum_{i=0}^{\infty} \frac{1}{z^i} \s_{R}[i]$, where $\{\s_{R}[i]\}$ is an ordered set of binary matrices. We say that a transfer function $R$ is in $\mathcal{S}_R$ if and only if $\Sp{R[i]} \subseteq \s_{R}[i]$ for all $i$, which we denote by $R \in \mathcal{S}_R$. We also define $\bar{\mathcal{S}_R} := \sum_{i=0}^{\infty} \s_{R}[i]$, which is the union of sparsity patterns over all spectral components of the constraint space.

\subsection{System Model}
Consider a discrete time distributed system described by
\begin{eqnarray}
x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber \\
y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics}
\end{eqnarray}
where $x=(x_i)$, $u=(u_i)$, and $y=(y_i)$ are stacked vectors of local state, control, and measurement, respectively, and $\delta_x = (\delta_x)_i$ and $\delta_y = (\delta_y)_i$ are the stacked perturbations on each state and measurement, respectively. 


%\subsection{Notation}
%We adopt the following notation.
%
%Stable transfer function: $RH_{\infty}$
%\subsection{Notations} 
%$\mathcal{RH}_{\infty}$ denotes the set of all real-rational stable proper transfer functions. $z$ is the variable of the z-transform. 
%Throughout this paper, we use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system.
%\subsection{System Model}
%\input{model_v2}
%- Global system model v.s. Local model
%- Figure example for local model
%- Distance d
%Consider an interconnected network system described by a graph.
%- Graphical model: Assume that the network structure is given by a graph
%Without losing generality, we assume that each 
%\subsection{System Model}
%\input{model_v2}


%- Define subspace constraint on stable transfer function (generalized to arbitrary topology)
%- Algebra
%- Illustrate by figure (column / row)
%- (h, d, T) constraint for this paper, but can extend to any convex constraint
%\input{st_cons_v1}

%\subsection{Distributed Optimal Control}
%\input{DOC_v1}

%\subsection{}


==> Prelim_v2.tex <==
We begin by introducing the interconnected system model that we consider in this paper. We then discuss the limitations of the conventional distributed optimal control framework on large-scale system. This section ends with the main results in \cite{2015_PartI} and the problem statement for this paper.

%\subsection{Mathematical Notations} 
%This paper works on discrete time linear time invariant systems. Let $z$ be the variable of z-transform. As standard, let $\mathcal{H}_2$ be the set of square integrable functions on the unit circle with analytic extension in $| z | > 1$ in the complex plane, $\mathcal{H}_\infty$ the set of functions essentially bounded on the unit circle with analytic extension in $| z | > 1$. The prefix $\mathcal{R}$ to a set $\mathcal{X}$ indicates the restriction to real-rational members of $\mathcal{X}$. Therefore, $\mathcal{RH}_{\infty}$ denote the set of all real-rational stable proper transfer functions. We also denote $\frac{1}{z} \mathcal{RH}_{\infty}$ the set of all real-rational, stable, and strictly proper transfer functions. 
%We use $G[i]$ to denote the $i$-th spectral component of a transfer function $G$, i.e. $G(z) = \sum_{i=0}^{\infty} \frac{1}{z^i} G[i]$ for $| z | > 1$. Let $G[i]^\top$ be the conjugate transpose of $G[i]$. The $\mathcal{H}_2$ norm of a transfer function $G \in \mathcal{H}_2$ can be computed by the identity 
%\begin{equation}
%|| G ||_{\mathcal{H}_2}^2 = \sum_{i=0}^{\infty} \Trace(G[i]^\top G[i]). \label{eq:FIR}
%\end{equation}
%In time domain, the order set $\{G[i]\}_{i=0}^{\infty}$ describes the impulse response of the system. 
%Unless specified otherwise, we use $G_j$ to represent the $j$-th column of a matrix-valued transfer function $G$, and $G_{ij}$ the $(i,j)$-entry of $G$. For a vector $x$, $x_j$ represents the $j$-th component of $x$.

%\input{st_cons_simple}
%\input{st_cons_v1}
%Sparsity constraints

\subsection{Interconnected System Model}
Consider a network of linear systems connected through a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\mathcal{V} = \{1, \dots, n\}$ is the set of sub-systems, and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these sub-systems. Each sub-system $i$ is associated with a state vector $x_i$, control action $u_i$, and measurement $y_i$. We assume that the dynamics of each sub-system $i$ is given in the form of
\begin{eqnarray}
x_i[k+1] &=& A_{ii} x_i[k] + B_{ii} u_i[k] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[k] + \delta{x_i}[k]\nonumber\\
y_i[k] &=& C_{ii} x_i[k] + \delta{y_i}[k], \label{eq:interconnected}
\end{eqnarray}
where $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ are constant matrices with compatible dimensions, $\delta{x_i}$ and $\delta{y_i}$ the perturbation on state and measurement, respectively, and $\mathcal{N}_i$ the (upstream) neighboring set of $i$ defined by $\mathcal{N}_i = \{j | (j,i) \in \mathcal{E}\}$. The following is a simple example in the form of \eqref{eq:interconnected}, which is used to illustrate several ideas throughout this paper.
\begin{example}
Consider a network system with interconnected topology given by Fig. \ref{fig:Chart105}. Each sub-system $x_i$ is assumed to have two interacting scalar states $x_{i,1}, x_{i,2}$, a sensor on $x_{i,1}$, and an actuator on $x_{i,2}$. The interaction between two neighboring sub-systems is illustrated in Fig. \ref{fig:inter}, where $x_{i,1}$ can affect $x_{j,2}$ if $i$ and $j$ are neighbor. This model is inspired from the second-order dynamics in power network or mechanical system. Specifically, consider a second-order equation
\begin{equation}
m_i \ddot{\theta_i} + d_i \dot{\theta_i} = -\sum_{j \in \mathcal{N}_i} k_{ij} (\theta_i - \theta_j) + w_i + u_i \nonumber
\end{equation}
for some scalar $\theta_i$.
If we define the state vector by $x_i = [\theta_i \quad \dot{\theta_i}]^\top$, take the measurement on $\theta_i$, and use $e^{A \Delta t} \approx I + A \Delta t$ to discretize the plant, we get a discretized plant model with interaction graph described by Fig. \ref{fig:inter}.
\end{example}
\begin{figure}[t!]
      \centering
      \subfigure[Interconnected topology]{%
      \includegraphics[width=0.35\textwidth]{./figure/Topology.pdf}
      \label{fig:Chart105}}      
      \subfigure[Interaction between neighboring sub-systems]{%
      \includegraphics[width=0.35\textwidth]{./figure/Interaction.pdf}
      \label{fig:inter}}      
      \caption{Illustrative Example}
\end{figure}

More generally, we can construct the global plant model in the form
\begin{eqnarray}
x[k+1] &=& A x[k] + B_1 w[k] + B_2 u[k] \nonumber \\
\bar{z}[k] &=& C_1 x[k] + D_{11} w[k] + D_{12} u[k] \nonumber \\
y[k] &=& C_2 x[k] + D_{21} w[k] + D_{22} u[k] \label{eq:dynamics}
\end{eqnarray}
where $x=(x_i)$, $u=(u_i)$, $y=(y_i)$, $w=(w_i)$, and $\bar{z}=(\bar{z}_i)$ are stacked vectors of local state, control, measurement, external disturbance, and regulated output, respectively. Equation \eqref{eq:dynamics} can be written in state space form as
\begin{equation}
P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & D_{11} & D_{12} \\ C_2 & D_{21} & D_{22} \end{array} \right] = \begin{bmatrix} P_{11} & P_{12} \\ P_{21} & P_{22} \end{bmatrix} \nonumber
\end{equation}
where $P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. In this paper, we are particular interested in the case that the matrices in \eqref{eq:dynamics} are \emph{large} and \emph{sparse}. We aim to develop a method that exploits the sparsity structure of these matrices to enhance scalability of controller synthesis and implementation. 

Well-posed and internal stability on state space


%\subsection{Sparsity Pattern}
%\textbf{NOT SURE WHETHER TO INCLUDE THIS IN THIS SECTION}
%In order to describe the sparsity pattern of a matrix, we define the support operator $\Sp{\cdot}: \mathbb{R}^{m \times n} \to \{0,1\}^{m \times n}$, where $\{\Sp{A}\}_{ij}=1$ if and only if $A_{ij}\neq0$, and $\{\Sp{A}\}_{ij}=0$ otherwise. We use $\cup$ and $\cap$ to represent the OR and AND operator on binary variables, respectively. The addition of two binary matrices $\s_1,\s_2 \in \{0,1\}^{m \times n}$ is defined by the rule
%\begin{equation}
%(\s_1 + \s_2)_{ij} = (\s_1)_{ij} \cup (\s_2)_{ij}. \nonumber
%\end{equation}
%In addition, we write $\s_1\subseteq \s_2$ when $\s_1 + \s_2=\s_2$. The product $\s_1 = \s_2 \s_3$ with binary matrices of compatible dimension is defined by the rule
%\begin{equation}
%(\s_1)_{ij} = \underset{k}{\cup} \, [ \, (\s_2)_{ik} \cap (\s_3)_{kj} \, ]. \nonumber
%\end{equation}
%where the $\cup$ operator is taken over all possible $k$. 
%
%We can define a subspace constraint $\mathcal{S}_R(z) := \sum_{i=0}^{\infty} \frac{1}{z^i} \s_{R}[i]$ on a transfer function $R$ by an ordered set of binary matrices $\{\s_{R}[i]\}$. This is usually interpreted as a spatio-temporal constraint or an information sharing constraint on a transfer function. We say that a transfer function $R$ is in $\mathcal{S}_R$ if and only if $\Sp{R[i]} \subseteq \s_{R}[i]$ for all $i$, which we denote by $R \in \mathcal{S}_R$. 
%We also define $\bar{\mathcal{S}_R} := \sum_{i=0}^{\infty} \s_{R}[i]$, which is the union of sparsity patterns over all spectral components of the subspace constraint.

\subsection{Distributed Optimal Control Problem}
Assume a dynamic output feedback control law $u = K y$. The distributed optimal control problem of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$.} of the closed loop transfer function from $w$ to $\bar{z}$ is formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} &&|| P_{11} + P_{12} K(I-P_{22}K)^{-1} P_{21}|| \nonumber\\
\text{subject to } && K \text{ stabilizes } P \nonumber\\
&& K \in \mathcal{S}_c  \label{eq:trad}
\end{eqnarray}
where $\mathcal{S}_c$ is a subspace constraint that $K$ must satisfy in order to be implementable on the communication network of the system. It can be seen that the objective function in \eqref{eq:trad} is not convex in $K$. As a result, Youla parameterization is used to reformulate \eqref{eq:trad} in terms of the Youla parameter, and it admits a convex reformulation if and only if $\mathcal{S}_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \mathcal{S}_c$ for all $K \in \mathcal{S}_c$.
%Traditionally, Youla parameterization is used to reformulate \eqref{eq:trad} into a convex manner. It is known that the constraint $\mathcal{S}_c$ remains convex on the Youla parameter if and only if $\mathcal{S}_c$ is QI with respect to $P_{22}$, i.e. $K P_{22} K \in \mathcal{S}_c$ for all $K \in \mathcal{S}_c$.


The delay constraint for QI

As alluded to in the introduction, the class of QI constraint is not amenable for large-scale problem. This is due to the fact that the sparsity constraint on $K$ is generally not QI for a plant with strongly connected topology\footnote{This means that $P_{22}$ is not sparse} \cite{2010_Rotkowitz_QI_delay, 2009_Swigart_graph_QI}. Even when $A$ in \eqref{eq:dynamics} is as sparse as a tridiagonal matrix, the QI condition requires all the local measurements to be shared among \emph{every controllers} in the network. Such a controller implementation is not scalable to large systems. In addition, \eqref{eq:trad} is a large-scale optimization problem, and it is generally hard to solve in a scalable way.

In this paper, we reformulate \eqref{eq:trad} in terms of the \emph{closed loop transfer matrices} rather than the Youla parameter. With a slightly change in the last constraint in \eqref{eq:trad}, we characterize a much broader class of convex problems in the field of distributed control. In the next section, we will start with a characterization of ``$K$ stabilizes $P$" in \eqref{eq:trad} in terms of the closed loop transfer matrices.



==> Sensor_regularization.tex <==
\subsection{Localized $\mathcal{H}_2$ with Sensor Regularization}
In the previous subsection, we assume that each subsystem in the toy power network has a phase and a frequency sensor. In this subsection, we use the localized $\mathcal{H}_2$ problem with sensor regularization (a special case of \eqref{eq:h2l1}) to co-design the localized $\mathcal{H}_2$ controller \emph{and} the sensor placement of a large network.
%the locations of the sensors of the network is given in advanced. In this subsection, we try to co-design the localized $\mathcal{H}_2$ controller \emph{and} the sensor placement of a large network. This is done by solving the localized $\mathcal{H}_2$ problem with sensor regularization, which is shown to be decomposable and thus admits a scalable algorithm.

In order to allow more flexibility on sensor placement, we slightly increase the locality constraint $\Ell$ and the length of the FIR constraint $\FT$. Specifically, the transfer matrices $\tf R, \tf M$, and $\tf N$ in \eqref{eq:desired} are allowed to be $2$-localized, and $\tf L$ is allowed to be $3$-localized. We set $T = 10$ for the FIR constraint. The results are summarized in Table \ref{Table:3}.

\begin{table}[h]
 \caption{Results of localized $\mathcal{H}_2$ with Sensor Regularization}
 \label{Table:3}
 %\normalsize
\begin{center}
    \begin{tabular}{ |c|c|c|c|c|c|}
    %\begin{tabular}{|c|c|c|c|}
    \hline
     $\#$ of states & 200 & 450 & 800 & 1800 & 3200 \\ \hline
     $\mathcal{H}_2$ norm (before) & 13.66 & 20.42 & 27.13 & 40.71 & 54.37 \\ \hline
     $\#$ of removed sensor & 29 & 98 & 162 & 376 & 654 \\ \hline
     $\mathcal{H}_2$ norm (after) & 14.49 & 22.11 & 29.10 & 43.73 & 58.11 \\ \hline
     Comp. time (s) & 109 &  606 & 1012 & 2437 & 5193 \\ \hline
     \end{tabular}
\end{center}
\end{table}

The first row of Table \ref{Table:3} is the total number of states of the networked system. We synthesize the localized $\mathcal{H}_2$ controller with the given spatiotemporal constraint, and list the $\mathcal{H}_2$ norm of the closed loop in the second row. We then solve the localized $\mathcal{H}_2$ problem with sensor regularization to determine the tradeoff between the localized $\mathcal{H}_2$ cost and the number of sensors used in the network. We initially give equal penalty on each sensor, then iteratively update the penalty using the reweighted $\ell_1$ algorithm described in Section \ref{sec:sar}. After $8$ times of reweighting, we remove the sensors for those with their sensor norm smaller than $0.02$. The numbers of removed sensors are listed in the third row of Table \ref{Table:3}, and the localized $\mathcal{H}_2$ cost (in terms of $\mathcal{H}_2$ norm) for the system with reduced number of sensors are listed in the fourth row. The fifth row of Table \ref{Table:3} is the total computation time to synthesize the initial localized $\mathcal{H}_2$ controller, solve the localized $\mathcal{H}_2$ problem with sensor regularization, and resynthesize the localized $\mathcal{H}_2$ controller for the system with reduced number of sensors.

According to Table \ref{Table:3}, our algorithm can successfully remove about $20\%$ of the sensors while maintaining the localizability of the network. The $\mathcal{H}_2$ norm of the closed loop degrades about $7\%$ after removing these sensors. The total computation time is significantly larger than the one in the previous subsection due to two different reasons. First, we increase the locality constraint $\Ell$ and the FIR constraint $\FT$, which increases the complexity of each localized $\mathcal{H}_2$ subproblem. Second, the localized $\mathcal{H}_2$ with sensor regularization takes much more iterations to converge. Even though the ADMM update for localized $\mathcal{H}_2$ with sensor regularization can be evaluated in closed form, the computation time for the reweighted $\ell_1$ iteration still contributes to $70\%$ of the total computation time. Nevertheless, our method is still much more scalable than the centralized method. For a randomized network with $3200$ states, it takes $13$ minutes to synthesize the initial localized $\mathcal{H}_2$ controller, $56$ minutes to run the reweighted $\ell_1$ iteration, and $17$ minutes to synthesize the localized $\mathcal{H}_2$ controller for the system with reduced number of sensors. In contrast, according to Figure \ref{fig:Time}, it takes more than $3$ hours to synthesize the initial centralized $\mathcal{H}_2$ optimal controller, and much longer time to run the sensor regularization algorithm. Figure \ref{fig:Sensor} shows the locations of the removed sensors for this $3200$-state example.

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.47\textwidth]{figure/Sensor_loc.pdf}
      \caption{The upward-pointing triangles represent the subsystems in which the phase sensor is removed. The downward-pointing triangles represent the subsystems in which the frequency sensor is removed.}
      \label{fig:Sensor}
\end{figure}

==> Simu_v1.tex <==
In this section, we demonstrate the LLQG algorithm with sensor actuator regularization on a toy power network. After introducing the power system model, we discuss how to set the constraints $\Ell$ and $\FT$ to enhance the scalability of controller implementation and synthesis. We show that the LLQG controller, with the additional sparsity constraint, FIR constraint, and communication delay constraint, can achieve similar transient performance to an idealized $\mathcal{H}_2$ optimal one, but far more superior than the centralized and the distributed methods in terms of the scalability of controller synthesis and implementation. Specifically, we synthesize the LLQG controller for a randomized heterogeneous networked system with $12800$ states, where the centralized and distributed counterparts cannot be computed. We also solve the LLQG problem with sensor actuator regularization to co-design the LLQG controller and the sensor and actuator placement of the power network. %Finally, we demonstrate our algorithm on a large system, and show that our method is far more superior than the centralized or the distributed methods in terms of the scalability of controller synthesis and implementation.

\subsection{Power System Model}
We begin with a $10 \times 10$ mesh network representing the interconnection between subsystems, and drop each edge with probability $0.25$. The resulting interconnected topology is shown in Fig. \ref{fig:mesh} -- we assume that all edges are undirected.
\begin{figure}[ht!]
      \centering
      \subfigure[Interconnected topology]{%
      \includegraphics[width=0.36\columnwidth]{figure/Mesh10.pdf}
      \label{fig:mesh}}      
      \subfigure[Interaction between neighboring subsystems]{%
      \includegraphics[width=0.45\columnwidth]{./figure/Inter.pdf}
      \label{fig:inter}} 
      \caption{Simulation example interaction graph.}
\end{figure}
%\begin{figure}[ht!]
%      \centering
%      \includegraphics[width=0.28\textwidth]{figure/Mesh8.pdf}
%      \caption{Interconnected topology for the simulation example}
%      \label{fig:mesh}
%\end{figure}
The dynamics of each subsystem is given by the discretized swing equation for power network. Consider the swing dynamic equation
\begin{equation}
m_i \ddot{\theta_i} + d_i \dot{\theta_i} = -\sum_{j \in \mathcal{N}_i} k_{ij} (\theta_i - \theta_j) + w_i + u_i \label{eq:swing}
\end{equation}
where $\theta_i$, $\dot{\theta_i}$, $m_i$, $d_i$, $w_i$, $u_i$ are the phase angle deviation, frequency deviation, inertia, damping, external disturbance, and control action at power station $i$. The coefficient $k_{ij}$ is the coupling term between stations $i$ and $j$. We let $x_i := [\theta_i \quad \dot{\theta_i}]^\top$ be the state of power station $i$ and use $e^{A \Delta t} \approx I + A \Delta t$ to discretize the swing dynamics. Equation \eqref{eq:swing} can then be expressed in the form of \eqref{eq:interconnected} with
\begin{equation}
A_{ii} = \begin{bmatrix} 1 & \quad \Delta{t} \\ -\frac{k_i}{m_i} \Delta{t} & \quad 1-\frac{d_i}{m_i} \Delta{t} \end{bmatrix}, \quad A_{ij} = \begin{bmatrix} 0 & 0 \\ \frac{k_{ij}}{m_i} \Delta{t} & 0 \end{bmatrix}, \nonumber
\end{equation}
and $B_{ii} = \begin{bmatrix} 0 & 1 \end{bmatrix}^\top$. We set $\Delta{t} = 0.2$ and $k_i = \sum_{j \in \mathcal{N}_i} k_{ij}$. In addition, the parameters $k_{ij}, d_i$, and $m_i^{-1}$ are randomly generated and uniformly distributed between $[0.5, 1]$, $[1, 1.5]$, and $[0, 2]$, respectively. The instability of the plant is characterized by the spectral radius of the matrix $A$, which is $1$ in the simulated example. The interactions between neighboring subsystems of the discretized model is described by Figure \ref{fig:inter}.

From \eqref{eq:swing}, the external disturbance $w_i$ only affects the frequency deviation $\dot{\theta_i}$. In the discretized plant model in Fig. \ref{fig:inter}, we assume that the process noise affects both the frequency deviation $\dot{\theta_i}$ and the phase deviation $\theta_i$ with different strength -- the disturbance on frequency and phase are uncorrelated AWGNs with covariance matrices given by $I$ and $10^{-4}I$, respectively. We assume that both the phase deviation and the frequency deviation are measured with some sensor noise. The sensor noise of phase and frequency measurements are uncorrelated AWGNs with covariance matrix given by $10^{-2}I$. We choose equal penalty on the state deviation and control effort, i.e., $\begin{bmatrix} C_1 & D_{12} \end{bmatrix} = I$. 

Based on the above setting, we can formulate a $\mathcal{H}_2$ optimal control problem that minimizes the $\mathcal{H}_2$ norm of the transfer matrix from the process and sensor noises to the regulated output. The $\mathcal{H}_2$ norm of the closed loop is given by $13.5356$ when a proper optimal $\mathcal{H}_2$ controller is applied, and $17.0972$ when a strictly proper optimal $\mathcal{H}_2$ controller is applied.
% 10.7354, 13.4280

%\begin{figure}[ht!]
%      \centering
%      \includegraphics[width=0.28\textwidth]{figure/inter.pdf}
%      \caption{The interaction between neighboring subsystems}
%      \label{fig:inter}
%\end{figure}

\subsection{LLQG}
The underlying assumption of the centralized optimal control scheme is that the measurement can be transmitted \emph{instantaneously} with \emph{every subsystem} in the network. To incorporate the communication delay constraint and facilitate the scalability of controller design, we impose additional constraint on the closed loop transfer matrices as in \eqref{eq:h2l1-3}. With the additional spatiotemporal constraint, the $\mathcal{H}_2$ control problem becomes a LLQG problem. We introduce the communication delay constraint, the locality constraint, and the FIR constraint in \eqref{eq:h2l1-3} in a sequential order as follows.

For the communication delay constraint $\C$, we assume that each subsystem takes one time step to transmit the information to its neighbor. Mathematically, the control action $u_i[t]$ at time $t$ can receive $(y_j[\tau],\beta_j[\tau])$ for all $\tau \leq t-k$ if the distance between subsystems $i$ and $j$ is $k$.
%$\dist{j}{i}=k$. 
The interaction between subsystems illustrated in Fig. \ref{fig:inter} implies that it takes two time steps for a disturbance at subsystem $j$ to propagate to its neighboring subsystems, and hence the communication speed is twice as fast as propagation speed of disturbances through the plant. For the given communication delay constraint $\C$, we use the method in \cite{2015_Wang_Reg} to design the sparsest locality constraint $\Ell$. In this example, we enforce the locality constraint such that the transfer matrices $\tf R$ and $\tf N$ in \eqref{eq:desired} are $1$-localized and $\tf M$ and $\tf L$ in \eqref{eq:desired} are $2$-localized. This implies that each subsystem $j$ only needs to exchange the information within its two-hop neighbors, and use the restricted plant model within its two-hop neighbors to synthesize the LLQG controller. 

Once the communication delay constraint $\C$ and the locality constraint $\Ell$ are specified, we perform some simulation to exploit the tradeoff between the length of the FIR constraint $\FT$ and the transient performance. Figure \ref{fig:T} shows the tradeoff curve between the transient performance of the LLQG controller and the length $T$ of the FIR constraint.
%(the $\mathcal{H}_2$ norm of the closed loop when LLQG controller with the constraint $\C \cap \Ell \cap \FT$ is applied)  (the length $T$ of the FIR constraint $\FT$). 
For the given communication delay constraint $\C$ and the locality constraint $\Ell$, the LLQG controller is feasible with the FIR constraint $\FT$ for all $T \geq 3$. When the length of the FIR constraint increases, the $\mathcal{H}_2$ norm of the closed loop converges quickly to the unconstrained optimal value. For instance, for FIR length $T=7, 10,$ and $20$, the performance degradation compared to the unconstrained $\mathcal{H}_2$ optimal controller are given by $3.8\%$, $1.0\%$, and $0.1\%$, respectively. This further means that the performance degradation due to the additional communication delay constraint $\C$ and the locality constraint $\Ell$ is less than $0.1\%$. From Figure \ref{fig:T}, we show that the LLQG controller, with additional communication delay constraint, locality constraint, and FIR constraint, can achieve similar transient performance to an unconstrained optimal $\mathcal{H}_2$ controller.

%Figure \ref{fig:T} illustrates the fundamental tradeoff between transient performance ($\mathcal{H}_2$ norm) and the settling time (the length of the FIR constraint).
\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.4\textwidth]{figure/T_plot.pdf}
      \caption{The vertical axis is the $\mathcal{H}_2$ norm of the closed loop when LLQG controller is applied. The LLQG controller is subject to the constraint $\C \cap \Ell \cap \FT$. The horizontal axis is the horizon $T$ of the FIR constraint $\FT$, which is also the settling time of the closed loop response. We plot the $\mathcal{H}_2$ norm for the centralized unconstrained optimal controller (proper and strictly proper) in the same figure.}
      \label{fig:T}
\end{figure}

To further illustrate the advantages of the LLQG optimal controller, we choose $T = 20$ and compare the LLQG controller and the $\mathcal{H}_2$ optimal controller in terms of closed loop performance, the complexity of controller synthesis, and the complexity of controller implementation in Table \ref{Table:2}. It can be seen that the LLQG optimal controller is vastly preferable in all aspects, except for a slight degradation in the closed-loop performance. In particular, the locality constraint $\Ell$ in this example has almost no effect on the closed loop performance. 

\begin{table}[h]
 \caption{Comparison Between Centralized and Localized Control}
 \label{Table:2}
 %\normalsize
\begin{center}
    \begin{tabular}{ | l | l | l | l | }
    %\begin{tabular}{|c|c|c|c|}
    \hline
     & & Centralized & Localized \\ \hline
     & Affected region & Global & $2$-hop \\ \cline{2-4}
     Closed Loop & Affected time & Long & $20$ steps \\ \cline{2-4}
     & Normalized $\mathcal{H}_2$ & $1$ & $1.001$ \\ \hline \hline
     & Comp. complexity & $O(n^3)$ & $O(n)$ \\ \cline{2-4}
     Synthesis & Plant model & Global & $2$-hop \\ \cline{2-4}
     & Redesign & Offline & Real-time \\ \hline \hline
     Implementation & Comm. Speed & $\infty$ & $2$x \\ \cline{2-4}
     & Comm. Range & Global & $2$-hop \\ \hline 
     \end{tabular}
\end{center}
\end{table}

%\begin{table}[h]
% \caption{Comparison Between Centralized and Localized Scheme}
% \label{Table:2}
%\begin{center}
%    \begin{tabular}{ | l | l | l | l | }
%    \hline
%     & & Centralized & Localized \\ \hline
%     & Affected region & Global & $2$-hop \\ \cline{2-4}
%     Closed Loop & Affected time & Long & $10$ steps \\ \cline{2-4}
%     & Normalized $\mathcal{H}_2$ & 1 & 1.035 \\ \hline \hline
%     & Comp. complexity & $O(n^3)$ & $O(n)$ \\ \cline{2-4}
%     & Comp. time (s)& $138.49$ & $55.67$ \\ \cline{2-4}
%     Synthesis & Time per node (s) & $138.49$ & $0.07$ \\ \cline{2-4}
%     & Plant model & Global & $3$-hop \\ \cline{2-4}
%     & Redesign & Offline & Real-time \\ \hline \hline
%     Implementation & Comm. Speed & Inf & $2$ \\ \cline{2-4}
%     & Comm. Range & Global & $3$-hop \\ \hline 
%     \end{tabular}
%\end{center}
%\end{table}

%We now vary the size of the system, and compare the computation time needed to synthesize
We now allow the size of the problem to vary and compare the computation time needed to synthesize a centralized, distributed, and LLQG optimal controller. The distributed optimal controller is computed using the methods described in \cite{2014_Lamperski_H2_journal}\footnote{The edge dropping probability is set to zero in this scheme as the method requires strong connectedness of the plant. This does not change the computation time much.}, in which we assume the same communication constraint $\C$ as LLQG. The empirical relationship obtained between computation time and problem size for different control schemes is illustrated in Figure \ref{fig:Time}. As can be seen in Figure \ref{fig:Time}, the computation time needed for the distributed controller grows rapidly when the size of problem increases. For the centralized one, the slope in the log-log plot in Figure \ref{fig:Time} is $3$, which matches the theoretical complexity $O(n^3)$. The slope for the LLQG controller is about $1.5$, which is larger than the theoretical value $1$. We believe this overhead is caused by other computational issue such as memory management and data structure. We note that the computational bottleneck that we faced in computing our large-scale example was that we were using a single workstation to compute the controller (and hence the LLQG subproblems were essentially solved in serial) -- in practice, if each local subsystem is capable of solving its corresponding LLQG subproblem, our approach scales to systems of arbitrary size as all computations can be done in parallel. For the largest example we have, we can finish the LLQG synthesis (for $T = 7$) for a system with $12800$ states in about $55$ minutes using a single computer. If the computation is parallelized into all $6400$ sub-systems, the synthesis algorithm can be done within a second. In contrast, the theoretical time to compute the centralized $\mathcal{H}_2$ optimal controller for the same example is more than a week.
%For the largest example that we computed, we are able to synthesize an LLQG optimal controller for a 
%To illustrate the extreme scalability of the LLQG controller, we compare the computation time of the LLQG controller to the centralized $\mathcal{H}_2$ controller and the distributed controller with QI communication delay constraint \cite{2014_Lamperski_H2_journal}. Figure \ref{fig:Time} shows the 

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.47\textwidth]{figure/Comp_time.pdf}
      \caption{The horizontal axis denotes the number of states of the system, and the vertical axis is the computation time in seconds.}
      \label{fig:Time}
\end{figure}

\subsection{LLQG with Sensor Regularization}
In the previous subsection, we assume that each subsystem in the toy power network has a phase and a frequency sensor. In this subsection, we use the LLQG problem with sensor regularization (a special case of \eqref{eq:h2l1}) to co-design the LLQG controller \emph{and} the sensor placement of a large network.
%the locations of the sensors of the network is given in advanced. In this subsection, we try to co-design the LLQG controller \emph{and} the sensor placement of a large network. This is done by solving the LLQG problem with sensor regularization, which is shown to be decomposable and thus admits a scalable algorithm.

In order to allow more flexibility on sensor placement, we slightly increase the locality constraint $\Ell$ and the length of the FIR constraint $\FT$. Specifically, the transfer matrices $\tf R, \tf M$, and $\tf N$ in \eqref{eq:desired} are allowed to be $2$-localized, and $\tf L$ is allowed to be $3$-localized. We set $T = 10$ for the FIR constraint. The results are summarized in Table \ref{Table:3}.

\begin{table}[h]
 \caption{Results of LLQG with Sensor Regularization}
 \label{Table:3}
 %\normalsize
\begin{center}
    \begin{tabular}{ |c|c|c|c|c|c|}
    %\begin{tabular}{|c|c|c|c|}
    \hline
     $\#$ of states & 200 & 450 & 800 & 1800 & 3200 \\ \hline
     $\mathcal{H}_2$ norm (before) & 13.66 & 20.42 & 27.13 & 40.71 & 54.37 \\ \hline
     $\#$ of removed sensor & 29 & 98 & 162 & 376 & 654 \\ \hline
     $\mathcal{H}_2$ norm (after) & 14.49 & 22.11 & 29.10 & 43.73 & 58.11 \\ \hline
     Comp. time (s) & 109 &  606 & 1012 & 2437 & 5193 \\ \hline
     \end{tabular}
\end{center}
\end{table}

The first row of Table \ref{Table:3} is the total number of states of the networked system. We synthesize the LLQG controller with the given spatiotemporal constraint, and list the $\mathcal{H}_2$ norm of the closed loop in the second row. We then solve the LLQG problem with sensor regularization to determine the tradeoff between the LLQG cost and the number of sensors used in the network. We initially give equal penalty on each sensor, then iteratively update the penalty using the reweighted $\ell_1$ algorithm described in Section \ref{sec:sar}. After $8$ times of reweighting, we remove the sensors for those with their sensor norm smaller than $0.02$. The numbers of removed sensors are listed in the third row of Table \ref{Table:3}, and the LLQG cost (in terms of $\mathcal{H}_2$ norm) for the system with reduced number of sensors are listed in the fourth row. The fifth row of Table \ref{Table:3} is the total computation time to synthesize the initial LLQG controller, solve the LLQG problem with sensor regularization, and resynthesize the LLQG controller for the system with reduced number of sensors.

According to Table \ref{Table:3}, our algorithm can successfully remove about $20\%$ of the sensors while maintaining the localizability of the network. The $\mathcal{H}_2$ norm of the closed loop degrades about $7\%$ after removing these sensors. The total computation time is significantly larger than the one in the previous subsection due to two different reasons. First, we increase the locality constraint $\Ell$ and the FIR constraint $\FT$, which increases the complexity of each LLQG subproblem. Second, the LLQG with sensor regularization takes much more iterations to converge. Even though the ADMM update for LLQG with sensor regularization can be evaluated in closed form, the computation time for the reweighted $\ell_1$ iteration still contributes to $70\%$ of the total computation time. Nevertheless, our method is still much more scalable than the centralized method. For a randomized network with $3200$ states, it takes $13$ minutes to synthesize the initial LLQG controller, $56$ minutes to run the reweighted $\ell_1$ iteration, and $17$ minutes to synthesize the LLQG controller for the system with reduced number of sensors. In contrast, according to Figure \ref{fig:Time}, it takes more than $3$ hours to synthesize the initial centralized $\mathcal{H}_2$ optimal controller, and much longer time to run the sensor regularization algorithm. Figure \ref{fig:Sensor} shows the locations of the removed sensors for this $3200$-state example.

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.47\textwidth]{figure/Sensor_loc.pdf}
      \caption{The upward-pointing triangles represent the subsystems in which the phase sensor is removed. The downward-pointing triangles represent the subsystems in which the frequency sensor is removed.}
      \label{fig:Sensor}
\end{figure}

\subsection{LLQG with Sensor Actuator Regularization}
We also co-design the LLQG controller with its actuator and sensor interface simultaneously by solving the general form of problem \eqref{eq:h2l1}. Problem \eqref{eq:h2l1} is decomposable, and thus can be solved in a localized and distributed way. Here we only demonstrate the algorithm for the example shown in Figure \ref{fig:mesh}. 

In order to allow more flexibility on sensor actuator placement, we set $T = 20$ for the FIR constraint. In addition, the transfer matrices $\tf R, \tf M$, and $\tf N$ in \eqref{eq:desired} are allowed to be $3$-localized, and $\tf L$ is allowed to be $4$-localized. The initial LLQG cost is given by $13.5397$, which is $0.03\%$ degradation compared to the idealized centralized $\mathcal{H}_2$ controller. Originally, we have $100$ actuators and $200$ sensors in the network. After solving the LLQG problem with sensor actuator regularization, we can successfully remove $8$ actuators and $52$ sensors. The idealized centralized $\mathcal{H}_2$ cost becomes $14.4709$ for the proper case, and $17.6036$ for the strictly proper case. The LLQG cost becomes $14.9472$, which is $3.3\%$ degradation compared to the idealized centralized one.
 
% 13.4302

==> State_v1.tex <==
%In the previous section, we showed how the constraints $\Ell$ and $\FT$ in \eqref{eq:localized} can be used to enhance the scalability of controller implementation. In the coming two sections, we show that the constraints $\Ell$ and $\FT$ also enhance the scalability of controller synthesis if the objective function $g(\cdot)$ and the localizability constraint $\s$ satisfy certain technical conditions.

In this section, we consider a special case of \eqref{eq:LOC} which either $B_2$ or $C_2$ is invertible. 
The discussion primarily focuses on the state feedback problem, i.e., $C_2 = I$. 
%In this section, we consider a special case of \eqref{eq:LOC} with $C_2 = I$ (state feedback).
We identify the technical conditions on the objective function $g(\cdot)$ and the $\mathcal{S}$-localizability constraint such that the optimization problem \eqref{eq:LOC} can be decomposed directly into parallel local optimization subproblems without using distributed optimization. This technique is crucial for the general algorithm proposed in Section \ref{sec:of}.

The section begins with some mathematical notations that will be used in the rest of the paper. We then introduce the notion of direct decomposability of the objective function and the localizability constraint. Once the global optimization problem is decomposed into parallel subproblems, we exploit the locality constraint $\Ell$ to further reduce the dimension of each subproblem from global scale to local scale. To help the reader understand the intuition of direct decomposability and the dimension reduction technique, we explain the physical interpretation of our method in Section \ref{sec:physical}. 
%This section ends with the summary of localized synthesis and re-synthesis algorithm for directly decomposable problems.

%and the localized controller re-synthesis algorithm to support the plug-and-play feature
%discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Mathematical Notations}
Let $\mathbb{Z}^+$ be the set of all positive integers. We use calligraphic lower case letters such as $\Set q$ to denote subsets of $\mathbb{Z}^+$. 
%The cardinality of a set $\Set q$ is denoted by $| \Set q |$. 
We say that $\{ \Set p_1, \dots \Set p_m \}$ is a partition of the set $\Set q \subset \mathbb{Z}^+$ if and only if $\Set p_i \not = \emptyset$ for all $i$, $\cup_{i=1}^m p_i = \Set q$, and $\Set p_i \cap \Set p_j = \emptyset$ for all $i \not = j$. 

Consider a transfer matrix $\ttf{\Phi}$ with $n_r$ rows and $n_c$ columns. Let $\Set p$ be a subset of $\{1, \dots, n_r \}$ and $\Set q$ be a subset of $\{1, \dots, n_c \}$. We use $\Sub{\ttf{\Phi}}{\Set p}{\Set q}$ to denote the submatrix of $\ttf{\Phi}$ by selecting the rows according to the set $\Set p$ and columns according to the set $\Set q$. When $\Set p = \{1, \dots, n_r \}$ is the set of all rows, we use the symbol $:$ to denote the set $\Set p$. Similarly, when $\Set q = \{1, \dots, n_c \}$ is the set of all columns, we use $:$ to denote the set $\Set q$. We have $\ttf{\Phi} = \Sub{\ttf{\Phi}}{:}{:}$. Let $\{ \Set p_1, \dots \Set p_m \}$ be a partition of the set $\{1, \dots, n_c\}$. Then $\{ \Sub{\ttf{\Phi}}{:}{\Set p_1}, \dots,  \Sub{\ttf{\Phi}}{:}{\Set p_m} \}$ is a column-wise partition of the transfer matrix $\ttf{\Phi}$.

%Partition of a set, column/row-wise partition, cardinality of a set, complement of a set
%Submatrices notation, transfer matrices (with FIR constraint)
A permutation matrix is a square binary matrix that has exactly one entry of $1$ in each row and each column and zeros elsewhere.
%Block-wise sparsity pattern, multiplication of sparsity patterns

\subsection{Direct Decomposability}
Assume that the matrix $C_2$ is invertible. In this case, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
\begin{eqnarray}
\tf N &=& [ \tf R (zI-A) - I ] C_2^{-1} \nonumber\\
\tf L &=& \tf M (zI-A) C_2^{-1}. \nonumber
\end{eqnarray}
%For $C_2 = I$, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%\begin{eqnarray}
%\tf N &=& [ \tf R (zI-A) - I ] \nonumber\\
%\tf L &=& \tf M (zI-A). \nonumber
%\end{eqnarray}
%The optimization problem \eqref{eq:LOC} is then simplified into
We then use these relations to simplify the optimization problem \eqref{eq:LOC} into
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && g'(\tf R, \tf M) \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \s' \cap \frac{1}{z} \mathcal{RH}_\infty,\label{eq:sf_lop}
\end{eqnarray}
%for some objective function $g'(\cdot)$ and localizability constraint $\mathcal{S}'$. 
where $g'(\cdot)$ is the original objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, and $\s'$ is the intersection of the set $\s$ and the affine space \eqref{eq:main_2}. 
We sometimes refer to \eqref{eq:sf_lop} a state feedback problem, i.e., $C_2 = I$ is invertible.
%The function $g'(\cdot)$ in \eqref{eq:sf_lop} is the original convex objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, which is convex. The set $\s'$ is the intersection of the original convex set constraint $\s$ and the affine space \eqref{eq:main_2}, which remains a convex set. Therefore, problem \eqref{eq:sf_lop} remains a convex optimization problem.

\begin{remark}
When $B_2$ is invertible, we can solve \eqref{eq:main_1} analytically to express the transfer matrices $(\tf M, \tf L)$ as a function of $(\tf R, \tf N)$.
%We focus on the state feedback problem (i.e., $C_2 = I$). After solving \eqref{eq:sf_lop}, the controller achieving the desired closed loop response can be implemented by \cite{2015_PartI}
%\begin{eqnarray}
%\tf{\hat{w}} &=& C_2^{-1} (\tf y - \tf{\hat{y}}) \nonumber\\
%\tf u &=& z \tf M \hat{w} \nonumber\\
%\tf{\hat{y}} &=& C_2 (z \tf R - I) \tf{\hat{w}}. \nonumber
%\end{eqnarray}
%Although this implementation holds for arbitrary invertible $C_2$, the computation of the inverse of $C_2$ can be prohibited for large-scale systems unless $C_2$ has certain sparsity structure, e.g., block diagonal.
\end{remark}
%For a state feedback system, we have $C_2 = I$.
%The general formulation for a localized state feedback problem is given by
%In particular, we consider the case in which the localizability constraint $\mathcal{S}$ is a spatio-temporal constraint. We aim to exploit the sparsity of $\mathcal{S}$ to provide a scalable algorithm to solve the optimization problem \eqref{eq:sf_lop}.

To simplify the notation, we use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. We ignore the superscript of $g$ and $\mathcal{S}$ in \eqref{eq:sf_lop} and denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$. The optimization problem \eqref{eq:sf_lop} can then be written as 
\begin{subequations} \label{eq:sf_lop2}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:lop-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = I \label{eq:lop-2} \\
& \ttf{\Phi} \in \s. \label{eq:lop-3}
\end{align}
\end{subequations}
Here we include the stability constraint $\frac{1}{z}\RHinf$ into the constraint set $\s$ in \eqref{eq:lop-3}. 
%Similar to \eqref{eq:localized}, 
Note that the localizability constraint $\s$ considered in this section is an intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the remaining convex set constraint $\Sother$, i.e., $\s = \Ell \cap \FT \cap \Sother$.
The goal of this section is to identify the technical conditions on $g(\cdot)$ and $\s$ in \eqref{eq:sf_lop2} so that the global optimization problem \eqref{eq:sf_lop2} can be solved in a localized and distributed way. 

%In addition, the localizability constraint $\s$ is expressed as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.
%We can also express the localizability constraint $\s$ as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.

%\subsubsection{Column-wise Partition}
%In order to make the optimization problem \emph{decomposable}, we make the following assumptions on the problem. 

%In order to solve the optimization problem \eqref{eq:sf_lop2} in an efficient way, we attempt to decompose the problem \eqref{eq:sf_lop2} into several subproblems with smaller scale. 
We first observe that the matrix variable $\ttf{\Phi}$ in constraint \eqref{eq:lop-2} can be examined column at a time. It is then natural to see if the objective \eqref{eq:lop-1} and the localizability constraint \eqref{eq:lop-3} can also be decomposed in a column-wise manner. This leads to the notion of \emph{direct decomposability} of the problem.

%Let $n_x + n_u$ and $n_x$ denote the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2}. 
From the definition of the closed loop transfer matrices \eqref{eq:desired}, the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2} are given by $(n_x + n_u)$ and $n_x$, respectively. Let $\{ \Set p_1, \dots, \Set p_m\}$ be a partition of the set $\{1, \dots, n_x\}$. The optimization variable $\ttf{\Phi}$ can then be partitioned column-wisely into the set $\{ \Sub{\ttf{\Phi}}{ : }{\Set p_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\Set p_m} \}$. The direct decomposability of the objective function in \eqref{eq:sf_lop2} is defined as follows.
\begin{definition} \label{dfn:dd}
The objective function $g(\ttf{\Phi})$ in \eqref{eq:sf_lop2} is said to be \emph{directly decomposable} with respect to the column-wise partition $\{ \Set p_1, \dots, \Set p_m\}$ if
\begin{equation}
g(\ttf{\Phi}) = \sum_{j=1}^m g_j(\Sub{\ttf{\Phi}}{ : }{\Set p_j}) \label{eq:decom_obj}
\end{equation}
for some functions $g_j(\cdot)$ for $j = 1, \dots, m$. 
\end{definition}
%$\Sub{\ttf{\Phi}}{ : }{\Set p_j}$
%Consider a column-wise partition $\{ \Phi_j \}_{j=1}^n$ of the closed loop transfer matrix $\Phi$. This partition can be interpreted as a partition of process noise, where $\Phi_j$ is the closed loop transfer matrix from disturbance $\delta{x_j}$ to $[x^\top u^\top]^\top$.
%Given a partition of the global state vector $\{ \Set p_j \}_{j=1}^n$, we can decompose the closed loop transfer matrices $(R,M)$ block column-wisely according to the partition $\{ \Set p_j \}_{j=1}^n$. Specifically, we use $R_{\Set p_j}$ and $M_{\Set p_j}$ to denote the $j$th block column of $R$ and $M$, respectively. By definition, $R_{\Set p_j}$ and $M_{\Set p_j}$ are the closed loop transfer matrices from $\delta{x_{\Set p_j}}$ to $x$ and $u$, respectively. 
%Note that the set $\{R_j,M_j\}$ encodes the information of the underlying partition. In the following, we use $\{R_j,M_j\}$ to represent a partition without explicitly specify the partition $\{ \Set p_j \}$. 
%We define the decomposable objective function and the decomposable localizability constraint as follows.
%Using this notation, 

Here we give some examples of directly decomposable objective functions. 
\begin{example}
Consider the objective function in \eqref{eq:trad_obj2} with $B_1 = I$ and $D_{21} = 0$. This is the state feedback problem with uncorrelated process noise, i.e., $B_1 = I$. We pick the objective function \eqref{eq:lop-1} as $|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2$. We have
%If we take the square of the $\mathcal{H}_2$ norm of the closed loop map, then the objective function is given by
%One concrete example of a column-wise decomposable objective is the $\mathcal{H}_2$ norm with identity noise matrix $B_1 = I$. For instance, we have
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{m} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\Set p_j} ||_{\mathcal{H}_2}^2 \nonumber
\end{equation}
for arbitrary column-wise partition $\{ \Set p_1, \dots, \Set p_m\}$. This holds for arbitrary $C_1$ and $D_{12}$.
\end{example}
\begin{example} \label{ex:perm}
Continue from the previous example.
%The previous example can be extended to a more general case. 
Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\Pi B_1$ is block diagonal. This happens when the global process noise vector can be partitioned into uncorrelated subsets. The objective function is given by
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} B_1 ||_{\mathcal{H}_2}^2  =  || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} \Pi^\top \Pi B_1 ||_{\mathcal{H}_2}^2. \nonumber
\end{equation}
Note that $\ttf{\Phi} \Pi^\top$ is a column-wise permutation of the optimization variable. We can define a column-wise partition on $\ttf{\Phi} \Pi^\top$ according to the block diagonal structure of the matrix $\Pi B_1$ to decompose the objective function in a column-wise manner. 
\end{example}
\begin{example} \label{ex:l1}
In the previous two examples, we rely on the inherent decomposable property of the $\mathcal{H}_2$ norm. Specifically, the square of the $\mathcal{H}_2$ norm of a FIR transfer matrix $\tf G \in \FT$ is given by
\begin{eqnarray}
|| \tf G ||_{\mathcal{H}_2}^2  &=&  \sum_i \sum_j || \tf g_{ij} ||_{\mathcal{H}_2}^2 \nonumber\\
&=& \sum_i \sum_j \sum_{t=1}^T ( g_{ij}[t] )^2. \label{eq:h2_comp}
\end{eqnarray}
Motivated by the $\mathcal{H}_2$ norm, we define the element-wise $\ell_1$ norm (denoted by $e\ell_1$) of a transfer matrix $\tf G \in \FT$ as
\begin{equation}
|| \tf G ||_{e\ell_1}  =  \sum_i \sum_j \sum_{t=1}^T | g_{ij}[t] |. \nonumber
\end{equation}
The previous two examples still hold if we change the square of the $\mathcal{H}_2$ norm to the element-wise $\ell_1$ norm.
\end{example}

We now define the direct decomposability of the localizability constraint \eqref{eq:lop-3} as follows.
\begin{definition} \label{dfn:s}
The set constraint $\s$ in \eqref{eq:lop-3} is said to be \emph{directly decomposable} with respect to the column-wise partition $\{ \Set p_1, \dots, \Set p_m\}$ if the following condition is satisfied:
\begin{equation}
\ttf{\Phi} \in \s \quad \text{if and only if} \quad \Sub{\ttf{\Phi}}{ : }{\Set p_j} \in \s_j \text{  for  } j = 1, \dots, m  \nonumber
\end{equation}
for some set $\s_j$ for $j = 1, \dots, m$. Mathematically, this condition is expressed as
\begin{equation}
\ttf{\Phi} \in \s \quad \Longleftrightarrow \quad \bigcap_{j=1}^m \Sub{\ttf{\Phi}}{ : }{\Set p_j} \in \s_j.  \label{eq:decom_scon}
\end{equation}
\end{definition}

Equation \eqref{eq:decom_scon} is interpreted as follows. Suppose that the set constraint $\ttf{\Phi} \in \s$ is directly decomposable with respect to the column-wise partition $\{ \Set p_1, \dots, \Set p_m\}$. To check whether the transfer matrix $\ttf{\Phi}$ belongs to the set $\s$, we can equivalently check whether the set constraint $\Sub{\ttf{\Phi}}{ : }{\Set p_j} \in \s_j$ is satisfied for each $j$. 
\begin{remark}
Let $\s = \Ell \cap \FT \cap \Sother$ be the localizability constraint in \eqref{eq:sf_lop2}. It can be readily shown that the locality constraint $\Ell$ and the FIR constraint $\FT$ are directly decomposable with respect to any column-wise partition. Therefore, the direct decomposability of the set constraint $\s$ in \eqref{eq:sf_lop2} is determined by the direct decomposability of the constraint $\Sother$. If $\s$ is directly decomposable, then we can express the set constraint $\s_j$ in \eqref{eq:decom_scon} as $\s_j = \Sub{\Ell}{:}{\Set p_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$ for each $j$.
%For the $j$th element of the partition, we can express the set constraint $\s_j$ as $\s_j = \Sub{\Ell}{:}{\Set p_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$.
%We can express the set constraint $\s_j$ as an intersection of the locality constraint, FIR constraint, and other set components as $\s_j = \Sub{\Ell}{:}{\Set p_j} \cap \FT \cap \Sother_j$.
\end{remark}

Assume that the objective function \eqref{eq:lop-1} and the localizability constraint \eqref{eq:lop-3} are both directly decomposable with respect to a column-wise partition $\{ \Set p_1, \dots, \Set p_m\}$. The optimization problem \eqref{eq:sf_lop2} can then be partitioned into $m$ parallel subproblems as
\begin{subequations} \label{eq:decom}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{ : }{\Set p_j}}{\text{minimize }} \quad & g_j(\Sub{\ttf{\Phi}}{ : }{\Set p_j}) \label{eq:decom-1}\\
\text{subject to } \quad & \tf Z_{AB} \Sub{\ttf{\Phi}}{ : }{\Set p_j} = \Sub{I}{ : }{\Set p_j} \label{eq:decom-2} \\
& \Sub{\ttf{\Phi}}{ : }{\Set p_j} \in \Sub{\Ell}{:}{\Set p_j} \cap \FT \cap \Sother_j \label{eq:decom-3}
\end{align}
\end{subequations}
for $j = 1, \dots, m$. 
%Note that the $m$ subproblems can be computed in an independent and parallel way.
%\begin{eqnarray}
%\underset{\Sub{\ttf{\Phi}}{ : }{\Set p_j}}{\text{minimize    }} && g_j(\Sub{\ttf{\Phi}}{ : }{\Set p_j}) \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\Set p_j} = \Sub{I}{ : }{\Set p_j} \nonumber \\
%&& \Sub{\ttf{\Phi}}{ : }{\Set p_j} \in \s_j \label{eq:sf_lopd}
%\end{eqnarray}
%\begin{example}
%Localized LQR with spatio-temporal constraint
%\end{example}
%This is the general formulation for the localized LQR (LLQR) problem proposed in \cite{2014_Wang_CDC}. In \cite{2014_Wang_CDC}, we showed that the global LLQR problem admits a localized decomposition. Specifically, the global LLQR solution can be obtained by solving multiple LLQR sub-problems in a parallel way, with each sub-problem depending only on the \emph{local plant model}. 
%The key observation is noting that the optimization problem \eqref{eq:llqr} admits a \emph{column-wise} decomposition. Specifically, the objective function in \eqref{eq:llqr} can be rewritten as
%\begin{equation}
%\sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber
%\end{equation}
%where the subscript $j$ represents the $j$-th column of the transfer matrix, and $n_x$ is the number of states. Note that the constraints in \eqref{eq:llqr} can be decomposed in a column-wise way as well. Let $\mathcal{S}_j$ denotes the convex set constraint on column $j$. We can solve
%\begin{eqnarray}
%\underset{\{R_j,M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber \\
%&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-s}
%\end{eqnarray}
%for $j = 1, \dots, n_x$ instead of solving \eqref{eq:llqr}, in a parallel way. We now focus on a specific $j$. When $\mathcal{S}_j$ is a locality (sparsity) constraint, we can reduce the dimension of \label{eq:llqr-s} \emph{from global scale to local scale}. 

\subsection{Dimension Reduction}
%When the problem \eqref{eq:sf_lop2} is directly decomposable, we can partition the original problem \eqref{eq:sf_lop2} into parallel subproblems as in \eqref{eq:decom}. 
Note that each subproblem in \eqref{eq:decom} remains a large-scale optimization problem -- each subproblem in \eqref{eq:decom} depends on the knowledge of the global plant model $\tf Z_{AB}$. In this subsection, we exploit the locality constraint $\Sub{\Ell}{:}{\Set p_j}$ in \eqref{eq:decom-3} to reduce the complexity of \eqref{eq:decom}. 
The physical interpretation of our approach is explained in the next subsection.
%In fact, the primary reason to decompose the global optimization problem \eqref{eq:sf_lop2} into parallel subproblems \eqref{eq:decom} is to facilitate the dimensional reduction -- this will be illustrated in the example in the next subsection.

Consider problem \eqref{eq:decom} with a specific $j$. Recall that the number of rows of the transfer matrix $\Sub{\ttf{\Phi}}{:}{\Set p_j}$ is given by $(n_x + n_u)$. Let $\Set c_j$ be the largest subset of $\{1, \dots, n_x + n_u\}$ such that the locality constraint $\Sub{\Ell}{\Set c_j}{\Set p_j}$ in \eqref{eq:decom-3} is exactly a zero matrix. When the locality constraint is imposed, we must have $\Sub{\ttf{\Phi}}{\Set c_j}{\Set p_j} = 0$. This part can be eliminated in objective \eqref{eq:decom-1} and constraint \eqref{eq:decom-2}. Let $\Set r_j = \{1, \dots, n_x + n_u\} - \Set c_j$ be the complement set of $\Set c_j$. When the locality constraint is imposed, problem \eqref{eq:decom} can be simplified into
\begin{subequations} \label{eq:decom2}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j}}{\text{minimize }} \quad & g'_j(\Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j}) \label{eq:decom2-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{:}{\Set r_j} \Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j} = \Sub{I}{ : }{\Set p_j} \label{eq:decom2-2} \\
& \Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j} \in \Sub{\Ell}{\Set r_j}{\Set p_j} \cap \FT \cap \Sother'_j \label{eq:decom2-3}
\end{align}
\end{subequations}
where $g'_j(\cdot)$ and $\Sother'_j$ are the restriction of $g_j(\cdot)$ and $\Sother_j$ on the constraint $\Sub{\ttf{\Phi}}{\Set c_j}{\Set p_j} = 0$, respectively. From the definition of the set $\Set r_j$, it is straightforward to see that \eqref{eq:decom2} is equivalent to $\eqref{eq:decom}$.

Next, when the system matrices $(A,B_2)$ are fairly sparse, the transfer matrix $\tf Z_{AB}$ is also sparse. Recall that the number of rows of $\tf Z_{AB}$ is given by $n_x$. Let $\Set d_j$ be the largest subset of $\{1, \dots, n_x\}$ such that the augmented matrix $\begin{bmatrix}\Sub{\tf Z_{AB}}{\Set d_j}{\Set r_j} & \Sub{I}{\Set d_j}{\Set p_j}\end{bmatrix}$ is a zero matrix. Let $\Set t_j = \{1, \dots, n_x\} - \Set d_j$ be the complement set of $\Set d_j$. We can further reduce \eqref{eq:decom2} into
\begin{subequations} \label{eq:decom3}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j}}{\text{minimize }} \quad & g'_j(\Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j}) \label{eq:decom3-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{\Set t_j}{\Set r_j} \Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j} = \Sub{I}{\Set t_j}{\Set p_j} \label{eq:decom3-2} \\
& \Sub{\ttf{\Phi}}{\Set r_j}{\Set p_j} \in \Sub{\Ell}{\Set r_j}{\Set p_j} \cap \FT \cap \Sother'_j. \label{eq:decom3-3}
\end{align}
\end{subequations}
From the definition of the set $\Set t_j$, we know that \eqref{eq:decom3} is equivalent to \eqref{eq:decom2} and therefore equivalent to \eqref{eq:decom}.

The dimension of problem \eqref{eq:decom3} is determined by the cardinality of the sets $\Set p_j$, $\Set r_j$, and $\Set t_j$. When the locality constraint and the system matrices are highly sparse, it is possible to make the size of these sets much smaller than the size of the global network. In this case, the global optimization problem \eqref{eq:decom} reduces to a local optimization problem \eqref{eq:decom3} which depends on the local plant model $\Sub{\tf Z_{AB}}{\Set t_j}{\Set r_j}$ only. The physical meaning of the sets $\Set p_j$, $\Set r_j$, and $\Set t_j$ are explained in detail in the next subsection.
%dimension reduction technique from \eqref{eq:decom} to \eqref{eq:decom3} is explained in detail in the next subsection.
%In the next subsection, we explain the physical meaning of the decomposability assumption from \eqref{eq:sf_lop2} to \eqref{eq:decom} and the dimension reduction from \eqref{eq:decom} to \eqref{eq:decom3}.

\begin{remark} \label{rmk:1}
The dimension reduction algorithm proposed in this paper is the generalization of the algorithms proposed in our prior works \cite{2014_Wang_CDC, 2015_Wang_H2}. Specifically, the algorithms in \cite{2014_Wang_CDC, 2015_Wang_H2} can only handle a particular type of locality constraint (called the $d$-localized constraint), while the algorithm proposed here can handle arbitrary sparsity constraint.
\end{remark}

%, and show how to simplify the optimization problem when $\mathcal{S}_j$ is highly sparse. Recall that $\mathcal{S}_j$ is a constraint imposed on the closed loop response from $\delta{x_j}$ to $x$ and $u$. Therefore, the block row-wise sparsity pattern of $\mathcal{S}_j$ encodes the set of affected states and activated control actions under disturbance $\delta{x_j}$. We can construct a localized region, local state vector, and local plant model based on this information. Consider the following illustrative example.

\subsection{Physical Interpretation} \label{sec:physical}
In this subsection, we explain the physical meaning of the sets $\Set p_j$, $\Set r_j$, and $\Set t_j$ in \eqref{eq:decom3} through a linear quadratic regulator (LQR) problem.
We show that the physical meaning of $\Set p_j$ is the $j$th uncorrelated subset of the noise vector, $\Set r_j$ is the collection of optimization variables contained within the localized region defined by the locality constraint $\Ell$ and the set $\Set p_j$, and $\Set t_j$ is the set of states that can be directly affected by the variables in $\Set r_j$.

%direct decomposability and the dimension reduction technique through a concrete example. For simplicity, 
Consider an arbitrary large $n$-chain network with interaction graph shown in Figure \ref{fig:chain}. The global system dynamic is described by $x[k+1] = A x[k] + B_2 u[k] + w[k]$, where $A$ is an $n$-dimensional tridiagonal matrix and $B_2$ is identity. We assume that the disturbance $w$ is the zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. The objective function is the expected value of the time-average LQR cost. Let $\tf R$ be the closed loop mapping from $\tf w$ to $\tf x$, and $\tf M$ the closed loop mapping from $\tf w$ to $\tf u$. We showed in \cite{2014_Wang_CDC} that the LQR problem can be formulated as
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize  }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \frac{1}{z} \mathcal{RH}_\infty. \label{eq:lqr}
\end{eqnarray}

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Chain.pdf}
     \caption{The $n$-chain example}
     \label{fig:chain}
\end{figure}
To facilitate the scalability of controller synthesis and implementation of \eqref{eq:lqr}, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within some localized region within $T$ time steps.
For instance, let $\Ell_R$ and $\Ell_M$ be the locality constraints that force the transfer matrices $\tf R$ and $\tf M$ being tridiagonal and pentadiagonal, respectively.
%To make both the controller implementation and controller synthesis of \eqref{eq:lqr} scalable to large systems, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within its within $T$ time steps. For instance, when $d = 2$, we can impose a pentadiagonal sparsity pattern on $\tf R$ and $\tf M$ in \eqref{eq:lqr}. 
This leads to an approximated formulation of \eqref{eq:lqr} given by
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix} \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr}
\end{eqnarray}
%where $\Ell_R$ and $\Ell_M$ are the sparsity constraints that force the transfer matrices $\tf R$ and $\tf M$ being pentadiagonal, respectively.

It can be shown that problem \eqref{eq:llqr} is directly decomposable with respect to arbitrary column-wise partition. By definition, the $j$th column of $\tf R$ and $\tf M$ are the closed loop mapping from $\tf w_j$ to $\tf x$ and $\tf u$, respectively. The direct decomposability of the problem therefore suggests that we can analyze the effect of each local disturbance $w_j$ in an independent and parallel way. More specifically, the direct decomposability of the constraint implies that each disturbance $w_j$ can be analyzed independently to ensure the \emph{feasibility} of the original problem, while the direct decomposability of the objective function further ensures the \emph{optimality} of the original problem when the analysis is performed for each $w_j$ in a distributed way. In the above example, the direct decomposability of the constraint is implied by the superposition principle of LTI systems. The direct decomposability of the objective is from the property of the $\mathcal{H}_2$ norm. It should be noted that a key assumption to make the problem decomposable is that the disturbance $w_j$ are uncorrelated to each other, i.e., $w \sim \mathcal{N}(0,I)$. For a more general case, suppose that we can partition the noise vector into $m$ uncorrelated subsets $\{\Set p_1, \dots, \Set p_m\}$. From Example \ref{ex:perm}, the objective function is directly decomposable with respect to the column-wise partition $\{\Set p_1, \dots, \Set p_m\}$. Therefore, the physical meaning of $\Set p_j$ is the $j$th uncorrelated subset of the noise vector.

%, the objective function is directly decomposable with respect to that partition.
%If the disturbance $w_j$ are correlated to each other globally, then we lose the direct decomposability of the objective function. In the $\mathcal{H}_2$ example, as long as we can partition the noise vector into uncorrelated subsets, the objective function is directly decomposable with respect to that partition.

Once the problem is decomposed, we can analyze each $w_j$ in an independent and parallel way. Without losing generality, we focus on the closed loop response of $w_1$ in the chain example. 
%Here, the locality constraints $\Ell_R$ and $\Ell_M$ allow us to analyze the effect of $w_1$ within its \emph{localized region}. 
Let $a_{ij}$ be the $(i,j)$-th entry of matrix $A$. Using the dimension reduction technique described in the previous subsection, the optimization problem solving the closed loop response of $w_1$ eventually reduces to
\begin{align}
&\underset{\tf v}{\text{minimize}} \quad || \begin{bmatrix} C_1^{'} & D_{12}^{'} \end{bmatrix} \tf v ||_{\mathcal{H}_2}^2 \nonumber\\
&\text{subject to} \quad \tf v \in \FT \cap \frac{1}{z} \mathcal{RH}_\infty \nonumber \\
&\begin{bmatrix} z-a_{11} & -a_{12} & -1 & 0 & 0 \\ -a_{21} & z-a_{22} & 0 & -1 & 0 \\ 0 & -a_{32} & 0 & 0 & -1 \end{bmatrix} \tf v = \begin{bmatrix} 1 \\ 0 \\ 0 \end{bmatrix} \label{eq:llqr-r}
\end{align}
with $\tf v = \begin{bmatrix} \tf R_{11} & \tf R_{21} & \tf M_{11} & \tf M_{21} & \tf M_{31} \end{bmatrix}^\top$ a column vector, and $C_1^{'}$ and $D_{12}^{'}$ some appropriate sub-matrices of $C_1$ and $D_{12}$, respectively. Clearly, the dimension of problem \eqref{eq:llqr-r} is completely independent with respect to the size of the global network $n$. In addition, \eqref{eq:llqr-r} is specified by only some of the entries of $A$, which means that problem \eqref{eq:llqr-r} only depends on the plant model locally.

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Localized2.pdf}
     \caption{The localized region for $w_1$}
     \label{fig:localized}
\end{figure}
The physical interpretation of \eqref{eq:llqr-r} can be illustrated by Figure \ref{fig:localized}. When the locality constraints $\Ell_R$ and $\Ell_M$ are imposed, all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
From the last equality constraint in \eqref{eq:llqr-r}, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$.
%It is clear that we only need to analyze the closed loop response of $w_1$ in the localized region specified in Figure \ref{fig:localized}. 
%Specifically, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$ from the last equality constraint in \eqref{eq:llqr-r}. 
This is a necessary and sufficient condition for the state $x_3$ at the third sub-system to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}, i.e., $\tf R_{31} = 0$. As long as $\tf R_{31} = 0$, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$. In this case, we can analyze the closed loop response of $w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region.
It should be noted that the condition $\tf M_{31} = -a_{32} \tf R_{21}$ is feasible only when the communication speed between sub-controllers is sufficiently faster than the speed of disturbance propagation in the plant. The technical conditions to ensure the feasibility of \eqref{eq:llqr-r} is discussed extensively in the first part of this two-part paper \cite{2015_PartI}.
%to analyze the effect of each local disturbance within its \emph{localized region}. 
%In the above example, the localized region for the disturbance $w_1$ is given by its $2$-outgoing set $\Down{1}{2}$. As long as \eqref{eq:llqr-r} is feasible, the effect of the disturbance $w_1$ is contained within the set $\Down{1}{2}$. Note that there is an implicit boundary constraint imposed by the last equality constraint in \eqref{eq:llqr-r}. Specifically, if $a_{43}$ is nonzero, we must have $\tf R_{31} = 0$. This means that the state $x_3$ has to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}. If this condition can be achieved, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ -- the effect of the disturbance $w_1$ is localized within the set $\Down{1}{2}$. When $\tf R_{31} = 0$, we have $\tf M_{31} = -a_{32} \tf R_{21}$ from the second last equality constraint in \eqref{eq:llqr-r}. This means that we need to apply the control action $u_3$ for disturbance $w_1$ properly to cancel the coupling effect from $x_2$ to $x_3$ in order to make $x_3$ uncorrelated to $w_1$. This implicitly requires the communication speed between the sub-controllers to be faster than the speed of disturbance propagation in the plant. 

%The physical meaning of the set $\Set r_j$ and $\Set t_j$ in \eqref{eq:decom3} can be explained using the $d$-outgoing sets. Suppose that the locality constraint $\Ell$ is $d$-localized and the noise at different subsystem are uncorrelated to each other (which means $\Set p_j = j$). In this case, the set $\Set r_j$ is the collection of optimization variables contained within the localized region $\Down{j}{d}$, and the set $\Set t_j$ is the extended localized region $\Down{j}{d+1}$. %region that can be affected by the variables in $\Set r_j$. In the chain example \eqref{eq:llqr-r}, the set $\Set t_j$ is given by the extended localized region $\Down{j}{d+1}$. 
%As long as the boundary set $\Down{j}{d+1} - \Down{j}{d}$ can be made uncorrelated to the disturbance $w_j$, the closed loop response of $w_j$ can be analyzed completely within its localized region $\Down{j}{d}$.

Combining the column-wise decomposition with dimension reduction, our approach to make the controller synthesis task scalable is to analyze the effect of each uncorrelated disturbance within its own localized region in a parallel way. The direct decomposability of the problem ensures that global optimality is achieved even when these localized regions overlap. 
The scalability and the efficiency of the algorithm primarily depend on the size of each localized region -- the algorithm is more efficient for smaller localized regions. 
The primary role of column-wise decomposition is to make each localized region small. For instance, if we analyze the closed loop response of $w_i$ and $w_j$ simultaneously, then the localized region becomes the union of their own localized regions. If we do not decompose the problem \eqref{eq:llqr} column-wisely first, we cannot reduce the dimension of \eqref{eq:llqr} into \eqref{eq:llqr-r}.

%Take \eqref{eq:llqr} as an example. Recall that $\Ell_R$ and $\Ell_M$ are pentadiagonal sparsity patterns, so $\Ell_R$ and $\Ell_M$ do not possess any zero row. If we do not perform a column-wise decomposition, we cannot reduce the dimension of the problem. On the other hand, if we decompose $\Ell_R$ and $\Ell_M$ column-wisely first, then we can reduce the dimension of each subproblem effectively since each column of $\Ell_R$ and $\Ell_M$ are highly sparse.
%For instance, suppose that the disturbances $\{w_1, w_2, w_3\}$ are correlated to each other, but uncorrelated to any other disturbances. The localized region for the disturbances $\{w_1, w_2, w_3\}$
%Dimension reduction -- localized region (implicit boundary constraint) 
%\input{Physical_v1}

%\subsection{Localized Synthesis and Re-synthesis}
%The controller synthesis procedure for directly decomposable problems is summarized in Algorithm \ref{ag:1}.
%
%%\begin{algorithm}[h!]
%%Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
%%Set feasible = 1\;
%%\For {each state $x_j$}
%%{    
%%     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
%%     \If {not feasible}
%%     {  
%%       feasible = 0\;
%%       break\;
%%     } 
%%}
%%
%%\If {feasible}
%%{    \For {each $j$-th LLQR sub-problem}
%%    {   
%%        Distribute the solution to the local controllers within its localized region \;
%%    }
%%}
%%\caption{Localized Synthesis} \label{ag:1}
%%\end{algorithm}
%\begin{algorithm}[h!]
%Given global plant model $(A, B_2)$, and sparse FIR constraint $\mathcal{S}$\;
%\For {each state perturbation $\delta{x_j}$}
%{    
%     Define localized region based on the block column sparsity of $\mathcal{S}$\;
%     Solve \eqref{eq:llqr-l} and derive $x_\ell, u_\ell$ within its localized region\;
%}
%
%\If {all sub-problems are feasible}
%{
%    \For {each sub-problem}
%    {   
%        Distribute the solution $x_\ell, u_\ell$ to the local controllers within its localized region \;
%    }
%}
%\caption{Localized Controller Synthesis for Directly Decomposable Problems} \label{ag:1}
%\end{algorithm}
%
%%Note that all the for loops in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.
%Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. 
%
%In addition, when the plant model change locally, we only need to resolve \emph{some} of the sub-problems. This suggests the possibility to do real-time \emph{re-synthesis} subject to model change that also maintains global optimality.



==> State_v2.tex <==
%In the previous section, we showed how the constraints $\Ell$ and $\FT$ in \eqref{eq:localized} can be used to enhance the scalability of controller implementation. In the coming two sections, we show that the constraints $\Ell$ and $\FT$ also enhance the scalability of controller synthesis if the objective function $g(\cdot)$ and the localizability constraint $\s$ satisfy certain technical conditions.

In this section, we consider a special case of \eqref{eq:localized} in which either $B_2$ or $C_2$ is invertible. 
The discussion primarily focuses on the state feedback problem, i.e., $C_2 = I$. 
%In this section, we consider a special case of \eqref{eq:LOC} with $C_2 = I$ (state feedback).
We identify the technical conditions on the objective function $g(\cdot)$ and the set constraint $\s = \Ell \cap \FT \cap \Sother$ such that the optimization problem \eqref{eq:localized} can be decomposed directly into parallel local optimization subproblems without using distributed optimization. This technique is crucial for the general algorithm proposed in Section \ref{sec:of}.

The section begins with some mathematical notations that will be used in the rest of the paper. We then introduce the notion of direct decomposability of the objective function and the set constraint. Once the global optimization problem is decomposed into parallel subproblems, we exploit the locality constraint $\Ell$ to further reduce the dimension of each subproblem from global scale to local scale. To help the reader understand the intuition of direct decomposability and the dimension reduction technique, we explain the physical meaning of our method in Section \ref{sec:physical}. 
%This section ends with the summary of localized synthesis and re-synthesis algorithm for directly decomposable problems.

%and the localized controller re-synthesis algorithm to support the plug-and-play feature
%discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Mathematical Notations}
Let $\mathbb{Z}^+$ be the set of all positive integers. We use calligraphic lower case letters such as $\Set q$ to denote subsets of $\mathbb{Z}^+$. 
%The cardinality of a set $\Set q$ is denoted by $| \Set q |$. 
We say that $\{ \Set p_1, \dots \Set p_m \}$ is a partition of a set $\Set q \subset \mathbb{Z}^+$ if and only if $\Set p_i \not = \emptyset$ for all $i$, $\cup_{i=1}^m p_i = \Set q$, and $\Set p_i \cap \Set p_j = \emptyset$ for all $i \not = j$. 

Consider a transfer matrix $\ttf{\Phi}$ with $n_r$ rows and $n_c$ columns. Let $\rowps$ be a subset of $\{1, \dots, n_r \}$ and $\colps$ a subset of $\{1, \dots, n_c \}$. We use $\Sub{\ttf{\Phi}}{\rowps}{\colps}$ to denote the submatrix of $\ttf{\Phi}$ by selecting the rows according to the set $\rowps$ and columns according to the set $\colps$. When $\rowps = \{1, \dots, n_r \}$ is the set of all rows, we use the symbol $:$ to denote the set $\rowps$. Similarly, when $\colps = \{1, \dots, n_c \}$ is the set of all columns, we use $:$ to denote the set $\colps$. We have $\ttf{\Phi} = \Sub{\ttf{\Phi}}{:}{:}$. Let $\{ \colps_1, \dots \colps_p \}$ be a partition of the set $\{1, \dots, n_c\}$. Then $\{ \Sub{\ttf{\Phi}}{:}{\colps_1}, \dots,  \Sub{\ttf{\Phi}}{:}{\colps_p} \}$ is a column-wise partition of the transfer matrix $\ttf{\Phi}$.

%Partition of a set, column/row-wise partition, cardinality of a set, complement of a set
%Submatrices notation, transfer matrices (with FIR constraint)
A permutation matrix is a square binary matrix that has exactly one entry of $1$ in each row and each column and zeros elsewhere.
%Block-wise sparsity pattern, multiplication of sparsity patterns

\subsection{Direct Decomposability}
Assume that the matrix $C_2$ is invertible. In this case, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
\begin{eqnarray}
\tf N &=& [ \tf R (zI-A) - I ] C_2^{-1} \nonumber\\
\tf L &=& \tf M (zI-A) C_2^{-1}. \nonumber
\end{eqnarray}
%For $C_2 = I$, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%\begin{eqnarray}
%\tf N &=& [ \tf R (zI-A) - I ] \nonumber\\
%\tf L &=& \tf M (zI-A). \nonumber
%\end{eqnarray}
%The optimization problem \eqref{eq:LOC} is then simplified into
We then use these relations to simplify the optimization problem \eqref{eq:LOC} into
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && \bar{g}(\tf R, \tf M) \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \bar{\s},\label{eq:sf_lop}
\end{eqnarray}
%for some objective function $\bar{g}(\cdot)$ and localizability constraint $\mathcal{S}'$. 
where $\bar{g}(\cdot)$ is the original objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, and $\bar{\s}$ is the intersection of the set $\s$ and the affine space \eqref{eq:main_2} and \eqref{eq:main_stable}. 
%We sometimes refer to \eqref{eq:sf_lop} a state feedback problem, i.e., $C_2 = I$ is invertible.
%The function $\bar{g}(\cdot)$ in \eqref{eq:sf_lop} is the original convex objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, which is convex. The set $\s'$ is the intersection of the original convex set constraint $\s$ and the affine space \eqref{eq:main_2}, which remains a convex set. Therefore, problem \eqref{eq:sf_lop} remains a convex optimization problem.

\begin{remark}
When $B_2$ is invertible, we can solve \eqref{eq:main_1} analytically to express the transfer matrices $(\tf M, \tf L)$ as a function of $(\tf R, \tf N)$.
%We focus on the state feedback problem (i.e., $C_2 = I$). After solving \eqref{eq:sf_lop}, the controller achieving the desired closed loop response can be implemented by \cite{2015_PartI}
%\begin{eqnarray}
%\tf{\hat{w}} &=& C_2^{-1} (\tf y - \tf{\hat{y}}) \nonumber\\
%\tf u &=& z \tf M \hat{w} \nonumber\\
%\tf{\hat{y}} &=& C_2 (z \tf R - I) \tf{\hat{w}}. \nonumber
%\end{eqnarray}
%Although this implementation holds for arbitrary invertible $C_2$, the computation of the inverse of $C_2$ can be prohibited for large-scale systems unless $C_2$ has certain sparsity structure, e.g., block diagonal.
\end{remark}
%For a state feedback system, we have $C_2 = I$.
%The general formulation for a localized state feedback problem is given by
%In particular, we consider the case in which the localizability constraint $\mathcal{S}$ is a spatio-temporal constraint. We aim to exploit the sparsity of $\mathcal{S}$ to provide a scalable algorithm to solve the optimization problem \eqref{eq:sf_lop}.

To simplify the notation, we use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. We ignore the bar-symbol of $g$ and $\s$ in \eqref{eq:sf_lop} and denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$. The optimization problem \eqref{eq:sf_lop} can then be written as 
\begin{subequations} \label{eq:sf_lop2}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:lop-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = I \label{eq:lop-2} \\
& \ttf{\Phi} \in \s. \label{eq:lop-3}
\end{align}
\end{subequations}
%Here we include the stability constraint $\frac{1}{z}\RHinf$ into the constraint set $\s$ in \eqref{eq:lop-3}. 
%Similar to \eqref{eq:localized}, 
Note that the set constraint $\s$ considered in this section is an intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the remaining convex set constraint $\Sother$, i.e., $\s = \Ell \cap \FT \cap \Sother$.
The goal of this section is to identify the technical conditions on $g(\cdot)$ and $\s$ in \eqref{eq:sf_lop2} so that the global optimization problem \eqref{eq:sf_lop2} can be solved in a localized and distributed way. 

%In addition, the localizability constraint $\s$ is expressed as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.
%We can also express the localizability constraint $\s$ as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.

%\subsubsection{Column-wise Partition}
%In order to make the optimization problem \emph{decomposable}, we make the following assumptions on the problem. 

%In order to solve the optimization problem \eqref{eq:sf_lop2} in an efficient way, we attempt to decompose the problem \eqref{eq:sf_lop2} into several subproblems with smaller scale. 
We first observe that the matrix variable $\ttf{\Phi}$ in constraint \eqref{eq:lop-2} can be examined column at a time. It is then natural to see if the objective \eqref{eq:lop-1} and the set constraint \eqref{eq:lop-3} can also be decomposed in a column-wise manner. This leads to the notion of \emph{direct decomposability} of the problem.
%Let $n_x + n_u$ and $n_x$ denote the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2}. 
%From the definition of the closed loop transfer matrices \eqref{eq:desired}, the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2} are given by $(n_x + n_u)$ and $n_x$, respectively. 
Let $\{ \colps_1, \dots, \colps_p\}$ be a partition of the set $\{1, \dots, n_x\}$. The optimization variable $\ttf{\Phi}$ can then be partitioned column-wisely into a set $\{ \Sub{\ttf{\Phi}}{ : }{\colps_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\colps_p} \}$. The direct decomposability of the objective function in \eqref{eq:sf_lop2} is defined as follows.
\begin{definition} \label{dfn:dd}
The objective function $g(\ttf{\Phi})$ in \eqref{eq:sf_lop2} is said to be \emph{directly decomposable} with respect to the column-wise partition $\{ \colps_1, \dots, \colps_p\}$ if
\begin{equation}
g(\ttf{\Phi}) = \sum_{j=1}^p g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \label{eq:decom_obj}
\end{equation}
for some functions $g_j(\cdot)$ for $j = 1, \dots, p$. 
\end{definition}
%$\Sub{\ttf{\Phi}}{ : }{\colps_j}$
%Consider a column-wise partition $\{ \Phi_j \}_{j=1}^n$ of the closed loop transfer matrix $\Phi$. This partition can be interpreted as a partition of process noise, where $\Phi_j$ is the closed loop transfer matrix from disturbance $\delta{x_j}$ to $[x^\top u^\top]^\top$.
%Given a partition of the global state vector $\{ \colps_j \}_{j=1}^n$, we can decompose the closed loop transfer matrices $(R,M)$ block column-wisely according to the partition $\{ \colps_j \}_{j=1}^n$. Specifically, we use $R_{\colps_j}$ and $M_{\colps_j}$ to denote the $j$th block column of $R$ and $M$, respectively. By definition, $R_{\colps_j}$ and $M_{\colps_j}$ are the closed loop transfer matrices from $\delta{x_{\colps_j}}$ to $x$ and $u$, respectively. 
%Note that the set $\{R_j,M_j\}$ encodes the information of the underlying partition. In the following, we use $\{R_j,M_j\}$ to represent a partition without explicitly specify the partition $\{ \colps_j \}$. 
%We define the decomposable objective function and the decomposable localizability constraint as follows.
%Using this notation, 

Here we give some examples of directly decomposable objective functions. 
\begin{example}
Consider the objective function in \eqref{eq:trad_obj2} with $B_1 = I$ and $D_{21} = 0$. This is the state feedback problem with uncorrelated process noise, i.e., $B_1 = I$. We pick the objective function \eqref{eq:lop-1} as $|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2$. We have
%If we take the square of the $\mathcal{H}_2$ norm of the closed loop map, then the objective function is given by
%One concrete example of a column-wise decomposable objective is the $\mathcal{H}_2$ norm with identity noise matrix $B_1 = I$. For instance, we have
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{p} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\colps_j} ||_{\mathcal{H}_2}^2 \nonumber
\end{equation}
for arbitrary column-wise partition $\{ \colps_1, \dots, \colps_p\}$. This holds for arbitrary $C_1$ and $D_{12}$.
\end{example}
\begin{example} \label{ex:perm}
Continue from the previous example.
%The previous example can be extended to a more general case. 
Suppose that there exists a permutation matrix $\Pi$ such that the matrix $\Pi B_1$ is block diagonal. This happens when the global process noise vector can be partitioned into uncorrelated subsets. The objective function is given by
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} B_1 ||_{\mathcal{H}_2}^2  =  || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} \Pi^\top \Pi B_1 ||_{\mathcal{H}_2}^2. \nonumber
\end{equation}
Note that $\ttf{\Phi} \Pi^\top$ is a column-wise permutation of the optimization variable. We can define a column-wise partition on $\ttf{\Phi} \Pi^\top$ according to the block diagonal structure of the matrix $\Pi B_1$ to decompose the objective function in a column-wise manner. 
\end{example}
\begin{example} \label{ex:l1}
In the previous two examples, we rely on the inherent decomposable property of the $\mathcal{H}_2$ norm. Specifically, the square of the $\mathcal{H}_2$ norm of a FIR transfer matrix $\tf G \in \FT$ is given by
\begin{eqnarray}
|| \tf G ||_{\mathcal{H}_2}^2  &=&  \sum_i \sum_j || \tf g_{ij} ||_{\mathcal{H}_2}^2 \nonumber\\
&=& \sum_i \sum_j \sum_{t=0}^T ( g_{ij}[t] )^2. \label{eq:h2_comp}
\end{eqnarray}
Motivated by the $\mathcal{H}_2$ norm, we define the element-wise $\ell_1$ norm (denoted by $e_1$) of a transfer matrix $\tf G \in \FT$ as
\begin{equation}
|| \tf G ||_{e_1}  =  \sum_i \sum_j \sum_{t=0}^T | g_{ij}[t] |. \nonumber
\end{equation}
The previous two examples still hold if we change the square of the $\mathcal{H}_2$ norm to the element-wise $\ell_1$ norm.
\end{example}

We now define the direct decomposability of the set constraint \eqref{eq:lop-3} as follows.
\begin{definition} \label{dfn:s}
The set constraint $\s$ in \eqref{eq:lop-3} is said to be \emph{directly decomposable} with respect to the column-wise partition $\{ \colps_1, \dots, \colps_p\}$ if the following condition is satisfied:
\begin{equation}
\ttf{\Phi} \in \s \quad \text{if and only if} \quad \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j \text{  for  } j = 1, \dots, p  \nonumber
\end{equation}
for some set $\s_j$ for $j = 1, \dots, p$. Mathematically, this condition is expressed as
\begin{equation}
\ttf{\Phi} \in \s \quad \Longleftrightarrow \quad \bigcap_{j=1}^p \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j.  \label{eq:decom_scon}
\end{equation}
\end{definition}

Equation \eqref{eq:decom_scon} is interpreted as follows. Suppose that the set constraint $\ttf{\Phi} \in \s$ is directly decomposable with respect to the column-wise partition $\{ \colps_1, \dots, \colps_p\}$. To check whether the transfer matrix $\ttf{\Phi}$ belongs to the set $\s$, we can equivalently check whether the set constraint $\Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j$ is satisfied for each $j$. 
\begin{remark}
%Let $\s = \Ell \cap \FT \cap \Sother$ be the localizability constraint in \eqref{eq:sf_lop2}. 
It can be readily shown that the locality constraint $\Ell$ and the FIR constraint $\FT$ are directly decomposable with respect to any column-wise partition. Therefore, the direct decomposability of the set constraint $\s = \Ell \cap \FT \cap \Sother$ in \eqref{eq:sf_lop2} is determined by the direct decomposability of the constraint $\Sother$. If $\s$ is directly decomposable, then we can express the set constraint $\s_j$ in \eqref{eq:decom_scon} as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$ for each $j$.
%For the $j$th element of the partition, we can express the set constraint $\s_j$ as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$.
%We can express the set constraint $\s_j$ as an intersection of the locality constraint, FIR constraint, and other set components as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$.
\end{remark}

Assume that the objective function \eqref{eq:lop-1} and the localizability constraint \eqref{eq:lop-3} are both directly decomposable with respect to a column-wise partition $\{ \colps_1, \dots, \colps_p\}$. The optimization problem \eqref{eq:sf_lop2} can then be partitioned into $p$ parallel subproblems as
\begin{subequations} \label{eq:decom}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{ : }{\colps_j}}{\text{minimize }} \quad & g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \label{eq:decom-1}\\
\text{subject to } \quad & \tf Z_{AB} \Sub{\ttf{\Phi}}{ : }{\colps_j} = \Sub{I}{ : }{\colps_j} \label{eq:decom-2} \\
& \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j \label{eq:decom-3}
\end{align}
\end{subequations}
for $j = 1, \dots, p$. 
%Note that the $p$ subproblems can be computed in an independent and parallel way.
%\begin{eqnarray}
%\underset{\Sub{\ttf{\Phi}}{ : }{\colps_j}}{\text{minimize    }} && g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\colps_j} = \Sub{I}{ : }{\colps_j} \nonumber \\
%&& \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j \label{eq:sf_lopd}
%\end{eqnarray}
%\begin{example}
%Localized LQR with spatio-temporal constraint
%\end{example}
%This is the general formulation for the localized LQR (LLQR) problem proposed in \cite{2014_Wang_CDC}. In \cite{2014_Wang_CDC}, we showed that the global LLQR problem admits a localized decomposition. Specifically, the global LLQR solution can be obtained by solving multiple LLQR sub-problems in a parallel way, with each sub-problem depending only on the \emph{local plant model}. 
%The key observation is noting that the optimization problem \eqref{eq:llqr} admits a \emph{column-wise} decomposition. Specifically, the objective function in \eqref{eq:llqr} can be rewritten as
%\begin{equation}
%\sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber
%\end{equation}
%where the subscript $j$ represents the $j$-th column of the transfer matrix, and $n_x$ is the number of states. Note that the constraints in \eqref{eq:llqr} can be decomposed in a column-wise way as well. Let $\mathcal{S}_j$ denotes the convex set constraint on column $j$. We can solve
%\begin{eqnarray}
%\underset{\{R_j,M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber \\
%&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-s}
%\end{eqnarray}
%for $j = 1, \dots, n_x$ instead of solving \eqref{eq:llqr}, in a parallel way. We now focus on a specific $j$. When $\mathcal{S}_j$ is a locality (sparsity) constraint, we can reduce the dimension of \label{eq:llqr-s} \emph{from global scale to local scale}. 

\subsection{Dimension Reduction} \label{sec:reduction}
%When the problem \eqref{eq:sf_lop2} is directly decomposable, we can partition the original problem \eqref{eq:sf_lop2} into parallel subproblems as in \eqref{eq:decom}. 
Note that each subproblem in \eqref{eq:decom} remains a large-scale optimization problem -- each subproblem in \eqref{eq:decom} depends on the knowledge of the global plant model $\tf Z_{AB}$. In this subsection, we exploit the locality constraint $\Sub{\Ell}{:}{\colps_j}$ in \eqref{eq:decom-3} to reduce the complexity of \eqref{eq:decom}. 
The physical interpretation of the dimension reduction technique is explained in the next subsection.
%In fact, the primary reason to decompose the global optimization problem \eqref{eq:sf_lop2} into parallel subproblems \eqref{eq:decom} is to facilitate the dimensional reduction -- this will be illustrated in the example in the next subsection.

Consider problem \eqref{eq:decom} with a specific $j$. Recall from \eqref{eq:desired} that the number of rows of the transfer matrix $\Sub{\ttf{\Phi}}{:}{\colps_j}$ is given by $(n_x + n_u)$. Let $\bar{\rone}_j$ be the largest subset of $\{1, \dots, n_x + n_u\}$ such that the locality constraint $\Sub{\Ell}{\bar{\rone}_j}{\colps_j}$ in \eqref{eq:decom-3} is exactly a zero matrix. When the locality constraint is imposed, we must have $\Sub{\ttf{\Phi}}{\bar{\rone}_j}{\colps_j} = 0$. This part can be eliminated in the objective \eqref{eq:decom-1} and the constraint \eqref{eq:decom-2}. Let $\rone_j = \{1, \dots, n_x + n_u\} - \bar{\rone}_j$ be the complement set of $\bar{\rone}_j$. When the locality constraint is imposed, problem \eqref{eq:decom} can be simplified into
\begin{subequations} \label{eq:decom2}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}}{\text{minimize }} \quad & \bar{g}_j(\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}) \label{eq:decom2-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{:}{\rone_j} \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} = \Sub{I}{ : }{\colps_j} \label{eq:decom2-2} \\
& \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} \in \Sub{\Ell}{\rone_j}{\colps_j} \cap \FT \cap \bar{\Sother}_j \label{eq:decom2-3}
\end{align}
\end{subequations}
where $\bar{g}_j(\cdot)$ and $\bar{\Sother}_j$ are the restriction of $g_j(\cdot)$ and $\Sother_j$ on the constraint $\Sub{\ttf{\Phi}}{\bar{\rone}_j}{\colps_j} = 0$, respectively. From the definition of the set $\rone_j$, it is straightforward to see that \eqref{eq:decom2} is equivalent to $\eqref{eq:decom}$.

Next, when the system matrices $(A,B_2)$ are fairly sparse, the transfer matrix $\tf Z_{AB}$ is also sparse. Recall that the number of rows of $\tf Z_{AB}$ is given by $n_x$. Let $\bar{\rtwo}_j$ be the largest subset of $\{1, \dots, n_x\}$ such that the augmented matrix $\begin{bmatrix}\Sub{\tf Z_{AB}}{\bar{\rtwo}_j}{\rone_j} & \Sub{I}{\bar{\rtwo}_j}{\colps_j}\end{bmatrix}$ is a zero matrix. Let $\rtwo_j = \{1, \dots, n_x\} - \bar{\rtwo}_j$ be the complement set of $\bar{\rtwo}_j$. We can further reduce \eqref{eq:decom2} into
\begin{subequations} \label{eq:decom3}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}}{\text{minimize }} \quad & \bar{g}_j(\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}) \label{eq:decom3-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{\rtwo_j}{\rone_j} \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} = \Sub{I}{\rtwo_j}{\colps_j} \label{eq:decom3-2} \\
& \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} \in \Sub{\Ell}{\rone_j}{\colps_j} \cap \FT \cap \bar{\Sother}_j. \label{eq:decom3-3}
\end{align}
\end{subequations}
From the definition of the set $\rtwo_j$, we know that \eqref{eq:decom3} is equivalent to \eqref{eq:decom2} and therefore equivalent to \eqref{eq:decom}.

The dimension of \eqref{eq:decom3} is determined by the cardinality of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$. When the locality constraint and the system matrices are highly sparse, it is possible to make the size of these sets much smaller than the size of the global network. In this case, the global optimization problem \eqref{eq:decom} reduces to a local optimization problem \eqref{eq:decom3} which depends on the local plant model $\Sub{\tf Z_{AB}}{\rtwo_j}{\rone_j}$ only. The physical meaning of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$ are explained in detail in the next subsection.
%dimension reduction technique from \eqref{eq:decom} to \eqref{eq:decom3} is explained in detail in the next subsection.
%In the next subsection, we explain the physical meaning of the decomposability assumption from \eqref{eq:sf_lop2} to \eqref{eq:decom} and the dimension reduction from \eqref{eq:decom} to \eqref{eq:decom3}.

\begin{remark} \label{rmk:1}
The dimension reduction algorithm proposed in this paper is a generalization of the algorithms proposed in our prior works \cite{2014_Wang_CDC, 2015_Wang_H2}. Specifically, the algorithms in \cite{2014_Wang_CDC, 2015_Wang_H2} only work for a particular type of locality constraint (called the $d$-localized constraint), while the algorithm proposed here can handle arbitrary sparsity constraint.
\end{remark}

%, and show how to simplify the optimization problem when $\mathcal{S}_j$ is highly sparse. Recall that $\mathcal{S}_j$ is a constraint imposed on the closed loop response from $\delta{x_j}$ to $x$ and $u$. Therefore, the block row-wise sparsity pattern of $\mathcal{S}_j$ encodes the set of affected states and activated control actions under disturbance $\delta{x_j}$. We can construct a localized region, local state vector, and local plant model based on this information. Consider the following illustrative example.

\subsection{Physical Interpretation} \label{sec:physical}
In this subsection, we explain the physical meaning of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$ in \eqref{eq:decom3} through a linear quadratic regulator (LQR) example.
We show that the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector, $\rone_j$ is the collection of optimization variables contained within the localized region defined by the locality constraint $\Sub{\Ell}{:}{\colps_j}$, and $\rtwo_j$ is the set of states that can be directly affected by the variables in $\rone_j$.

%direct decomposability and the dimension reduction technique through a concrete example. For simplicity, 
Consider the $n$-chain example shown in Figure \ref{fig:interconnected}. We assume that each subsystem's state $x_i$ is a scalar.
%network with interaction graph shown in Figure \ref{fig:chain}. 
The global system dynamic is described by $x[t+1] = A x[t] + B_2 u[t] + w[t]$, where $A$ is an $n$-dimensional tridiagonal matrix and $B_2$ is identity. We assume that the disturbance $w$ is a zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. The objective function is the expected value of the time-average LQR cost. Let $\tf R$ be the closed loop mapping from $\tf w$ to $\tf x$, and $\tf M$ the closed loop mapping from $\tf w$ to $\tf u$. We showed in \cite{2014_Wang_CDC} that the LQR problem can be formulated as
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize  }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \frac{1}{z} \mathcal{RH}_\infty. \label{eq:lqr}
\end{eqnarray}

%\begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.35\textwidth]{./figure/Chain.pdf}
%     \caption{The $n$-chain example}
%     \label{fig:chain}
%\end{figure}
To facilitate the scalability of controller synthesis and implementation of \eqref{eq:lqr}, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within some localized region within $T$ time steps.
For instance, let $\Ell_R$ and $\Ell_M$ be the locality constraints that force the transfer matrices $\tf R$ and $\tf M$ being tridiagonal and pentadiagonal, respectively.
%To make both the controller implementation and controller synthesis of \eqref{eq:lqr} scalable to large systems, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within its within $T$ time steps. For instance, when $d = 2$, we can impose a pentadiagonal sparsity pattern on $\tf R$ and $\tf M$ in \eqref{eq:lqr}. 
This leads to an approximation of \eqref{eq:lqr} given by
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix} \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr}
\end{eqnarray}
%where $\Ell_R$ and $\Ell_M$ are the sparsity constraints that force the transfer matrices $\tf R$ and $\tf M$ being pentadiagonal, respectively.

It can be shown that \eqref{eq:llqr} is directly decomposable with respect to arbitrary column-wise partition. By definition, the $j$th column of $\tf R$ and $\tf M$ are the closed loop mapping from $\tf w_j$ to $\tf x$ and $\tf u$, respectively. The direct decomposability of the problem therefore suggests that we can analyze the closed loop response of each local disturbance $w_j$ in an independent and parallel manner. More specifically, the direct decomposability of the constraint implies that each disturbance $w_j$ can be analyzed independently to ensure the \emph{feasibility} of the original problem, while the direct decomposability of the objective function further ensures the \emph{optimality} of the original problem when the analysis is performed for each $w_j$ in a distributed way. In the example of \eqref{eq:llqr}, the direct decomposability of the constraint is implied by the superposition principle of LTI systems. The direct decomposability of the objective follows from the property of the $\mathcal{H}_2$ norm. It should be noted that a key assumption to make the problem decomposable is that the disturbance $w_j$ are uncorrelated to each other, i.e., $w \sim \mathcal{N}(0,I)$. For a more general case, suppose that we can partition the noise vector into $p$ uncorrelated subsets $\{\colps_1, \dots, \colps_p\}$. From Example \ref{ex:perm}, we know that the objective function is directly decomposable with respect to the column-wise partition $\{\colps_1, \dots, \colps_p\}$. Therefore, the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector.

%, the objective function is directly decomposable with respect to that partition.
%If the disturbance $w_j$ are correlated to each other globally, then we lose the direct decomposability of the objective function. In the $\mathcal{H}_2$ example, as long as we can partition the noise vector into uncorrelated subsets, the objective function is directly decomposable with respect to that partition.

Once the problem is decomposed, we analyze the closed loop response of each $w_j$ in an independent and parallel way. Without losing generality, we focus on the closed loop response of $w_1$ in the chain example. 
%Here, the locality constraints $\Ell_R$ and $\Ell_M$ allow us to analyze the effect of $w_1$ within its \emph{localized region}. 
Let $a_{ij}$ be the $(i,j)$-th entry of matrix $A$. Using the dimension reduction technique described in the previous subsection, the optimization problem solving the closed loop response of $w_1$ eventually reduces to
\begin{align}
&\underset{\tf v}{\text{minimize}} \quad || \begin{bmatrix} \bar{C}_1 & \bar{D}_{12} \end{bmatrix} \tf v ||_{\mathcal{H}_2}^2 \nonumber\\
&\text{subject to} \quad \tf v \in \FT \cap \frac{1}{z} \mathcal{RH}_\infty \nonumber \\
&\begin{bmatrix} z-a_{11} & -a_{12} & -1 & 0 & 0 \\ -a_{21} & z-a_{22} & 0 & -1 & 0 \\ 0 & -a_{32} & 0 & 0 & -1 \end{bmatrix} \tf v = \begin{bmatrix} 1 \\ 0 \\ 0 \end{bmatrix} \label{eq:llqr-r}
\end{align}
with $\tf v = \begin{bmatrix} \tf R_{11} & \tf R_{21} & \tf M_{11} & \tf M_{21} & \tf M_{31} \end{bmatrix}^\top$ a column vector, and $\bar{C}_1$ and $\bar{D}_{12}$ some appropriate sub-matrices of $C_1$ and $D_{12}$, respectively. Clearly, the dimension of problem \eqref{eq:llqr-r} is completely independent with respect to the size of the global network $n$. In addition, \eqref{eq:llqr-r} is specified by only some of the entries of $A$, which means that we only need to know some local plant model information to solve \eqref{eq:llqr-r}.
%problem \eqref{eq:llqr-r} only depends on the plant model locally.

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Localized2.pdf}
     \caption{The localized region for $w_1$}
     \label{fig:localized}
\end{figure}
The physical interpretation of \eqref{eq:llqr-r} is illustrated by Figure \ref{fig:localized}. When the locality constraints $\Ell_R$ and $\Ell_M$ are imposed, all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
From the last equality constraint in \eqref{eq:llqr-r}, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$.
%It is clear that we only need to analyze the closed loop response of $w_1$ in the localized region specified in Figure \ref{fig:localized}. 
%Specifically, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$ from the last equality constraint in \eqref{eq:llqr-r}. 
This is a necessary and sufficient condition to make the state $x_3$ at the third sub-system uncorrelated to the disturbance $w_1$ in \emph{closed loop}, i.e., $\tf R_{31} = 0$. As long as $\tf R_{31} = 0$, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ in closed loop. In this case, we can analyze the closed loop response of $w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region.
It should be noted that the condition $\tf M_{31} = -a_{32} \tf R_{21}$ is feasible only when the communication speed between sub-controllers is sufficiently faster than the speed of disturbance propagation in the plant. The technical conditions to ensure the feasibility of \eqref{eq:llqr-r} is discussed extensively in the first part of this two-part paper \cite{2015_PartI}.
%to analyze the effect of each local disturbance within its \emph{localized region}. 
%In the above example, the localized region for the disturbance $w_1$ is given by its $2$-outgoing set $\Down{1}{2}$. As long as \eqref{eq:llqr-r} is feasible, the effect of the disturbance $w_1$ is contained within the set $\Down{1}{2}$. Note that there is an implicit boundary constraint imposed by the last equality constraint in \eqref{eq:llqr-r}. Specifically, if $a_{43}$ is nonzero, we must have $\tf R_{31} = 0$. This means that the state $x_3$ has to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}. If this condition can be achieved, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ -- the effect of the disturbance $w_1$ is localized within the set $\Down{1}{2}$. When $\tf R_{31} = 0$, we have $\tf M_{31} = -a_{32} \tf R_{21}$ from the second last equality constraint in \eqref{eq:llqr-r}. This means that we need to apply the control action $u_3$ for disturbance $w_1$ properly to cancel the coupling effect from $x_2$ to $x_3$ in order to make $x_3$ uncorrelated to $w_1$. This implicitly requires the communication speed between the sub-controllers to be faster than the speed of disturbance propagation in the plant. 
In this example, the set $\rone_1$ is the collection of the colored nodes shown in Figure \ref{fig:localized}, and the set $\rtwo_1$ is the collection of the states contained within the localized region in Figure \ref{fig:localized}.
%The physical meaning of the set $\rone_j$ and $\rtwo_j$ in \eqref{eq:decom3} can be explained using the $d$-outgoing sets. Suppose that the locality constraint $\Ell$ is $d$-localized and the noise at different subsystem are uncorrelated to each other (which means $\colps_j = j$). In this case, the set $\rone_j$ is the collection of optimization variables contained within the localized region $\Down{j}{d}$, and the set $\rtwo_j$ is the extended localized region $\Down{j}{d+1}$. %region that can be affected by the variables in $\rone_j$. In the chain example \eqref{eq:llqr-r}, the set $\rtwo_j$ is given by the extended localized region $\Down{j}{d+1}$. 
%As long as the boundary set $\Down{j}{d+1} - \Down{j}{d}$ can be made uncorrelated to the disturbance $w_j$, the closed loop response of $w_j$ can be analyzed completely within its localized region $\Down{j}{d}$.

Combining the column-wise decomposition with dimension reduction, our approach to make the controller synthesis task scalable is to analyze the closed loop response of each uncorrelated disturbance within its own localized region in a parallel way. The direct decomposability of the problem ensures that global feasibility and optimality are achieved even when the localized regions for each disturbance overlap.
The scalability and the efficiency of the algorithm primarily depend on the size of each localized region -- the algorithm is more efficient for smaller localized regions. 
The primary role of column-wise decomposition is to make each localized region small. For instance, if we analyze the closed loop response of $w_i$ and $w_j$ simultaneously, then the localized region becomes the union of their own localized regions. If we do not decompose the problem \eqref{eq:llqr} column-wisely first, we cannot reduce the dimension of \eqref{eq:llqr} from global scale to local scale.

%Take \eqref{eq:llqr} as an example. Recall that $\Ell_R$ and $\Ell_M$ are pentadiagonal sparsity patterns, so $\Ell_R$ and $\Ell_M$ do not possess any zero row. If we do not perform a column-wise decomposition, we cannot reduce the dimension of the problem. On the other hand, if we decompose $\Ell_R$ and $\Ell_M$ column-wisely first, then we can reduce the dimension of each subproblem effectively since each column of $\Ell_R$ and $\Ell_M$ are highly sparse.
%For instance, suppose that the disturbances $\{w_1, w_2, w_3\}$ are correlated to each other, but uncorrelated to any other disturbances. The localized region for the disturbances $\{w_1, w_2, w_3\}$
%Dimension reduction -- localized region (implicit boundary constraint) 
%\input{Physical_v1}

%\subsection{Localized Synthesis and Re-synthesis}
%The controller synthesis procedure for directly decomposable problems is summarized in Algorithm \ref{ag:1}.
%
%%\begin{algorithm}[h!]
%%Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
%%Set feasible = 1\;
%%\For {each state $x_j$}
%%{    
%%     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
%%     \If {not feasible}
%%     {  
%%       feasible = 0\;
%%       break\;
%%     } 
%%}
%%
%%\If {feasible}
%%{    \For {each $j$-th LLQR sub-problem}
%%    {   
%%        Distribute the solution to the local controllers within its localized region \;
%%    }
%%}
%%\caption{Localized Synthesis} \label{ag:1}
%%\end{algorithm}
%\begin{algorithm}[h!]
%Given global plant model $(A, B_2)$, and sparse FIR constraint $\mathcal{S}$\;
%\For {each state perturbation $\delta{x_j}$}
%{    
%     Define localized region based on the block column sparsity of $\mathcal{S}$\;
%     Solve \eqref{eq:llqr-l} and derive $x_\ell, u_\ell$ within its localized region\;
%}
%
%\If {all sub-problems are feasible}
%{
%    \For {each sub-problem}
%    {   
%        Distribute the solution $x_\ell, u_\ell$ to the local controllers within its localized region \;
%    }
%}
%\caption{Localized Controller Synthesis for Directly Decomposable Problems} \label{ag:1}
%\end{algorithm}
%
%%Note that all the for loops in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.
%Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. 
%
%In addition, when the plant model change locally, we only need to resolve \emph{some} of the sub-problems. This suggests the possibility to do real-time \emph{re-synthesis} subject to model change that also maintains global optimality.



==> State_v3.tex <==
%In the previous section, we showed how the constraints $\Ell$ and $\FT$ in \eqref{eq:localized} can be used to enhance the scalability of controller implementation. In the coming two sections, we show that the constraints $\Ell$ and $\FT$ also enhance the scalability of controller synthesis if the objective function $g(\cdot)$ and the localizability constraint $\s$ satisfy certain technical conditions.

In this section, we consider the state feedback localized SLS problem \eqref{eq:sf_lop}, which is a special case of \eqref{eq:localized}.
%in which the matrix $C_2$ is invertible. In this case, we can solve the constraint \eqref{eq:main_2} analytically and express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%\begin{eqnarray}
%\tf N &=& [ \tf R (zI-A) - I ] C_2^{-1} \nonumber\\
%\tf L &=& \tf M (zI-A) C_2^{-1}. \nonumber
%\end{eqnarray}
%%For $C_2 = I$, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%%\begin{eqnarray}
%%\tf N &=& [ \tf R (zI-A) - I ] \nonumber\\
%%\tf L &=& \tf M (zI-A). \nonumber
%%\end{eqnarray}
%%The optimization problem \eqref{eq:LOC} is then simplified into
%This allows us to simplify the optimization problem \eqref{eq:localized} into
%\begin{eqnarray}
%\underset{\{\tf R, \tf M\}}{\text{minimize    }} && \bar{g}(\tf R, \tf M) \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
%&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \begin{bmatrix} \Ell_R \\ \Ell_M \end{bmatrix} \cap \FT \cap \bar{\Sother},\label{eq:sf_lop}
%\end{eqnarray}
%%for some objective function $\bar{g}(\cdot)$ and localizability constraint $\mathcal{S}'$. 
%where $\bar{g}(\cdot)$ is the original objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, $(\Ell_R, \Ell_M)$ the locality constraint imposed on the transfer matrices $(\tf R, \tf M)$, and $\bar{\Sother}$ the intersection of the set $\Sother$, the affine space \eqref{eq:main_2} and \eqref{eq:main_stable}, and the locality constraint imposed on the system response $(\tf N, \tf L)$. 
%The discussion primarily focuses on the state feedback problem, i.e., $C_2 = I$. 
%In this section, we consider a special case of \eqref{eq:LOC} with $C_2 = I$ (state feedback).
We identify the technical conditions on the SLO and the SLC in \eqref{eq:sf_lop} such that the optimization problem \eqref{eq:sf_lop} can be decomposed into parallel local optimization subproblems without using distributed optimization. This technique is crucial for the general algorithm proposed in Section \ref{sec:of}.

This section begins with the localized linear quadratic regulator (LLQR) as a special case of \eqref{eq:sf_lop} to illustrate the key idea of our optimization decomposition algorithm. We then extend the LLQR to a more general class of problem, which we call the \emph{column-wise separable problems}. This section ends with the highlight of row-wise separable problems as dual of column-wise separable problems.
%discuss the extension of LLQR to more general objectives and constraints. Finally, we introduce the notion of \emph{column-wise separable problems}, and show that we can use the proposed optimization decomposition algorithm to solve column-wise separable problems in a localized and scalable way.
%Finally, we introduce the notion of \emph{column-wise separability} of the problem, and show that a column-wise separable problem can be solved using our optimization decomposition algorithm in a scalable way. 
%We end this section with the notion of column-wise separability of the problem

%some mathematical notations that will be used in the rest of the paper. We then introduce the notion of direct decomposability of the objective function and the set constraint. Once the global optimization problem is decomposed into parallel subproblems, we exploit the locality constraint $\Ell$ to further reduce the dimension of each subproblem from global scale to local scale. To help the reader understand the intuition of direct decomposability and the dimension reduction technique, we explain the physical meaning of our method in Section \ref{sec:physical}. 
%This section ends with the summary of localized synthesis and re-synthesis algorithm for directly decomposable problems.

%and the localized controller re-synthesis algorithm to support the plug-and-play feature
%discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 
%This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Localized Linear Quadratic Regulator} \label{sec:physical}
%In this subsection, we explain the physical meaning of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$ in \eqref{eq:decom3} through a linear quadratic regulator (LQR) example.
%We show that the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector, $\rone_j$ is the collection of optimization variables contained within the localized region defined by the locality constraint $\Sub{\Ell}{:}{\colps_j}$, and $\rtwo_j$ is the set of states that can be directly affected by the variables in $\rone_j$.
%direct decomposability and the dimension reduction technique through a concrete example. For simplicity, 
%Consider the $n$-chain example shown in Figure \ref{fig:interconnected}. We assume that each subsystem's state $x_i$ is a scalar.
%network with interaction graph shown in Figure \ref{fig:chain}. 
%The global system dynamic is described by $x[t+1] = A x[t] + B_2 u[t] + w[t]$, where $A$ is an $n$-dimensional tridiagonal matrix and $B_2$ is identity. We assume that the disturbance $w$ is a zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. The objective function is the expected value of the time-average LQR cost. Let $\tf R$ be the system response from disturbance $\tf w$ to state $\tf x$, and $\tf M$ the system response from disturbance $\tf w$ to control action $\tf u$. We showed in \cite{2014_Wang_CDC} that the traditional LQR problem can be formulated as
Consider the system dynamic equation $x[t+1] = A x[t] + B_2 u[t] + w[t]$ with state feedback. We assume that the disturbance $w$ is a zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. Let $\tf R$ be the system response from disturbance $\tf w$ to state $\tf x$, and $\tf M$ the system response from disturbance $\tf w$ to control action $\tf u$. Let the objective function be the expected value of the time-average energy of the signal $(C_1 \tf x + D_{12} \tf u)$. Then the LQR problem can be formulated as \cite{2014_Wang_CDC}
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize  }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \frac{1}{z} \mathcal{RH}_\infty. \label{eq:lqr}
\end{eqnarray}

%\begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.35\textwidth]{./figure/Chain.pdf}
%     \caption{The $n$-chain example}
%     \label{fig:chain}
%\end{figure}
To facilitate the scalability of controller synthesis and implementation of \eqref{eq:lqr}, we additionally impose a spatiotemporal constraint on the system response to \emph{localize} the effect of each disturbance $w_j$ within some localized region within $T$ time steps.
Let $\Ell_R$ and $\Ell_M$ be the locality constraints imposed on the system response $\tf R$ and $\tf M$, respectively. %When the locality constraint is enforced, we try to localize the response of each disturbance $w_j$ within its two-hop neighbors.
%To make both the controller implementation and controller synthesis of \eqref{eq:lqr} scalable to large systems, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within its within $T$ time steps. For instance, when $d = 2$, we can impose a pentadiagonal sparsity pattern on $\tf R$ and $\tf M$ in \eqref{eq:lqr}. 
The localized LQR (LLQR) \cite{2014_Wang_CDC} problem is then given by
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix} \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr}
\end{eqnarray}
%where $\Ell_R$ and $\Ell_M$ are the sparsity constraints that force the transfer matrices $\tf R$ and $\tf M$ being pentadiagonal, respectively.
Note that \eqref{eq:llqr} is a special case of \eqref{eq:sf_lop}. The goal of this subsection is to propose a scalable algorithm to solve \eqref{eq:llqr}. %exploit the locality constraints $\Ell_R$ and $\Ell_M$ to decompose \eqref{eq:llqr} into parallel local optimization subproblems.

We first notice that \eqref{eq:llqr} admits a \emph{column-wise separation} -- we can solve for the transfer matrices $\tf R$ and $\tf M$ column at a time. Denote $\tf G_j$ the $j$th column of any transfer matrix $\tf G$. The objective in \eqref{eq:llqr} can be written as
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j ||_{\mathcal{H}_2}^2. \nonumber
\end{equation}
%and the constraint in \eqref{eq:llqr} can be checked column at a time. 
This allows us to decompose \eqref{eq:llqr} into $n_x$ parallel subproblems as
\begin{eqnarray}
\underset{\{\tf R_j, \tf M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j = e_j \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix}_j \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty \label{eq:llqr-r}
\end{eqnarray}
for $j = 1, \dots, n_x$. By definition, the $j$th column of $\tf R$ and $\tf M$ are the system response of disturbance $\tf w_j$ to $\tf x$ and $\tf u$, respectively. The column-wise separation property therefore suggests that we can analyze the system response of each local disturbance $w_j$ in an independent and parallel way. This separation property is implied by two different characteristics of the LLQR problem: (i) the system is LTI, so the constraint in \eqref{eq:llqr} admits a column-wise separation, and (ii) the objective function is the LQR cost with uncorrelated disturbances $w \sim \mathcal{N}(0,I)$, which can be separated into column-wise sum as above. 
%Denote $\tf G_j$ the $j$th column of any transfer matrix $\tf G$. 
%More specifically, the direct decomposability of the constraint implies that each disturbance $w_j$ can be analyzed independently to ensure the \emph{feasibility} of the original problem, while the direct decomposability of the objective function further ensures the \emph{optimality} of the original problem when the analysis is performed for each $w_j$ in a distributed way. In the example of \eqref{eq:llqr}, the direct decomposability of the constraint is implied by the superposition principle of LTI systems. The direct decomposability of the objective follows from the property of the $\mathcal{H}_2$ norm. 
%It should be noted that a key assumption to make the problem decomposable is that the disturbance $w_j$ are uncorrelated to each other, i.e., $w \sim \mathcal{N}(0,I)$. For a more general case, suppose that we can partition the noise vector into $p$ uncorrelated subsets $\{\colps_1, \dots, \colps_p\}$. From Example \ref{ex:perm}, we know that the objective function is directly decomposable with respect to the column-wise partition $\{\colps_1, \dots, \colps_p\}$. Therefore, the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector.

%, the objective function is directly decomposable with respect to that partition.
%If the disturbance $w_j$ are correlated to each other globally, then we lose the direct decomposability of the objective function. In the $\mathcal{H}_2$ example, as long as we can partition the noise vector into uncorrelated subsets, the objective function is directly decomposable with respect to that partition.

%Once the problem is decomposed, we analyze the closed loop response of each $w_j$ in an independent and parallel way. 
%Here, the locality constraints $\Ell_R$ and $\Ell_M$ allow us to analyze the effect of $w_1$ within its \emph{localized region}. 
%Let $a_{ij}$ be the $(i,j)$-th entry of matrix $A$. Using the dimension reduction technique described in the previous subsection, the optimization problem solving the closed loop response of $w_1$ eventually reduces to
%\begin{align}
%&\underset{\tf v}{\text{minimize}} \quad || \begin{bmatrix} \bar{C}_1 & \bar{D}_{12} \end{bmatrix} \tf v ||_{\mathcal{H}_2}^2 \nonumber\\
%&\text{subject to} \quad \tf v \in \FT \cap \frac{1}{z} \mathcal{RH}_\infty \nonumber \\
%&\begin{bmatrix} z-a_{11} & -a_{12} & -1 & 0 & 0 \\ -a_{21} & z-a_{22} & 0 & -1 & 0 \\ 0 & -a_{32} & 0 & 0 & -1 \end{bmatrix} \tf v = \begin{bmatrix} 1 \\ 0 \\ 0 \end{bmatrix} \label{eq:llqr-r}
%\end{align}
%with $\tf v = \begin{bmatrix} \tf R_{11} & \tf R_{21} & \tf M_{11} & \tf M_{21} & \tf M_{31} \end{bmatrix}^\top$ a column vector, and $\bar{C}_1$ and $\bar{D}_{12}$ some appropriate sub-matrices of $C_1$ and $D_{12}$, respectively. Clearly, the dimension of problem \eqref{eq:llqr-r} is completely independent with respect to the size of the global network $n$. In addition, \eqref{eq:llqr-r} is specified by only some of the entries of $A$, which means that we only need to know some local plant model information to solve \eqref{eq:llqr-r}.
%problem \eqref{eq:llqr-r} only depends on the plant model locally.

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Localized3.pdf}
     \caption{The localized region for $w_1$}
     \label{fig:localized}
\end{figure}
For each subproblem in \eqref{eq:llqr-r}, we can further exploit the locality constraint to reduce the dimension of each subproblem from global scale to local scale. The technical details of the dimensional reduction algorithm can be found in our prior work \cite{2014_Wang_CDC}, and we will discuss a generalized version in the next subsection and in Appendix \ref{sec:reduction}. 
%and the issues regarding the feasibility of each \eqref{eq:llqr-r} is discussed in \cite{2015_Wang_Reg}. 
Here we just illustrate the idea through a simple example.
\begin{example}
Consider a chain of $n$ LTI subsystems with a single local disturbance $\tf w_1$. In \eqref{eq:llqr-r}, the optimization variables are the system response from the disturbance $\tf w_1$ to the global state $\tf x$ and global control action $\tf u$.  Assume that the locality constraint in \eqref{eq:llqr-r} is given by $x_3 = \dots = x_n = 0$ and $u_4 = \dots = u_n = 0$. In this case, we can solve \eqref{eq:llqr-r} using only the information contained within the localized region shown in Figure \ref{fig:localized}. Intuitively, as long as the boundary constraint $x_3 = 0$ is enforced, the system response of $w_1$ can never escape from the localized region. In other words, the condition $x_i = 0$ for $i = 4, \dots n$ is implicitly implied by the boundary constraint $x_3 = 0$. In order to make $x_3$ unaffected by the disturbance $w_1$, the actuator $u_3$ at the third subsystem must actuate properly to cancel the coupling from the state $x_2$ at the second subsystem. 
Finally, as the system is LTI, we can analyze the system response for each $w_j$ within its own localized region, and use superposition principle to compute the system response for arbitrary linear combination of disturbances. 
\end{example}


%%%%%%%%%%
%Without loss of generality, we focus on the first subproblem $j = 1$ of \eqref{eq:llqr-r}, which corresponds to the system response of $w_1$. Recall that we enforce the locality constraint $(\Ell_R, \Ell_M)$ to localize the response of each local disturbance to its two-hop neighbors. We plot the desired response of $w_1$ in Figure \ref{fig:localized}, where all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
%The physical interpretation of \eqref{eq:llqr-r} is illustrated by Figure \ref{fig:localized}. When the locality constraints $\Ell_R$ and $\Ell_M$ are imposed, all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
%From the last equality constraint in \eqref{eq:llqr-r}, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$.
%It is clear that we only need to analyze the closed loop response of $w_1$ in the localized region specified in Figure \ref{fig:localized}. 
%Specifically, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$ from the last equality constraint in \eqref{eq:llqr-r}. 
%This is a necessary and sufficient condition to make 
%Note that we require the state $x_3$ at the third sub-system to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}, i.e., $\tf R_{31} = 0$. Implicit in this statement is the requirement of fast enough information sharing between sub-controllers. 
%Figure \ref{fig:delay} shows the information delay (the sum of the sensing delay from $x_1$ to $u_1$, the communication delay from $u_1$ to $u_3$, and the actuation delay from $u_3$ to $x_3$) and the physical delay (the delay from $x_1$ to $x_3$ through dynamic coupling) between the first three sub-systems of the chain.
%We require the information delay to be \emph{less than or equal to} the physical delay. In this case, the sub-controller $\tf u_3$ at the third sub-system receives advanced warning about the disturbance information $\tf w_1$ from the first sub-controller. The sub-controller $\tf u_3$ can then apply suitable control action to cancel the disturbance propagating through the second sub-system $\tf x_2$, and make the state $\tf x_3$ unaffected by the disturbance $\tf w_1$ in closed loop. As long as the state $\tf x_3$ is unaffected by the disturbance $\tf w_1$ in closed loop, all the state $\tf x_i$ for $i > 3$ are unaffected by the disturbance $\tf w_1$ in closed loop. 
%In this situation, we can analyze the system response of $\tf w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region. In particular, the complexity of analyzing the system response of $\tf w_1$ is independent to the size of the chain network, which means that our algorithm is scalable to arbitrary large network. From \eqref{eq:llqr-r}, we can analyze the system response for each $\tf w_j$ in their own localized region in a parallel way. The feasibility and optimality of the original problem \eqref{eq:llqr} are achieved even when the localized regions of each disturbance overlap.

%\begin{figure}[h!]
%      \centering
%      \includegraphics[width=0.4\textwidth]{./figure/Delay2.pdf}
%      \caption{Information delay and physical delay}
%      \label{fig:delay}
%\end{figure}

%As long as $\tf R_{31} = 0$, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ in closed loop. In this case, we can analyze the closed loop response of $w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region.
%It should be noted that the condition $\tf M_{31} = -a_{32} \tf R_{21}$ is feasible only when the communication speed between sub-controllers is sufficiently faster than the speed of disturbance propagation in the plant. The technical conditions to ensure the feasibility of \eqref{eq:llqr-r} is discussed extensively in the first part of this two-part paper \cite{2015_PartI}.
%to analyze the effect of each local disturbance within its \emph{localized region}. 
%In the above example, the localized region for the disturbance $w_1$ is given by its $2$-outgoing set $\Down{1}{2}$. As long as \eqref{eq:llqr-r} is feasible, the effect of the disturbance $w_1$ is contained within the set $\Down{1}{2}$. Note that there is an implicit boundary constraint imposed by the last equality constraint in \eqref{eq:llqr-r}. Specifically, if $a_{43}$ is nonzero, we must have $\tf R_{31} = 0$. This means that the state $x_3$ has to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}. If this condition can be achieved, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ -- the effect of the disturbance $w_1$ is localized within the set $\Down{1}{2}$. When $\tf R_{31} = 0$, we have $\tf M_{31} = -a_{32} \tf R_{21}$ from the second last equality constraint in \eqref{eq:llqr-r}. This means that we need to apply the control action $u_3$ for disturbance $w_1$ properly to cancel the coupling effect from $x_2$ to $x_3$ in order to make $x_3$ uncorrelated to $w_1$. This implicitly requires the communication speed between the sub-controllers to be faster than the speed of disturbance propagation in the plant. 
%In this example, the set $\rone_1$ is the collection of the colored nodes shown in Figure \ref{fig:localized}, and the set $\rtwo_1$ is the collection of the states contained within the localized region in Figure \ref{fig:localized}.
%The physical meaning of the set $\rone_j$ and $\rtwo_j$ in \eqref{eq:decom3} can be explained using the $d$-outgoing sets. Suppose that the locality constraint $\Ell$ is $d$-localized and the noise at different subsystem are uncorrelated to each other (which means $\colps_j = j$). In this case, the set $\rone_j$ is the collection of optimization variables contained within the localized region $\Down{j}{d}$, and the set $\rtwo_j$ is the extended localized region $\Down{j}{d+1}$. %region that can be affected by the variables in $\rone_j$. In the chain example \eqref{eq:llqr-r}, the set $\rtwo_j$ is given by the extended localized region $\Down{j}{d+1}$. 
%As long as the boundary set $\Down{j}{d+1} - \Down{j}{d}$ can be made uncorrelated to the disturbance $w_j$, the closed loop response of $w_j$ can be analyzed completely within its localized region $\Down{j}{d}$.

In summary, our approach to make the LLQR synthesis task scalable consists of two steps: (i) we perform a \emph{column-wise separation} of the problem, which allows us to analyze the system response of each local disturbance in an independent and parallel way, and (ii) we exploit the locality constraint $\Ell_R$ and $\Ell_M$ in \eqref{eq:llqr-r} to analyze the response of each local disturbance within its own localized region. 

%In the rest of this section, we generalize the LLQR problem to a broader class of problem which we called \emph{column-wise separable problems}. We show that all the column-wise separable problem can be solved using this decomposition technique in a localized and scalable way.

%to analyze the closed loop response of each uncorrelated disturbance within its own localized region in a parallel way. The direct decomposability of the problem ensures that global feasibility and optimality are achieved even when the localized regions for each disturbance overlap.
%The scalability and the efficiency of the algorithm primarily depend on the size of each localized region -- the algorithm is more efficient for smaller localized regions. 
%The primary role of column-wise decomposition is to make each localized region small. For instance, if we analyze the closed loop response of $w_i$ and $w_j$ simultaneously, then the localized region becomes the union of their own localized regions. If we do not decompose the problem \eqref{eq:llqr} column-wisely first, we cannot reduce the dimension of \eqref{eq:llqr} from global scale to local scale.

%Take \eqref{eq:llqr} as an example. Recall that $\Ell_R$ and $\Ell_M$ are pentadiagonal sparsity patterns, so $\Ell_R$ and $\Ell_M$ do not possess any zero row. If we do not perform a column-wise decomposition, we cannot reduce the dimension of the problem. On the other hand, if we decompose $\Ell_R$ and $\Ell_M$ column-wisely first, then we can reduce the dimension of each subproblem effectively since each column of $\Ell_R$ and $\Ell_M$ are highly sparse.
%For instance, suppose that the disturbances $\{w_1, w_2, w_3\}$ are correlated to each other, but uncorrelated to any other disturbances. The localized region for the disturbances $\{w_1, w_2, w_3\}$
%Dimension reduction -- localized region (implicit boundary constraint) 
%\input{Physical_v1}

%\subsection{Localized Synthesis and Re-synthesis}
%The controller synthesis procedure for directly decomposable problems is summarized in Algorithm \ref{ag:1}.
%
%%\begin{algorithm}[h!]
%%Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
%%Set feasible = 1\;
%%\For {each state $x_j$}
%%{    
%%     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
%%     \If {not feasible}
%%     {  
%%       feasible = 0\;
%%       break\;
%%     } 
%%}
%%
%%\If {feasible}
%%{    \For {each $j$-th LLQR sub-problem}
%%    {   
%%        Distribute the solution to the local controllers within its localized region \;
%%    }
%%}
%%\caption{Localized Synthesis} \label{ag:1}
%%\end{algorithm}
%\begin{algorithm}[h!]
%Given global plant model $(A, B_2)$, and sparse FIR constraint $\mathcal{S}$\;
%\For {each state perturbation $\delta{x_j}$}
%{    
%     Define localized region based on the block column sparsity of $\mathcal{S}$\;
%     Solve \eqref{eq:llqr-l} and derive $x_\ell, u_\ell$ within its localized region\;
%}
%
%\If {all sub-problems are feasible}
%{
%    \For {each sub-problem}
%    {   
%        Distribute the solution $x_\ell, u_\ell$ to the local controllers within its localized region \;
%    }
%}
%\caption{Localized Controller Synthesis for Directly Decomposable Problems} \label{ag:1}
%\end{algorithm}
%
%%Note that all the for loops in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.
%Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. 
%
%In addition, when the plant model change locally, we only need to resolve \emph{some} of the sub-problems. This suggests the possibility to do real-time \emph{re-synthesis} subject to model change that also maintains global optimality.

%\subsection{Extensions Beyond LLQR}
%In this subsection, we highlight the generalization of LLQR to a more broader class of problem, which we call the column-wise separable problem. 
%Let $\mathbb{Z}^+$ be the set of all positive integers. We use calligraphic lower case letters such as $\Set q$ to denote subsets of $\mathbb{Z}^+$. 
%%The cardinality of a set $\Set q$ is denoted by $| \Set q |$. 
%We say that $\{ \Set p_1, \dots \Set p_m \}$ is a partition of a set $\Set q \subset \mathbb{Z}^+$ if and only if $\Set p_i \not = \emptyset$ for all $i$, $\cup_{i=1}^m \Set p_i = \Set q$, and $\Set p_i \cap \Set p_j = \emptyset$ for all $i \not = j$. 
%
%Consider a transfer matrix $\ttf{\Phi}$ with $n_r$ rows and $n_c$ columns. Let $\rowps$ be a subset of $\{1, \dots, n_r \}$ and $\colps$ a subset of $\{1, \dots, n_c \}$. We use $\Sub{\ttf{\Phi}}{\rowps}{\colps}$ to denote the submatrix of $\ttf{\Phi}$ by selecting the rows according to the set $\rowps$ and columns according to the set $\colps$. When $\rowps = \{1, \dots, n_r \}$ is the set of all rows, we use the symbol $:$ to denote the set $\rowps$. Similarly, when $\colps = \{1, \dots, n_c \}$ is the set of all columns, we use $:$ to denote the set $\colps$. We have $\ttf{\Phi} = \Sub{\ttf{\Phi}}{:}{:}$. Let $\{ \colps_1, \dots \colps_p \}$ be a partition of the set $\{1, \dots, n_c\}$. Then $\{ \Sub{\ttf{\Phi}}{:}{\colps_1}, \dots,  \Sub{\ttf{\Phi}}{:}{\colps_p} \}$ is a column-wise partition of the transfer matrix $\ttf{\Phi}$.
%
%%Partition of a set, column/row-wise partition, cardinality of a set, complement of a set
%%Submatrices notation, transfer matrices (with FIR constraint)
%A permutation matrix is a square binary matrix that has exactly one entry of $1$ in each row and each column and zeros elsewhere.
%Block-wise sparsity pattern, multiplication of sparsity patterns

\subsection{Column-wise Separable Problems} \label{sec:CWSP}
%Assume that the matrix $C_2$ is invertible. In this case, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%\begin{eqnarray}
%\tf N &=& [ \tf R (zI-A) - I ] C_2^{-1} \nonumber\\
%\tf L &=& \tf M (zI-A) C_2^{-1}. \nonumber
%\end{eqnarray}
%%For $C_2 = I$, we can solve the constraint \eqref{eq:main_2} analytically to express the transfer matrices $(\tf N, \tf L)$ as a function of $(\tf R, \tf M)$ by
%%\begin{eqnarray}
%%\tf N &=& [ \tf R (zI-A) - I ] \nonumber\\
%%\tf L &=& \tf M (zI-A). \nonumber
%%\end{eqnarray}
%%The optimization problem \eqref{eq:LOC} is then simplified into
%We then use these relations to simplify the optimization problem \eqref{eq:LOC} into
%\begin{eqnarray}
%\underset{\{\tf R, \tf M\}}{\text{minimize    }} && \bar{g}(\tf R, \tf M) \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
%&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \bar{\s},\label{eq:sf_lop}
%\end{eqnarray}
%%for some objective function $\bar{g}(\cdot)$ and localizability constraint $\mathcal{S}'$. 
%where $\bar{g}(\cdot)$ is the original objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, and $\bar{\s}$ is the intersection of the set $\s$ and the affine space \eqref{eq:main_2} and \eqref{eq:main_stable}. 
%%We sometimes refer to \eqref{eq:sf_lop} a state feedback problem, i.e., $C_2 = I$ is invertible.
%%The function $\bar{g}(\cdot)$ in \eqref{eq:sf_lop} is the original convex objective function $g(\cdot)$ restricted on the affine space defined by \eqref{eq:main_2}, which is convex. The set $\s'$ is the intersection of the original convex set constraint $\s$ and the affine space \eqref{eq:main_2}, which remains a convex set. Therefore, problem \eqref{eq:sf_lop} remains a convex optimization problem.
%For a state feedback system, we have $C_2 = I$.
%The general formulation for a localized state feedback problem is given by
%In particular, we consider the case in which the localizability constraint $\mathcal{S}$ is a spatio-temporal constraint. We aim to exploit the sparsity of $\mathcal{S}$ to provide a scalable algorithm to solve the optimization problem \eqref{eq:sf_lop}.
%We note that a key assumption in the LLQR problem \eqref{eq:llqr} is that the disturbances $w_i$ and $w_j$ are uncorrelated to each other.
We now extend the LLQR to the state feedback localized SLS problem \eqref{eq:sf_lop}. The goal of this subsection is to identify the technical conditions on $g(\cdot)$ and $\Sother$ in \eqref{eq:sf_lop} so that the global optimization problem \eqref{eq:sf_lop} can be solved in a localized and distributed way using the column-wise separation method introduced in the previous subsection.
To simplify the notation of \eqref{eq:sf_lop}, we use
\begin{equation}
\ttf{\Phi} = \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \nonumber
\end{equation}
to represent the system response we want to optimize for, and we denote $\tf Z_{AB}$ the transfer matrix $\begin{bmatrix} zI-A & -B_2 \end{bmatrix}$. The state feedback localized SLS problem \eqref{eq:sf_lop} can then be written as 
\begin{subequations} \label{eq:sf_lop2}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:lop-1}\\
\text{subject to } \quad & \tf Z_{AB} \ttf{\Phi} = I \label{eq:lop-2} \\
& \ttf{\Phi} \in \s, \label{eq:lop-3}
\end{align}
\end{subequations}
%Here we include the stability constraint $\frac{1}{z}\RHinf$ into the constraint set $\s$ in \eqref{eq:lop-3}. 
%Similar to \eqref{eq:localized},
with $\s = \Ell \cap \FT \cap \Sother$.
%Note that the set constraint $\s$ considered in this subsection is an intersection of the locality constraint $\Ell$, the FIR constraint $\FT$, and the remaining convex set constraint $\Sother$, i.e., $\s = \Ell \cap \FT \cap \Sother$.

%In addition, the localizability constraint $\s$ is expressed as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.
%We can also express the localizability constraint $\s$ as an intersection of the locality constraint $\Ell$, FIR constraint $\FT$, and other convex set constraint $\Sother$ as in \eqref{eq:localized}.

%\subsubsection{Column-wise Partition}
%In order to make the optimization problem \emph{decomposable}, we make the following assumptions on the problem. 

%In order to solve the optimization problem \eqref{eq:sf_lop2} in an efficient way, we attempt to decompose the problem \eqref{eq:sf_lop2} into several subproblems with smaller scale. 
Similar to the LLQR problem, we note that the matrix variable $\ttf{\Phi}$ in constraint \eqref{eq:lop-2} can be examined column at a time. It is then natural to see if the SLO \eqref{eq:lop-1} and the SLC \eqref{eq:lop-3} can also be decomposed in a column-wise manner. 
More generally, we note that it suffices to find a column-wise \emph{partition} of the optimization variable to decompose \eqref{eq:sf_lop2} into parallel subproblems. Recall that we use calligraphic lower case letters such as $\Set c$ to denote subsets of positive integer. 
%This leads to the notion of \emph{column-wise separable problems}.
%Let $n_x + n_u$ and $n_x$ denote the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2}. 
%From the definition of the closed loop transfer matrices \eqref{eq:desired}, the number of rows and columns of the transfer matrix $\ttf{\Phi}$ in \eqref{eq:sf_lop2} are given by $(n_x + n_u)$ and $n_x$, respectively. 
Let $\{ \colps_1, \dots, \colps_p\}$ be a partition of the set $\{1, \dots, n_x\}$. The optimization variable $\ttf{\Phi}$ can then be partitioned column-wisely into the set $\{ \Sub{\ttf{\Phi}}{ : }{\colps_1}, \dots, \Sub{\ttf{\Phi}}{ : }{\colps_p} \}$. The column-wise separability of the SLO \eqref{eq:lop-1} is defined as follows.
\begin{definition} \label{dfn:dd}
The system level objective $g(\ttf{\Phi})$ in \eqref{eq:lop-1} is said to be \emph{column-wise separable} with respect to the column-wise partition $\{ \colps_1, \dots, \colps_p\}$ if
\begin{equation}
g(\ttf{\Phi}) = \sum_{j=1}^p g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \label{eq:decom_obj}
\end{equation}
for some functionals $g_j(\cdot)$ for $j = 1, \dots, p$. 
\end{definition}
%$\Sub{\ttf{\Phi}}{ : }{\colps_j}$
%Consider a column-wise partition $\{ \Phi_j \}_{j=1}^n$ of the closed loop transfer matrix $\Phi$. This partition can be interpreted as a partition of process noise, where $\Phi_j$ is the closed loop transfer matrix from disturbance $\delta{x_j}$ to $[x^\top u^\top]^\top$.
%Given a partition of the global state vector $\{ \colps_j \}_{j=1}^n$, we can decompose the closed loop transfer matrices $(R,M)$ block column-wisely according to the partition $\{ \colps_j \}_{j=1}^n$. Specifically, we use $R_{\colps_j}$ and $M_{\colps_j}$ to denote the $j$th block column of $R$ and $M$, respectively. By definition, $R_{\colps_j}$ and $M_{\colps_j}$ are the closed loop transfer matrices from $\delta{x_{\colps_j}}$ to $x$ and $u$, respectively. 
%Note that the set $\{R_j,M_j\}$ encodes the information of the underlying partition. In the following, we use $\{R_j,M_j\}$ to represent a partition without explicitly specify the partition $\{ \colps_j \}$. 
%We define the decomposable objective function and the decomposable localizability constraint as follows.
%Using this notation, 

We note that the objective functional of the LLQR problem \eqref{eq:llqr} is column-wise separable with respect to arbitrary column-wise partition. Here we give some more examples of column-wise separable SLOs. 
%\begin{example}
%Consider the objective function in \eqref{eq:trad_obj2} with $B_1 = I$ and $D_{21} = 0$. This is the state feedback problem with uncorrelated process noise, i.e., $B_1 = I$. We pick the objective function \eqref{eq:lop-1} as $|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2$. We have
%%If we take the square of the $\mathcal{H}_2$ norm of the closed loop map, then the objective function is given by
%%One concrete example of a column-wise decomposable objective is the $\mathcal{H}_2$ norm with identity noise matrix $B_1 = I$. For instance, we have
%\begin{equation}
%|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{p} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\colps_j} ||_{\mathcal{H}_2}^2 \nonumber
%\end{equation}
%for arbitrary column-wise partition $\{ \colps_1, \dots, \colps_p\}$. This holds for arbitrary $C_1$ and $D_{12}$.
%\end{example}
\begin{example} \label{ex:perm}
Consider the LLQR problem \eqref{eq:llqr}, but now we assume that the covariance of the disturbance is given by $B_1^\top B_1$ for some matrix $B_1$, i.e., $w \sim \mathcal{N}(0,B_1^\top B_1)$. 
%Continue from the previous example.
%The previous example can be extended to a more general case. 
In addition, suppose that there exists a permutation matrix $\Pi$ such that the matrix $\Pi B_1$ is block diagonal. This happens when the global noise vector $\tf w$ can be partitioned into uncorrelated subsets. The objective is given by
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} B_1 ||_{\mathcal{H}_2}^2  =  || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \ttf{\Phi} \Pi^\top \Pi B_1 ||_{\mathcal{H}_2}^2. \nonumber
\end{equation}
Note that $\ttf{\Phi} \Pi^\top$ is a column-wise permutation of the optimization variable. We can define a column-wise partition on $\ttf{\Phi} \Pi^\top$ according to the block diagonal structure of the matrix $\Pi B_1$ to decompose the objective in a column-wise manner. 
\end{example}
\begin{example} \label{ex:l1}
In the LLQR examples, we rely on the inherent separable property of the $\mathcal{H}_2$ norm. Specifically, the square of the $\mathcal{H}_2$ norm of a FIR transfer matrix $\tf G \in \FT$ is given by
\begin{equation}
|| \tf G ||_{\mathcal{H}_2}^2  =  \sum_i \sum_j || \tf g_{ij} ||_{\mathcal{H}_2}^2 =  \sum_i \sum_j \sum_{t=0}^T ( g_{ij}[t] )^2. \label{eq:h2_comp}
\end{equation}
Motivated by the $\mathcal{H}_2$ norm, we define the element-wise $\ell_1$ norm (denoted by $e_1$) of a transfer matrix $\tf G \in \FT$ as
\begin{equation}
|| \tf G ||_{e_1}  =  \sum_i \sum_j \sum_{t=0}^T | g_{ij}[t] |. \nonumber
\end{equation}
The previous example still holds if we change the square of the $\mathcal{H}_2$ norm to the element-wise $\ell_1$ norm.
\end{example}

The column-wise separability of the SLC \eqref{eq:lop-3} is defined as follows.
\begin{definition} \label{dfn:s}
The system level constraint $\s$ in \eqref{eq:lop-3} is said to be \emph{column-wise separable} with respect to the column-wise partition $\{ \colps_1, \dots, \colps_p\}$ if the following condition is satisfied:
\begin{equation}
\ttf{\Phi} \in \s \quad \text{if and only if} \quad \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j \text{  for  } j = 1, \dots, p  \nonumber
\end{equation}
for some sets $\s_j$ for $j = 1, \dots, p$. Mathematically, this condition is expressed as
\begin{equation}
\ttf{\Phi} \in \s \quad \Longleftrightarrow \quad \bigcap_{j=1}^p \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j.  \label{eq:decom_scon}
\end{equation}
\end{definition}

Equation \eqref{eq:decom_scon} is interpreted as follows. Suppose that the SLC $\ttf{\Phi} \in \s$ is column-wise separable with respect to the partition $\{ \colps_1, \dots, \colps_p\}$. To check whether the transfer matrix $\ttf{\Phi}$ belongs to the set $\s$, we can equivalently check whether the set constraint $\Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j$ is satisfied for each $j$. 
\begin{remark}
%Let $\s = \Ell \cap \FT \cap \Sother$ be the localizability constraint in \eqref{eq:sf_lop2}. 
It can be readily shown that the locality constraint $\Ell$ and the FIR constraint $\FT$ are column-wise separable with respect to any column-wise partition. Therefore, the column-wise separability of the SLC $\s = \Ell \cap \FT \cap \Sother$ in \eqref{eq:sf_lop2} is determined by the column-wise separability of the constraint $\Sother$. If $\s$ is column-wise separable, then we can express the set constraint $\s_j$ in \eqref{eq:decom_scon} as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$ for each $j$.
%For the $j$th element of the partition, we can express the set constraint $\s_j$ as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$ for some $\Sother_j$.
%We can express the set constraint $\s_j$ as an intersection of the locality constraint, FIR constraint, and other set components as $\s_j = \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j$.
\end{remark}

Assume that the SLO \eqref{eq:lop-1} and the SLC \eqref{eq:lop-3} are both column-wise separable with respect to a column-wise partition $\{ \colps_1, \dots, \colps_p\}$. In this case, we say that the state feedback localized SLS problem \eqref{eq:sf_lop2} is a \emph{column-wise separable problem}. Specifically, \eqref{eq:sf_lop2} can be partitioned into $p$ parallel subproblems as
\begin{subequations} \label{eq:decom}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{ : }{\colps_j}}{\text{minimize }} \quad & g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \label{eq:decom-1}\\
\text{subject to } \quad & \tf Z_{AB} \Sub{\ttf{\Phi}}{ : }{\colps_j} = \Sub{I}{ : }{\colps_j} \label{eq:decom-2} \\
& \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \Sub{\Ell}{:}{\colps_j} \cap \FT \cap \Sother_j \label{eq:decom-3}
\end{align}
\end{subequations}
for $j = 1, \dots, p$. 

Then, similar to the LLQR method, we exploit the locality constraint $\Sub{\Ell}{:}{\colps_j}$ in \eqref{eq:decom-3} to reduce the dimension of \eqref{eq:decom} for each $j$ from global scale to local scale. 
%The dimension reduction algorithm for certain class of locality constraint has been proposed in our prior works \cite{2014_Wang_CDC, 2015_Wang_H2}. 
We defer a detailed dimension reduction algorithm for arbitrary locality constraint in Appendix \ref{sec:reduction}. Here we just highlight the results.
In Appendix \ref{sec:reduction}, we show that the optimization subproblem \eqref{eq:decom} can be reduced into
\begin{subequations} \label{eq:decom40}
\begin{align} 
\underset{\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}}{\text{minimize }} \quad & \bar{g}_j(\Sub{\ttf{\Phi}}{\rone_j}{\colps_j}) \label{eq:decom40-1}\\
\text{subject to } \quad & \Sub{\tf Z_{AB}}{\rtwo_j}{\rone_j} \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} = \Sub{I}{\rtwo_j}{\colps_j} \label{eq:decom40-2} \\
& \Sub{\ttf{\Phi}}{\rone_j}{\colps_j} \in \Sub{\Ell}{\rone_j}{\colps_j} \cap \FT \cap \bar{\Sother}_j \label{eq:decom40-3}
\end{align}
\end{subequations}
where $\rone_j$ and $\rtwo_j$ are sets of positive integer defined in Appendix \ref{sec:reduction}, and $\bar{g}_j$ and $\bar{\Sother}_j$ the objective and constraint in the reduced dimension, respectively. 
Roughly speaking, the set $\rone_j$ is the collection of optimization variables contained within the localized region specified by $\Sub{\Ell}{:}{\colps_j}$, and the set $\rtwo_j$ is the collection of states that are directly affected by the optimization variables in $\rone_j$.
The complexity of solving \eqref{eq:decom40} is determined by the cardinality of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$, which are determined by the sparsity of the locality constraint and the system matrices. For instance, the cardinality of the set $\rone_j$ is equal to the number of nonzero rows of the locality constraint $\Sub{\Ell}{:}{\colps_j}$.
When the locality constraint and the system matrices are suitably sparse, it is possible to make the size of these sets much smaller than the size of the global network. In this case, the global optimization subproblem \eqref{eq:decom} reduces to a local optimization subproblem \eqref{eq:decom40} which depends on the local plant model $\Sub{\tf Z_{AB}}{\rtwo_j}{\rone_j}$ only. 

%Note that each subproblem in \eqref{eq:decom} remains a large-scale optimization problem -- each subproblem in \eqref{eq:decom} depends on the knowledge of the global plant model $\tf Z_{AB}$. In this subsection, we exploit the locality constraint $\Sub{\Ell}{:}{\colps_j}$ in \eqref{eq:decom-3} to reduce the complexity of \eqref{eq:decom}. 

%Note that the $p$ subproblems can be computed in an independent and parallel way.
%\begin{eqnarray}
%\underset{\Sub{\ttf{\Phi}}{ : }{\colps_j}}{\text{minimize    }} && g_j(\Sub{\ttf{\Phi}}{ : }{\colps_j}) \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \Sub{\ttf{\Phi}}{ : }{\colps_j} = \Sub{I}{ : }{\colps_j} \nonumber \\
%&& \Sub{\ttf{\Phi}}{ : }{\colps_j} \in \s_j \label{eq:sf_lopd}
%\end{eqnarray}
%\begin{example}
%Localized LQR with spatio-temporal constraint
%\end{example}
%This is the general formulation for the localized LQR (LLQR) problem proposed in \cite{2014_Wang_CDC}. In \cite{2014_Wang_CDC}, we showed that the global LLQR problem admits a localized decomposition. Specifically, the global LLQR solution can be obtained by solving multiple LLQR sub-problems in a parallel way, with each sub-problem depending only on the \emph{local plant model}. 
%The key observation is noting that the optimization problem \eqref{eq:llqr} admits a \emph{column-wise} decomposition. Specifically, the objective function in \eqref{eq:llqr} can be rewritten as
%\begin{equation}
%\sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber
%\end{equation}
%where the subscript $j$ represents the $j$-th column of the transfer matrix, and $n_x$ is the number of states. Note that the constraints in \eqref{eq:llqr} can be decomposed in a column-wise way as well. Let $\mathcal{S}_j$ denotes the convex set constraint on column $j$. We can solve
%\begin{eqnarray}
%\underset{\{R_j,M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber \\
%&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-s}
%\end{eqnarray}
%for $j = 1, \dots, n_x$ instead of solving \eqref{eq:llqr}, in a parallel way. We now focus on a specific $j$. When $\mathcal{S}_j$ is a locality (sparsity) constraint, we can reduce the dimension of \label{eq:llqr-s} \emph{from global scale to local scale}. 

%\subsection{Dimension Reduction} 

\subsection{Row-wise Separable Problems}
%\begin{remark}
The technique described in the previous subsection can be readily extended to row-wise separable problems.
For instance, we formulate the localized distributed Kalman filter (LDKF) problem in \cite{2015_Wang_LDKF} as
\begin{eqnarray}
\underset{\{\tf R, \tf N\}}{\text{minimize    }} && || \begin{bmatrix} \tf R & \tf N \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} \tf R & \tf N \end{bmatrix} \begin{bmatrix} zI-A \\ -C_2 \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R & \tf N \end{bmatrix} \in \begin{bmatrix} \Ell_{R} & \Ell_{N} \end{bmatrix} \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty, \nonumber%\label{eq:ldkf}
\end{eqnarray}
which is the dual of LLQR. The LDKF problem belongs to the class of row-wise separable problem. Consider a state estimation SLS problem \cite{2015_PartI} given by
\begin{subequations} \label{eq:sf_lop20}
\begin{align} 
\underset{\ttf{\Phi}}{\text{minimize }} \quad & g(\ttf{\Phi}) \label{eq:lop-10}\\
\text{subject to } \quad & \ttf{\Phi} \tf Z_{AC} = I \label{eq:lop-20} \\
& \ttf{\Phi} \in \s. \label{eq:lop-30}
\end{align}
\end{subequations}
with $\ttf{\Phi} = \begin{bmatrix} \tf R & \tf N \end{bmatrix}$ and $\tf Z_{AC} = \begin{bmatrix} zI-A^\top & -C_2^\top \end{bmatrix}^\top$.
%The general form of the row-wise separable problem is given by
Let $\{ \rowps_1, \dots, \rowps_q\}$ be a partition of the set $\{1, \dots, n_x\}$. The row-wise separability of the SLO and SLC in \eqref{eq:sf_lop20} are defined as follows.
\begin{definition} \label{dfn:dd_row}
The system level objective $g(\ttf{\Phi})$ in \eqref{eq:lop-10} is said to be \emph{row-wise separable} with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_q\}$ if
\begin{equation}
g(\ttf{\Phi}) = \sum_{j=1}^q g_j(\Sub{\ttf{\Phi}}{\rowps_j}{ : }) \label{eq:decom_obj_row}
\end{equation}
for some functionals $g_j(\cdot)$ for $j = 1, \dots, q$. 
\end{definition}
\begin{definition} \label{dfn:s_row}
The system level constraint $\s$ in \eqref{eq:lop-30} is said to be \emph{row-wise separable} with respect to the row-wise partition $\{ \rowps_1, \dots, \rowps_p\}$ if 
\begin{equation}
\ttf{\Phi} \in \s \quad \Longleftrightarrow \quad \bigcap_{j=1}^q \Sub{\ttf{\Phi}}{\rowps_j}{ : } \in \s_j  \label{eq:decom_scon_row}
\end{equation}
for some sets $\s_j$ for $j = 1, \dots, q$.
%the following condition is satisfied:
%\begin{equation}
%\ttf{\Phi} \in \s \quad \text{if and only if} \quad \Sub{\ttf{\Phi}}{\rowps_j}{ : } \in \s_j \text{  for  } j = 1, \dots, q  \nonumber
%\end{equation}
%Mathematically, this condition is expressed as
\end{definition}

%When $B_2$ is invertible, we solve \eqref{eq:main_1} analytically to express the transfer matrices $(\tf M, \tf L)$ as a function of $(\tf R, \tf N)$. We can define row-wise separable objective and constraint accordingly.
%We focus on the state feedback problem (i.e., $C_2 = I$). After solving \eqref{eq:sf_lop}, the controller achieving the desired closed loop response can be implemented by \cite{2015_PartI}
%\begin{eqnarray}
%\tf{\hat{w}} &=& C_2^{-1} (\tf y - \tf{\hat{y}}) \nonumber\\
%\tf u &=& z \tf M \hat{w} \nonumber\\
%\tf{\hat{y}} &=& C_2 (z \tf R - I) \tf{\hat{w}}. \nonumber
%\end{eqnarray}
%Although this implementation holds for arbitrary invertible $C_2$, the computation of the inverse of $C_2$ can be prohibited for large-scale systems unless $C_2$ has certain sparsity structure, e.g., block diagonal.
%\end{remark}



==> Synthesis_v1.tex <==
In particular, when sparsity constraint is imposed on the closed loop transfer matrices, the controller achieving the desired closed loop response can be implemented in a localized way -- this allows the control scheme to be applied on an arbitrary large-scale system.


In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.

\subsection{Locality Constraints}
Assume that $P_{22}$ is strictly proper, i.e. $D_{22} = 0$. Similar to the FIR constraint, the sparsity constraints imposed on $R, M, N, L$ in \eqref{eq:main_SS} can have added benefit on the scalability of controller implementation. As our controller is implemented by $R, M, N, L$ directly as in Figure \ref{fig:of}, a localized (sparse) closed loop response implies a localized (sparse) controller implementation. For simplicity of presentation, we use the chain model to illustrate the idea. The method described in this paper can generalize to arbitrary plant topology immediately as in \cite{2014_Wang_ACC, 2014_Wang_CDC, 2014_Wang_Allerton}.

When sparsity constraints is imposed

The problem of structural realizability is automatically satisfied

\subsection{Localized LQR}
Consider the state feedback problem \eqref{eq:sfplant} with a quadratic cost, the distributed optimal control problem can be formulated as
\begin{eqnarray}
\underset{\{R,M\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} R \\ M \end{bmatrix} \in \mathcal{S} \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr}
\end{eqnarray}
This is the general formulation for the localized LQR (LLQR) problem proposed in \cite{2014_Wang_CDC}. In \cite{2014_Wang_CDC}, we showed that the global LLQR problem admits a localized decomposition. Specifically, the global LLQR solution can be obtained by solving multiple LLQR sub-problems in a parallel way, with each sub-problems depending only on the \emph{local plant model}. We will outline the LLQR decomposition procedure here since the output feedback problem use the same decomposition technique as a subroutine. Interested readers can refer to \cite{2014_Wang_CDC} for more details.

The key observation is noting that the optimization problem \eqref{eq:llqr} admits a \emph{column-wise} decomposition. Specifically, the objective function in \eqref{eq:llqr} can be rewritten as
\begin{equation}
\sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber
\end{equation}
where the subscript $j$ represents the $j$-th column of the transfer matrix, and $n_x$ is the number of states. Note that the constraints in \eqref{eq:llqr} can be decomposed in a column-wise way as well. Let $\mathcal{S}_j$ denotes the convex set constraint on column $j$. We can solve
\begin{eqnarray}
\underset{\{R_j,M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber \\
&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-s}
\end{eqnarray}
for $j = 1, \dots, n_x$ instead of solving \eqref{eq:llqr}, in a parallel way. We now focus on a specific $j$. When $\mathcal{S}_j$ is a locality (sparsity) constraint, we can reduce the dimension of \label{eq:llqr-s} \emph{from global scale to local scale}. In order to illustrate the idea, we consider the chain example again.

Chain example

With this dimension reduction, each LLQR sub-problem can be expressed in the form as
\begin{eqnarray}
\underset{\{x_\ell, u_\ell \}}{\text{minimize    }} && || C_\ell x_\ell + D_\ell u_\ell ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A_\ell & -B_\ell \end{bmatrix} \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} = e_\ell \nonumber \\
&& \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} \in \mathcal{S}_\ell \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-l}
\end{eqnarray}

The complete synthesis procedure is summarized in Algorithm \ref{ag:1}.

\begin{algorithm}[h!]
Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
Set feasible = 1\;
\For {each state $x_j$}
{    
     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
     \If {not feasible}
     {  
       feasible = 0\;
       break\;
     } 
}

\If {feasible}
{    \For {each $j$-th LLQR sub-problem}
    {   
        Distribute the solution to the local controllers within its localized region \;
    }
}
\caption{Localized Synthesis} \label{ag:1}
\end{algorithm}

Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.

\subsection{Sparse $\mathcal{H}_2$}
Consider the optimization problem
\begin{subequations}
\begin{align}
\underset{\{R,M,N,L\}}{\text{minimize    }} & || \begin{bmatrix} R & \sigma_y N \\ \sigma_u M & \sigma_u \sigma_y L \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:h2_obj}\\
\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:h2_1} \\
& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:h2_2} \\
&  R, M, N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad L \in \mathcal{RH}_{\infty} \label{eq:h2_stable}\\
& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:h2_S}
\end{align}
\end{subequations}
where $\sigma_u$ is the relative penalty between state deviation and control effort, $\sigma_y$ the relative magnitude of process disturbance and sensor disturbance. This corresponds to the case for some sparse $C_1, D_{21}, B_1, D_{21}$. Theoretically, the method described in this paper can generalize to arbitrary $C_1, D_{21}, B_1, D_{21}$, but it is effective only when those matrices are highly sparse.

Without the constraint \eqref{eq:h2_2}, this optimization problem admits a column-wise decomposition as the LLQR problem. Similarly, without the constraint \eqref{eq:h2_1}, the optimization problem admits a row-wise decomposition. Specifically, we solve
\begin{eqnarray}
\begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
\text{subject to }  && \eqref{eq:h2_1}, \eqref{eq:h2_stable}, \eqref{eq:h2_S} \label{eq:sub1}
\end{eqnarray}
and
\begin{eqnarray}
\begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
\text{subject to }  && \eqref{eq:h2_2}, \eqref{eq:h2_stable}, \eqref{eq:h2_S}. \label{eq:sub2}
\end{eqnarray}
When the constraint \eqref{eq:h2_S} is a locality constraint, we can utilize the technique of LLQR to solve both \eqref{eq:sub1} and \eqref{eq:sub2} in a completely localized and parallel way.

The optimal solution in \eqref{eq:sub1} and \eqref{eq:sub2} may not be the same. Therefore, we need to solve an extra optimization problem as
\begin{eqnarray}
\underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
\text{subject to }  && \begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix}. \label{eq:sub3}
\end{eqnarray}
Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}.



==> Synthesis_v2.tex <==
In this section, we discuss how to solve the optimization problem \eqref{eq:main_SS} in a scalable manner when the objective function and the $\mathcal{S}$-localizability constraint are \emph{decomposable}. In this case, the optimization problem \eqref{eq:main_SS} decomposes naturally into several localized optimization problems with much smaller scale. For each localized optimization problem, the solution only depends on the system model locally. This offers a localized and scalable controller synthesis method for large-scale systems. 

This section begins with some mathematical notations. We then focus on a special class of state feedback system in which the optimization problem admits a direct decomposition. Finally, we combine the state feedback decomposition technique with distributed optimization to deal with a more general class of output feedback systems.
%State feedback is discussed first due to

%can further be \emph{solved} in a completely localized and scalable way.
%In this section, we will discuss on how to solve the optimization problem \eqref{eq:main_SS}. In particular, for some specific objective function, when sparsity constraint is imposed in \eqref{eq:main_SS}, the optimization problem can be decomposed into several sub-problems with much smaller scale. This offers a localized and scalable controller synthesis method for large-scale systems. We will first discuss the state feedback problem with linear quadratic regulator (LQR) cost. Then, the output feedback problem with $\mathcal{H}_2$ norm will be discussed.
%\subsection{Locality Constraints}

\subsection{Mathematical Notations}
Column/row-wise partition, permutation, block-wise sparsity pattern, multiplication of sparsity patterns

\subsection{State Feedback with Direct Decomposition}
%Assume that the matrix $C_2$ is invertible. In this case, equation \eqref{eq:output_fb2} implies that the closed loop transfer matrices $(N, L)$ can be expressed as a function of $(R, M)$ by
%\begin{eqnarray}
%N &=& (R(zI-A) - I) C_2^{-1} \nonumber\\
%L &=& M(zI-A) C_2^{-1}. \nonumber
%\end{eqnarray}
%For a state feedback system, we have $C_2 = I$.
The general formulation for a localized state feedback problem is given by
\begin{eqnarray}
\underset{\{R,M\}}{\text{minimize    }} && g(R,M) \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} R \\ M \end{bmatrix} \in \mathcal{S} \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:sf_lop}
\end{eqnarray}
In particular, we consider the case in which the localizability constraint $\mathcal{S}$ is a spatio-temporal constraint. We aim to exploit the sparsity of $\mathcal{S}$ to provide a scalable algorithm to solve the optimization problem \eqref{eq:sf_lop}.

To further simplify the notation, we use
\begin{equation}
\Phi = \begin{bmatrix} R \\ M \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. The optimization problem \eqref{eq:sf_lop} can then be written as 
\begin{eqnarray}
\underset{\Phi}{\text{minimize    }} && g(\Phi) \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \Phi = I \nonumber \\
&& \Phi \in \mathcal{S} \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:sf_lop2}
\end{eqnarray}

\subsubsection{Column-wise Partition}
In order to make the optimization problem \emph{decomposable}, we make the following assumptions on the problem. Consider a column-wise partition $\{ \Phi_j \}_{j=1}^n$ of the closed loop transfer matrix $\Phi$. This partition can be interpreted as a partition of process noise, where $\Phi_j$ is the closed loop transfer matrix from disturbance $\delta{x_j}$ to $[x^\top u^\top]^\top$.
%Given a partition of the global state vector $\{ p_j \}_{j=1}^n$, we can decompose the closed loop transfer matrices $(R,M)$ block column-wisely according to the partition $\{ p_j \}_{j=1}^n$. Specifically, we use $R_{p_j}$ and $M_{p_j}$ to denote the $j$th block column of $R$ and $M$, respectively. By definition, $R_{p_j}$ and $M_{p_j}$ are the closed loop transfer matrices from $\delta{x_{p_j}}$ to $x$ and $u$, respectively. 
%Note that the set $\{R_j,M_j\}$ encodes the information of the underlying partition. In the following, we use $\{R_j,M_j\}$ to represent a partition without explicitly specify the partition $\{ p_j \}$. 
%We define the decomposable objective function and the decomposable localizability constraint as follows.
%Using this notation, 
We define column-wise decomposable objective functions as follows.

\begin{definition}
The objective function $g(\Phi)$ is said to be column-wise decomposable with respect to the partition $\{ \Phi_j \}_{j=1}^n$ if
\begin{equation}
g(\Phi) = \sum_{j=1}^n g_j(\Phi_j) \label{eq:decom_obj}
\end{equation}
for some objective functions $g_j(.)$ for $j = 1, \dots, n$. 
\end{definition}
\begin{example}
One concrete example of a column-wise decomposable objective is the $\mathcal{H}_2$ norm with identity noise matrix $B_1 = I$. For instance, we have
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Phi ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{n} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \Phi_j ||_{\mathcal{H}_2}^2 \nonumber
\end{equation}
for arbitrary cost function $C_1$ and $D_{12}$ with arbitrary partition $\{ \Phi_j \}_{j=1}^n$. Other decomposable objectives include the entry-wise $\ell_1$ objective. 
\end{example}
\begin{example}
LQR objective with block diagonal noise matrix, the partition $\Phi_j$ is the partition of uncorrelated process noise
\end{example}

We can also define a column-wise decomposable constraint as follows.
\begin{definition}
The localizability constraint $\mathcal{S}$ is said to be column-wise decomposable with respect to the partition $\{ \Phi_j \}_{j=1}^n$ if 
\begin{equation}
\Phi \in \mathcal{S} \, \Longleftrightarrow \, \Phi_j \in \mathcal{S}_j \text{  for  } j = 1, \dots, n  \nonumber
\end{equation}
for some set $\mathcal{S}_j$ for $j = 1, \dots, n$. 
\end{definition}
\begin{example}
It can be readily shown that the spatio-temporal constraint $\mathcal{S}$ defined in the previous section is column-wise decomposable with respect to any partition.
\end{example}

Assume that the objective function and the localizability constraint are both decomposable with respect to the partition $\{ \Phi_j \}_{j=1}^n$. Let $[I]_j$ denote the column-wise partition of the identity matrix corresponding to $\Phi_j$. It is straightforward to show that the optimization \eqref{eq:sf_lop2} can be decomposed into
\begin{eqnarray}
\underset{\Phi_j}{\text{minimize    }} && g_j(\Phi_j) \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \Phi_j = [I]_j \nonumber \\
&& \Phi_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty \label{eq:sf_lopd}
\end{eqnarray}
for $j = 1, \dots, n$.

\begin{example}
Localized LQR with spatio-temporal constraint
\end{example}

The benefit of this decomposition is that we can possibly reduce the dimension of \eqref{eq:sf_lopd} \emph{from global scale to local scale} when each $\mathcal{S}_j$ is highly sparse. 
Due to the decomposable assumptions, we can analyze the closed loop response for each local disturbance $\delta{x_j}$ in its own localized region in a parallel and independent way, even when their localized regions are \emph{overlapped}.

%This is the general formulation for the localized LQR (LLQR) problem proposed in \cite{2014_Wang_CDC}. In \cite{2014_Wang_CDC}, we showed that the global LLQR problem admits a localized decomposition. Specifically, the global LLQR solution can be obtained by solving multiple LLQR sub-problems in a parallel way, with each sub-problem depending only on the \emph{local plant model}. 
%The key observation is noting that the optimization problem \eqref{eq:llqr} admits a \emph{column-wise} decomposition. Specifically, the objective function in \eqref{eq:llqr} can be rewritten as
%\begin{equation}
%\sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber
%\end{equation}
%where the subscript $j$ represents the $j$-th column of the transfer matrix, and $n_x$ is the number of states. Note that the constraints in \eqref{eq:llqr} can be decomposed in a column-wise way as well. Let $\mathcal{S}_j$ denotes the convex set constraint on column $j$. We can solve
%\begin{eqnarray}
%\underset{\{R_j,M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
%\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber \\
%&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \mathcal{S}_j \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-s}
%\end{eqnarray}
%for $j = 1, \dots, n_x$ instead of solving \eqref{eq:llqr}, in a parallel way. We now focus on a specific $j$. When $\mathcal{S}_j$ is a locality (sparsity) constraint, we can reduce the dimension of \label{eq:llqr-s} \emph{from global scale to local scale}. 

\subsubsection{Localized Region}
We now focus on a specific $j$ in \eqref{eq:sf_lopd}, and show how to simplify the optimization problem when $\mathcal{S}_j$ is highly sparse. Recall that $\mathcal{S}_j$ is a constraint imposed on the closed loop response from $\delta{x_j}$ to $x$ and $u$. Therefore, the block row-wise sparsity pattern of $\mathcal{S}_j$ encodes the set of affected states and activated control actions under disturbance $\delta{x_j}$. We can construct a localized region, local state vector, and local plant model based on this information. Consider the following illustrative example.
\begin{example}
Consider Fig. \ref{fig:Chart105} with state feedback (full sensing). Assume that the disturbance $\delta{x_1}$ at node $1$ is only allowed to affect the state $x_1$ and $x_2$ at node $1$ and node $2$ in closed loop. In addition, we want to achieve this by activating the control action $u_i$ from node $i = 1, \dots, 4$. In this case, a localized region for disturbance $\delta{x_1}$ can be constructed by Region$(x_1) = \{x_1, x_2, x_3, x_4\}$ as shown in Fig. \ref{fig:region}. The boundary of this localized region is the set $\{x_3, x_4\}$. Intuitively, by keeping the boundary being zero for all time, there is no way for the disturbance to \emph{escape} from the localized region through state propagation. In addition, the effects of all control actions are limited within the localized region. We can then solve \eqref{eq:sf_lopd} using the local state, control, and plant model defined within this localized region. \label{ex:3}
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.4\textwidth]{figure/Region.pdf}
      \caption{Localized Region}
      \label{fig:region}
\end{figure}
%Clearly, we need to activate $u_1, u_2, u_3$ in order to localize the disturbance. In this case, we can define $Region(x_1) = \{x_1, x_2, x_3\}$, $Ext(x_1) = \{x_4, x_5\}$, and $Bound(x_1) = \{x_3\}$. Note that $x_3$ is contained within the localized region since $u_3$ is actuated.
\end{example}

1. Formally define "affected states" and "activated control actions"
Split $\mathcal{S}_j$ into $\mathcal{S}_{R_j}$ and $\mathcal{S}_{M_j}$. 
To be specific, the notion of affected states and activated control actions are formally defined as follows.
\begin{definition}
The affected states and the activated control actions, nonzero position of $\mathcal{S}_j$
\end{definition}
\begin{example}
Graph example, intuition
\end{example}

2. Define the localized region as a union set (need to define the partition of matrix A)
For a particular local disturbance $\delta{x_j}$ with the spatio-temporal constraint $\mathcal{S}_j$, we can construct a localized region by taking the union of the following three sets:
\begin{enumerate}[(i)]
\item the affected states %($\{x_1, x_2\}$ in Example \ref{ex:3})
\item the states that can be affected by the activated control actions directly %($\{x_1, \dots, x_4\}$ in Example \ref{ex:3})
\item the states that are connected from the affected states, i.e. the set $\{ x_i | A_{ik} \not = 0, x_k \in \text{ affected states}\}$. %($\{x_1, \dots, x_4\}$ in Example \ref{ex:3})
\end{enumerate}
We denote the localized region for $\delta{x_j}$ by Region($x_j$).
\begin{example}
Graph example, intuition
\end{example}

For a localized region, the external region Ext$(.)$ is defined as its complement set. The boundary of a localized region is defined as the set of states that connect the localized region toward the external region, i.e. $\{ x_k | A_{ik} \not = 0, x_k \in \text{Region}(x_j), x_i \in \text{Ext}(x_j)\}$. Intuitively, the affected states can be considered as the \emph{internal region} of the localized region, and the boundary is the set that \emph{separates} the internal region from the external region. As long as the boundary states are keeping zero for all time, and the control actions do not affect the external region (which is ensured by construction rule (ii)), the solution of \eqref{eq:llqr-s} can be analyzed completely within the localized region. Construction rule (iii) ensures that the boundary states are included in the localized region. 

Algebraically, we can also calculate the localized region for $\delta{x_{p_j}}$ by checking the block row-wise sparsity pattern of
\begin{equation}
SL = \Sp{\begin{bmatrix} zI - A & -B_2 \end{bmatrix}} \Sp{\mathcal{S}_j}. \nonumber
\end{equation}
The localized region can be alternatively defined as
\begin{equation}
\text{Region}(x_j) = \{i | SL_i \not = 0 \}.
\end{equation}

With the notion of localized region, we define the local state vector $x_{\ell}$ the stacked vector of $x_i$ for all $x_i \in \text{Region}(x_j)$. The local control vector $u_{\ell}$ is stacked vector of all activated local control action $u_i$. The local plant model $(A_\ell,B_{2 \ell})$ associated with Region$(x_j)$ is defined by selecting submatrices of $(A,B_2)$ consisting of the columns and rows associated with $x_\ell$ and $u_\ell$.

Let $e_\ell$ be the initial condition of the source of disturbance. The local convex set constraint $\mathcal{S}_\ell$ can be defined by selecting the block rows of $\mathcal{S}_j$ associated with $[x_\ell^\top u_\ell^\top]^\top$, and column corresponding to $e_\ell$.

%The construction of the localized region
%For completeness, we prove the equivalence in Appendix (see LLQR paper)

%To be specific, we define the localized region for state $j$ by a column sparsity pattern as
%\begin{equation}
%\text{sp}(\begin{bmatrix} zI - A & -B_2 \end{bmatrix}) \Sp{\mathcal{S}_j}. \nonumber
%\end{equation}
%Region(j) = \begin{bmatrix} \Sp{\bar{A}} & \Sp{B_2} \end{bmatrix} \Sp{\mathcal{S}_j}, \nonumber
%By an abuse of notation, we also interpret Region$(j)$ as a set of the positions of its nonzero entries. 

%Recall that $\mathcal{V}$ is the set of all sub-systems. We use a set $Region(j) \subseteq \mathcal{V}$ to denote the localized region for sub-system $j$, and $External(j) = \mathcal{V} \setminus Region(j)$ to denote the external region for sub-system $j$. The boundary of $Region(j)$ is defined as follows.
%\begin{definition}
%The boundary of $Region(j)$ is the set of all sub-systems that connect $Region(j)$ toward $External(j)$ and is denoted by $Bound(j)$. Specifically, we have
%\begin{equation}
%Bound(j) = \{ k | A_{ik} \not = 0, k \in Region(j), i \in External(j) \}. \nonumber
%%\footnote{The $A_{ik}$ here denotes the $(i,k)$-entries of $A$.} \nonumber
%\end{equation}
%\end{definition}

The general form

The algebraic definition can be calculated in a localized way.

\begin{example}
Each LLQR sub-problem can be expressed in the form as
\begin{eqnarray}
\underset{\{x_\ell, u_\ell \}}{\text{minimize    }} && || C_\ell x_\ell + D_\ell u_\ell ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A_\ell & -B_\ell \end{bmatrix} \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} = e_\ell \nonumber \\
&& \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} \in \mathcal{S}_\ell \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr-l}
\end{eqnarray}
\end{example}

The complete synthesis procedure is summarized in Algorithm \ref{ag:1}.

%\begin{algorithm}[h!]
%Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
%Set feasible = 1\;
%\For {each state $x_j$}
%{    
%     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
%     \If {not feasible}
%     {  
%       feasible = 0\;
%       break\;
%     } 
%}
%
%\If {feasible}
%{    \For {each $j$-th LLQR sub-problem}
%    {   
%        Distribute the solution to the local controllers within its localized region \;
%    }
%}
%\caption{Localized Synthesis} \label{ag:1}
%\end{algorithm}
\begin{algorithm}[h!]
Given global plant model $(A, B_2)$, objective $(C_1, D_{12})$, and sparse FIR constraint $\mathcal{S}$\;
\For {each state perturbation $\delta{x_j}$}
{    
     Define localized region based on the block column sparsity of $\mathcal{S}$\;
     Solve \eqref{eq:llqr-l} and derive $x_\ell, u_\ell$ within its localized region\;
}

\If {all sub-problems are feasible}
{
    \For {each sub-problem}
    {   
        Distribute the solution $x_\ell, u_\ell$ to the local controllers within its localized region \;
    }
}
\caption{State Feedback Synthesis} \label{ag:1}
\end{algorithm}

%Note that all the for loops in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.
Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. In addition, when the plant model change locally, we only need to resolve \emph{some} of the sub-problems. This suggests the possibility to do real-time \emph{re-synthesis} subject to model change that also maintains global optimality.


\subsection{Output Feedback with Distributed Optimization}
The column-wise decomposition technique does not apply to output feedback systems directly as the constraint \eqref{eq:output_fb2} does not admit a column-wise decomposition. However, we note that the constraint \eqref{eq:output_fb2} can be decomposed in a block row-wise manner. It is then natural to use the distributed optimization techniques such as the alternating direction method of multipliers (ADMM) to decouple the constraints \eqref{eq:output_fb1} and \eqref{eq:output_fb2}, and solve the localized output feedback optimal control problem in a localized yet iterative way. 

\subsubsection{Decomposability}
To simplify the notation, we use
\begin{equation}
\Phi = \begin{bmatrix} R & N \\ M & L \end{bmatrix} \nonumber
\end{equation}
to represent the closed loop transfer matrix we want to optimize for. 
Let $\{\Phi_j\}_{j=1}^n$ be a column-wise partition of $\Phi$, and $\{(\Phi^\top)_j\}_{j=1}^{n'}$ be a row-wise partition of $\Phi$ (a column-wise partition of $\Phi^\top$).
%Let $\{p_j\}_{j=1}^n$ be a column-wise partition for $CL$ (a partition on the perturbation $[\delta{x}; \delta{y}]$), and $\{p'_j\}_{j=1}^{n'}$ a row-wise partition for $CL$ (a partition on the internal variable $[x; u]$). 
The decomposability for the objective function and the localizability constraint are defined as follows.
\begin{definition}
The objective function $g(\Phi)$ is said to be decomposable with respect to the column-wise partition $\{\Phi_j\}_{j=1}^n$ and the row-wise partition $\{[\Phi^\top]_j\}_{j=1}^{n'}$ if $g(\Phi)$ can be written as
\begin{equation}
g(\Phi) = \tilde{g}(\Phi) + \hat{g}(\Phi) \nonumber\\
\end{equation}
where $\tilde{g}(\Phi)$ is column-wise decomposable with respect to $\{\Phi_j\}_{j=1}^n$ and $\hat{g}(\Phi)$ is row-wise decomposable with respect to $\{[\Phi^\top]_j\}_{j=1}^{n'}$. Specifically, we have 
\begin{eqnarray}
\tilde{g}(\Phi) &=& \sum_{j=1}^n \tilde{g}_j(\Phi_j) \nonumber\\
\hat{g}(\Phi) &=& \sum_{j=1}^{n'} \hat{g}_j([\Phi^\top]_{j})
\end{eqnarray}
for some objective functions $\tilde{g}_j(.)$ for $j = 1, \dots, n$, and $\hat{g}_j(.)$ for $j = 1, \dots, n'$. 
\end{definition}
\begin{example}
$\mathcal{H}_2$ norm with block diagonal noise matrix
\end{example}
\begin{example}
$\mathcal{H}_2$ norm with block diagonal cost matrix
\end{example}

\begin{definition}
The localizability constraint $\mathcal{S}$ is said to be decomposable with respect to the column-wise partition $\{\Phi_j\}_{j=1}^n$ and the row-wise partition $\{[\Phi^\top]_j\}_{j=1}^{n'}$ if 
\begin{eqnarray}
\Phi \in \mathcal{S} \, &\Longleftrightarrow & \, \Phi_j \in \mathcal{S}_j \text{  for  } j = 1, \dots, n  \nonumber\\
&\Longleftrightarrow & \, [\Phi^\top]_j \in [\mathcal{S}^\top]_j \text{  for  } j = 1, \dots, n'
%\Phi \in \mathcal{S} \quad &\Longleftrightarrow & \quad \bigcap_{j=1}^n \Phi_j \in \mathcal{S}_j \nonumber\\
%&\Longleftrightarrow & \quad \bigcap_{j=1}^{n'} [\Phi^\top]_j \in [\mathcal{S}^\top]_j
%CL \in \mathcal{S} &\Longleftrightarrow & [CL]_{p_j} \in [\mathcal{S}]_{p_j} \quad \forall j \nonumber\\
%&\Longleftrightarrow & [CL^\top]_{p'_j} \in [\mathcal{S}^\top]_{p'_j} \quad \forall j
\end{eqnarray}
for some set $\mathcal{S}_{j}$ for $j = 1, \dots, n$, and $[\mathcal{S}^\top]_{j}$ for $j = 1, \dots, n'$. 
\end{definition}
only need to be column-wise decomposable \emph{OR} row-wise decomposable

\begin{example}
Spatio-temporal constraint
\end{example}

\begin{example}
Mixed H2 / L1 problem
\end{example}

%Consider the optimization problem
%\begin{subequations}
%\begin{align}
%\underset{\{R,M,N,L\}}{\text{minimize    }} & || \begin{bmatrix} R & \sigma_y N \\ \sigma_u M & \sigma_u \sigma_y L \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:h2_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:h2_1} \\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:h2_2} \\
%&  R, M, N \in \frac{1}{z} \mathcal{RH}_{\infty}, \quad L \in \mathcal{RH}_{\infty} \label{eq:h2_stable}\\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix} \in \mathcal{S} \label{eq:h2_S}
%\end{align}
%\end{subequations}
%where $\sigma_u$ is the relative penalty between state deviation and control effort, $\sigma_y$ the relative magnitude of process disturbance and sensor disturbance. This corresponds to the case for some sparse $C_1, D_{21}, B_1, D_{21}$. Theoretically, the method described in this paper can generalize to arbitrary $C_1, D_{21}, B_1, D_{21}$, but it is effective only when those matrices are highly sparse.

\subsubsection{ADMM Algorithm}
%Assumptions (?)
Assume that the optimization problem is has a decomposable objective function with a decomposable localizability constraint. To decouple the constraints \eqref{eq:output_fb1} and \eqref{eq:output_fb2}, we define extended-real-value functions $\tilde{h}(\Phi)$ and $\hat{h}(\Psi)$ by
\begin{eqnarray}
&& \tilde{h}(\Phi) = \left\{ \begin{array}{ll}
\tilde{g}(\Phi) & \textrm{if } \eqref{eq:output_fb1}, \eqref{eq:output_fb3}, \Phi \in \mathcal{S}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber\\
&& \hat{h}(\Psi) = \left\{ \begin{array}{ll}
\hat{g}(\Psi) & \textrm{if } \eqref{eq:output_fb2}, \eqref{eq:output_fb3}, \Psi \in \mathcal{S}\\
\infty & \textrm{otherwise}
\end{array} \right. \nonumber
\end{eqnarray}
Problem \eqref{eq:main_SS} can then be equivalently formulated as
\begin{eqnarray}
\underset{\{\Phi, \Psi\}}{\text{minimize    }} && \tilde{h}(\Phi) + \hat{h}(\Psi) \nonumber\\
\text{subject to }  && \Phi = \Psi. \label{eq:sub3}
\end{eqnarray}
Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}. Specifically, the ADMM algorithm for \eqref{eq:sub3} can be written as
\begin{subequations}
\begin{align}
\Phi^{k+1} &= \underset{\Phi}{\text{argmin }} \Big( \tilde{h}(\Phi) + \frac{\rho}{2} || \Phi - \Psi^{k} + \Lambda^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm1} \\
\Psi^{k+1} &= \underset{\Psi}{\text{argmin }} \Big( \hat{h}(\Psi) + \frac{\rho}{2} || \Psi - \Phi^{k+1} - \Lambda^{k}||_{\mathcal{H}_2}^2 \Big) \nonumber \\
\label{eq:admm2} \\
\Lambda^{k+1} &= \Lambda^{k} + \Phi^{k+1} - \Psi^{k+1} \label{eq:admm3}
\end{align}
\end{subequations}
where the square of $\mathcal{H}_2$ norm can be computed by \eqref{eq:FIR}. 

Note that $\tilde{h}(\Phi)$ admits a block column-wise decomposition as both $\tilde{g}(\Phi)$ and the localizability constraint $\mathcal{S}$ are both column-wise decomposable. As the $\mathcal{H}_2$ norm admits a column-wise decomposition for any partition, subproblem \eqref{eq:admm1} can be solved using the state feedback decomposition technique described in the previous subsection. When the localizability constraint $\mathcal{S}$ is highly sparse, subproblem \eqref{eq:admm1} can be solved in a localized and scalable way. 
%From the decomposability assumptions on the objective function and the localizability constraint, function $\tilde{h}(\Phi)$ admits a block column-wise decomposition. 
%and function $\hat{h}(\Psi)$ admits a block row-wise decomposition. 
%From the decomposability of the
%Subproblem \eqref{eq:admm1} reduces to be form of state feedback 
%can be solved in a localized way using LLQR with a column-wise decomposition on the objective function and the constraint. 
Similarly, subproblem \eqref{eq:admm2} can also be solved using the state feedback decomposition technique through a row-wise decomposition. Equation \eqref{eq:admm3} can be decomposed either column-wise or row-wise. Therefore, \eqref{eq:admm1} - \eqref{eq:admm3} is a localized output feedback synthesis algorithm by using column-wise and row-wise decomposition alternatively and iteratively.

\begin{example}
LLQG
\end{example}

%Without the constraint \eqref{eq:h2_2}, this optimization problem admits a column-wise decomposition as the LLQR problem. Similarly, without the constraint \eqref{eq:h2_1}, the optimization problem admits a row-wise decomposition. Specifically, we solve
%\begin{eqnarray}
%\begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_1}, \eqref{eq:h2_stable}, \eqref{eq:h2_S} \label{eq:sub1}
%\end{eqnarray}
%and
%\begin{eqnarray}
%\begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix} = \underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \eqref{eq:h2_2}, \eqref{eq:h2_stable}, \eqref{eq:h2_S}. \label{eq:sub2}
%\end{eqnarray}
%When the constraint \eqref{eq:h2_S} is a locality constraint, we can utilize the technique of LLQR to solve both \eqref{eq:sub1} and \eqref{eq:sub2} in a completely localized and parallel way.
%
%The optimal solution in \eqref{eq:sub1} and \eqref{eq:sub2} may not be the same. Therefore, we need to solve an extra optimization problem as
%\begin{eqnarray}
%\underset{\{R,M,N,L\}}{\text{minimize    }} && \eqref{eq:h2_obj} \nonumber\\
%\text{subject to }  && \begin{bmatrix} R_1 & N_1 \\ M_1 & L_1 \end{bmatrix} = \begin{bmatrix} R_2 & N_2 \\ M_2 & L_2 \end{bmatrix}. \label{eq:sub3}
%\end{eqnarray}
%Problem \eqref{eq:sub3} can be solved via the standard ADMM approach \cite{BoydADMM}.

\subsubsection{Convergence and Stopping Criteria}



==> llqr.tex <==
\subsection{Localized Linear Quadratic Regulator} \label{sec:physical}
%In this subsection, we explain the physical meaning of the sets $\colps_j$, $\rone_j$, and $\rtwo_j$ in \eqref{eq:decom3} through a linear quadratic regulator (LQR) example.
%We show that the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector, $\rone_j$ is the collection of optimization variables contained within the localized region defined by the locality constraint $\Sub{\Ell}{:}{\colps_j}$, and $\rtwo_j$ is the set of states that can be directly affected by the variables in $\rone_j$.
%direct decomposability and the dimension reduction technique through a concrete example. For simplicity, 
%Consider the $n$-chain example shown in Figure \ref{fig:interconnected}. We assume that each subsystem's state $x_i$ is a scalar.
%network with interaction graph shown in Figure \ref{fig:chain}. 
%The global system dynamic is described by $x[t+1] = A x[t] + B_2 u[t] + w[t]$, where $A$ is an $n$-dimensional tridiagonal matrix and $B_2$ is identity. We assume that the disturbance $w$ is a zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. The objective function is the expected value of the time-average LQR cost. Let $\tf R$ be the system response from disturbance $\tf w$ to state $\tf x$, and $\tf M$ the system response from disturbance $\tf w$ to control action $\tf u$. We showed in \cite{2014_Wang_CDC} that the traditional LQR problem can be formulated as
Consider the system dynamic equation $x[t+1] = A x[t] + B_2 u[t] + w[t]$ with state feedback. We assume that the disturbance $w$ is a zero-mean additive white Gaussian noise (AWGN) with identity covariance matrix, i.e., $w \sim \mathcal{N}(0,I)$. Let $\tf R$ be the system response from disturbance $\tf w$ to state $\tf x$, and $\tf M$ the system response from disturbance $\tf w$ to control action $\tf u$. Let the objective function be the expected value of the time-average energy of the signal $(C_1 \tf x + D_{12} \tf u)$. Then the LQR problem can be formulated as \cite{2014_Wang_CDC}
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize  }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \frac{1}{z} \mathcal{RH}_\infty. \label{eq:lqr}
\end{eqnarray}

%\begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.35\textwidth]{./figure/Chain.pdf}
%     \caption{The $n$-chain example}
%     \label{fig:chain}
%\end{figure}
To facilitate the scalability of controller synthesis and implementation of \eqref{eq:lqr}, we additionally impose a spatiotemporal constraint on the system response to \emph{localize} the effect of each disturbance $w_j$ within some localized region within $T$ time steps.
Let $\Ell_R$ and $\Ell_M$ be the locality constraints imposed on the system response $\tf R$ and $\tf M$, respectively. %When the locality constraint is enforced, we try to localize the response of each disturbance $w_j$ within its two-hop neighbors.
%To make both the controller implementation and controller synthesis of \eqref{eq:lqr} scalable to large systems, we additionally impose a constraint to \emph{localize} the effect of each disturbance $w_j$ within its within $T$ time steps. For instance, when $d = 2$, we can impose a pentadiagonal sparsity pattern on $\tf R$ and $\tf M$ in \eqref{eq:lqr}. 
The localized LQR (LLQR) \cite{2014_Wang_CDC} problem is then given by
\begin{eqnarray}
\underset{\{\tf R, \tf M\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} = I \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix} \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty. \label{eq:llqr}
\end{eqnarray}
%where $\Ell_R$ and $\Ell_M$ are the sparsity constraints that force the transfer matrices $\tf R$ and $\tf M$ being pentadiagonal, respectively.
Note that \eqref{eq:llqr} is a special case of \eqref{eq:sf_lop}. The goal of this subsection is to propose a scalable algorithm to solve \eqref{eq:llqr}. %exploit the locality constraints $\Ell_R$ and $\Ell_M$ to decompose \eqref{eq:llqr} into parallel local optimization subproblems.

We first notice that \eqref{eq:llqr} admits a \emph{column-wise separation} -- we can solve for the transfer matrices $\tf R$ and $\tf M$ column at a time. Denote $\tf G_j$ the $j$th column of any transfer matrix $\tf G$. The objective in \eqref{eq:llqr} can be written as
\begin{equation}
|| \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix} ||_{\mathcal{H}_2}^2 = \sum_{j=1}^{n_x} || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j ||_{\mathcal{H}_2}^2. \nonumber
\end{equation}
%and the constraint in \eqref{eq:llqr} can be checked column at a time. 
This allows us to decompose \eqref{eq:llqr} into $n_x$ parallel subproblems as
\begin{eqnarray}
\underset{\{\tf R_j, \tf M_j\}}{\text{minimize    }} && || \begin{bmatrix} C_1 & D_{12} \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j = e_j \nonumber \\
&& \begin{bmatrix} \tf R \\ \tf M \end{bmatrix}_j \in \begin{bmatrix} \Ell_{R} \\ \Ell_{M} \end{bmatrix}_j \cap \FT \cap \frac{1}{z} \mathcal{RH}_\infty \label{eq:llqr-r}
\end{eqnarray}
for $j = 1, \dots, n_x$. By definition, the $j$th column of $\tf R$ and $\tf M$ are the system response of disturbance $\tf w_j$ to $\tf x$ and $\tf u$, respectively. The column-wise separation property therefore suggests that we can analyze the system response of each local disturbance $w_j$ in an independent and parallel way. This separation property is implied by two different characteristics of the LLQR problem: (i) the system is LTI, so the constraint in \eqref{eq:llqr} admits a column-wise separation, and (ii) the objective function is the LQR cost with uncorrelated disturbances $w \sim \mathcal{N}(0,I)$, which can be separated into column-wise sum as above. 
%Denote $\tf G_j$ the $j$th column of any transfer matrix $\tf G$. 
%More specifically, the direct decomposability of the constraint implies that each disturbance $w_j$ can be analyzed independently to ensure the \emph{feasibility} of the original problem, while the direct decomposability of the objective function further ensures the \emph{optimality} of the original problem when the analysis is performed for each $w_j$ in a distributed way. In the example of \eqref{eq:llqr}, the direct decomposability of the constraint is implied by the superposition principle of LTI systems. The direct decomposability of the objective follows from the property of the $\mathcal{H}_2$ norm. 
%It should be noted that a key assumption to make the problem decomposable is that the disturbance $w_j$ are uncorrelated to each other, i.e., $w \sim \mathcal{N}(0,I)$. For a more general case, suppose that we can partition the noise vector into $p$ uncorrelated subsets $\{\colps_1, \dots, \colps_p\}$. From Example \ref{ex:perm}, we know that the objective function is directly decomposable with respect to the column-wise partition $\{\colps_1, \dots, \colps_p\}$. Therefore, the physical meaning of $\colps_j$ is the $j$th uncorrelated subset of the noise vector.

%, the objective function is directly decomposable with respect to that partition.
%If the disturbance $w_j$ are correlated to each other globally, then we lose the direct decomposability of the objective function. In the $\mathcal{H}_2$ example, as long as we can partition the noise vector into uncorrelated subsets, the objective function is directly decomposable with respect to that partition.

%Once the problem is decomposed, we analyze the closed loop response of each $w_j$ in an independent and parallel way. 
%Here, the locality constraints $\Ell_R$ and $\Ell_M$ allow us to analyze the effect of $w_1$ within its \emph{localized region}. 
%Let $a_{ij}$ be the $(i,j)$-th entry of matrix $A$. Using the dimension reduction technique described in the previous subsection, the optimization problem solving the closed loop response of $w_1$ eventually reduces to
%\begin{align}
%&\underset{\tf v}{\text{minimize}} \quad || \begin{bmatrix} \bar{C}_1 & \bar{D}_{12} \end{bmatrix} \tf v ||_{\mathcal{H}_2}^2 \nonumber\\
%&\text{subject to} \quad \tf v \in \FT \cap \frac{1}{z} \mathcal{RH}_\infty \nonumber \\
%&\begin{bmatrix} z-a_{11} & -a_{12} & -1 & 0 & 0 \\ -a_{21} & z-a_{22} & 0 & -1 & 0 \\ 0 & -a_{32} & 0 & 0 & -1 \end{bmatrix} \tf v = \begin{bmatrix} 1 \\ 0 \\ 0 \end{bmatrix} \label{eq:llqr-r}
%\end{align}
%with $\tf v = \begin{bmatrix} \tf R_{11} & \tf R_{21} & \tf M_{11} & \tf M_{21} & \tf M_{31} \end{bmatrix}^\top$ a column vector, and $\bar{C}_1$ and $\bar{D}_{12}$ some appropriate sub-matrices of $C_1$ and $D_{12}$, respectively. Clearly, the dimension of problem \eqref{eq:llqr-r} is completely independent with respect to the size of the global network $n$. In addition, \eqref{eq:llqr-r} is specified by only some of the entries of $A$, which means that we only need to know some local plant model information to solve \eqref{eq:llqr-r}.
%problem \eqref{eq:llqr-r} only depends on the plant model locally.

\begin{figure}[h!]
     \centering
     \includegraphics[width=0.35\textwidth]{./figure/Localized3.pdf}
     \caption{The localized region for $w_1$}
     \label{fig:localized}
\end{figure}
For each subproblem in \eqref{eq:llqr-r}, we can further exploit the locality constraint to reduce the dimension of each subproblem from global scale to local scale. The technical details of the dimensional reduction algorithm can be found in our prior work \cite{2014_Wang_CDC}, and we will discuss a generalized version in the next subsection and in Appendix \ref{sec:reduction}. 
%and the issues regarding the feasibility of each \eqref{eq:llqr-r} is discussed in \cite{2015_Wang_Reg}. 
Here we just illustrate the idea through a simple example.
\begin{example}
Consider a chain of $n$ LTI subsystems with a single local disturbance $\tf w_1$. In \eqref{eq:llqr-r}, the optimization variables are the system response from the disturbance $\tf w_1$ to the global state $\tf x$ and global control action $\tf u$.  Assume that the locality constraint in \eqref{eq:llqr-r} is given by $x_3 = \dots = x_n = 0$ and $u_4 = \dots = u_n = 0$. In this case, we can solve \eqref{eq:llqr-r} using only the information contained within the localized region shown in Figure \ref{fig:localized}. Intuitively, as long as the boundary constraint $x_3 = 0$ is enforced, the system response of $w_1$ can never escape from the localized region. In other words, the condition $x_i = 0$ for $i = 4, \dots n$ is implicitly implied by the boundary constraint $x_3 = 0$. In order to make $x_3$ unaffected by the disturbance $w_1$, the actuator $u_3$ at the third subsystem must actuate properly to cancel the coupling from the state $x_2$ at the second subsystem. 
Finally, as the system is LTI, we can analyze the system response for each $w_j$ within its own localized region, and use superposition principle to compute the system response for arbitrary linear combination of disturbances. 
\end{example}


%%%%%%%%%%
%Without loss of generality, we focus on the first subproblem $j = 1$ of \eqref{eq:llqr-r}, which corresponds to the system response of $w_1$. Recall that we enforce the locality constraint $(\Ell_R, \Ell_M)$ to localize the response of each local disturbance to its two-hop neighbors. We plot the desired response of $w_1$ in Figure \ref{fig:localized}, where all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
%The physical interpretation of \eqref{eq:llqr-r} is illustrated by Figure \ref{fig:localized}. When the locality constraints $\Ell_R$ and $\Ell_M$ are imposed, all the uncolored nodes in Figure \ref{fig:localized} are required to be zero. 
%From the last equality constraint in \eqref{eq:llqr-r}, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$.
%It is clear that we only need to analyze the closed loop response of $w_1$ in the localized region specified in Figure \ref{fig:localized}. 
%Specifically, we have the relation $\tf M_{31} = -a_{32} \tf R_{21}$ from the last equality constraint in \eqref{eq:llqr-r}. 
%This is a necessary and sufficient condition to make 
%Note that we require the state $x_3$ at the third sub-system to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}, i.e., $\tf R_{31} = 0$. Implicit in this statement is the requirement of fast enough information sharing between sub-controllers. 
%Figure \ref{fig:delay} shows the information delay (the sum of the sensing delay from $x_1$ to $u_1$, the communication delay from $u_1$ to $u_3$, and the actuation delay from $u_3$ to $x_3$) and the physical delay (the delay from $x_1$ to $x_3$ through dynamic coupling) between the first three sub-systems of the chain.
%We require the information delay to be \emph{less than or equal to} the physical delay. In this case, the sub-controller $\tf u_3$ at the third sub-system receives advanced warning about the disturbance information $\tf w_1$ from the first sub-controller. The sub-controller $\tf u_3$ can then apply suitable control action to cancel the disturbance propagating through the second sub-system $\tf x_2$, and make the state $\tf x_3$ unaffected by the disturbance $\tf w_1$ in closed loop. As long as the state $\tf x_3$ is unaffected by the disturbance $\tf w_1$ in closed loop, all the state $\tf x_i$ for $i > 3$ are unaffected by the disturbance $\tf w_1$ in closed loop. 
%In this situation, we can analyze the system response of $\tf w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region. In particular, the complexity of analyzing the system response of $\tf w_1$ is independent to the size of the chain network, which means that our algorithm is scalable to arbitrary large network. From \eqref{eq:llqr-r}, we can analyze the system response for each $\tf w_j$ in their own localized region in a parallel way. The feasibility and optimality of the original problem \eqref{eq:llqr} are achieved even when the localized regions of each disturbance overlap.

%\begin{figure}[h!]
%      \centering
%      \includegraphics[width=0.4\textwidth]{./figure/Delay2.pdf}
%      \caption{Information delay and physical delay}
%      \label{fig:delay}
%\end{figure}

%As long as $\tf R_{31} = 0$, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ in closed loop. In this case, we can analyze the closed loop response of $w_1$ completely within the localized region specified in Figure \ref{fig:localized} without knowing the plant model information outside its localized region.
%It should be noted that the condition $\tf M_{31} = -a_{32} \tf R_{21}$ is feasible only when the communication speed between sub-controllers is sufficiently faster than the speed of disturbance propagation in the plant. The technical conditions to ensure the feasibility of \eqref{eq:llqr-r} is discussed extensively in the first part of this two-part paper \cite{2015_PartI}.
%to analyze the effect of each local disturbance within its \emph{localized region}. 
%In the above example, the localized region for the disturbance $w_1$ is given by its $2$-outgoing set $\Down{1}{2}$. As long as \eqref{eq:llqr-r} is feasible, the effect of the disturbance $w_1$ is contained within the set $\Down{1}{2}$. Note that there is an implicit boundary constraint imposed by the last equality constraint in \eqref{eq:llqr-r}. Specifically, if $a_{43}$ is nonzero, we must have $\tf R_{31} = 0$. This means that the state $x_3$ has to be uncorrelated to the disturbance $w_1$ in \emph{closed loop}. If this condition can be achieved, we can infer that all the states $x_i$ for $i \geq 3$ are also uncorrelated to $w_1$ -- the effect of the disturbance $w_1$ is localized within the set $\Down{1}{2}$. When $\tf R_{31} = 0$, we have $\tf M_{31} = -a_{32} \tf R_{21}$ from the second last equality constraint in \eqref{eq:llqr-r}. This means that we need to apply the control action $u_3$ for disturbance $w_1$ properly to cancel the coupling effect from $x_2$ to $x_3$ in order to make $x_3$ uncorrelated to $w_1$. This implicitly requires the communication speed between the sub-controllers to be faster than the speed of disturbance propagation in the plant. 
%In this example, the set $\rone_1$ is the collection of the colored nodes shown in Figure \ref{fig:localized}, and the set $\rtwo_1$ is the collection of the states contained within the localized region in Figure \ref{fig:localized}.
%The physical meaning of the set $\rone_j$ and $\rtwo_j$ in \eqref{eq:decom3} can be explained using the $d$-outgoing sets. Suppose that the locality constraint $\Ell$ is $d$-localized and the noise at different subsystem are uncorrelated to each other (which means $\colps_j = j$). In this case, the set $\rone_j$ is the collection of optimization variables contained within the localized region $\Down{j}{d}$, and the set $\rtwo_j$ is the extended localized region $\Down{j}{d+1}$. %region that can be affected by the variables in $\rone_j$. In the chain example \eqref{eq:llqr-r}, the set $\rtwo_j$ is given by the extended localized region $\Down{j}{d+1}$. 
%As long as the boundary set $\Down{j}{d+1} - \Down{j}{d}$ can be made uncorrelated to the disturbance $w_j$, the closed loop response of $w_j$ can be analyzed completely within its localized region $\Down{j}{d}$.

In summary, our approach to make the LLQR synthesis task scalable consists of two steps: (i) we perform a \emph{column-wise separation} of the problem, which allows us to analyze the system response of each local disturbance in an independent and parallel way, and (ii) we exploit the locality constraint $\Ell_R$ and $\Ell_M$ in \eqref{eq:llqr-r} to analyze the response of each local disturbance within its own localized region. 

%In the rest of this section, we generalize the LLQR problem to a broader class of problem which we called \emph{column-wise separable problems}. We show that all the column-wise separable problem can be solved using this decomposition technique in a localized and scalable way.

%to analyze the closed loop response of each uncorrelated disturbance within its own localized region in a parallel way. The direct decomposability of the problem ensures that global feasibility and optimality are achieved even when the localized regions for each disturbance overlap.
%The scalability and the efficiency of the algorithm primarily depend on the size of each localized region -- the algorithm is more efficient for smaller localized regions. 
%The primary role of column-wise decomposition is to make each localized region small. For instance, if we analyze the closed loop response of $w_i$ and $w_j$ simultaneously, then the localized region becomes the union of their own localized regions. If we do not decompose the problem \eqref{eq:llqr} column-wisely first, we cannot reduce the dimension of \eqref{eq:llqr} from global scale to local scale.

%Take \eqref{eq:llqr} as an example. Recall that $\Ell_R$ and $\Ell_M$ are pentadiagonal sparsity patterns, so $\Ell_R$ and $\Ell_M$ do not possess any zero row. If we do not perform a column-wise decomposition, we cannot reduce the dimension of the problem. On the other hand, if we decompose $\Ell_R$ and $\Ell_M$ column-wisely first, then we can reduce the dimension of each subproblem effectively since each column of $\Ell_R$ and $\Ell_M$ are highly sparse.
%For instance, suppose that the disturbances $\{w_1, w_2, w_3\}$ are correlated to each other, but uncorrelated to any other disturbances. The localized region for the disturbances $\{w_1, w_2, w_3\}$
%Dimension reduction -- localized region (implicit boundary constraint) 
%\input{Physical_v1}

%\subsection{Localized Synthesis and Re-synthesis}
%The controller synthesis procedure for directly decomposable problems is summarized in Algorithm \ref{ag:1}.
%
%%\begin{algorithm}[h!]
%%Given global plant model $(A, B_2)$ and a locality constraints $\mathcal{S}$ that described the localized region for each state\;
%%Set feasible = 1\;
%%\For {each state $x_j$}
%%{    
%%     Solve LLQR sub-problem \eqref{eq:llqr-l} on its localized region based on localized plant model\;
%%     \If {not feasible}
%%     {  
%%       feasible = 0\;
%%       break\;
%%     } 
%%}
%%
%%\If {feasible}
%%{    \For {each $j$-th LLQR sub-problem}
%%    {   
%%        Distribute the solution to the local controllers within its localized region \;
%%    }
%%}
%%\caption{Localized Synthesis} \label{ag:1}
%%\end{algorithm}
%\begin{algorithm}[h!]
%Given global plant model $(A, B_2)$, and sparse FIR constraint $\mathcal{S}$\;
%\For {each state perturbation $\delta{x_j}$}
%{    
%     Define localized region based on the block column sparsity of $\mathcal{S}$\;
%     Solve \eqref{eq:llqr-l} and derive $x_\ell, u_\ell$ within its localized region\;
%}
%
%\If {all sub-problems are feasible}
%{
%    \For {each sub-problem}
%    {   
%        Distribute the solution $x_\ell, u_\ell$ to the local controllers within its localized region \;
%    }
%}
%\caption{Localized Controller Synthesis for Directly Decomposable Problems} \label{ag:1}
%\end{algorithm}
%
%%Note that all the for loops in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. This not only facilitates real-time controller synthesis, but also suggests the possibility to do real-time \emph{re-synthesis} subject to model change that maintains global optimality.
%Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. 
%
%In addition, when the plant model change locally, we only need to resolve \emph{some} of the sub-problems. This suggests the possibility to do real-time \emph{re-synthesis} subject to model change that also maintains global optimality.

%\subsection{Extensions Beyond LLQR}
%In this subsection, we highlight the generalization of LLQR to a more broader class of problem, which we call the column-wise separable problem. 
%Let $\mathbb{Z}^+$ be the set of all positive integers. We use calligraphic lower case letters such as $\Set q$ to denote subsets of $\mathbb{Z}^+$. 
%%The cardinality of a set $\Set q$ is denoted by $| \Set q |$. 
%We say that $\{ \Set p_1, \dots \Set p_m \}$ is a partition of a set $\Set q \subset \mathbb{Z}^+$ if and only if $\Set p_i \not = \emptyset$ for all $i$, $\cup_{i=1}^m \Set p_i = \Set q$, and $\Set p_i \cap \Set p_j = \emptyset$ for all $i \not = j$. 
%
%Consider a transfer matrix $\ttf{\Phi}$ with $n_r$ rows and $n_c$ columns. Let $\rowps$ be a subset of $\{1, \dots, n_r \}$ and $\colps$ a subset of $\{1, \dots, n_c \}$. We use $\Sub{\ttf{\Phi}}{\rowps}{\colps}$ to denote the submatrix of $\ttf{\Phi}$ by selecting the rows according to the set $\rowps$ and columns according to the set $\colps$. When $\rowps = \{1, \dots, n_r \}$ is the set of all rows, we use the symbol $:$ to denote the set $\rowps$. Similarly, when $\colps = \{1, \dots, n_c \}$ is the set of all columns, we use $:$ to denote the set $\colps$. We have $\ttf{\Phi} = \Sub{\ttf{\Phi}}{:}{:}$. Let $\{ \colps_1, \dots \colps_p \}$ be a partition of the set $\{1, \dots, n_c\}$. Then $\{ \Sub{\ttf{\Phi}}{:}{\colps_1}, \dots,  \Sub{\ttf{\Phi}}{:}{\colps_p} \}$ is a column-wise partition of the transfer matrix $\ttf{\Phi}$.
%
%%Partition of a set, column/row-wise partition, cardinality of a set, complement of a set
%%Submatrices notation, transfer matrices (with FIR constraint)
%A permutation matrix is a square binary matrix that has exactly one entry of $1$ in each row and each column and zeros elsewhere.
%Block-wise sparsity pattern, multiplication of sparsity patterns

==> old/Abstract_v1.tex <==
%This paper proposes a novel control paradigm for large-scale network systems that achieves both scalability and near global optimality.
%Specifically, we introduce the notion of localizability for state and output feedback 
%This paper presents a novel feedback control scheme for localizable distributed systems subject to delay.
%These are systems for which the effect of both process noise and sensor noise can be localized in closed loop despite communications delays between controllers, akin to spatio-temporal dead-beat control with delays.
%We formulate the localized distributed optimal control problem in terms of the closed loop transfer matrices from perturbations to controlled output as a finite dimensional affinity constrained convex program.
%We then show that this convex program can be solved by distributed optimization technique in a localized manner, resulting a scalable way to synthesize near optimal controller for large-scale network.
%The controller can be implemented in a localized and thus scalable manner as well, which is essential when applying the scheme to large-scale systems.
%Simulation shows that for certain systems, our optimal controller, with its constraints on locality, settling time, and communication delay, can achieve similar performance to a idealized centralized optimal one.
%This paper proposes a novel optimal control theory for large-scale systems. 
This paper presents a novel state feedback control scheme for localizable distributed systems subject to delay.
These are systems for which the effect of each local disturbance can be localized in closed loop despite communications delays between controllers, akin to spatio-temporal dead-beat control with delays.
Specifically, we introduce the idea of state feedback localizability as a generalization of controllability into space-time domain, and characterize state feedback localizable systems in terms of the feasibility of a set of linear equations.
We then formulate the localized LQR (LLQR) problem for state feedback localizable system, and show that the global optimal solution can be computed in a completely localized and parallel way. 
The solution of each LLQR sub-problem can be used for controller synthesis by a local update algorithm, and each local controller only need to collect information from a localized region to compute its control action.
All these properties are extremely favorable for large-scale control systems, as the synthesis and the implementation of the controller can all be done in a localized and parallel way, regardless the dimension of the global system. 
Specifically, we show that when a model changes locally, we only need to re-synthesize some of the local controllers to ensure global optimality, which supports incremental design of the plant. 
%This supports the optimal plug-and-play feature, and is particularly favorable for large-scale systems.
Simulation shows that our optimal controller, with its constraints on locality, settling time, and communication delay, can achieve similar performance to an idealized centralized optimal one.
In particular, we synthesize a localized optimal controller for a large-scale unstable system with $10^{6}$ states, and achieve $99\%$ global optimality.




==> old/Chain.tex <==
\begin{figure*}[t!]
      \centering
      \includegraphics[width=0.85\textwidth]{./figure/Chart_black.pdf}
      \caption{Chain Model: Each $\mathbf{P_i}$ is a local plant and $\mathbf{C_i}$ a local controller. The numbers represent the delay between nodes. The actuation and plant propagation delay are one time step. The communication delay is $0.5$ time step, which means that the information is forwarded to both first and second neighbors at each time step.}
      \label{fig:Chart105}
\end{figure*}

In this section, we will use a simple chain model to illustrate various concepts throughout the paper. The key concepts include $d$-localized plant model, localized closed loop response, localized controller implementation, and localized controller synthesis. 

Consider a chain of $n$ dynamically coupled linear systems as shown in Figure \ref{fig:Chart105}. Denote $x_i$ the state of system $i$, and $u_i$ the control action of system $i$. We assume that each $x_i$ and $u_i$ are scalar variables. The dynamics of $x_i$ is given by the following equation
\begin{equation}
x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} a_{ij} x_j[k] + u_i[k] + w_i[k] \label{eq:purely_local}
\end{equation}
where $k$ is the time index, $w_i$ is the disturbance on system $i$, and $\mathcal{N}_i$ is the set of neighboring systems of system $i$. In this example, $\mathcal{N}_i = \{i-1, i+1\}$ for $i = 2, \dots, n-1$, $\mathcal{N}_1 = \{2\}$, and $\mathcal{N}_n = \{n-1\}$. In \eqref{eq:purely_local}, the first term is the local dynamics, and the second term is the coupling term induced by the interconnection of the systems.

Define the global state vector $\mathbf{x} = [x_1^\top, \dots, x_n^\top]^\top$, global control vector $\mathbf{u} = [u_1^\top, \dots, u_n^\top]^\top$, and global disturbance vector $\mathbf{w} = [w_1^\top, \dots, w_n^\top]^\top$. The global system model can then be written as
\begin{equation}
\mathbf{x}[k+1] = \mathbf{A} \mathbf{x}[k] + \mathbf{u}[k] + \mathbf{w}[k] \label{eq:global}
\end{equation}
where $\mathbf{A}$ is a $n \times n$ tridiagonal matrix.

In practice, the global plant model in \eqref{eq:global} may not be available for all system $i$ when the number of system $n$ is large. On the other hand, using the local model 

==> old/Chain2.tex <==
\begin{figure*}[t!]
      \centering
      \includegraphics[width=0.85\textwidth]{./figure/Chart_black.pdf}
      \caption{Chain Model: Each $\mathbf{P_i}$ is a local plant and $\mathbf{C_i}$ a local controller. The numbers represent the delay between nodes. The actuation and plant propagation delay are one time step. The communication delay is $0.5$ time step, which means that the information is forwarded to both first and second neighbors at each time step.}
      \label{fig:Chart105}
\end{figure*}

Consider $n$ dynamically coupled linear systems with interconnection described by a directed graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$. Each node $i \in \mathcal{V}$ represents a linear system, and each edge in $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction of these systems. Denote $x_i$ the state of system $i$, and $u_i$ the control action of system $i$. For ease of explanation, we first assume that all $x_i$ and $u_i$ are scalar variables. Define the neighboring systems of system $i$ by $\mathcal{N}_i = \{j | (j,i) \in \mathcal{E} \}$. Assume that the dynamics of $x_i$ is given by the following equation
\begin{equation}
x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} a_{ij} x_j[k] + b_i u_i[k] + w_i[k] \label{eq:purely_local}
\end{equation}
where $k$ is the time index and $w_i$ is the disturbance on system $i$. The first term in \eqref{eq:purely_local} is the local dynamics, and the second term in \eqref{eq:purely_local} is the coupling term induced by the interconnection of these systems. In addition, if system $i$ does not have a controller, we can simply set $b_i = 0$.

Define the global state vector $\mathbf{x} = [x_1^\top, \dots, x_n^\top]^\top$, global control vector $\mathbf{u} = [u_1^\top, \dots, u_n^\top]^\top$, and global disturbance vector $\mathbf{w} = [w_1^\top, \dots, w_n^\top]^\top$. The global system dynamics can then be written into a single equation as
\begin{equation}
\mathbf{x}[k+1] = A \mathbf{x}[k] + B_2 \mathbf{u}[k] + \mathbf{w}[k] \label{eq:global}
\end{equation}
where $A$ and $B_2$ are $n \times n$ matrices.

%In practice, the global plant model in \eqref{eq:global} may not be available for all system $i$ when the number of system $n$ is large. On the other hand, using the local model

\begin{example}
Chain
\end{example}

The objective of this paper is to design a distributed dynamic state-feedback controller such that the transfer functions from $\mathbf{w}$ to $\mathbf{x}$ and $\mathbf{w}$ to $\mathbf{u}$ satisfy some spatio-temporal (locality) constraints. Throughout this paper, we use $R$ to denote the closed loop transfer function from $\mathbf{w}$ to $\mathbf{x}$ and $M$ the closed loop transfer function from $\mathbf{w}$ to $\mathbf{u}$. The key idea in this paper is to force $R$ and $M$ to satisfy some spatio-temporal constraints, then show that the controller achieving the desired closed loop response can be synthesized and implemented by $R$ and $M$.

The spatio-temporal constraints can be defined based on the graphical structure $\mathcal{G}$ of the interconnected system. Note that $\mathcal{G}$ can be completely characterized by the sparsity pattern of $A$. Specifically, the transpose of $A$ has the same sparsity pattern as the adjacency matrix of $\mathcal{G}$. In the next subsection, we will exploit the sparseness of matrix $A$ and use it as a basis to define the notion of spatio-temporal constraints.


%Consider an interconnected network system described by a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where each node in $\mathcal{V}$ represents a sub-system, and the set $\mathcal{E}$ encodes the interaction between these sub-systems. We start with a simple case that each node contains a scalar state variable $x_i$ and a scalar control signal $u_i$. Assume that the value of the state variable evolves according to the following rule
%\begin{equation}
%x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{U}_{(i,1)}} a_{ij} x_j[k] + u_i[k] + w_i[k]
%\end{equation}
%where $k$ is the time index and $w_i$ is the disturbance on system $i$. Define the global state vector $\mathbf{x} = [x_1^\top, \dots, x_n^\top]^\top$ and global control vector $\mathbf{u} = [u_1^\top, \dots, u_n^\top]^\top$. The global system model can then be written as
%\begin{equation}
%\mathbf{x}[k+1] = \mathbf{A} \mathbf{x}[k] + \mathbf{u}[k] + \mathbf{w}[k]
%\end{equation}

%Denote $\mathcal{N}_i$ the set of systems that has a direct effect on the state of system $i$. 
%where each node $v \in \mathcal{V}$ represents a sub-system and each link $e \in mathcal{E}$ represents the interaction of different sub-systems. We start with a simple case that each node contain

%We start with a chain of $n$ interconnected sub-systems as shown in Figure \ref{fig:Chart105}. We assume that each sub-system contains a single scalar state $x_i$ associated with a scalar control action $u_i$, for $i = 1, \dots, n$. The value of the state is evolved according to the following rule
%\begin{equation}
%x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} a_{ij} x_j[k] + u_i[k]
%\end{equation}

%\begin{eqnarray}
%x_1[k+1] &=& a_{1,1} x_1[k] + a_{1,2} x_{2}[k] + u_1[k] \nonumber\\
%x_i[k+1] &=& a_{i,i} x_i[k] + a_{i,i-1} x_{i-1}[k] + a_{i,i+1} x_{i+1}[k] + u_i[k] \text{ for } i = 2, \dots, n-1 \nonumber\\
%x_n[k+1] &=& a_{n,n-1} x_{n-1}[k] + a_{n,n} x_{n}[k] + u_n[k]
%\end{eqnarray}
%where $k$ is the time index and all $a_{i,j}$ are parameters.
 

==> old/Chain3.tex <==
\begin{figure*}[t!]
      \centering
      \includegraphics[width=0.85\textwidth]{./figure/Chart_black.pdf}
      \caption{Chain Model: Each $\mathbf{P_i}$ is a local plant and $\mathbf{C_i}$ a local controller. The numbers represent the delay between nodes. The actuation and plant propagation delay are one time step. The communication delay is $0.5$ time step, which means that the information is forwarded to both first and second neighbors at each time step.}
      \label{fig:Chart105}
\end{figure*}

In this section, we introduce a simple chain model to illustrate various concepts in the paper. We will explain why this simple model raises significant challenge to current control theory, and such problem cannot be solved by existing methods in the field of distributed optimal control. We also use this model to give intuition on the ideas about localized plant model, localized closed loop response, localized controller implementation, and localized controller synthesis, where the generalization of these concepts will be defined in a formal way in the next few sections.

Consider a chain of $n$ dynamically coupled linear systems as shown in Figure \ref{fig:Chart105}. Denote $x_i$ the state of system $i$, and $u_i$ the control action of system $i$. For ease of explanation, we first assume that each $x_i$ and $u_i$ are scalar variables. Assume that the dynamics of $x_i$ is given by the following equation
\begin{equation}
x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} a_{ij} x_j[k] + b_i u_i[k] + w_i[k] \label{eq:purely_local}
\end{equation}
where $k$ is the time index, $w_i$ is the disturbance on system $i$, and $\mathcal{N}_i$ is the set of neighboring systems of system $i$. Specifically, $\mathcal{N}_i = \{i-1, i+1\}$ for $i = 2, \dots, n-1$, $\mathcal{N}_1 = \{2\}$, and $\mathcal{N}_n = \{n-1\}$. In \eqref{eq:purely_local}, the first term is the local dynamics, and the second term is the coupling term induced by the interconnection of the systems. In addition, if system $i$ does not have an actuator, we can simply set $b_i = 0$.

Define the global state vector $\mathbf{x} = [x_1^\top, \dots, x_n^\top]^\top$, global control vector $\mathbf{u} = [u_1^\top, \dots, u_n^\top]^\top$, and global disturbance vector $\mathbf{w} = [w_1^\top, \dots, w_n^\top]^\top$. The global system dynamics can then be summarized into a single equation as
\begin{equation}
\mathbf{x}[k+1] = A \mathbf{x}[k] + B_2 \mathbf{u}[k] + \mathbf{w}[k] \label{eq:global}
\end{equation}
where $B_2 = \text{diag}(b_1, \dots, b_n)$ and $A$ is a $n \times n$ tridiagonal matrix.

The goal


In practice, the global plant model in \eqref{eq:global} may not be available for all system $i$ when the number of system $n$ is large. On the other hand, using the local model 

%Consider $n$ dynamically coupled linear systems with interconnection described by a directed graph $

%In practice, the global plant model in \eqref{eq:global} may not be available for all system $i$ when the number of system $n$ is large. On the other hand, using the local model

\begin{example}
Chain
\end{example}

The objective of this paper is to design a distributed dynamic state-feedback controller such that the transfer functions from $\mathbf{w}$ to $\mathbf{x}$ and $\mathbf{w}$ to $\mathbf{u}$ satisfy some spatio-temporal (locality) constraints. Throughout this paper, we use $R$ to denote the closed loop transfer function from $\mathbf{w}$ to $\mathbf{x}$ and $M$ the closed loop transfer function from $\mathbf{w}$ to $\mathbf{u}$. The key idea in this paper is to force $R$ and $M$ to satisfy some spatio-temporal constraints, then show that the controller achieving the desired closed loop response can be synthesized and implemented by $R$ and $M$.

The spatio-temporal constraints can be defined based on the graphical structure $\mathcal{G}$ of the interconnected system. Note that $\mathcal{G}$ can be completely characterized by the sparsity pattern of $A$. Specifically, the transpose of $A$ has the same sparsity pattern as the adjacency matrix of $\mathcal{G}$. In the next subsection, we will exploit the sparseness of matrix $A$ and use it as a basis to define the notion of spatio-temporal constraints.


%Consider an interconnected network system described by a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where each node in $\mathcal{V}$ represents a sub-system, and the set $\mathcal{E}$ encodes the interaction between these sub-systems. We start with a simple case that each node contains a scalar state variable $x_i$ and a scalar control signal $u_i$. Assume that the value of the state variable evolves according to the following rule
%\begin{equation}
%x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{U}_{(i,1)}} a_{ij} x_j[k] + u_i[k] + w_i[k]
%\end{equation}
%where $k$ is the time index and $w_i$ is the disturbance on system $i$. Define the global state vector $\mathbf{x} = [x_1^\top, \dots, x_n^\top]^\top$ and global control vector $\mathbf{u} = [u_1^\top, \dots, u_n^\top]^\top$. The global system model can then be written as
%\begin{equation}
%\mathbf{x}[k+1] = \mathbf{A} \mathbf{x}[k] + \mathbf{u}[k] + \mathbf{w}[k]
%\end{equation}

%Denote $\mathcal{N}_i$ the set of systems that has a direct effect on the state of system $i$. 
%where each node $v \in \mathcal{V}$ represents a sub-system and each link $e \in mathcal{E}$ represents the interaction of different sub-systems. We start with a simple case that each node contain

%We start with a chain of $n$ interconnected sub-systems as shown in Figure \ref{fig:Chart105}. We assume that each sub-system contains a single scalar state $x_i$ associated with a scalar control action $u_i$, for $i = 1, \dots, n$. The value of the state is evolved according to the following rule
%\begin{equation}
%x_i[k+1] = a_{ii} x_i[k] + \sum_{j \in \mathcal{N}_i} a_{ij} x_j[k] + u_i[k]
%\end{equation}

%\begin{eqnarray}
%x_1[k+1] &=& a_{1,1} x_1[k] + a_{1,2} x_{2}[k] + u_1[k] \nonumber\\
%x_i[k+1] &=& a_{i,i} x_i[k] + a_{i,i-1} x_{i-1}[k] + a_{i,i+1} x_{i+1}[k] + u_i[k] \text{ for } i = 2, \dots, n-1 \nonumber\\
%x_n[k+1] &=& a_{n,n-1} x_{n-1}[k] + a_{n,n} x_{n}[k] + u_n[k]
%\end{eqnarray}
%where $k$ is the time index and all $a_{i,j}$ are parameters.
 

==> old/DOC_v1.tex <==
Consider a stable discrete time plant model given by
\begin{equation}
P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & 0 & D_{12} \\ C_2 & D_{21} & 0 \end{array} \right] = \begin{bmatrix}
P_{11} & P_{12} \\ P_{21} & P_{22} \end{bmatrix}. \label{eq:g_plant}
\end{equation}

Let $K$ be the transfer function from $y$ to $u$, i.e. $u = K y$. The optimal control problem of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$, although our formulation is amenable to any convex measure of closed loop performance.} of the closed loop transfer function from the disturbances to the controlled output is formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} &&|| P_{11} + P_{12} K(I-P_{22}K)^{-1} P_{21}|| \nonumber\\
\text{subject to } && K \in \mathcal{S}_c  \nonumber\\
&& K(I-P_{22}K)^{-1} \in \RHinf \label{eq:matching_0}
\end{eqnarray}
where $\mathcal{S}_c$ is the information sharing constraint that $K$ must satisfy in order to be implementable on the communication network of the system.  As can be seen, this problem is not convex in $K$, and as alluded to in the introduction, only certain classes of $\mathcal{S}_c$ can be reformulated in a convex manner.

The information sharing constraint $\mathcal{S}_c$ is said to be QI \cite{2006_Rotkowitz_QI_TAC} under $P_{22}$ if $K P_{22} K \in \mathcal{S}_c$ for all $K \in \mathcal{S}_c$. If $\mathcal{S}_c$ is QI under $P_{22}$, then $K \in \mathcal{S}_c$ is equivalent to $Q \in \mathcal{S}_c\cap\RHinf$, where $Q = K(I-P_{22}K)^{-1}$ is the Youla parametrization\cite{2006_Rotkowitz_QI_TAC}. Thus, we can convexify \eqref{eq:matching_0} by a change of variable as 
\begin{eqnarray}
\underset{Q}{\text{minimize  }} &&|| P_{11} + P_{12} Q P_{21}|| \nonumber\\
\text{subject to } && Q \in \mathcal{S}_c\cap\RHinf. \label{eq:matching}
\end{eqnarray}
The controller is then implemented by $K = (I + Q P_{22})^{-1} Q$, and $K \in \mathcal{S}_c$.

As discussed previously, the primary limitation of this formulation is that locality constraints are not QI for strongly connected plants -- thus the aforementioned reparameterization does not yield a $K$ that satisfies the locality constraints, even if such a $Q$ could be computed. However, it is important to note that this does not mean that the controller cannot be implemented in a localized way. In the next section, we will reformulate \eqref{eq:matching} in terms of the closed loop transfer matrix from the perturbations $(\delta_x, \delta_y)$ to $(x,u)$, upon which we can impose the locality constraint. We will show that the localized distributed controller can be synthesized directly from this closed loop transfer matrix. 


==> old/Extension.tex <==
Up to this point, our localized control scheme is based on a fixed $(d,T)$-localized FIR constraint $(\mathcal{S}_R, \mathcal{S}_M)$. In this section, we will discuss how to determine the parameter $(d,T)$  for a system $(A, B_2)$ to ensure that the transient performance is close to unconstrained global optimal. Next, we will discuss how to \emph{design} the plant model $(A, B_2)$ to ensure localizability. 

\subsection{Localized Lower Bound}


The general strategy to determine the 

\subsection{Spatial Localizability}

==> old/Graph.tex <==
%\subsection{Preliminaries on Graph Theory}
For a square matrix $A$, we define the state transition graph as follows.
\begin{definition}
The state transition graph of a $n \times n$ matrix $A$ is a directed graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V} = \{x_1, \dots, x_n\}$ is the set of vertices, and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the set of directed edges. In particular, $(x_i, x_j) \in \mathcal{E}$ if and only if $A_{ji} \not = 0$.
\end{definition}

\begin{example}
For a tridiagonal $n \times n$ matrix $A$, the state transition graph is given by the physical plant in Figure \ref{fig:Chart105}.
\end{example}

A \emph{directed path} of a graph is a sequence of directed edges which connect a sequence of vertices, with all edges directed in the same direction. The \emph{length} of a path is the number of edges of that path. The \emph{distance} from $x_i$ to $x_j$ is the length of a shortest path which connect $x_i$ to $x_j$. 


%In terms of the vertex adjacency matrix $\mathcal{A}$, the distance function can also be written as
%\begin{equation}
%\displaystyle \dist{v_i}{v_j}{\mathcal{A}}: = \min\{ k \in \mathbb{N} \cup 0 \, | \, \left(\mathcal{A}^{k}\right)_{ji} \neq 0\} \nonumber
%\end{equation}
%with the definition $\mathcal{A}^0 = I$.


==> old/Implementation.tex <==
In this section, we show how to synthesize and implement the controller that achieves the desired closed loop response specified in the previous section. Specifically, we show that the controller achieves the desired localized closed loop response can be synthesized and implemented in a localized manner as well. Finally, we show how to re-synthesize the optimal controller in a localized way when the plant model changes locally. This allows incremental design when the physical system expands.

\subsection{Localized Implementation}
To achieve a desired closed loop response $R = \sum_{i=1}^{T} \frac{1}{z^i}R[i]$ and $M = \sum_{i=1}^{T} \frac{1}{z^i}M[i]$, the controller can be implemented by the following equations
\begin{eqnarray}
w_e [k] &=& x[k] - x_r [k] \label{eq:rhc_we} \\
u[k] &=& \sum_{\tau = 0}^{T-1} M[\tau+1] w_e [k-\tau] \label{eq:rhc_u}\\
x_r [k+1] &=& \sum_{\tau = 0}^{T-2} R[\tau+2] w_e [k-\tau]. \label{eq:rhc_xr}
\end{eqnarray}

In comparison to the column-wise decomposition for localized synthesis, the localized implementation can be seen from the row-wise decomposition of \eqref{eq:rhc_we} - \eqref{eq:rhc_xr}. Focus on the $i$-th row of \eqref{eq:rhc_xr}. From the definition of $(A,d)$ sparseness for $R$, $(x_r)_i$ can be generated by collecting the estimated disturbance from the set $Up(i,d)$. Let $u_{c_i}$ be the control action that affects $x_i$ only, i.e. the $(i, c_i)$-entry of $B_2$ is the only nonzero entry in the $c_i$-th column. The control action $u_{c_i}$ can be generated by collecting the estimated disturbance from the set $Up(i,d+1)$. Furthermore, as we impose communication delay constraint on $R$ and $M$, the implementation \eqref{eq:rhc_we} - \eqref{eq:rhc_xr} is realizable with finite communication speed.

The row-wise decomposition of \eqref{eq:rhc_we} - \eqref{eq:rhc_xr} imply that the controller can be implemented in a localized and parallel way. At each time step, every controller (i) measures its own state and computes its own estimated disturbance by \eqref{eq:rhc_we}, (ii) broadcasts its estimated disturbance out to its downstream set and collects estimated disturbances from its upstream sets, (iii) computes its control strategy and reference trajectory based on the collected estimated disturbances by \eqref{eq:rhc_u}-\eqref{eq:rhc_xr}, and (iv) applies the control action. 
%This general strategy, as implemented at a single node, can be illustrated through Figure \ref{fig:lightcones}.
%Similarly, each local controller $u_i$ only needs to collect $(w_e)_j$, for $j \in \bigcap_{\ell} \mathcal{E}_{(\ell,d+1)}$, with $l \in \{\ell \, | \, B_{\ell i} \not = 0\}$, to generate its control action. 
%In Figure \ref{fig:lightcones}, the 

\begin{example}
Recall that the affected region for each local disturbance in the chain model can be plotted in the space-time diagram as in Figure \ref{fig:region}. The localized controller implementation for the chain model can also be illustrated in a similar way. Figure \ref{fig:lightcones} shows the relation between the affected region of a local disturbance $w_j$ and the information collection region of a local control action $u_{c_i}$. Note that $i \in Down(j,d+1)$ is equivalent to $j \in Up(i,d+1)$. Therefore, $u_{c_i}$ is in the affected region of $w_j$ if and only if $w_j$ is in the information collection region of $u_{c_i}$. In terms of the sparsity pattern of $R$ and $M$, the affected regions are defined by the sparsity pattern of the columns of $R$ and $M$, and the information collection regions are defined by the sparsity pattern of the rows of $R$ and $M$.
\end{example}

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.48\textwidth]{figure/Forbackward.pdf}
      \caption{Local space-time region interpretation of proposed control strategy.}
      \label{fig:lightcones}
\end{figure}

%At each time step, every controller (i) collects estimated disturbances from its upstream sets, (ii) computes its control strategy and reference trajectory based on the collected estimated disturbances by \eqref{eq:rhc_u}-\eqref{eq:rhc_xr}, (iii) applies the control action and measures its own state, and (iv) computes its own estimated disturbance by \eqref{eq:rhc_we} and broadcasts it out to its downstream set. This general strategy, as implemented at a single node, is illustrated in Figure \ref{fig:lightcones}.

%\begin{figure}[ht!]
%      \centering
%      \includegraphics[width=0.48\textwidth]{figure/lightcones8.pdf}
%      \caption{Local space-time region interpretation of proposed control strategy.}
%      \label{fig:lightcones}
%\end{figure}

The implementation \eqref{eq:rhc_we}-\eqref{eq:rhc_xr} can also be realized by filters. As $R[1] = I$, \eqref{eq:rhc_we}-\eqref{eq:rhc_xr} can be written in the frequency domain as
\begin{eqnarray}
w_e &=& x - x_r \label{eq:rhc_we2} \\
u &=& zM w_e \label{eq:rhc_u2}\\
x_r &=& (zR - I) w_e. \label{eq:rhc_xr2}
\end{eqnarray}
We define $\tilde{R} = zR - I$ and $\tilde{M} = zM$. From \eqref{eq:freq}, we have $\tilde{R} = zR - I = A R + B_2 M$. As $R, M \in \mathcal{RH}_{\infty}^{sp}$, we have $\tilde{R} \in \mathcal{RH}_{\infty}^{sp}$ and $\tilde{M} \in \mathcal{RH}_{\infty}$. In addition, both $\tilde{R}$ and $\tilde{M}$ are FIRs. Equations \eqref{eq:rhc_we2}-\eqref{eq:rhc_xr2} leads to the controller structure given by Figure \ref{fig:structure}. In this figure, the red block is the plant model given by \eqref{eq:dynamics}, and the blue block is the controller. In the next subsection, we will show that the controller structure given in Figure \ref{fig:structure} internally stabilizes the plant, and indeed achieves the desired closed loop response $(R,M)$ for the process disturbance $w$. 
%Before going into the detail of analysis, we will first show that \eqref{eq:rhc_we2}-\eqref{eq:rhc_xr2} is a localized implementation, and is realizable with finite communication speed.

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.45\textwidth]{./figure/K_structure.pdf}
      \caption{The structure of localized feedback controller, with $\tilde{R} = zR - I$ and $\tilde{M} = zM$.}
      \label{fig:structure}
\end{figure}

\begin{remark}
The transfer function $K$ in Figure \ref{fig:structure} is usually not sparse due to the inverse relation $K = M R^{-1}$.  On the other hand, if $K$ is sparse and strictly proper, then $R$ will usually not be sparse except specific structures (non strongly connected) since $R = (zI - A - B_2 K)^{-1}$. This means that for a sparse $K$, the effect of a local disturbance will in general affect \emph{all} the states in closed loop, which makes local analysis difficult. This is part of the reason why the works in \cite{2004_Dullerud, 2013_Farokhi_model}  can be quite conservative. In this paper, we directly use $R$ and $M$ for controller implementation and synthesis, so the fundamental difficulty for sparse $K$ can be avoided.
\end{remark}

\subsection{Robustness Analysis}
The conventional way to check internal stability of a closed loop structure is testing the stability of the closed loop transfer functions from $(w, v_x, v_u)$ to $(x,u)$, where $v_x$ and $v_u$ are perturbation on $x$ and $u$, respectively. If all these six transfer functions are stable, then the controller internally stabilizes the plant. In Figure \ref{fig:structure}, we assume that the controller is decomposed into the $\tilde{R}$ loop and $\tilde{M}$ loop. To show that this specific structure is stabilizing, we need to introduce extra perturbation into the system. In Figure \ref{fig:internal}, five extra perturbation signals $(v_x, v_u, v_R, v_M, v_A)$ are introduced into the system, where $v_R$ and $v_M$ are extra perturbations inside the controller, and $v_A$ is a perturbation inside the plant. Any other possible perturbation can all be written as a linear combination of these five signals. It suffices to check the stability of the transfer function from $(w, v_x, v_u, v_R, v_M, v_A)$ to all internal variable $(w_e, x, u)$ to determine internal stability of the controller structure.

\begin{figure}[ht!]
      \centering
      \includegraphics[width=0.49\textwidth]{./figure/Internal.pdf}
      \caption{Perturbation test on internal stability. All circles in the figure represents addition.}
      \label{fig:internal}
\end{figure}

Table \ref{Table:1} summarizes the closed loop transfer functions from $(w, v_x, v_u, v_R, v_M, v_A)$ to $(w_e, x, u)$. Clearly, all transfer functions are stable, so the controller structure in Figure \ref{fig:structure} internally stabilizes the plant. In fact, all transfer functions in Table \ref{Table:1} are localized FIRs, meaning that the effect of the perturbation occurring anywhere in the structure can be limited spatially and temporally. For instance, the transfer function from $v_R$ to $x$ is $-(\tilde{R} - R A) \tilde{R}$. As $\tilde{R}$ and $R$ are $(A,d)$ sparse, this transfer function is $(A, 2d+1)$ sparse. In particular, when the perturbation is on the estimated disturbance, that is, $v_w = v_R = v_M$, the closed loop transfer functions from $v_w$ to $(w_e, x, u)$ are $(- \frac{1}{z} A, \tilde{R} - R A, \tilde{M} - M A)$. This implies that the closed loop system under perturbation $v_w$ will automatically be $(d+1,T)$ localizable. Finally, all the argument above is true regardless of the stability of the open loop system $A$. 

\begin{table*}[t]
 \caption{Transfer Functions from Perturbation to Internal Variables}
 \label{Table:1}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c | c | c | c | c | c |}
    \hline 
    & $w$ & $v_x$ & $v_u$ & $v_R$ & $v_M$ & $v_A$ \\ \hline
    $w_e$ & $\frac{1}{z} I$ & $I - \frac{1}{z} A$ & $\frac{1}{z} B_2$ & $-(I-\frac{1}{z}A)\tilde{R}$ & $\frac{1}{z}B_2 \tilde{M}$ & $\frac{1}{z} A$ \\ \hline
    $x$ & $R$ & $\tilde{R} - R A$ & $R B_2$ & $-(\tilde{R} - R A) \tilde{R}$ & $R B_2 \tilde{M}$ & $R A$ \\ \hline
    $u$ & $M$ & $\tilde{M} - M A$ & $I + M B_2$ & $-(\tilde{M} - M A) \tilde{R}$ & $(I + M B_2) \tilde{M}$ & $M A$ \\ \hline
    \end{tabular}
\end{center}
\end{table*}

We now consider the case that the system is not \emph{exactly} $(d,T)$ localizable, which means that \eqref{eq:freq} is not exactly feasible.
%In the above, the assumption is that the system is \emph{exactly} $(d,T)$ localizable, which means that \eqref{eq:freq} is feasible. 
The non-localizability may come from the small computation error, model uncertainty or model bias, or simply due to the fact that the system is no exactly localizable. The degree of non-localizability can be characterized by a perturbation transfer function $\Delta_{RM}$ on \eqref{eq:freq} as
%In practice, there may be some small computation error or model uncertainty that causes non-localizability. The analysis of those effects can be described by the following equations
\begin{eqnarray}
&& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I + \Delta_{RM}\nonumber\\
&& \begin{bmatrix} R \\ M \end{bmatrix} \in \begin{bmatrix} \mathcal{S}_R \\ \mathcal{S}_M \end{bmatrix}.  \label{eq:freq_delta}
\end{eqnarray}
%where $\Delta_{RM}$ is a perturbation transfer function that characterizes the degree of non-localizability. 
The following theorem gives a sufficient condition on global stability of the controller structure in Figure \ref{fig:structure} in the presence of $\Delta_{RM}$.

\begin{theorem}
If $(I + \Delta_{RM})^{-1}$ is stable, then the state feedback controller with structure given by Figure \ref{fig:structure} internally stabilizes the plant.
\end{theorem}
\begin{proof}
This can be done through the same perturbation analysis as in Figure \ref{fig:internal} by replacing \eqref{eq:freq} by \eqref{eq:freq_delta}. The closed loop transfer functions from $(w, v_x, v_u, v_R, v_M, v_A)$ to $(w_e, x, u)$ are summarized in Table \ref{Table:2}, where $I_\Delta = (I+\Delta_{RM})^{-1}$. Clearly, if $I_\Delta$ is stable, all the transfer functions in Table \ref{Table:2} will be stable, so the structure in Figure \ref{fig:structure} internally stabilizes the plant.
\end{proof}

\begin{table*}[t]
 \caption{Transfer Functions from Perturbation to Internal Variables with Non-localizability}
 \label{Table:2}
\begin{center}
\renewcommand{\arraystretch}{2}
    \begin{tabular}{| c | c | c | c | c | c | c | c |}
    \hline 
    & $w$ & $v_x$ & $v_u$ & $v_R$ & $v_M$ & $v_A$ \\ \hline
    $w_e$ & $\frac{1}{z} I_\Delta$ & $I_\Delta (I - \frac{1}{z} A)$ & $\frac{1}{z} I_\Delta B_2$ & $-I_\Delta(I-\frac{1}{z}A)\tilde{R}$ & $\frac{1}{z} I_\Delta B_2 \tilde{M}$ & $\frac{1}{z} I_\Delta A$ \\ \hline
    $x$ & $R I_\Delta$ & $(I+\tilde{R})I_\Delta(I-\frac{1}{z}A) - I$ & $R I_\Delta B_2$ & $[ I - (I+\tilde{R})I_\Delta(I-\frac{1}{z}A) ] \tilde{R}$ & $R I_\Delta B_2 \tilde{M}$ & $R I_\Delta A$ \\ \hline
    $u$ & $M I_\Delta$ & $\tilde{M}I_\Delta(I-\frac{1}{z}A)$ & $I + M I_\Delta B_2$ & $-\tilde{M}I_\Delta(I-\frac{1}{z}A)\tilde{R}$ & $[ I + M I_\Delta B_2 ]\tilde{M}$ & $M I_\Delta A$ \\ \hline
    %    & $w$ & $v_x$ & $v_u$ & $v_R$ & $v_M$ & $v_A$ \\ \hline
%    $w_e$ & $\frac{1}{z} (I + \Delta_{RM})^{-1}$ & $(I + \Delta_{RM})^{-1} (I - \frac{1}{z} A)$ & $\frac{1}{z} (I + \Delta_{RM})^{-1} B_2$ & $-(I + \Delta_{RM})^{-1}(I-\frac{1}{z}A)\tilde{R}$ & $\frac{1}{z}(I + \Delta_{RM})^{-1}B_2 \tilde{M}$ & $\frac{1}{z} (I + \Delta_{RM})^{-1}A$ \\ \hline
%    $x$ & $R(I + \Delta_{RM})^{-1}$ & $(I+\tilde{R})(I + \Delta_{RM})^{-1}(I-\frac{1}{z}A) - I$ & $R (I + \Delta_{RM})^{-1}B_2$ & $[ I - (I+\tilde{R})(I + \Delta_{RM})^{-1}(I-\frac{1}{z}A) ] \tilde{R}$ & $R(I + \Delta_{RM})^{-1} B_2 \tilde{M}$ & $R(I + \Delta_{RM})^{-1}A$ \\ \hline
%    $u$ & $M(I + \Delta_{RM})^{-1}$ & $\tilde{M}(I + \Delta_{RM})^{-1}(I-\frac{1}{z}A)$ & $I + M(I + \Delta_{RM})^{-1}B_2$ & $-\tilde{M}(I + \Delta_{RM})^{-1}(I-\frac{1}{z}A)\tilde{R}$ & $[ I + M(I + \Delta_{RM})^{-1}B_2 ]\tilde{M}$ & $M(I + \Delta_{RM})^{-1}A$ \\ \hline
    \end{tabular}
\end{center}
\end{table*}

Note that in the present of $\Delta_{RM}$, the closed loop response is no longer exactly localizable. However, when $\Delta_{RM}$ is small enough, $I_\Delta = (I+\Delta_{RM})^{-1}$ will be stable, and the structure in Figure \ref{fig:structure} is globally stable. This robustness allows approximated solution for localized controller implementation for nearly localizable systems.

\subsection{Localized Synthesis} \label{sec:syn}
The row-wise interpretation of \eqref{eq:rhc_we2}-\eqref{eq:rhc_xr2} indicates that the synthesis of each local controller only depends on the LLQR solution locally. From Figure \ref{fig:lightcones}, each local controller $u_{c_i}$ can be synthesized based on the LLQR sub-problems \eqref{eq:lqr_op_0} for $j \in Up(i,d+1)$. In other words, the global optimal LLQR controller can be synthesized by exchanging the solution of each LLQR sub-problem \eqref{eq:lqr_op_0} locally. We summarize this procedure into the following algorithm.

%In this subsection, we combine the result of LLQR and localized implementation as a localized synthesis algorithm as follows. 
%We conclude this section with an algorithm that summarizes our developments, and which provides a scalable, distributed and entirely local means of synthesizing a $(d,T)$-localizing state-feedback controller.

\begin{algorithm}[h!]
Given global plant model $(A,B_2)$ and a $(d,T)$-localized FIR constraints $(\mathcal{S}_R, \mathcal{S}_M)$\;
Set feasible = 1\;
\For {each state $x_j$}
{    
     Solve LLQR sub-problem \eqref{eq:lqr_op_0} on $Down(j,d+1)$ based on localized plant model\;
     \If {not feasible}
     {  
       feasible = 0\;
       break\;
     } 
}

\If {feasible}
{    \For {each $j$-th LLQR sub-problem}
    {   
        Distribute the solution of LLQR sub-problem (reference trajectory $x_r$ and control action $u$) to the set $Down_(j,d+1)$\; 
    }
    \For {each local controller}
    {     
          Collect the solution from its upstream set and synthesize each column of $R$ and $M$\;
 %         Implement the controller based on $R$ and $M$\;       
    }
}
\caption{Localized Synthesis} \label{ag:1}
\end{algorithm}

Note that all the for loop in Algorithm \ref{ag:1} can be implemented in a completely parallel, localized, and scalable way. As each LLQR sub-problem can be solved analytically, this also facilitates real-time controller synthesis, and is well-suited to model predictive control (MPC) architecture.

\subsection{Localized Re-synthesis}
As the LLQR controller can be synthesized in real-time, our control scheme also supports incremental design and plug-and-play (PnP) feature of an interconnected network system. Assume that the model changes locally, for instance, the value of $A_{ij}$ changes. We only need to resolve $k$-th LLQR sub-problems for $k \in Up(j,d)$, while all the other solution remaining the same. If all the LLQR sub-problems for $k \in Up(j,d)$ are feasible, then the global system is $(d,T)$ localizable. We then update the solution of these LLQR problems locally into the set $Down(k,d+1)$ for all $k \in Up(j,d)$, and the global system is keeping optimal. In particular, when the state transition graph of $A$ is undirected ($\Sp{A}$ is symmetric), we have $Up(j,d) = Down(j,d)$. So only the controller within the set $Down(j, 2d+1)$ need to be changed to maintain global optimality. This property is highly desirable for large-scale systems.


==> old/Intro_v1.tex <==
\IEEEPARstart{L}{arge-scale} networked systems permeate both modern life and academic research, with familiar examples including the Internet, smart grid, wireless sensor networks, and biological networks in science and medicine. Those systems pose fundamental challenge for controller design: simple local controllers generated by heuristics cannot guarantee global performance (or at times even stability), whereas a traditional centralized controller is neither scalable to compute, nor physically implementable. Specifically, the synthesis of the optimal centralized controller requires solving a large-scale optimization problem with the knowledge of \emph{global} plant model. In addition, the information in the network is assumed to be collected \emph{instantaneously}. The scale of the problem and the practical communication delay degrade the performance of centralized scheme substantially and make it unappealing to large systems.
 
In order to incorporate realistic communication constraints amongst sensors, actuators, and controllers into the control design process, the field of distributed (decentralized) optimal control has emerged. These communication constraints manifest themselves as subspace constraints in the optimal control problem, restricting the controller to respect specific delay and sparsity patterns. Specifically, a distributed optimal control problem is usually formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} && || f(P,K) || \nonumber\\
\text{subject to }  && K \text{ stabilizes } P \nonumber\\
&& K \in \mathcal{S}  \label{eq:intro}
\end{eqnarray}
where $P$ is the plant, $K$ the controller, $f(P,K)$ the closed-loop mapping, and $\mathcal{S}$ the subspace constraint that $K$ needs to satisfy.

The tractability of \eqref{eq:intro} depends on $\mathcal{S}$ and $P$. For example, the problem is known to be NP-hard in the worst case for a completely decentralized information structure (diagonal $\mathcal{S}$)\cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. In the seminal works \cite{2006_Rotkowitz_QI_TAC, 2014_Lessard_convexity}, the authors show that \eqref{eq:intro} admits a convex formulation if and only if $\mathcal{S}$ is quadratically invariant (QI) with respect to the plant. With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made on the field of distributed control.

%If the information sharing constraint is quadratically invariant (QI) with respect to the plant, then the distributed optimal control problem can be formulated in a convex manner \cite{2006_Rotkowitz_QI_TAC, 2010_Rotkowitz_QI_delay} by Youla parametrization \cite{1976_Youla_parameterization}.  With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made in finding finite dimensional reformulations of the optimal control problem.

In the case of QI constraints induced by strongly connected communication graphs, computing the optimal controller has been reduced to solving a finite dimensional convex program in \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal} ($\mathcal{H}_2$ criteria) and \cite{2014_Matni_Hinf} ($\mathcal{H}_{\infty}$ criteria).
Roughly speaking, constraints imposed by communication networks that allow exchange of information between controllers faster than dynamics propagate through the plant can be handled in a convex way.  In the case of sparsity constrained controllers, specific structures have been explicitly solved: including two-player \cite{2012_Lessard_two_player, 2014_Lessard_Hinf}, triangular  \cite{2013_Scherer_Hinf, 2014_Tanaka_Triangular}, partially nested  \cite{1972_Ho_info}, and poset-causal \cite{2010_Shah_H2_poset, 2011_Shah_poset_causal} systems.  It should also be noted that similar approaches to convex distributed optimal controller synthesis have been applied to spatially invariant systems satisfying a funnel causality property \cite{2002_Bamieh_spatially_invariant, 2005_Bamieh_spatially_invariant}.

As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}.  Although the computed controllers respect the information sharing constraints of the problem, in all of the above, the resulting optimal controller is as difficult to compute as its centralized counterpart, and even more demanding to implement.
In fact, for a plant with a strongly connected topology, even as simple as a chain, the QI condition implies that local measurements need to be shared among \emph{all local controllers} in the network (which can be inferred from \cite{2010_Rotkowitz_QI_delay} and \cite{2009_Swigart_graph_QI}).  This then implies that finding an optimal sparse controller $K$ (which is defined as the transfer function from measurement to control action) for a strongly connected plant cannot be formulated in a convex manner.

Based on this discussion, we argue that the closed loop behavior achieved by these distributed optimal controllers should be viewed as fundamental limits on performance, that we should strive to attain via more \emph{scalable} and \emph{realistically implementable} control schemes.

The idea of designing localized (sparse) controllers to improve scalability and ease of implementation is not a new one.  For example, regularization or approximation have been used in hopes of finding a sparse controller, such as sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting}, spatial truncation \cite{2009_Motee_spatial_truncation}, or on a spatial decaying system \cite{2014_Motee_spatially_decaying}.

The key observation in our work that distinguishes us from existing results in the literature is that a localized (and thus sparse and scalable) controller implementation does not necessarily imply that $K$ (which we recall is the transfer function from measurements to control actions) needs to be sparse. Indeed, most results in the field of distributed control is built based on the formulation \eqref{eq:intro}, while we argue that \eqref{eq:intro} is not the only way, and even not a good way, to formulate an optimal control problem with communication constraint. In fact, by using implicit implementations of the controller (which allow the communication of both \emph{ measurements and control actions}), we show how localized closed loop responses and implementations can indeed be compatible with each other, and computed in a convex way.

Specifically, in \cite{2014_Wang_ACC}, we introduced the notion of a state feedback localizable system, that is to say systems for which a localized closed loop response exists. 
We derived a direct relation between the closed loop response of the system and the controller implementation achieving the desired closed loop.  Building on these results, in \cite{2014_Wang_CDC} we showed how the computation and implementation of a linear quadratic regulator (LQR) optimal localizing state feedback law can be done in a completely localized (and hence scalable) manner. The result is further extended to output feedback in \cite{2014_Wang_Allerton}. Surprisingly, simulations in \cite{2014_Wang_CDC, 2014_Wang_Allerton} showed that the proposed localized controller achieved performance similar to that of a centralized optimal one, while being far superior in terms of the sparsity of implementation and the closed loop response.  We emphasize once again that this latter property is key for the scalability of this scheme.

This paper summarizes our previous results on localized distributed control into a generalized framework. Specifically, we extend the result in \cite{2014_Wang_Allerton} to unstable system by redefining the notion of internal stability. The notion of localizability is also restated as a generalization of controllability and observability. Based on that, the localized distributed optimal control problem is formulated as a finite dimensional affinely constrained convex program, which can be solved by a localized way by standard distributed optimization technique. The controller can also be implemented in a localized way, and the robustness of the implementation is analyzed. Simulation shows that our localized (scalable) controller implementation can achieve similar transient response to a centralized optimal one.

The rest of this paper is organized as follows. Section \ref{sec:prelim} introduces the system model, spatio-temporal constraints, and some preliminaries on graph theory and distributed control. Section \ref{sec:state} starts with an illustrative example, and formally defines the notion of state feedback localizability later on. The localized LQR (LLQR) problem is formulated in Section \ref{sec:LLQR}. In particular, we show that LLQR problem can be solved by a completely localized and distributed way, and the resulting controller can also be implemented in a localized way. Section \ref{sec:output} extends the result into output feedback, and the localized distributed optimal control problem is formulated and solved in \ref{sec:localized}. Once again, both the controller synthesis and implementation are localized. Simulation results are shown in Section \ref{sec:simu} to illustrate the effectiveness of our method. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%\subsection{Prior Work}
%\subsection{Contribution}
%\subsection{Outline}
%The rest of this paper is organized as follows.

%\textbf{Mathematical Notations: } $\mathcal{RH}_{\infty}$ denotes the set of all real-rational stable proper transfer functions.

==> old/Intro_v2.tex <==
\IEEEPARstart{L}{arge-scale} networked systems permeate both modern life and academic research, with familiar examples including the Internet, smart grid, wireless sensor networks, and biological networks in science and medicine. The scale of these systems pose fundamental challenge for controller design: simple local controllers generated by heuristics cannot guarantee global performance (or at times even stability), whereas a traditional centralized controller is neither scalable to compute, nor physically implementable. Specifically, the synthesis of the optimal centralized controller requires solving a large-scale optimization problem with the knowledge of \emph{global} plant model. In addition, the information in the network is assumed to be collected \emph{instantaneously}. The scale of the problem and the practical communication delay degrade the performance of centralized scheme substantially and make it unappealing to large systems.
 
In order to incorporate realistic communication constraints amongst sensors, actuators, and controllers into the control design process, the field of distributed (decentralized) optimal control has emerged. These communication constraints manifest themselves as subspace constraints in the optimal control problem, restricting the controller to respect specific delay and sparsity patterns. Specifically, a distributed optimal control problem is usually formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} && || f(P,K) || \nonumber\\
\text{subject to }  && K \text{ stabilizes } P \nonumber\\
&& K \in \mathcal{S}  \label{eq:intro}
\end{eqnarray}
where $P$ is the plant, $K$ the controller, $f(P,K)$ the closed-loop mapping, and $\mathcal{S}$ the subspace constraint that $K$ needs to satisfy.

The tractability of \eqref{eq:intro} depends on the relations between $\mathcal{S}$ and $P$. For instance, the problem is known to be NP-hard in the worst case for a completely decentralized information structure (diagonal $\mathcal{S}$)\cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. In the seminal works \cite{2006_Rotkowitz_QI_TAC, 2014_Lessard_convexity}, the authors show that \eqref{eq:intro} admits a convex formulation if and only if $\mathcal{S}$ is quadratically invariant (QI) with respect to the plant. 
%Roughly speaking, constraints imposed by communication networks that allow exchange of information between controllers faster than dynamics propagate through the plant can be handled in a convex way.
Roughly speaking, QI condition holds when the communication speed is faster than the speed of disturbance propagation in the physical system \cite{2010_Rotkowitz_QI_delay}. Much progress has been made \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal, 2014_Matni_Hinf, 2012_Lessard_two_player, 2014_Lessard_Hinf, 2013_Scherer_Hinf, 2014_Tanaka_Triangular, 2010_Shah_H2_poset, 2011_Shah_poset_causal} on extending the result of QI for specific structure or finite dimensional reformulation of the optimal control problem in recent years.

%With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made on the field of distributed control.
%If the information sharing constraint is quadratically invariant (QI) with respect to the plant, then the distributed optimal control problem can be formulated in a convex manner \cite{2006_Rotkowitz_QI_TAC, 2010_Rotkowitz_QI_delay} by Youla parametrization \cite{1976_Youla_parameterization}.  With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made in finding finite dimensional reformulations of the optimal control problem.

%Although the communication delay constraint is well-handled in the field of distributed control, the synthesis and the implementation of those controllers are still not scalable.
%As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}.  Although the computed controllers respect the information sharing constraints of the problem, 
As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}. 
In all of the above, the resulting optimal controller is as difficult to compute as its centralized counterpart, and even more demanding to implement.
In fact, for a plant with a strongly connected topology, even as simple as a chain, the QI condition implies that local measurements need to be shared among \emph{all local controllers} in the network (which can be inferred from \cite{2010_Rotkowitz_QI_delay} and \cite{2009_Swigart_graph_QI}). This then implies that finding an optimal sparse controller $K$ in \eqref{eq:intro} (which is defined as the transfer function from measurement to control action) for a strongly connected plant cannot be formulated in a convex manner. In addition, the synthesis of distributed optimal controller also requires solving large-scale optimization problem with the knowledge of global plant model beforehand, which is highly unrealistic.

Based on this discussion, we argue that the closed loop behavior achieved by these distributed optimal controllers should be viewed as fundamental limits on performance, that we should strive to attain via more \emph{scalable} and \emph{realistically implementable} control schemes.

Our key observation that breaks the fundamental limits on convexity is that a localized (and thus sparse and scalable) controller implementation does not necessarily imply that $K$ (which we recall is the transfer function from measurements to control actions) needs to be sparse. In fact, by using implicit implementations of the controller (which allow the communication of both \emph{measurements and control action}, or \emph{estimated disturbance and reference trajectory}), we show that the distributed controller can be implemented in a localized way even when $K$ is not sparse. With this innovation on controller implementation, we create a whole new control theory, which we call \emph{localized distributed control}, that is extremely favorable for large-scale systems.

%Specifically, we argue that \eqref{eq:intro} is not the only way, and even not a good way, to formulate the optimal control problem with communication constraint.

Specifically, in \cite{2014_Wang_ACC}, we introduced the notion of a state feedback localizable system. The basic concept is the following observation: when the communication speed is faster than the speed of disturbance propagation, it is possible to localize the effect of each local disturbance. We define this as the notion of state feedback localizability of a system, which is a natural extension of controllability in a space-time region. We show in \cite{2014_Wang_ACC, 2014_Wang_CDC} that a state feedback localizable system achieves the following properties.

\textbf{Closed Loop Response}

\begin{enumerate}
\item The effect of each local disturbance is limited in a localized region in finite time.
\item The transient performance is close to the idealized (undelayed) global optimal one. Traditional centralized control scheme can be considered as a degenerated case of localized distributed control. 
\end{enumerate}

\textbf{Controller Implementation}

\begin{enumerate}
\item The controller achieving the desired closed loop response can be implemented in a \emph{localized} way by FIR filters. In other words, each local controller only needs to communicate and collaborate with some of its neighbors to generate its control action.
\item The controller can be implemented with communication delay as long as the communication speed is faster than the speed of disturbance propagation.
\end{enumerate}

\textbf{Controller Synthesis}

\begin{enumerate}
\item The global optimal controller (subject to localized constraints) can be synthesized in a localized way by solving small scale affinely constrained convex optimization problems with local update procedure.
\item Each local optimization problem only depends on the plant model locally. This is to say that when the plant model changes locally, only some local optimization problems need to be resolved to maintain global optimality. This allows incremental design when the physical system expands.
\end{enumerate}

The implication of these properties is that we have a systematic way to practically synthesize and implement the controller for a large-scale system with nearly optimal transient performance. In addition, disturbance propagation can be limited in a localized region without using a centralized coordinator. Both features significantly enhance robustness and scalability for a large-scale system. Note that many of these properties can never be achieved with the formulation in \eqref{eq:intro}.

\subsection{Related Works}
In the case of QI constraints induced by strongly connected communication graphs, computing the optimal controller has been reduced to solving a finite dimensional convex program in \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal} ($\mathcal{H}_2$ criteria) and \cite{2014_Matni_Hinf} ($\mathcal{H}_{\infty}$ criteria).
Roughly speaking, constraints imposed by communication networks that allow exchange of information between controllers faster than dynamics propagate through the plant can be handled in a convex way.  In the case of sparsity constrained controllers, specific structures have been explicitly solved: including two-player \cite{2012_Lessard_two_player, 2014_Lessard_Hinf}, triangular \cite{2013_Scherer_Hinf, 2014_Tanaka_Triangular}, partially nested  \cite{1972_Ho_info}, and poset-causal \cite{2010_Shah_H2_poset, 2011_Shah_poset_causal} systems. 

It should also be noted that similar approaches to convex distributed optimal controller synthesis have been applied to spatially invariant systems satisfying a funnel causality property \cite{2002_Bamieh_spatially_invariant, 2005_Bamieh_spatially_invariant}.

The idea of designing localized (sparse) controllers to improve scalability and ease of implementation is not a new one.  For example, regularization or approximation have been used in hopes of finding a sparse controller, such as sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting}, spatial truncation \cite{2009_Motee_spatial_truncation}, or on a spatial decaying system \cite{2014_Motee_spatially_decaying}.

Disturbance localization

\subsection{Contribution}

We derived a direct relation between the closed loop response of the system and the controller implementation achieving the desired closed loop.  Building on these results, in \cite{2014_Wang_CDC} we showed how the computation and implementation of a linear quadratic regulator (LQR) optimal localizing state feedback law can be done in a completely localized (and hence scalable) manner. The result is further extended to output feedback in \cite{2014_Wang_Allerton}. Surprisingly, simulations in \cite{2014_Wang_CDC, 2014_Wang_Allerton} showed that the proposed localized controller achieved performance similar to that of a centralized optimal one, while being far superior in terms of the sparsity of implementation and the closed loop response.  We emphasize once again that this latter property is key for the scalability of this scheme.

This paper summarizes our previous results on localized distributed control into a generalized framework. Specifically, we extend the result in \cite{2014_Wang_Allerton} to unstable system by redefining the notion of internal stability. The notion of localizability is also restated as a generalization of controllability and observability. Based on that, the localized distributed optimal control problem is formulated as a finite dimensional affinely constrained convex program, which can be solved by a localized way by standard distributed optimization technique. The controller can also be implemented in a localized way, and the robustness of the implementation is analyzed. Simulation shows that our localized (scalable) controller implementation can achieve similar transient response to a centralized optimal one.

\subsection{Outline}
The rest of this paper is organized as follows. Section \ref{sec:prelim} introduces the system model, spatio-temporal constraints, and some preliminaries on graph theory and distributed control. Section \ref{sec:state} starts with an illustrative example, and formally defines the notion of state feedback localizability later on. The localized LQR (LLQR) problem is formulated in Section \ref{sec:LLQR}. In particular, we show that LLQR problem can be solved by a completely localized and distributed way, and the resulting controller can also be implemented in a localized way. Section \ref{sec:output} extends the result into output feedback, and the localized distributed optimal control problem is formulated and solved in \ref{sec:localized}. Once again, both the controller synthesis and implementation are localized. Simulation results are shown in Section \ref{sec:simu} to illustrate the effectiveness of our method. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%The rest of this paper is organized as follows.

%\textbf{Mathematical Notations: } $\mathcal{RH}_{\infty}$ denotes the set of all real-rational stable proper transfer functions. $z$ is the variable of the z-transform. 
%Throughout this paper, we use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system.


==> old/Intro_v3.tex <==
\IEEEPARstart{L}{arge-scale} networked systems permeate both modern life and academic research, with familiar examples including the Internet, smart grid, wireless sensor networks, and biological networks in science and medicine. The scale of these systems pose fundamental challenge for controller design: simple local controllers generated by heuristics cannot guarantee global performance (or at times even stability), whereas a traditional centralized controller is neither scalable to compute, nor physically implementable. Specifically, the synthesis of the optimal centralized controller requires solving a large-scale optimization problem with the knowledge of \emph{global} plant model. In addition, the information in the network is assumed to be collected \emph{instantaneously}. The scale of the problem and the practical communication delay degrade the performance of centralized scheme substantially and make it unappealing to large systems.
 
In order to incorporate realistic communication constraints amongst sensors, actuators, and controllers into the control design process, the field of distributed (decentralized) optimal control has emerged. These communication constraints manifest themselves as subspace constraints in the optimal control problem, restricting the controller to respect specific delay and sparsity patterns. Specifically, a distributed optimal control problem is usually formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} && || f(P,K) || \nonumber\\
\text{subject to }  && K \text{ stabilizes } P \nonumber\\
&& K \in \mathcal{S}  \label{eq:intro}
\end{eqnarray}
where $P$ is the plant, $K$ the controller, $f(P,K)$ the closed-loop mapping, and $\mathcal{S}$ the subspace constraint that $K$ needs to satisfy.

The tractability of \eqref{eq:intro} depends on the relations between $\mathcal{S}$ and $P$. For instance, the problem is known to be NP-hard in the worst case for a completely decentralized information structure (diagonal $\mathcal{S}$)\cite{1968_Witsenhausen_counterexample, 1984_Tsitsiklis_NP_hard}. In the seminal works \cite{2006_Rotkowitz_QI_TAC} and recently in \cite{2014_Lessard_convexity}, the authors show that \eqref{eq:intro} admits a convex formulation if and only if $\mathcal{S}$ is quadratically invariant (QI) with respect to the plant. 
%Roughly speaking, constraints imposed by communication networks that allow exchange of information between controllers faster than dynamics propagate through the plant can be handled in a convex way.
Roughly speaking, QI condition holds when the communication speed is faster than the speed of disturbance propagation in the physical system \cite{2010_Rotkowitz_QI_delay}. Much progress has been made \cite{2013_Lamperski_H2, 2014_Lamperski_H2_journal, 2014_Lamperski_state, 2014_Matni_Hinf, 2012_Lessard_two_player, 2014_Lessard_Hinf, 2013_Scherer_Hinf, 2014_Tanaka_Triangular, 2010_Shah_H2_poset, 2011_Shah_poset_causal} on extending the result of QI for specific structure or finite dimensional reformulation of the optimal control problem in recent years.

%With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made on the field of distributed control.
%If the information sharing constraint is quadratically invariant (QI) with respect to the plant, then the distributed optimal control problem can be formulated in a convex manner \cite{2006_Rotkowitz_QI_TAC, 2010_Rotkowitz_QI_delay} by Youla parametrization \cite{1976_Youla_parameterization}.  With the identification of quadratic invariance as an appropriate means of convexifying the distributed optimal control problem, much progress has been made in finding finite dimensional reformulations of the optimal control problem.

%Although the communication delay constraint is well-handled in the field of distributed control, the synthesis and the implementation of those controllers are still not scalable.
%As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}.  Although the computed controllers respect the information sharing constraints of the problem, 
As promising and impressive as all of the results have been, they ignore one key aspect of applying distributed control to large scale systems: \emph{scalability}. 
In all of the above, the resulting optimal controller is as difficult to compute as its centralized counterpart, and even more demanding to implement.
In fact, for a plant with a strongly connected topology, even as simple as a chain, the QI condition implies that local measurements need to be shared among \emph{all local controllers} in the network (which can be inferred from \cite{2010_Rotkowitz_QI_delay} and \cite{2009_Swigart_graph_QI}). This then implies that finding an optimal sparse controller $K$ in \eqref{eq:intro} (which is defined as the transfer function from measurement to control action) for a strongly connected plant cannot be formulated in a convex manner. Although the nonconvex problem is possible to be solved approximately \cite{2014_Fazelnia_ODC, 2011_Rotkowitz_subspace}, the synthesis of distributed optimal controller still requires solving large-scale optimization problem with the knowledge of global plant model beforehand, which is highly unrealistic.

Based on this discussion, we argue that the closed loop behavior achieved by these distributed optimal controllers should be viewed as fundamental limits on performance, that we should strive to attain via more \emph{scalable} and \emph{realistically implementable} control schemes.

Our key observation that breaks the fundamental limits on convexity is that a localized (and thus sparse and scalable) controller implementation does not necessarily imply that $K$ (which we recall is the transfer function from measurements to control actions) needs to be sparse. In fact, by using implicit implementations of the controller (which allow the communication of both \emph{measurements and control action}, or \emph{estimated disturbance and reference trajectory}), we show that the distributed controller can be implemented in a localized way even when $K$ is not sparse. With this innovation on controller implementation, we create a whole new control theory, which we call \emph{localized distributed control}, that is extremely favorable for large-scale systems.

%Specifically, we argue that \eqref{eq:intro} is not the only way, and even not a good way, to formulate the optimal control problem with communication constraint.

Specifically, in \cite{2014_Wang_ACC}, we introduced the notion of a state feedback localizable system. The basic concept is the following observation: when the communication speed is faster than the speed of disturbance propagation, it is possible to localize the effect of each local disturbance. We define this as the notion of state feedback localizability of a system, which is a natural extension of controllability in a space-time region. We show in \cite{2014_Wang_ACC, 2014_Wang_CDC} that a state feedback localizable system achieves the following properties.

\textbf{Closed Loop Response}
\begin{enumerate}
\item The effect of each local disturbance is limited in a localized region in finite time.
\item The transient performance can be close to the idealized centralized global optimal one by selecting the localized region appropriately. 
\end{enumerate}

\textbf{Controller Implementation}
\begin{enumerate}
\item The controller achieving the desired closed loop response can be implemented in a \emph{localized} way by FIR filters. Each local controller only needs to communicate with some of its neighbors to generate its control action.
\item The controller can be implemented with communication delay as long as the communication speed is faster than the speed of disturbance propagation.
\end{enumerate}

\textbf{Controller Synthesis}
\begin{enumerate}
\item For linear quadratic regulator (LQR) cost, the global optimal controller (subject to localized constraints) can be synthesized in a localized way by solving localized LQR (LLQR) problems following a local update procedure.
\item Each LLQR sub-problem only depends on the plant model locally. When the plant model changes locally, only some local optimization problems need to be resolved to maintain global optimality. This allows incremental design when the physical system expands.
\end{enumerate}

The implication of these properties is that we have a systematic way to practically synthesize and implement the controller for a large-scale system with nearly optimal transient performance. In addition, disturbance propagation can be limited in a localized region without using a centralized coordinator. Both features significantly enhance robustness and scalability for a large-scale system. Note that many of these properties cannot be achieved with the formulation in \eqref{eq:intro}.

\subsection{Related Works}
Besides the works in distributed optimal control, the idea of localized closed loop response, localized implementation, and localized synthesis have been addressed separately in different line of research.

The idea of designing localized (sparse) controllers to improve scalability and ease of implementation has been applied on spatially invariant systems \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant}, and the inverse optimality condition is analyzed in \cite{2005_Jovanovic_localized}.
%In fact, the distributed optimal controller for a spatially invariant system is shown to have an inherent degree of localization, which makes the 
%The spatial localization property of the distributed optimal controller have been analyzed
%For instance, the localized optimal controller has been applied on spatially invariant systems in \cite{2002_Bamieh_spatially_invariant, 2002_Castro_LSI, 2005_Bamieh_spatially_invariant}%For instance, it has been shown that the optimal controller for a spatially invariant system have an inherent degree of localization \cite{2002_Bamieh_spatially_invariant} and thus 
%It should also be noted that similar approaches to convex distributed optimal controller synthesis have been applied to spatially invariant systems satisfying a funnel causality property \cite{2002_Bamieh_spatially_invariant, 2005_Bamieh_spatially_invariant}.
The method is generalized into spatial decaying systems in \cite{2008_Motee_distributed, 2014_Motee_spatially_decaying}. Regularization or approximation have also been used in hopes of finding a sparse controller. Representative works include sparsity-promoting control \cite{2011_Fardad_sparsity_promoting, 2013_Lin_sparsity_promoting} and spatial truncation method \cite{2009_Motee_spatial_truncation}.

Although the above-mentioned methods provide a scalable way to implement the distributed controller, the synthesis procedure is still centralized, which requires global plant model beforehand. The methods described in 
\cite{2004_Dullerud, 2008_Borrelli_LQR, 2013_Farokhi_model} can provide scalable way to synthesize distributed controller with limited model information, but the method can be quite conservative. Part of the reason is that the controller synthesis and implementation of those methods are in the ``$K$" domain.

\subsection{Contribution}
%We derived a direct relation between the closed loop response of the system and the controller implementation achieving the desired closed loop.  Building on these results, in \cite{2014_Wang_CDC} we showed how the computation and implementation of a linear quadratic regulator (LQR) optimal localizing state feedback law can be done in a completely localized (and hence scalable) manner. The result is further extended to output feedback in \cite{2014_Wang_Allerton}. Surprisingly, simulations in \cite{2014_Wang_CDC, 2014_Wang_Allerton} showed that the proposed localized controller achieved performance similar to that of a centralized optimal one, while being far superior in terms of the sparsity of implementation and the closed loop response.  We emphasize once again that this latter property is key for the scalability of this scheme.
This paper provides a localized and thus scalable way to synthesize and implement the state feedback distributed controller for large-scale systems with arbitrary interconnected topology. 
It is an extension of our previous result in \cite{2014_Wang_ACC, 2014_Wang_CDC} in the following sense.
\begin{enumerate}
\item The robustness of the localized controller implementation is rigorously analyzed by an extended notion of internal stability.
\item A localized algorithm that computes the lower bound of global optimality is proposed. By comparing the relative cost of the feasible solution (upper bound) and the lower bound, one can dynamically choose the size of the localized region for each local disturbance.
\item A simple condition on the spatial localizability is given. This provides a guideline for actuator placement that ensures spatial localizability. 
\end{enumerate}
 
With these three extensions, we test our algorithm on a large-scale randomized example. With the scalable lower bound algorithm, we show that our controller achieve nearly global optimality without actually computing the cost of an idealized centralized controller. Finally, some of the notation and derivation in \cite{2014_Wang_ACC, 2014_Wang_CDC} are refined in this paper to enhance generality and readability.

%This paper summarizes our previous results on localized distributed control into a generalized framework. Specifically, we extend the result in \cite{2014_Wang_Allerton} to unstable system by redefining the notion of internal stability. The notion of localizability is also restated as a generalization of controllability and observability. Based on that, the localized distributed optimal control problem is formulated as a finite dimensional affinely constrained convex program, which can be solved by a localized way by standard distributed optimization technique. The controller can also be implemented in a localized way, and the robustness of the implementation is analyzed. Simulation shows that our localized (scalable) controller implementation can achieve similar transient response to a centralized optimal one.

\subsection{Outline}
The rest of this paper is organized as follows. Section \ref{sec:problem} introduces some preliminaries and formulate the LLQR problem. The spatio-temporal constraints in LLQR is then formally defined in Section \ref{sec:st_cons}. In Section \ref{sec:state}, we define the notion of state feedback localizability in terms of the feasibility of a set of linear equations, and show that the feasibility of the equations can be verified in a localized and parallel way. We then show that the LLQR problem can be decomposed in a similar way in Section \ref{sec:LLQR}. The localized implementation and synthesis procedure for the LLQR controller are provided in Section \ref{sec:imp}. Some extensions are discussed in Section \ref{sec:ext}, and the simulation results are shown in Section \ref{sec:simu}. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%The rest of this paper is organized as follows. Section \ref{sec:prelim} introduces the system model, spatio-temporal constraints, and some preliminaries on graph theory and distributed control. Section \ref{sec:state} starts with an illustrative example, and formally defines the notion of state feedback localizability later on. The localized LQR (LLQR) problem is formulated in Section \ref{sec:LLQR}. In particular, we show that LLQR problem can be solved by a completely localized and distributed way, and the resulting controller can also be implemented in a localized way. Section \ref{sec:output} extends the result into output feedback, and the localized distributed optimal control problem is formulated and solved in \ref{sec:localized}. Once again, both the controller synthesis and implementation are localized. Simulation results are shown in Section \ref{sec:simu} to illustrate the effectiveness of our method. Lastly, Section \ref{sec:conclusion} ends with conclusions and offers some future research directions.

%The rest of this paper is organized as follows.

%\textbf{Mathematical Notations: } $\mathcal{RH}_{\infty}$ denotes the set of all real-rational stable proper transfer functions. $z$ is the variable of the z-transform. 
%Throughout this paper, we use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system.


==> old/Output_local_v1.tex <==
- State estimation is dual to state feedback
- State feedback/estimation localizability imply output feedback localizability
- Not optimal, but this is a rule to meet structural localizability

==> old/Output_v1.tex <==

\subsection{Localized Synthesis through ADMM}
- Separable cost function
- Review on ADMM

\subsection{Localized Implementation}
- Three ways to implement controller
- Internal stability
- Robustness analysis


==> old/Prelim_LLQG.tex <==
\subsection{Interconnected System Model}
Consider a network of linear systems connected through a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\mathcal{V} = \{1, \dots, n\}$ is the set of sub-systems, and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ encodes the interaction between these sub-systems. Each sub-system $i$ is associated with a state vector $x_i$, control action $u_i$, and measurement $y_i$. We assume that the dynamics of each sub-system $i$ is given in the form of
\begin{eqnarray}
x_i[k+1] &=& A_{ii} x_i[k] + B_{ii} u_i[k] + \sum_{j \in \mathcal{N}_i} A_{ij}x_j[k] + \delta{x_i}[k]\nonumber\\
y_i[k] &=& C_{ii} x_i[k] + \delta{y_i}[k], \label{eq:interconnected}
\end{eqnarray}
where $A_{ii}, A_{ij}, B_{ii}, C_{ii}$ are constant matrices with compatible dimensions, $\delta{x_i}$ and $\delta{y_i}$ the perturbation on state and measurement, respectively, and $\mathcal{N}_i$ the (upstream) neighboring set of $i$ defined by $\mathcal{N}_i = \{j | (j,i) \in \mathcal{E}\}$. The following is a simple example in the form of \eqref{eq:interconnected}, which is used to illustrate several ideas throughout this paper.
\begin{example}
Consider a network system with interconnected topology given by Fig. \ref{fig:Chart105}. Each sub-system $x_i$ is assumed to have two interacting scalar states $x_{i,1}, x_{i,2}$, a sensor on $x_{i,1}$, and an actuator on $x_{i,2}$. The interaction between two neighboring sub-systems is illustrated in Fig. \ref{fig:inter}, where $x_{i,1}$ can affect $x_{j,2}$ if $i$ and $j$ are neighbor. This model is inspired from the second-order dynamics in power network or mechanical system. Specifically, consider a second-order equation
\begin{equation}
m_i \ddot{\theta_i} + d_i \dot{\theta_i} = -\sum_{j \in \mathcal{N}_i} k_{ij} (\theta_i - \theta_j) + w_i + u_i \nonumber
\end{equation}
for some scalar $\theta_i$.
If we define the state vector by $x_i = [\theta_i \quad \dot{\theta_i}]^\top$, take the measurement on $\theta_i$, and use $e^{A \Delta t} \approx I + A \Delta t$ to discretize the plant, we get a discretized plant model with interaction graph described by Fig. \ref{fig:inter}.
\end{example}
\begin{figure}[t!]
      \centering
      \subfigure[Interconnected topology]{%
      \includegraphics[width=0.35\textwidth]{./figure/Topology.pdf}
      \label{fig:Chart105}}      
      \subfigure[Interaction between neighboring sub-systems]{%
      \includegraphics[width=0.25\textwidth]{./figure/Interaction.pdf}
      \label{fig:inter}}      
      \caption{Illustrative Example}
\end{figure}

\subsection{Challenges to Traditional Method}
The interconnected systems pose great challenges to controller design when (i) the effect of sub-system interaction $A_{ij}$ cannot be neglected, and (ii) the number of sub-systems $n$ grows large. The distributed method and the completely local method can handle one of the situations above, but not both.

By completely local method, for an extreme case, the controller is implemented \emph{and} designed in a purely local way. Specifically, each local control rule is given by $u_i = K_i y_i$, where $K_i$ is designed with the local plant model $(A_{ii}, B_{ii}, C_{ii})$ \emph{only}. Clearly, such control scheme is scalable to arbitrary large $n$, but does not guarantee global stability if the effect of $A_{ij}$ is not negligible.

To show that the distributed optimal control method is not scalable to large $n$, we construct the global plant model as
\begin{eqnarray}
x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber \\
y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics}
\end{eqnarray}
where $x$, $u$, $y$, $\delta_x$, and $\delta_y$ are stacked vectors of local state, control, measurement, process disturbance, and sensor disturbance, respectively. The global plant model $(A,B_2,C_2)$ can be derived by combining the matrices in \eqref{eq:interconnected} in an appropriate way. Equation \eqref{eq:dynamics} can be written in state space form as
\begin{equation}
P = \left[ \begin{array}{c|cc} A & B_1 & B_2 \\ \hline C_1 & \mathbf{0} & D_{12} \\ C_2 & D_{21} & \mathbf{0} \end{array} \right] = \begin{bmatrix} P_{11} & P_{12} \\ P_{21} & P_{22} \end{bmatrix} \nonumber
\end{equation}
for some matrices $C_1, D_{12}, B_1, D_{21}$ representing the cost function and noise dynamics, and $P_{ij} = C_i(zI-A)^{-1}B_j + D_{ij}$. Assume a dynamic output feedback control law $u = K y$. The distributed optimal control problem is commonly formulated as
%of minimizing the norm\footnote{Typical choices for the norm include $\mathcal{H}_2$ and $\mathcal{H}_\infty$.} of the closed loop transfer function from $w$ to $\bar{z}$ is formulated as
\begin{eqnarray}
\underset{K}{\text{minimize  }} &&|| P_{11} + P_{12} K(I-P_{22}K)^{-1} P_{21}|| \nonumber\\
\text{subject to } && K \text{ stabilizes } P \nonumber\\
&& K \in \mathcal{S}_c  \label{eq:trad}
\end{eqnarray}
where $\mathcal{S}_c$ is a subspace constraint that $K$ must satisfy in order to be implementable on the communication network of the system. 

In order to have a scalable controller implementation, it is natural to impose sparsity constraints on $K$. For example, one may want the control action $u_1$ at node $1$ in Fig. \ref{fig:Chart105} to use the measurements $y_i$ from node $i = 1, \dots, 5$ only. This is equivalently saying that the delay from measurements $y_i$ for node $i = 6, \dots, 10$ to the control action $u_1$ at node $1$ is set to be infinity. This information sharing constraint is not QI, and \eqref{eq:trad} becomes non-convex. In fact, using the delay interpretation of QI in \cite{2010_Rotkowitz_QI_delay}, the sparsity constraint for a plant with strongly connected topology is not QI in general.

Although the non-convex problem corresponding to a sparse $\mathcal{S}_c$ may be solved via convex relaxation \cite{2014_Fazelnia_ODC} or other techniques, \eqref{eq:trad} (or the modification of \eqref{eq:trad}) is still a large-scale optimization problem depending on a global plant model, which cannot be solved in a scalable way.


%\subsection{Localized Distributed Control}
%In our previous works, we point out that the distributed controller does not need to be implemented directly by $K$, so $K$ need not be sparse. Instead, we introduce four closed loop transfer matrices $(R,M,N,L)$ to link the relation between closed loop response, controller implementation, and controller synthesis. For a system described by \eqref{eq:dynamics}, the closed loop transfer matrices $(R,M,N,L)$ are defined by
%\begin{equation}
%\begin{bmatrix} x \\ u \end{bmatrix} = \begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix}\delta_x \\ \delta_y \end{bmatrix}. \label{eq:desired}
%\end{equation}
%The \emph{localized} distributed optimal control problem is then formulated by
%\begin{subequations}
%\begin{align}
%\underset{\{R,M,N,L\}}{\text{minimize}} & \quad || \begin{bmatrix} C_1 & D_{12} \end{bmatrix}\begin{bmatrix} R & N \\ M & L \end{bmatrix} \begin{bmatrix} B_1 \\ D_{21} \end{bmatrix}|| \label{eq:local_obj}\\
%\text{subject to }  & \begin{bmatrix} zI - A & -B_2 \end{bmatrix}
%\begin{bmatrix} R & N \\ M & L \end{bmatrix} = 
%\begin{bmatrix} I & 0 \end{bmatrix} \label{eq:local1} \\
%& \begin{bmatrix} R & N \\ M & L \end{bmatrix}
%\begin{bmatrix} zI - A \\ -C_2 \end{bmatrix} = 
%\begin{bmatrix} I \\ 0 \end{bmatrix} \label{eq:local2} \\
%& \begin{bmatrix} zR & zN \\ zM & L \end{bmatrix} \in \mathcal{S} \cap \mathcal{RH}_{\infty} \label{eq:local_S}
%\end{align}
%\end{subequations}
%where $z$ is the variable of z-transform, $\mathcal{RH}_{\infty}$ the set of real rational stable proper transfer matrices, and $\mathcal{S}$ a spatio-temporal constraint on the closed loop transfer matrices. The following theorem is proposed in \cite{2014_Wang_Allerton} and extended in \cite{2015_Wang_LDC}.
%\begin{theorem}
%If \eqref{eq:local1} - \eqref{eq:local_S} is feasible, then the desired closed loop response \eqref{eq:desired} can be achieved by the controller implementation
%\begin{eqnarray}
%z \beta &=& \tilde{R}^+ \beta + \tilde{N} y \nonumber\\
%u &=& \tilde{M} \beta + L y \label{eq:implementation}
%\end{eqnarray}
%where $\tilde{R}^+ = z(I - zR)$, $\tilde{N} = -zN$, $\tilde{M} = zM$, $L$ are stable proper transfer matrices, $\beta$ the controller state. The implementation \eqref{eq:implementation} is internally stabilizing. \label{thm:1}
%\end{theorem}
%
%The implementation \eqref{eq:implementation} is similar to the state space realization of the controller, but we generalize the state space matrices into stable proper transfer matrices $(\tilde{R}^+, \tilde{N}, \tilde{M}, L)$. If \eqref{eq:local1} - \eqref{eq:local_S} is feasible for a sparse $\mathcal{S}$, Theorem \ref{thm:1} suggests that the controller achieving the desired closed loop response can also be implemented in a localized way by \eqref{eq:implementation}. 
%\begin{example}
%For Fig. \ref{fig:Chart105}, if there exists a control law such that the state $x_1$ and control action $u_1$ at node $1$ is affected only by disturbances $\delta{x_i}$ and $\delta{y_i}$ from node $i = 1, \dots, 5$ in closed loop. Then, using Theorem \ref{thm:1}, the control action $u_1$ at node $1$ can be computed by collecting measurements \emph{and} controller states $(y_i, \beta_i)$ from node $i = 1, \dots, 5$ to achieve the desired closed loop response.
%\end{example}
%
%%With this theorem, finding a locally implementable controller reduces to the problem of finding a localized closed loop response in \eqref{eq:local1} - \eqref{eq:local_S}, which is \emph{always} convex. 
%We emphasize the fact that both the synthesis and implementation of \eqref{eq:local_obj} - \eqref{eq:local_S} are done in the \emph{closed loop transfer matrices domain}, which avoids the non-convexity in \eqref{eq:trad}. 
%% and \eqref{eq:local_obj} - \eqref{eq:local_S} is \emph{always} convex. 
%This method can also be considered as a generalization of disturbance localization \cite{1982_Kobayashi} and the decoupled control law \cite{2014_Bullo}.
%% are developed in the $K$ domain similar to \eqref{eq:trad}. 
%Specifically, a centralized controller is required for the method in \cite{1982_Kobayashi}, and the method in \cite{2014_Bullo} only works when the interconnected systems have a non-overlapping partition (block diagonal sparsity constraint on $R$). 
%%It should also be noted that the traditional disturbance localization \cite{1982_Kobayashi} and the decoupled control law \cite{2014_Bullo} are developed in the $K$ domain similar to \eqref{eq:trad}, so these methods only work when the interconnected systems have a non-overlapping partition (block diagonal sparsity constraint on $R$). 
%%It should be noted that this method is a substantial generalization of the disturbance localization problem \cite{1970_Wonham, 1975_Hamano, 1982_Kobayashi} and the decoupled control law \cite{2014_Bullo}. Those methods only work when the interconnected systems have a non-overlapping partition (a block diagonal sparsity constraint in \eqref{eq:local_S}). 
%On the other hand, Theorem \ref{thm:1} can handle \emph{overlapping} localized regions, which arise when there are communication delays between local controllers. 
%
%However, the optimization problem \eqref{eq:local_obj} - \eqref{eq:local_S} does not decompose naturally due to the coupling between constraints \eqref{eq:local1} and \eqref{eq:local2}. The goal of this paper is to provide a scalable algorithm to \emph{solve} \eqref{eq:local_obj} - \eqref{eq:local_S} in a localized way with \eqref{eq:local_obj} being the LQG cost. In this paper, the spatio-temporal constraint $\mathcal{S}$ in \eqref{eq:local_S} is given before synthesis. Some simple rules to \emph{design} $\mathcal{S}$ and the actuator locations ($B_2$) are proposed in \cite{2015_Wang_Reg}.




==> old/State_local_v1.tex <==
In this section, we define the notion of state feedback localizability. We then give a feasibility test to characterize state feedback localizable systems, and show that this test can be performed in a localized and distributed way.

%\subsection{Localized FIR Constraints}
%We now define localized FIR constraints and state feedback localizability for a system $(A,B)$. Throughout this paper, we use $\mathcal{S}_x$ to denote the constraint space for $R$ (the transfer function from $w$ to $x$) and $\mathcal{S}_u$ the constraint space for $M$ (the transfer function from $w$ to $u$).
%\begin{definition}
%The constraint space pair $(\mathcal{S}_x, \mathcal{S}_u)$ is a $(d,T)$ localized FIR constraint for system $(A,B)$ if and only if
%\begin{enumerate}
%\item $\mathcal{S}_x$ and $\mathcal{S}_u$ are finite in time $T$.
%\item $\mathcal{S}_x$ is $(A,d)$ sparse.
%\item $\Sp{B}$ $\mathcal{S}_u$ is $(A,d+1)$ sparse.
%\end{enumerate}
%\label{dfn:2}
%\end{definition}
%
%The third condition of Definition \ref{dfn:2} is key to extending our previous results \cite{2014_Wang_ACC} to non-scalar sub-systems.\footnote{In this paper, each sub-system can contain several states and control signals. The $x_i$ and $u_i$  refer to a single state and a single control signal respectively, which are scalars. However, a scalar $u_i$ might affect several states at the same time, and a state might be affected by several control signals as well.} Here, we not only want to localize the closed loop from $w$ to $x$, but also want to achieve this by only using controllers in a localized region. For the scalar sub-system plant model that was considered in \cite{2014_Wang_ACC}, the latter condition is automatically satisfied. For non-scalar sub-systems, we need to explicitly impose this constraint on the controller.

\subsection{State Feedback Localizability}
We start with designing the desired closed loop response. 
%Consider a global plant model given by
%\begin{equation}
%x[k+1] = A x[k] + B_2 u[k] + w[k] \label{eq:sfb}
%\end{equation}
%with state measurement. The z-transform of \eqref{eq:sfb} is given by
Consider the z-transform of \eqref{eq:dynamics}
\begin{equation}
(zI - A) x = B_2 u + w. \label{eq:zsfb}
\end{equation}
Denote $R$ the closed loop transfer function from $w$ to $x$, $M$ the closed loop transfer function from $w$ to $u$. Equation \eqref{eq:zsfb} can be written as
\begin{equation}
\begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I.
\end{equation}

In order to achieve a localized closed loop response, we impose the spatio-temporal constraint $(\mathcal{S}_R, \mathcal{S}_M)$ on the transfer function $R$ and $M$, which leads to the following definition.

\begin{definition} [State Feedback Localizability]
Assume that $(\mathcal{S}_R, \mathcal{S}_M)$ is a $(d,T)$ localized constraint for system $(A,B_2)$. The system $(A, B_2)$ is $(d,T)$ state feedback localizable by $(\mathcal{S}_R, \mathcal{S}_M)$ if and only if there exists $R, M \in \mathcal{RH}_\infty^{sp}$ such that the following equation is feasible.
\begin{eqnarray}
&& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \nonumber\\
&& \begin{bmatrix} R \\ M \end{bmatrix} \in \begin{bmatrix} \mathcal{S}_R \\ \mathcal{S}_M \end{bmatrix}  \label{eq:freq}
\end{eqnarray}
%In particular, when $(A, B_2)$ is a scalar sub-system model, and $(\mathcal{S}_R, \mathcal{S}_M)$ is the $(h,d,T)$ spatio-temporal constraint, we say that the system is $(h,d,T)$ state feedback localizable.
\end{definition}

Let $(\mathcal{S}_R, \mathcal{S}_M)$ be a $(d,T)$ localized FIR constraint for $(A,B_2)$. To check whether $(A,B_2)$ is $(d,T)$-FIR localizable by $(\mathcal{S}_R, \mathcal{S}_M)$, we can expand the spectral component of $R$ and $M$ into an augmented matrix and formulate the global feasibility test as a finite dimensional linear programming (LP) as
\begin{eqnarray}
&&\begin{bmatrix}I & -A & \cdots & 0\\
0 & \ddots & \ddots & \vdots\\
\vdots & \ddots & \ddots & -A \\
0 & \cdots & 0 & I
\end{bmatrix}
\begin{bmatrix}R[T+1] \\ \vdots \\ R[1]\end{bmatrix} = 
\begin{bmatrix}B_2 M[T] \\ \vdots \\ B_2 M[1] \\ I \end{bmatrix} \nonumber \\ \nonumber\\
&&R \in \mathcal{S}_R, M \in \mathcal{S}_M. \label{eq:system}
\end{eqnarray}
Note that the FIR constraint imposed on $R$ and $M$ ensures that $R[T+1] = 0$. This then imply $R[k] = 0$ and $M[k] = 0$ for all $k > T$, resulting a finite dimensional LP test in \eqref{eq:system}.

State feedback localizability can be considered as a generalization of controllability for a discrete time system. Specifically, assume that $(\mathcal{S}_R$ only contains the FIR constraint $R[n+1] = 0$, where $n$ is the number of states. Equation \eqref{eq:system} can then be written into
\begin{eqnarray}
\begin{bmatrix}R[n+1] \\ \vdots \\ R[2]\end{bmatrix} = \begin{bmatrix}A^n \\ \vdots \\ A\end{bmatrix} R[1] +
\begin{bmatrix}B_2 & \cdots & A^{n-1}B_2\\
 & \ddots & \vdots\\
0 &  & B_2
\end{bmatrix}\begin{bmatrix}M[n] \\ \vdots \\ M[1]\end{bmatrix} \nonumber
\end{eqnarray}
with $R[1] = I$ and $R[n+1] = 0$. If $A^n$ is non-singular, the feasibility of the above equation reduces to the condition rank$(\begin{bmatrix}B_2 & \cdots & A^{n-1}B_2 \end{bmatrix}) = n$, which is the well known rank condition on the controllability matrix. 

State feedback localizability is a stricter notion than controllability, as we not only want the closed loop response being FIR, but also satisfy a prescribed spatio-temporal constraint. Yet we argue that this stricter condition is desirable for large-scale system, as a controllable network does not mean that it is stabilizable in the presence of locality constraint on controller implementation. 

%- A generalization of controllability
%- Relation to disturbance localization
%From local point of view
%From global point of view
%Independent with the stability of A

%State feedback localizability is then defined as follows.
%\begin{definition}
%Assume that $(\mathcal{S}_x, \mathcal{S}_u)$ is a $(d,T)$ localized FIR constraint for system $(A,B)$. The system $(A,B)$ is state feedback $(d,T)$-FIR localizable by $(\mathcal{S}_x, \mathcal{S}_u)$ if and only if there exists strictly proper transfer functions $R \in \mathcal{S}_x$ and $M \in \mathcal{S}_u$ such that
%\begin{equation}
%R[k+1] = A R[k] + B M[k] \label{eq:freq}
%\end{equation}
%with $R[1]=I$. \label{dfn:3}
%\end{definition}
%
%Equation \eqref{eq:freq} is a relation that $R$ and $M$ must satisfy when the system dynamics are given by \eqref{eq:dynamics}. To see this, apply an impulse disturbance at state $j$ in \eqref{eq:dynamics}, i.e. $w[k] = \delta[k] e_j$. The closed loop response of $x[k]$ and $u[k]$ in \eqref{eq:dynamics} is by definition the $j$-th column of $R[k]$ and $M[k]$ respectively. Therefore, a valid closed loop transfer function pair $(R, M)$ must satisfy \eqref{eq:freq}. In addition, $(\mathcal{S}_x, \mathcal{S}_u)$ being a $(d,T)$ localized FIR constraints implies that $R[k] = \mathbf{0}$ and $M[k] = \mathbf{0}$ for all $k\geq T+1$, meaning that $R$ and $M$ are both FIR as well.

%Definition \ref{dfn:3} has an intuitive interpretation in the time domain. For a $(d,T)$-FIR localizable system, a local disturbance $w_j$ only affects $x_i$ with $i \in Down(j,d)$, and the effect will be eliminated in time $T$. Furthermore, we only need to activate the local controllers $u_i$ for $\{\ell \, | \, B_{\ell i} \not = 0\} \subseteq Down(j,d+1)$ in order to localize the affected region. As illustrated in Figure \ref{fig:lightcones}, the affected region of $w_j$ is confined to the right section in the space-time diagram, which we call the forward space-time region for $w_j$.  %which is equal to the sparsity constraint in $j$-th column of $\mathcal{S}_x$. 

%\begin{figure}[ht!]
%      \centering
%      \includegraphics[width=0.48\textwidth]{figure/lightcones8.pdf}
%      \caption{Local space-time region interpretation of proposed control strategy.}
%      \label{fig:lightcones}
%\end{figure}

%Imposing space-time constraints on the closed loop has the added benefit that the controller can then be implemented in a localized manner. Assume that the disturbance $w$ can be perfectly estimated. Then, each local controller only needs to collect the estimated disturbances from a backward space-time region as shown in Figure \ref{fig:lightcones}. Hence we can impose communication delay constraints for information collection through this region by ensuring that the backward space-time region is contained within an allowable region.

\subsection{Local Feasibility Test}
In this subsection, we show that state feedback localizability can be checked in a localized and parallel way. Specifically, we show that the feasibility of \eqref{eq:freq} can be verified in a localized and parallel manner by column decomposition on $R$ and $M$. The fact that $(\mathcal{S}_R, \mathcal{S}_M)$ is a $(d,T)$ localized FIR constraint enables us to further reduce the dimension of the feasibly test of each column.

Consider the $j$-th column of \eqref{eq:freq} 
%The first step is noting that the feasibility of \eqref{eq:freq} can be checked by each column in a parallel way. For $j$-th column, the feasibility test becomes
\begin{eqnarray}
&& \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix}_j = e_j \nonumber\\
&& \begin{bmatrix} R \\ M \end{bmatrix}_j \in \begin{bmatrix} \mathcal{S}_R \\ \mathcal{S}_M \end{bmatrix}_j  \label{eq:freq_col}
\end{eqnarray}
where the subscript $j$ represents the $j$-th column of the corresponding transfer function. Equation \eqref{eq:freq_col} can also be interpreted by the system dynamics. Let $x[0] = 0$, $u[0] = 0$, and apply an impulse disturbance $w[k] = \delta[k] e_j$ to \eqref{eq:dynamics}. We then search the desired $x[k]$ and $u[k]$ such that the effect of the disturbance is contained within a prescribed space-time region. The decomposition from \eqref{eq:freq} to \eqref{eq:freq_col} imply that we can check the impulse disturbance $w[k] = \delta[k] e_j$ in a parallel way for each $j$, even when the localized region for each $j$ may be overlapping.

We now focus on system $j$'s point of view. As $(\mathcal{S}_R, \mathcal{S}_M)$ is a $(d,T)$ localized FIR constraint, equation \eqref{eq:freq_col} implies that the nonzero states in $x[k+1]$, $A x[k]$, and $B_2 u[k]$ are constrained to be in the set $Down(j,d+1)$. This motivates the definition of localized state, control, and plant model from $j$'s point of view.
%the nonzero entries in their $j$-th column is contained within the set $Down(j,d)$ and $Down(j,d+1)$, respectively. Recall that $Down(j,d+1)$ is the downstream set of system $j$ within distance $(d+1)$.

\begin{definition}
The $(j,d)$-localized state vector $x_{(j,d)}$ consists of all local state $x_i$ with $i \in Down(j,d+1)$. Similarly, the $(j,d)$-localized control vector $u_{(j,d)}$ consists of all local control $u_i$ such that their effect is strictly within the set $Down(j,d+1)$. Specifically, $u_{(j,d)}$ contains all $u_i$ with $\{k \, | \, B_{k i} \not = 0\} \subseteq Down(j,d+1)$.
\end{definition}

To lighten notational burden, we replace the subscript $(j,d)$ by simply $\ell$, which means ``localized". We consider an example on localized state vector and control action for a chain model.

\begin{example}
Let $(j,d) = (1,1)$ for the chain model in Figure \ref{fig:Chart105}. The set $Down(j,d+1) = \{1, 2, 3\}$. The $(1,1)$-localized state vector and control action are therefore $x_\ell = [x_1, x_2, x_3]^\top$ and $u_\ell = [u_1, u_2, u_3]^\top$.
\end{example}

For $\ell = (j,d)$, we can define the localized plant model $(A_\ell,B_{2 \ell})$ by selecting submatrices of $(A,B_2)$ consisting of the columns and rows associated with $x_\ell$ and $u_\ell$. We denote by $e_\ell$ the new location of the source of disturbance $j$ within the localized state $x_\ell$. The localized constraint space $(\mathcal{S}_{x \ell}, \mathcal{S}_{u \ell})$ can be defined by selecting the $j$-th column of $(\mathcal{S}_R, \mathcal{S}_M)$ and the rows associated with $(x_\ell, u_\ell)$.

\begin{example}
Continue with the previous example. The localized plant model with $(j,d) = (1,1)$ is given by the left-top $3 \times 3$ submatrix of global plant model $A$. For a chain model (tridiagonal $A$) with $d = 1$, the localized plant model for $j = 1, 3, 5$ are illustrated in Figure \ref{fig:local}.
\end{example}

\begin{figure}[t!]
      \centering
      \includegraphics[width=0.3\textwidth]{./figure/LocalModel.pdf}
      \caption{The sparsity pattern of the $A$ matrix for a chain model. With $d = 1$, the blue, red, black block represents the localized plant model for $j = 1, 3, 5$, respectively.}
      \label{fig:local}
\end{figure}

With the definition of localized plant model, equation \eqref{eq:freq_col} can be simplified into
\begin{eqnarray}
&& \begin{bmatrix} zI - A_\ell & -B_{2 \ell} \end{bmatrix} \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} = e_\ell \nonumber\\
&& \begin{bmatrix} x_\ell \\ u_\ell \end{bmatrix} \in \begin{bmatrix} \mathcal{S}_{x \ell} \\ \mathcal{S}_{u \ell} \end{bmatrix}.  \label{eq:freq_local}
\end{eqnarray}
Note that the dimension of the test in \eqref{eq:freq_local} depends only on the size of the localized plant model, regardless the size of the global plant model. We can also express \eqref{eq:freq_local} in the form of \eqref{eq:system} as
\begin{eqnarray}
&&\begin{bmatrix}I & -A_{\ell} & \cdots & 0\\
0 & \ddots & \ddots & \vdots\\
\vdots & \ddots & \ddots & -A_{\ell} \\
0 & \cdots & 0 & I
\end{bmatrix}
\begin{bmatrix}x_{\ell}[T+1] \\ \vdots \\ x_{\ell}[1]\end{bmatrix} = \begin{bmatrix}B_{2 \ell}u_{\ell}[T] \\ \vdots \\ B_{2 \ell}u_{\ell}[1] \\ e_{\ell} \end{bmatrix}\nonumber\\ \nonumber\\
&& x_\ell \in \mathcal{S}_{x \ell}, u_\ell \in \mathcal{S}_{u \ell}
\label{eq:system_1}
\end{eqnarray}
where $\ell = (j,d)$ for each $j = 1, \dots, n$. We emphasize the fact that the whole test can be performed in a parallel way for each $j$, even when the localized region may be overlapping. In addition, the size of each local feasibility test only depends on its localized plant model.
%without using any iteration.
%\begin{example}
%Run in a parallel manner, even when the localized region is overlapping.
%\end{example}

The equivalence between local and global feasibility test is formally stated in the following theorem.
%To prove the equivalence between the global feasibility test and local feasibility test, we define the embedding linear operators $E_x(\cdot)$ on $x_{(j,d)}[k]$ and $E_u(\cdot)$ on $u_{(j,d)}[k]$, which simply add appropriate zero padding such that $E_x(x_{(j,d)}[k]) = (R[k])_j$ and $E_u(u_{(j,d)}[k]) = (M[k])_j$, where $(R[k])_j$ and $(M[k])_j$ are the $j$-th column of $R[k]$ and $M[k]$ respectively. In particular, we have that $E_x(e_{w(j,d)}) = e_j$. The equivalence between local and global feasibility test is given by the following theorem.
%\begin{theorem}
%$(x_{(j,d)},u_{(j,d)})$ is a feasible solution for \eqref{eq:system_1} if and only if $(E_x(x_{(j,d)}),E_u(u_{(j,d)}))$ form the $j$-th column of $(R,M)$, where $(R,M)$ is a feasible solution for \eqref{eq:system}. 
%\label{thm:local_feasibility}
%\end{theorem}
\begin{theorem}
A system is $(d,T)$-localizable if and only if \eqref{eq:system_1} is feasible for all $j$ with $\ell = (j,d)$. \label{thm:local_feasibility}
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

\begin{remark}[Robustness to local changes]Equation \eqref{eq:system_1} indicates that the solution $(x_\ell, u_\ell)$ only depends on the local plant model $(A_\ell, B_{2 \ell})$. Therefore, when a plant model changes locally, we only need to resolve some of the local feasibility tests to check whether it is still localizable.
\end{remark}

%For each local feasibility test \eqref{eq:system_1}, we can explicitly express the state trajectory $x_{(j,d)}[k]$ over the horizon $k=2,\dots,T+1$ as a function of control input $u_{(j,d)}[k]$ as 
%\begin{eqnarray}
%X_{(j)} &=& W_{(j)} + C_{(j)} U_{(j)} \nonumber \\
%\Sp{X_{(j)}} &\subseteq& ST_x^{(j)} \nonumber \\
%\Sp{U_{(j)}} &\subseteq& ST_u^{(j)}
%\label{eq:local_feas}
%\end{eqnarray}
%where
%\begin{eqnarray}
%&X_{(j)}& = \begin{bmatrix}x_{(j,d)}[T+1] \\ \vdots \\ x_{(j,d)}[2]\end{bmatrix}, 
%W_{(j)} = \begin{bmatrix}A_{(j,d)}^T \\ \vdots \\ A_{(j,d)}\end{bmatrix} e_{w(j,d)}, \nonumber\\
%&C_{(j)}& = \begin{bmatrix}B_{(j,d)} & \cdots & A_{(j,d)}^{T-1}B_{(j,d)}\\
% & \ddots & \vdots\\
%0 &  & B_{(j,d)}
%\end{bmatrix}, \nonumber\\ 
%&U_{(j)}& = \begin{bmatrix}u_{(j,d)}[T] \\ \vdots \\ u_{(j,d)}[1] \end{bmatrix} \nonumber
%\end{eqnarray}
%with $x_{(j,d)}[1] = e_{w(j,d)}$, and $ST_x^{(j)}$ and $ST_u^{(j)}$ the stacked sparsity constraints that can be derived directly from \eqref{eq:system_1}. The form of \eqref{eq:local_feas} is the same as the traditional way to check controllability of a system. We can then interpret state feedback localizability as a generalization of controllability  within a space-time region. 

==> old/State_v1.tex <==
In this section, we give a general formulation of the localized distributed optimal control problem. We then show that when the objective function is a quadratic cost, the localized LQR (LLQR) problem admits a localized decomposition similar to the way to perform localized verification. This allows a localized synthesis procedure for the optimal controller.

\subsection{Optimal Control Problem Formulation}
In general, the localized optimal control problem can be formulated as the following affinely constrained convex program:
\begin{eqnarray}
\underset{R, M \in \mathcal{RH}_\infty}{\text{minimize  }} &&f(R, M) \nonumber\\
\text{subject to } &&\eqref{eq:freq} \label{eq:convex}
\end{eqnarray}
for some convex function $f$. Localizability is determined by the feasibility of this optimization problem. Note that as the closed loop system is constrained to be FIR, traditionally infinite dimensional objectives and constraints, such as those present in $\mathcal{H}_2$ optimal control, trivially admit a finite dimensional representation.

\subsection{Localized LQR}
For a general objective function in \eqref{eq:convex}, the optimization may not necessarily be solved in a localized way. However, when the cost function is chosen to be LQR, leading to a LLQR optimal control problem, \eqref{eq:convex} can be decomposed in exactly the same way as the local feasibility test. Thus, the LLQR problem can be solved by solving multiple local optimization problems in a parallel fashion.
%Thus, the optimal LLQR controller can be synthesized based on local optimizations followed by local update procedures.

The general formulation for the LLQR problem is given by
\begin{eqnarray}
\underset{R, M \in \mathcal{RH}_\infty^{sp}}{\text{minimize  }} &&||\begin{bmatrix}C_1 & D_{12} \end{bmatrix} \begin{bmatrix}R \\ M \end{bmatrix} ||_{\mathcal{H}_2}^2 \nonumber\\
\text{subject to } &&\eqref{eq:freq}. \label{eq:lqr_obj0}
\end{eqnarray}
The objective function in \eqref{eq:lqr_obj0} can be written as
%This then leads to a formulation as
%\begin{align}
%\underset{R, M \in \mathcal{RH}_\infty}{\text{minimize }} &\sum_{k=1}^{T} \text{Trace}(\begin{bmatrix}R[k] \\ M[k] \end{bmatrix}^\top \begin{bmatrix}C_1^\top C_1 & C_1^\top D_{12} \\ D_{12}^\top C_1 & D_{12}^\top D_{12} \end{bmatrix} \begin{bmatrix}R[k] \\ M[k] \end{bmatrix}) \nonumber\\
%\text{subject to } &\eqref{eq:freq}. \label{eq:lqr_obj}
%\end{align}
\begin{equation}
\sum_{k=1}^{T} \text{Trace}(\begin{bmatrix}R[k] \\ M[k] \end{bmatrix}^\top \begin{bmatrix}C_1^\top C_1 & C_1^\top D_{12} \\ D_{12}^\top C_1 & D_{12}^\top D_{12} \end{bmatrix} \begin{bmatrix}R[k] \\ M[k] \end{bmatrix}). \label{eq:lqr_obj}
\end{equation}
To see why \eqref{eq:lqr_obj0} is called the LLQR problem, assume that
\begin{equation}
\begin{bmatrix}C_1^\top C_1 & C_1^\top D_{12} \\ D_{12}^\top C_1 & D_{12}^\top D_{12} \end{bmatrix} = \begin{bmatrix}\mathcal{Q} & 0 \\ 0 & \mathcal{R} \end{bmatrix}
\end{equation}
for some semi-positive definite matrix $\mathcal{Q}$ and positive definite matrix $\mathcal{R}$.
%To compare with the normal LQR formulation, we assume that $\mathcal{Q} = C_1^\top C_1$ is a semi-positive definite matrix, $\mathcal{R} = D_{12}^\top D_{12}$ a positive definite matrix, and $C_1^\top D_{12} = 0$. 
Letting $n$ be the number of states, the objective in \eqref{eq:lqr_obj} can be further written as
\begin{equation}
\sum_{j=1}^{n} \sum_{k=1}^{T} \text{Trace}(\begin{bmatrix}R[k] \\ M[k] \end{bmatrix}^\top \begin{bmatrix}\mathcal{Q} & 0 \\ 0 & \mathcal{R} \end{bmatrix} \begin{bmatrix}R[k] \\ M[k] \end{bmatrix} e_j e_j^\top). \label{eq:lqr_trace}
\end{equation}
As trace is invariant under cyclic permutation, we can write \eqref{eq:lqr_trace} as
\begin{equation}
\sum_{j=1}^{n} \sum_{k=1}^{T} \begin{bmatrix}R[k] \\ M[k] \end{bmatrix}_j^\top \begin{bmatrix}\mathcal{Q} & 0 \\ 0 & \mathcal{R} \end{bmatrix} \begin{bmatrix}R[k] \\ M[k] \end{bmatrix}_j. \nonumber
\end{equation}
Using Theorem \ref{thm:local_feasibility}, each $(R[k])_j$ and $(M[k])_j$ can be solved for via the $j$-th local feasibility test. Thus, we can decompose the full objective in \eqref{eq:lqr_obj} into the sum of local objectives. Let $\ell = (j,d)$, the LLQR sub-problem for the reduced trajectory $x_{\ell}[k]$ and $u_{\ell}[k]$ can be formulated as
\begin{align}
\underset{\{x_{\ell}[k], u_{\ell}[k]\}_{k=1}^T}{\text{minimize }}& \sum_{k=1}^{T} x_{\ell}[k]^\top \mathcal{Q}_\ell x_{\ell}[k] + u_{\ell}[k]^\top \mathcal{R}_\ell u_{\ell}[k] \nonumber\\
\text{subject to } &\eqref{eq:freq_local} \label{eq:lqr_op_0}
\end{align}
where $\mathcal{Q}_\ell$ and $\mathcal{R}_\ell$ are submatrices of $(\mathcal{Q},\mathcal{R})$ consisting of the columns and rows associated with $x_{\ell}$ and $u_{\ell}$. We solve \eqref{eq:lqr_op_0} with $\ell = (j,d)$ for $j = 1, \dots, n$ in a parallel way.

%To lighten notational burden, we drop all subscripts and write \eqref{eq:local_feas} as $X = W + C U$, $\Sp{X} \subseteq ST_x$, and $\Sp{U} \subseteq ST_u$. In addition, we define $(\mathcal{\overline{Q}}_j, \mathcal{\overline{R}}_j)$ as the augmented block diagonal matrix with $(\mathcal{Q}_j, \mathcal{R}_j)$ along the block diagonal. The objective in \eqref{eq:lqr_op_0} can therefore be written in a single term $X^\top \mathcal{\overline{Q}}_j X + U^\top \mathcal{\overline{R}}_j U$. The analytic solution of \eqref{eq:lqr_op_0} can be derived as follows.
%
%Noting that $\Sp{U} \subseteq ST_u$ is an affine constraint that forces some of the elements of $U$ to be zero, we can eliminate this constraint by selecting the appropriate columns of matrix $C$ to form a reduced matrix $C_{r}$ such that
%\begin{equation}
%C U = C_{r} U_{r} \nonumber
%\end{equation}
%where $U_{r}$ is the reduced \emph{unconstrained} control signal.% by imposing the constraint $\Sp{U} \subseteq ST_u$. 
%
%Similarly, we can impose the constraint $\Sp{X} \subseteq ST_x$ by selecting the corresponding rows on $W$ and $C_{r}$. Specifically, we define matrices $W_a$ and $C_a$ by selecting the rows of $W$ and $C_r$ according to the positions of the zero entries in $ST_x$, and the rows of $W_b$ and $C_b$ according to the positions of the nonzero entries in $ST_x$. The equation $X = W + C_r U_r$ is then separated into two parts: 
%\begin{eqnarray}
%0 &=& W_{a} + C_{a} U_{r} \label{eq:lqr_1}\\
%X_{r} &=& W_{b} + C_{b} U_{r} \label{eq:lqr_2}
%\end{eqnarray}
%where \eqref{eq:lqr_1} corresponds to the sparsity constraints imposed by $ST_x$, and \eqref{eq:lqr_2} enforces that the non-zero states $X_r$ satisfy the dynamics. 
%
%We define $(\mathcal{Q}_{r}, \mathcal{R}_{r})$ the submatrices of $(\mathcal{\overline{Q}}_j, \mathcal{\overline{R}}_j)$ associated with the support of $ST_x$ and $ST_u$ respectively. Then, \eqref{eq:lqr_op_0} becomes
%\begin{align}
%&\underset{X_r, U_r}{\text{minimize }} X_{r}^\top \mathcal{Q}_{r} X_{r} + U_{r}^\top \mathcal{R}_{r} U_{r} \nonumber\\
%&\text{subject to } \textit{\eqref{eq:lqr_1} and \eqref{eq:lqr_2}} \label{eq:lqr_op}
%\end{align}
%Substituting \eqref{eq:lqr_2} into the objective function, we have
%\begin{eqnarray}
%\underset{U_r}{\text{minimize }}  &&U_{r}^\top (\mathcal{R}_{r}+C_{b}^\top  \mathcal{Q}_{r} C_{b}) U_{r}+ 2 U_{r}^\top (C_{b}^\top  \mathcal{Q}_{r} W_{b}) \nonumber\\
%\text{subject to }  &&0 = W_{a} + C_{a} U_{r} \label{eq:convex_lqr}
%\end{eqnarray}
%
%If this problem is feasible, then we can solve the quadratic optimization via its optimality conditions
%\begin{eqnarray}
%\begin{bmatrix} \mathcal{R}_{r}+C_{b}^\top  \mathcal{Q}_{r} C_{b} & C_{a}^{\top}\\
% C_{a} & 0
%\end{bmatrix}
%\begin{bmatrix} U_r^{*}\\
%\lambda^{*}
%\end{bmatrix}=
%\begin{bmatrix} -C_{b}^\top  \mathcal{Q}_{r} W_{b}\\
%-W_{a}
%\end{bmatrix}. \label{eq:optimality}
%\end{eqnarray}

Note that \eqref{eq:lqr_op_0} is an affinely constrained quadratic program. We can use the technique of Lagrange multiplier and write the optimality condition of \eqref{eq:lqr_op_0} as a linear equation. In addition, the size of the problem is independent to the size of the global plant model $A$ since we only need to know the local plant model $A_\ell$ for each LLQR sub-problem. This property is especially favorable for large scale distributed systems. 

The LLQR problem derived in this Section is based on the assumption that $w[k]$ is an impulse disturbance on each state. In \cite{2014_Wang_CDC}, we further show that the controller synthesized by \eqref{eq:lqr_op_0} is mean square error optimal with respect to additive white Gaussian noise (AWGN), i.e. $E[w[k]] = 0$ and $E[w[i] w[j]^\top] = \delta_{ij} I$ for all $i,j,k$.

%to solve the optimal solution analytically. 

%In other words, we can solve the feasibility of this problem as well as the optimal solution by a set of linear equations. Although the problem size of \eqref{eq:optimality} is proportional to time $T$, it is independent to the size of the global plant model $A$ since we only need to know the local plant model $A_\ell$ for each LLQR feasibility test. This property is especially favorable for large scale distributed systems. Future work will look to find a dynamic programming based solution to remove this linear scaling with $T$.

%- Analytic solution in Appendix

%- AWGN expected optimal

%In summary, the reduced LLQR problem is subject to the constraint in \eqref{eq:convex_lqr}, and has the optimal solution given by \eqref{eq:optimality}, implying that the LLQR optimal controller can be synthesized by solving a set of linear equations. Although the problem size of \eqref{eq:optimality} is proportional to time $T$, it is independent to the size of the global plant model $A$ since we only need to know the local plant model $A_{(j,d)}$ for each $j$-th LLQR feasibility test. This property is especially favorable for large scale distributed systems. Future work will look to find a dynamic programming based solution to remove this linear scaling with $T$.




==> old/model_v1.tex <==
Consider a discrete time distributed system described by
\begin{eqnarray}
x[k+1] &=& A x[k] + B_2 u[k] + \delta_x [k] \nonumber \\
y[k] &=& C_2 x[k] + \delta_y [k] \label{eq:dynamics}
\end{eqnarray}
where $x=(x_i)$, $u=(u_i)$, and $y=(y_i)$ are stacked vectors of local state, control, and measurement, respectively, and $\delta_x = (\delta_x)_i$ and $\delta_y = (\delta_y)_i$ are the stacked perturbations on each state and measurement, respectively. These perturbation may represent the process noise and sensor noise of the system, but may include other sources of disturbance. For example, actuator saturation and/or quantization on the control action can be modeled as $\delta_x = B_2 \delta_u$ for appropriately defined $\delta_u$.  

The objective is to design a distributed controller that generates a control signal $u$, based on the measurements $y$ (subject to the information sharing constraints of the system) such that the closed loop transfer functions from the perturbations $(\delta_x, \delta_y)$ to $(x, u)$ satisfy some spatio-temporal constraints (which will be defined in the next subsection). We will show that if the closed loop transfer functions can be localized, then the controller can be implemented in a localized manner. Throughout this paper, we use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system.

==> old/model_v2.tex <==
\subsection{Mathematical Notations and Preliminaries} 
Let $z$ be the variable of the z-transform. We use $L[i]$ to denote the $i$-th spectral component of any transfer function $L$, $L = \sum_{i=0}^{\infty} \frac{1}{z^i} L[i]$. In time domain, the order set $\{L[i]\}_{i=0}^{\infty}$ describes the impulse response of the system. If $L$ is a matrix transfer function, $L_j$ represents the $j$-th column of the transfer function $L$ unless specified otherwise, and $L_{ij}$ represents the $(i,j)$-entry of $L$. For a vector $x$, $x_j$ represents the $j$-th component of $x$.

In this paper, we denote $\mathcal{RH}_{\infty}$ the set of all stable, real-rational, and proper transfer functions, $\mathcal{RH}_{\infty}^{sp}$ the set of all stable, real-rational, and strictly proper transfer functions. $|| \cdot ||_{\mathcal{H}_2}$ is the $\mathcal{H}_2$ norm of a transfer function.

Given a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$. $\mathcal{V} = \{v_1, \dots, v_n\}$ is the set of vertices, and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the set of directed edges. A \emph{directed path} of a graph is a sequence of directed edges which connect a sequence of vertices, with all edges directed in the same direction. The \emph{length} of a path is the number of edges of that path. The \emph{distance} from $v_i$ to $v_j$ is the length of a shortest path which connect $v_i$ to $v_j$. 

\subsection{System Model}
Consider a discrete time linear time invariant (LTI) system with dynamics given by
\begin{equation}
x[k+1] = A x[k] + B_2 u[k] + w[k] \label{eq:dynamics}
\end{equation}
where $x = (x_i)$, $u = (u_i)$ and $w = (w_i)$ are stacked vector of local state, control action, and disturbance, respectively. In this paper, we are particular interested in the case that $A$ and $B_2$ are large sparse matrices. We aim to develop a method that exploits the sparsity structure of $A$ and $B_2$ to enhance scalability of controller synthesis and implementation. To illustrate the idea, we start with a simple model that is consisted of a chain of $n$ dynamically coupled linear systems as shown in Figure \ref{fig:Chart105}. In this figure, all $x_i, u_i, w_i$ are assumed to be scalar, and the numbers represent the delay between nodes. The dynamics of the system in Figure \ref{fig:Chart105} is given by \eqref{eq:dynamics}, where $A$ is a tridiagonal matrix and $B_2$ a diagonal matrix. We will use this chain model to illustrate various ideas throughout this paper.
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.48\textwidth]{./figure/Long_chain3.pdf}
      \caption{Chain Model: Each $x_i$ is a local state and $u_i$ a local control action. The numbers represent the delay between nodes. The actuation, sensing, and plant propagation delay are one time step. The communication speed is $h > 1$ times faster than the speed of plant propagation. Therefore, the communication delay between two nearby nodes is $1/h$. The system dynamics is given by \eqref{eq:dynamics}, with $A$ a tridiagonal matrix and $B_2$ a diagonal matrix.}
      \label{fig:Chart105}
\end{figure}

Note from Figure \ref{fig:Chart105} that the sparsity pattern of $(A, B_2)$ can be described by the underlying graph structure of the system model. We define the state transition graph of a matrix $A$ as follows.
%The sparsity pattern of $A$ can be described by the state transition graph as follows.
%Specifically, for a square matrix $A$, we define the state transition graph as follows.
\begin{definition} [State Transition Graph]
The state transition graph of a $n \times n$ matrix $A$ is a directed graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with $\mathcal{V} = \{x_1, \dots, x_n\}$, and $(x_i, x_j) \in \mathcal{E}$ if and only if $A_{ji} \not = 0$.
\end{definition}

The sparsity pattern of $B_2$ is described column by column -- each represents the set of states that is affected directly by a scalar control action. For ease of explanation, we focus our discussion on the scalar sub-system model, which is defined as follows.

\begin{definition} [Scalar Sub-system]
A system given by \eqref{eq:dynamics} is called a \emph{scalar sub-system} model if $B_2$ has at most one non-zero entry per column. \label{df:1}
\end{definition}

Definition \ref{df:1} means that each control action in \eqref{eq:dynamics} can only affect at most one state directly. In this case, we can treat each state as a scalar sub-system. The method described in this paper focus on, but not limit to, scalar sub-system model.

%\begin{example}
%For a tridiagonal $n \times n$ matrix $A$, the state transition graph is given by the lower part of Figure \ref{fig:Chart105}.
%\end{example}

\subsection{Problem Formulation}
%Although the chain model in Figure \ref{fig:Chart105} looks simple, it gives significant difficulties for controller synthesis and implementation when $n$ becomes large. 
The first problem we are going to solve is designing a distributed dynamic state-feedback controller such that the transfer functions from $w$ to $x$ and $w$ to $u$ satisfy some spatio-temporal (locality) constraints. Throughout this paper, we use $R$ to denote the closed loop transfer function from $w$ to $x$ and $M$ the closed loop transfer function from $w$ to $u$. The key idea in this paper is to force $R$ and $M$ to satisfy some spatio-temporal constraints, then show that the controller achieving the desired closed loop response can be synthesized and implemented by $R$ and $M$. 

%Instead of imposing the communication and sparsity constraint on $K$ as in \eqref{eq:intro}, we impose the communication and sparsity constraint on the \emph{closed loop transfer functions} $R$ and $M$ and formulate the \emph{localized distributed optimal control} problem as
Specifically, we formulate the \emph{localized distributed optimal control} problem as
\begin{eqnarray}
\underset{R, M \in \mathcal{RH}_\infty^{sp}}{\text{minimize  }} &&||\begin{bmatrix}C_1 & D_{12} \end{bmatrix} \begin{bmatrix}R \\ M \end{bmatrix} ||_{\mathcal{H}_2}^2 \label{eq:intro2}\\
\text{subject to } && \begin{bmatrix} zI - A & -B_2 \end{bmatrix} \begin{bmatrix} R \\ M \end{bmatrix} = I \label{eq:intro3}\\
&& \begin{bmatrix} R \\ M \end{bmatrix} \in \begin{bmatrix} \mathcal{S}_R \\ \mathcal{S}_M \end{bmatrix}  \label{eq:intro4}
\end{eqnarray}
where \eqref{eq:intro2} is a convex objective of the closed loop transfer functions $(R,M)$, \eqref{eq:intro3} is the system dynamics, and \eqref{eq:intro4} is the spatio-temporal constraints on $(R,M)$. The formal definition of spatio-temporal constraints \eqref{eq:intro4} will be introduced in Section \ref{sec:st_cons}. In Section \ref{sec:state}, we consider \eqref{eq:intro3} and \eqref{eq:intro4} together and define the feasibility of \eqref{eq:intro3} - \eqref{eq:intro4} as \emph{state feedback localizability}. In Section \ref{sec:LLQR}, we consider the whole optimization problem \eqref{eq:intro2} - \eqref{eq:intro4} together, and explain why this is called the LLQR problem. Then in Section \ref{sec:imp}, we show how to achieve localized synthesis and implementation from the solution of this optimization problem.




==> st_cons_simple.tex <==
For a matrix $A$, we use $A_{ij}$ to denote its $(i,j)$-th entry. Define the support operator $\Sp{\cdot}: \mathbb{R}^{m \times n} \to \{0,1\}^{m \times n}$, where $\{\Sp{A}\}_{ij}=1$ if and only if $A_{ij}\neq0$, and $\{\Sp{A}\}_{ij}=0$ otherwise. 
%Block-wise sparsity pattern(?) Or define this after the interconnected system model
We use $\cup$ to denote the OR operator, and $\cap$ to denote the AND operator on binary variables.
%We define the OR operator $\cup$ and AND operator $\cap$ on binary variables by the following rules
%\begin{eqnarray}
%&& 0 \cup 0 = 0 \quad 0 \cup 1 = 1 \quad 1 \cup 0 = 1 \quad 1 \cup 1 = 1 \nonumber\\
%&& 0 \cap 0 = 0 \quad 0 \cap 1 = 0 \quad 1 \cap 0 = 0 \quad 1 \cap 1 = 1. \nonumber
%\end{eqnarray}
The addition of two binary matrices $\s_1,\s_2 \in \{0,1\}^{m \times n}$ is defined in an element-wise manner by 
\begin{equation}
(\s_1 + \s_2)_{ij} = (\s_1)_{ij} \cup (\s_2)_{ij}. \nonumber
\end{equation}
In addition, we write $\s_1\subseteq \s_2$ when $\s_1 + \s_2=\s_2$. 
%The product $\s_1 = \s_2 \s_3$ with binary matrices of compatible dimension is defined by the rule
%\begin{equation}
%(\s_1)_{ij} = \underset{k}{\cup} \, [ \, (\s_2)_{ik} \cap (\s_3)_{kj} \, ].
%\end{equation}
%where the $\cup$ operator is taken over all possible $k$. For a square binary matrix $\mathcal{S}_0$, we define the power $\mathcal{S}_{0}^{i+1} := \mathcal{S}_{0}^i \mathcal{S}_{0}$ for all positive integer $i$, and $\mathcal{S}_{0}^0 = I$. 

The sparsity patterns defined on a matrix can be extended to the spatio-temporal constraints defined on a transfer function. Specifically, the spatio-temporal constraints for a transfer function $R$ is described by a constraint space $\mathcal{S}_R := \sum_{i=0}^{\infty} \frac{1}{z^i} \s_{R}[i]$, where $\{\s_{R}[i]\}$ is an ordered set of binary matrices. We say that a transfer function $R$ is in $\mathcal{S}_R$ if and only if $\Sp{R[i]} \subseteq \s_{R}[i]$ for all $i$, which we denote by $R \in \mathcal{S}_R$. 

==> st_cons_v1.tex <==
%In this section, we start with the definition of state transition graph, which is an intuitive graphical interpretation of the sparsity patterns of system $A$. We then define the operation on sparsity pattern and the distance between two states algebraically. Finally, we extend the notion of sparsity pattern of a matrix into the spatio-temporal constraints on a transfer function, and define the $(d,T)$ localized FIR constraint for a distributed system $(A, B_2)$.
In this section, we define the operation on sparsity pattern and the distance between two states in an algebraic way. We then extend the notion of sparsity pattern of a matrix into the spatio-temporal constraints on a transfer function, and define the $(d,T)$ localized FIR constraint for a distributed system $(A, B_2)$.
%\subsection{State Transition Graph}
%\input{Graph}

\subsection{Sparsity Patterns}
Define the support operator $\Sp{\cdot}: \mathbb{R}^{m \times n} \to \{0,1\}^{m \times n}$, where $\{\Sp{A}\}_{ij}=1$ if and only if $A_{ij}\neq0$, and $\{\Sp{A}\}_{ij}=0$ otherwise. We define the OR operator $\cup$ and AND operator $\cap$ on binary variables by the following rules
\begin{eqnarray}
&& 0 \cup 0 = 0 \quad 0 \cup 1 = 1 \quad 1 \cup 0 = 1 \quad 1 \cup 1 = 1 \nonumber\\
&& 0 \cap 0 = 0 \quad 0 \cap 1 = 0 \quad 1 \cap 0 = 0 \quad 1 \cap 1 = 1. \nonumber
\end{eqnarray}
The addition of two binary matrices $\s_1,\s_2 \in \{0,1\}^{m \times n}$ is defined by 
\begin{equation}
(\s_1 + \s_2)_{ij} = (\s_1)_{ij} \cup (\s_2)_{ij}. \nonumber
\end{equation}
In addition, we write $\s_1\subseteq \s_2$ when $\s_1 + \s_2=\s_2$. The product $\s_1 = \s_2 \s_3$ with binary matrices of compatible dimension is defined by the rule
\begin{equation}
(\s_1)_{ij} = \underset{k}{\cup} \, [ \, (\s_2)_{ik} \cap (\s_3)_{kj} \, ].
\end{equation}
%\begin{eqnarray}
%&&(\s_1)_{ij} = 1 \textit{ iff there exists a $k$ such that} \nonumber\\
%&&(\s_2)_{ik} = 1 \textit{ and } (\s_3)_{kj} = 1. \nonumber
%\end{eqnarray}
where the $\cup$ operator is taken over all possible $k$. For a square binary matrix $\mathcal{S}_0$, we define the power $\mathcal{S}_{0}^{i+1} := \mathcal{S}_{0}^i \mathcal{S}_{0}$ for all positive integer $i$, and $\mathcal{S}_{0}^0 = I$. 

Let $\mathcal{A} = \Sp{A}$, which characterizes the underlying topology of the state transition graph. The distance from state $k$ to $j$ can be defined by 
\begin{equation}
\displaystyle \dist{k}{j}{\mathcal{A}}: = \min\{ i \in \mathbb{N} \cup 0 \, | \, \left(\mathcal{A}^{i}\right)_{jk} \neq 0\}. \nonumber
\end{equation}
Note that this definition is compatible with the definition of distance function on a graph.
%Note that this definition is compatible with the common notion of distance function on a graph, which is defined by the length of the shortest path connecting from one state to the other. 

We then characterize the localized region for each state $j$ by defining the following two sets
\begin{eqnarray}
Up(j,d) &=& \{s \, | \, \dist{s}{j}{\mathcal{A}} \leq d \} \nonumber\\
Down(j,d) &=& \{s \, | \, \dist{j}{s}{\mathcal{A}} \leq d \} \nonumber
\end{eqnarray}
where $Up(j,d)$ is the upstream set of state $j$ within distance $d$, and $Down(j,d)$ is the downstream set of state $j$ within distance $d$. If the topology of $\mathcal{A}$ is represented by an undirected graph, $\mathcal{A}$ is symmetric and $Up(j,d) = Down(j,d)$ for all $j$ and $d$.

From the definition of distance function, we have
\begin{eqnarray}
Up(j,d) &=& \{s \, | \, \dist{s}{j}{\mathcal{A}} \leq d \} \nonumber\\
&=& \{s \, | \, \left(\mathcal{A}^{i}\right)_{js} \neq 0 \text{ for some } i \leq d \} \nonumber\\
&=& \bigcup_{i=0}^d \{s \, | \, \left(\mathcal{A}^{i}\right)_{js} \neq 0 \} \nonumber
\end{eqnarray}
where $\bigcup$ is the set union operation. Define $\bar{\mathcal{A}} = \Sp{I} + \Sp{A}$. It can be shown that
\begin{eqnarray}
Up(j,d) &=& \{s \, | \, \left(\bar{\mathcal{A}}^{d}\right)_{js} \neq 0 \} \nonumber \\
Down(j,d) &=& \{s \, | \, \left(\bar{\mathcal{A}}^{d}\right)_{sj} \neq 0 \}. \label{eq:updown}
\end{eqnarray}
Note that $Up(j,d)$ is the set of all (possibly) nonzero elements in $j$-th row of $\bar{\mathcal{A}}^d$, and $Down(j,d)$ is the set of all (possibly) nonzero elements in $j$-th column of $\bar{\mathcal{A}}^d$. This motivates the definition of $(A,d)$ sparseness, which provides a compact way to encode $Up(j,d)$ and $Down(j,d)$ for all $j$.
%natural measure of sparsity with respect to the underlying topology of a given matrix $A$.
\begin{definition} [$(A,d)$ Sparseness]
Let $\bar{\mathcal{A}} = \Sp{I} + \Sp{A}$. A real matrix $X$ is \textit{$(A,d)$ sparse} if and only if
\begin{equation*}
\Sp{X} \subseteq \bar{\mathcal{A}}^d.
\end{equation*}
\end{definition}
%From \eqref{eq:updown}, $Up(j,d)$ is the set of all (possibly) nonzero elements in $j$-th row of $\bar{\mathcal{A}}^d$, and $Down(j,d)$ is the set of all (possibly) nonzero elements in $j$-th column of $\bar{\mathcal{A}}^d$. In other words, $(A,d)$ sparseness is a compact way to encode $Up(j,d)$ and $Down(j,d)$ for all $j$.
%A simple way to check $(A,d)$ sparseness is by defining $\bar{\mathcal{A}} = \Sp{I} + \Sp{A}$. In this case, $\bar{\mathcal{A}}^i \subseteq \bar{\mathcal{A}}^{i+1}$ and thus we have
%\begin{equation}
%\sum_{i=0}^{d} \mathcal{A}^i = \bar{\mathcal{A}}^d.
%\end{equation}

%We describe locality constraints in terms of $(A,d)$ sparseness, which is defined as follows.
%\begin{definition}
%A real matrix $X$ is \textit{$(A,d)$ sparse} if
%\begin{equation*}
%\Sp{X} \subseteq \bigcup_{i=0}^{d} \Sp{A}^i.
%\end{equation*}

%We define the union of two binary matrices $\s_1, \s_2\in \{0,1\}^{m \times n}$ by the rule
%\begin{equation*}
%\{\s_1\bigcup\s_2\}_{ij} = 1 \textit{ iff } \{\s_1\}_{ij} = 1 \textit{ or } \{\s_2\}_{ij} = 1.
%\end{equation*}
%We may then naturally say that $\s_1\subseteq \s_2$ if $\s_1\bigcup\s_2=\s_2$.

\subsection{Spatio-Temporal Constraints}
The sparsity patterns defined on a matrix can be extended to the spatio-temporal constraints defined on a transfer function. Specifically, the spatio-temporal constraints for a transfer function $R$ is described by a constraint space $\mathcal{S}_R := \sum_{i=0}^{\infty} \frac{1}{z^i} \s_{R}[i]$, where $\{\s_{R}[i]\}$ is an ordered set of binary matrices. We say that a transfer function $R$ is in $\mathcal{S}_R$ if and only if $\Sp{R[i]} \subseteq \s_{R}[i]$ for all $i$, which we denote by $R \in \mathcal{S}_R$. 

In this paper, we consider locality constraints, finite impulse response (FIR) constraints, and communication delay constraints as follows.
%-- the combination of these three constraints allow for the control problem to be formulated as a finite dimensional convex program that leads to a scalable implementation, all the while respecting the information sharing constraints of the system.

\subsubsection{Locality constraints}
A constraint space $\mathcal{S}_R$ is $(A,d)$ sparse if and only if $\s_{R}[i]$ is $(A,d)$ sparse for all $i$.\footnote{For a large $d$, it is possible that $\bar{\mathcal{A}}^d = \mathbf{1}$ - this simply means that the ``localized" region is the entire system.} A transfer function is $(A,d)$ sparse if and only if all of its spectral components are $(A,d)$ sparse.

\subsubsection{FIR constraints}  If $\s_{R}[i] = \mathbf{0}$ for all $i > T$, we say that $\mathcal{S}_R$ is finite in time $T$, and any stable transfer function in $\mathcal{S}_R$ has a FIR.

%which in our case will be intimately related to how perturbations spread across the physical topology of the plant.

\subsubsection{Communication delay constraints}
The communication delay constraints can be imposed on the first few spectral components of a transfer function. In this paper, we characterize communication delay constraint on a parameter $h > 1$, which represents the relative communication speed compared to the speed of disturbance propagation in the plant.
%The constraints depend on the implementation of the controller as well as the topology of the communication network. 

\begin{example}
One example that combines the locality constraints, FIR constraints, and communication delay constraints, is given by
\begin{equation}
\mathcal{S}_R = \sum_{i=1}^T \frac{1}{z^i} \bar{\mathcal{A}}^{\min(d, \lfloor h(i-1) \rfloor)}. \nonumber
\end{equation}
\end{example}

For a system $(A, B_2)$, the spatio-temporal constraint is described by a pair $(\mathcal{S}_R, \mathcal{S}_M)$ on the closed loop transfer function $(R,M)$ (the transfer function from $w$ to $x$ and $w$ to $u$, respectively). We define a $(d,T)$ localized FIR constraint for a system $(A,B_2)$ as follows.
\begin{definition} [$(d,T)$ Localized FIR Constraint]
The constraint space pair $(\mathcal{S}_R, \mathcal{S}_M)$ is a $(d,T)$ localized FIR constraint for system $(A, B_2)$ if and only if
\begin{enumerate}
\item $\mathcal{S}_R$ and $\mathcal{S}_M$ are finite in time $T$.
\item $\mathcal{S}_R$ is $(A,d)$ sparse.
\item $\Sp{B_2}$ $\mathcal{S}_M$ is $(A,d+1)$ sparse.
%\item $\mathcal{S}_x[i]$ is $(A,d)$ sparse for $i = 1, \dots, T$.
%\item $\Sp{B}$ $\mathcal{S}_u[i]$ is $(A,d+1)$ sparse for $i = 1, \dots, T$.
\end{enumerate}
\label{dfn:3}
\end{definition}

Before discussing the physical meaning of Definition \ref{dfn:3}, we consider an example of a $(d,T)$ localized FIR constraint for a scalar sub-system model $(A, B_2)$.
\begin{example}
Let $(A, B_2)$ be a scalar sub-system model and $h > 1$ the relative communication speed. The following constraint space pair $(\mathcal{S}_R, \mathcal{S}_M)$ is a $(d,T)$ localized FIR constraint for system $(A, B_2)$.
\begin{eqnarray}
\mathcal{S}_R &=& \sum_{i=1}^T \frac{1}{z^i} \bar{\mathcal{A}}^{\min(d, \lfloor h(i-1) \rfloor)} \nonumber\\
\mathcal{S}_M &=& \frac{1}{z^{t_s}}\sum_{i=1}^T \frac{1}{z^i} \Sp{B_2^\top} \bar{\mathcal{A}}^{\min(d+1, \lfloor h(i-1) \rfloor)} \label{eq:SRM}
\end{eqnarray}
where $t_s$ is the sensing delay, e.g. $t_s = 1$ for a strictly proper controller, and $t_s = 0$ for a proper controller. It can be verified that all the conditions in Definition \ref{dfn:3} are satisfied.
\label{ex:rm}
\end{example}
%In our control scheme, the required communication delay constraints depend on the implementation of the controller, and therefore, we hold off on defining these until after we have introduced the controller implementation in Section \ref{sec:implementation}.

The parameters $(d,T,h)$ in \eqref{eq:SRM} has a fairly intuitive physical meaning. For a local disturbance $w[k] = \delta[k] e_j$ in \eqref{eq:dynamics}, the state $x$ is constrained by the $j$-th column of $\mathcal{S}_R$ in \eqref{eq:SRM}. Similarly, the control $u$ is constrained by the $j$-th column of $\mathcal{S}_M$. Therefore, the parameter $d$ in \eqref{eq:SRM} means that the affected region of disturbance $j$ is limited within the set $Down(j,d)$ for each $j$, and the effect of the disturbance can be eliminated within time $T$. The parameter $h$ characterize how fast the information of the disturbance is propagated within the controller network, which needs to be faster than the speed of disturbance propagation in the plant in order to localize the effect of the disturbance.
%we can parameterize the spatio-temporal constraints by $(d,T,h)$, where $d$ is the radius of the affected region for each disturbance, $T$ the affected time for each disturbance, and $h > 1$ is the required relative communication speed compared to the speed of disturbance propagation in the plant.

\begin{example}
For the chain model, the constraints in \eqref{eq:SRM} for a local disturbance $w_j$ can be visualized by a space-time diagram in Figure \ref{fig:region}. The vertical axis in this diagram represents the space of different states (an ordered set $\{x_i\}$), and the horizontal axis is the time evolution. The constraints in \eqref{eq:SRM} require that the the effect of $w_j$ being contained within the affected region in this space-time diagram. For multiple disturbances, linearity ensures that the effect of each local disturbance is contained within their own (possibly overlapping) affected region as shown in Figure \ref{fig:Overlap}.
\label{ex:chain}
\end{example}
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.38\textwidth]{./figure/Forward_region2.pdf}
      \caption{The affected region of a local disturbance $w_j$ for a chain model. The vertical axis in this diagram represents the space of different states (an ordered set $\{x_i\}$), and the horizontal axis is the time evolution.}
      \label{fig:region}
\end{figure}
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.35\textwidth]{./figure/Overlapping.pdf}
      \caption{Overlapping affected regions for different local disturbances.}
      \label{fig:Overlap}
\end{figure}

\begin{remark}
The problem of finding a localized closed loop response can be considered as a generalization of disturbance localization problems. Those problems are first formulated in \cite{1970_Wonham} for the centralized case, \cite{1975_Hamano} for the decentralized case, and \cite{1982_Kobayashi} for an extension. It should be noted that the methods described in those papers cannot deal with multiple disturbance with overlapping affected regions, as the solution becomes simply infeasible. This is again due to the fact that the problem is formulated in the ``$K$" domain. It is also noteworthy that \cite{1982_Kobayashi} uses the term \emph{localizability} in their paper with a different meaning. In their method, localizability can only be achieved by a large centralized supervisory controller, which cannot be applied on large-scale system. 
\end{remark}

The physical meaning of Definition \ref{dfn:3} for scalar sub-system is explained by the discussion in Example \ref{ex:rm} and \ref{ex:chain}. For non-scalar sub-system, there may exist control action that affects multiple states at the same time. The third condition means that no cross-boundary control action should be activated to localize the disturbance. Consider the non-scalar sub-system model in Figure \ref{fig:non} with $d = 2$. The red block in this figure represents the localized region including the boundary for disturbance $w_1$. The states affected by $u_1$ lies strictly within the red block, so $u_1$ can be activated for disturbance $w_1$. On the other hand, $u_2$ is a cross-boundary control action since it affects $x_5$. Therefore, a $(d,T)$ localized FIR constraint with $d = 2$ requires $u_2 = 0$.

\begin{figure}[t!]
      \centering
      \includegraphics[width=0.35\textwidth]{./figure/Nonscalar.pdf}
      \caption{The red / blue block represents the localized region with / without the boundary for disturbance $w_1$. $u_2$ is a cross-boundary control action.}
      \label{fig:non}
\end{figure}

Note that $(d,T)$ localized FIR constraint is just one type of structural constraint on the closed loop transfer function. The methods described in this paper is compatible with other constraints such as the upper and lower bound on the entries of $R$ and $M$ as well.


